Trading off Accuracy for Speedup: Multiplier Bootstraps for Subgraph Counts

We propose a new class of multiplier bootstraps for count functionals, ranging from a fast, approximate linear bootstrap tailored to sparse, massive graphs to a quadratic bootstrap procedure that offers refined accuracy for smaller, denser graphs. For the fast, approximate linear bootstrap, we show that $\sqrt{n}$-consistent inference of the count functional is attainable in certain computational regimes that depend on the sparsity level of the graph. Furthermore, even in more challenging regimes, we prove that our bootstrap procedure offers valid coverage and vanishing confidence intervals. For the quadratic bootstrap, we establish an Edgeworth expansion and show that this procedure offers higher-order accuracy under appropriate sparsity conditions. We complement our theoretical results with a simulation study and real data analysis and verify that our procedure offers state-of-the-art performance for several functionals.

==> cicoverage.tex <==
So far, we have proposed a family of bootstrapped methods for standardized count functionals of networks. Note that studentized statistics are typically preferred because they produce higher order correct confidence intervals. However it is well known~\citep{hall-bootstrap-edgeworth} that in many situations like correlation coefficients,  pivoting may not be suitable, because the variance estimate can be unstable. On the other hand, standardized bootstrap procedures produce first order correct confidence intervals. In this section, we show how to correct these intervals to get higher order coverage. \bk


From our proposed bootstrap, we construct a two-sided confidence interval with nominal coverage $\alpha$ $\mathcal{I}_1=\left(\hat{y}_{\frac{1-\alpha}{2}},\hat{y}_{\frac{1+\alpha}{2}}\right)$,
%\begin{align}\label{eq:cifirst}
 %   \mathcal{I}_1=\left(\hat{y}_{\frac{1-\alpha}{2}},\hat{y}_{\frac{1+\alpha}{2}}\right),
%\end{align}
where we define function $\hat{L}(t)=P(\hat{T}_n^* < t \mid  A,X)$ for bootstrap samples $\{\hat{T}^*_n\}$, and $\hat{y}_\alpha=\hat{L}^{-1}(\alpha)$.
Let $z_{\alpha}$ denote standard normal critical point at $\alpha$ where $\Phi(z_{\alpha})=\alpha$, then $\hat{y}_\alpha=\hat{L}^{-1}(\Phi(z_{\alpha}))$.
%Coverage error of a confidence interval is the difference of its true coverage and nominal coverage, $P(\theta \in \mathcal{I}_1)-\alpha$. %First-order correct CIs have coverage error of order $O(n^{-1/2})$, whereas second-order correct CIs have coverage error of $O(n^{-1})$. 
%A confidence interval is first-order correct if its coverage error is of order $O(n^{-1/2})$, but is second-order correct if its coverage error is of order $O(n^{-1})$. Alternatively, 
Equivalently, define $\hat{u}_{\alpha}$ as the critical point at $\alpha$ for standardized bootstrap sample $(\hat{T}^*_n-\hat{T}_n)/\hat{\sigma}_n$ distribution and $\hat{v}_{\alpha}$ as the critical point at $\alpha$ for studentized bootstrap sample $(\hat{T}^*_n-\hat{T}_n)/\hat{\sigma}^*_n$ distribution.
Standardized and studentized bootstrap CIs  $\mathcal{I}_1$ and  $\mathcal{I}_2$ can be written as 
\begin{align*}
    &\mathcal{I}_1=(\hat{T}_n+n^{-1/2}\hat{\sigma}_n\hat{u}_{\frac{1-\alpha}{2}},\hat{T}_n+n^{-1/2}\hat{\sigma}_n\hat{u}_{\frac{1+\alpha}{2}}) ,\\
    &\mathcal{I}_2=(\hat{T}_n+n^{-1/2}\hat{\sigma}_n\hat{v}_{\frac{1-\alpha}{2}},\hat{T}_n+n^{-1/2}\hat{\sigma}_n\hat{v}_{\frac{1+\alpha}{2}}).
\end{align*}

$\mathcal{I}_1$ and  $\mathcal{I}_2$ are bootstrap estimates of theoretical $\alpha$ coverage percentile CIs $\mathcal{J}_1$ and $\mathcal{J}_2$ respectively,
\begin{align*}
     &\mathcal{J}_1=(\hat{T}_n+n^{-1/2}\sigma_nu_{\frac{1-\alpha}{2}},\hat{T}_n+n^{-1/2}\sigma_nu_{\frac{1+\alpha}{2}}) ,\\
    &\mathcal{J}_2=(\hat{T}_n+n^{-1/2}\hat{\sigma}_n v_{\frac{1-\alpha}{2}},\hat{T}_n+n^{-1/2}\hat{\sigma}_n v_{\frac{1+\alpha}{2}}),
\end{align*}
where $u_{\alpha}$ is the critical point at $\alpha$ of the distribution for $(\hat{T}_n-T_n)/\sigma_n$ and $v_{\alpha}$  is the critical point at $\alpha$ of the distribution for $(\hat{T}_n-T_n)/\hat{\sigma}_n$.
Our standardized bootstrap confidence interval $\mathcal{I}_1$ is only first-order correct, as the end points of $\mathcal{I}_1$ differ from  $\mathcal{J}_1$ by $O(n^{-1})$ (or equivalently, they agree only to and including terms of order $O(n^{-1/2})$). In contrast, studentized bootstrap confidence interval $\mathcal{I}_2$ is second-order correct; the end points of $\mathcal{I}_2$ differs from  $\mathcal{J}_2$ by $O(n^{-3/2})$.   However, $\mathcal{I}_1$ can be shifted to be second-order correct as follows:% (also see~\cite{hall-bootstrap-edgeworth}). %\cite{hall-bootstrap-edgeworth} Section 3.10 gives an explicit form of shifting $\mathcal{I}_1$ to $\mathcal{I}'_1$ and $\mathcal{I}'_1$ is second-order correct. 
\begin{align}\label{eq:ci-correction}
    \mathcal{I}'_1 = \left(\hat{y}_{\frac{1-\alpha}{2}}+n^{-1}\hat{\sigma}\left\{\hat{p}_1(z_{\frac{1-\alpha}{2}})+\hat{q}_1(z_{\frac{1-\alpha}{2}})\right\},\  \hat{y}_{\frac{1+\alpha}{2}}+n^{-1}\hat{\sigma}\left\{\hat{p}_1(z_{\frac{1+\alpha}{2}})+\hat{q}_1(z_{\frac{1+\alpha}{2}})\right\} \right)
\end{align}
where for any $x \in \mathbb{R}$, $\hat{p}_1(x)$ and   $\hat{q}_1(x)$ are estimates for $p_1(x)$ and $q_1(x)$. $p_1(x)$ is polynomial coefficient of $n^{-1/2}\phi(x)$ in standardized Edgeworth Expansion $G_n(x)$ developed in Eq~\ref{eq:edgeworth-gn} and $q_1(x)$ is the polynomial in front of $n^{-1/2}\phi(x)$ in studentized Edgeworth Expansion $G_n'(x)$ developed in previous work. Therefore, we can write
\begin{align*}
    &\hat{p}_1(\mathit{z}_{\alpha})= \frac{(1-\mathit{z}_{\alpha}^2)}{6\hat{\tau}_n^3}\biggl[\mathbb{E}\{\hat{g}_1^3(X_1)\}+3(r-1)\mathbb{E}\{\hat{g}_1(X_1)\hat{g}_1(X_2)\hat{g}_2(X_1,X_2)\} \biggr], \\
    &\hat{q}_1(\mathit{z}_{\alpha})=\frac{1}{\hat{\tau}_n^3}\biggl[\frac{2\mathit{z}_{\alpha}^2+1}{6}\mathbb{E}\{\hat{g}_1^3(X_1)\}+\frac{r-1}{2}(\mathit{z}_{\alpha}^2+1)\mathbb{E}\{\hat{g}_1(X_1)\hat{g}_1(X_2)\hat{g}_2(X_1,X_2)\} \biggr].
\end{align*}

\rd 
Now, for smooth functions of conditional expectation of count functionals, we have derived $\sigma$ and $p_1(x)$ in Section~\ref{sec:smf}. % needed for correction.
We now present the form of $q_1(x)$ for the studentized version of this. Define the studentized functional $S_n'=n^{1/2}(f(\bu)-f(\bmu))/\hat{\sigma}$, where $\bu$ and $\bmu$ are defined as the conditional and unconditional expectations of the count statistics. We use this form to correct our confidence intervals.
\bk

The derivation of $q_1$ is much more complicated than deriving $p_1$, since one needs to append to $\bu$ more terms so that the variance of $f(\bu)$ can be written as a function of the elongated mean vector $E[\bu]$. For example, for estimating mean of i.i.d univariate random variables one will use a two dimensional vector $(x_1,x_2)$ with $x_1=X_i$ and $x_2=X_i^2$. for smooth functions of count  statistics the variance of the smooth function of $f(\bu)$ is $\sigma^2/n$, where $\sigma$ is given in Eq~\ref{eq:p1sigma}. In order to write this as a function of $\bmu$, we create the following mean vector.

\begin{equation*}
\begin{split}
   \cbu=\bigg{\{}\underbrace{\frac{\tnt{(1)}}{\rho_n^{s_1}},\ldots, \frac{\tnt{(d)}}{\rho_n^{s_d}}}_{d \text{ terms}},\underbrace{\frac{r_1r_2\sum_{i=1}^n\hat{h}_1^{(1)}(X_i)\hat{h}_1^{(2)}(X_i)}{n\rho_n^{s_1}\rho_n^{s_2}},\ldots,\frac{r_{d-1}r_d\sum_{i=1}^n\hat{h}_1^{(d-1)}(X_i)\hat{h}_1^{(d)}(X_i)}{n\rho_n^{s_1}\rho_n^{s_2}}}_{{d \choose 2} \text{ terms}},\\
   \underbrace{\frac{r_1^2\sum_{i=1}^n\hat{h}_1^{(1)}(X_i)^2}{n\rho_n^{2s_1}},\ldots,\frac{r_d^2\sum_{i=1}^n\hat{h}_1^{(d)}(X_i)^2}{n\rho_n^{2s_d}}}_{d \text{ terms}}\bigg{\}}, 
\end{split}
\end{equation*}
where $\hat{h}_1(X_i)$ is given by:
\begin{align*}
    \hat{h}_1(X_i)=\frac{1}{{n-1 \choose r-1}}\sum_{1\leq i_1<\ldots< i_r\leq n, i_1,\ldots,i_r \neq i } \hat{h}(X_i,X_{i_1},\ldots,X_{i_r}).
\end{align*}

Under similar conditions required to establish the Edgeworth expansion of Eq~\ref{eq:EW-SMF}, we have
 \begin{align*}
    P(S_n' < x) = \Phi(x) + n^{-1/2}q_1(x)\phi(x) + o\left(n^{-1/2}\right),
\end{align*}
\begin{align*}
    q_1(x)=-\{B_1+\frac{1}{6}B_2(x^2-1)\},
    \end{align*}
    where 
    \begin{align}
        B_1= A_1\sigma^{-1}-\frac{1}{2}\sigma^{-3}n\sum_{i=1}^{d'}\sum_{j=1}^{d'}a_ic_j\E\{(\cbu-\cbmu)^{(i)}(\cbu-\cbmu)^{(j)}\}.
    \end{align}
   % We provide the form of $B_1$ explicitly in Supplementary Section~ \ref{sec:supp:proof-smf-ew-stu-and-ci-abc}. 
   Note that the CDF of the studentized and standardized statistics match at $x=0$, i.e. $p_1(0)=q_1(0)$. Hence one can estimate $B_2$ if $A_1,A_2$, and $B_1$ are available.
    
    Estimating the moments in the above expression requires one to expand out the expression and we do this in detail in the Supplement Section~\ref{sec:supp:proof-smf-ew-stu-and-ci-abc}.
    
    
    In the following figures we compare the absolute deviation of the empirical Edgeworth expansion of the transitivity coefficient from the true distribution with that of the Gaussian approximation for the \smg graphon. It is easy to see that the Edgeworth expansion is much more accurate than the Gaussian approximation.
    
    \begin{figure}[h]
%\vskip 0.2in
\centering
%\text{no log}\\
\begin{tabular}{c}
    \includegraphics[width=  0.4\textwidth]{plots2/Smg-p1-error.pdf} 
     \includegraphics[width=  0.4\textwidth]{plots2/Smg-q1-error.pdf}
  %   \vspace{-2em}
     %  \includegraphics[trim=0em 1em 0em 5em, clip, width=  \textwidth]{plots/EW-MB-trans-nobar.pdf}
  %     \vspace{-1em}
    %\vspace{-4em}
%    \includegraphics[width=  0.8\textwidth,height=0.4\textwidth]{plots/EW-MB-twostars-nobar.pdf}\\
\end{tabular}
%\\\vspace{5mm}\text{taking log}\\
%\begin{tabular}{c}
%    \includegraphics[width=  0.4\textwidth]{plots2/sbm-triangles-log.pdf} 
%    \includegraphics[width=  0.4\textwidth]{plots2/ng2-triangles-log.pdf}\\
%    \includegraphics[width=  0.4\textwidth]{plots2/sbm-triangles-centerbytnhat-log.pdf}\includegraphics[width=  0.4\textwidth]{plots2/ng2-triangles-centerbytnhat-log.pdf}
  %   \vspace{-2em}
     %  \includegraphics[trim=0em 1em 0em 5em, clip, width=  \textwidth]{plots/EW-MB-trans-nobar.pdf}
  %     \vspace{-1em}
    %\vspace{-4em}
%    \includegraphics[width=  0.8\textwidth,height=0.4\textwidth]{plots/EW-MB-twostars-nobar.pdf}\\
%\end{tabular}
 \caption{\rd Standardized and studentized transitivity: Y axis is absolute error $|Fn(u) - F^*(u)|$ of CDFs, X axis is  X axis is $u$ $\in$ $[-3:3]$. Left is absolute error of standardized Edgeworth expansion to standardized truth compare to absolute error of N(0,1) to standardized truth. Right is absolute error of studentized Edgeworth expansion to studentized truth compared with absolute error of N(0,1) to studentized truth. }.
%\begin{center}
\label{fig:cdf-error}
\end{figure}
\rd
In the Supplement, we also provide a table for different statistics like linear combinations of triangle and two star densities, the product of triangle and two-star densities, the product of the squares of triangle and two-star densities. The general observation is that if the derivatives $a_i,a_{ij}$ have to be estimated from data, then the error of the empirical Edgeworth gets worse.
\bk
%The explicit form of $B_1$ and $B_2$ are provided in Supplementary Section~ \ref{sec:supp:proof-smf-ew-stu-and-ci-abc}. 
\iffalse
However, because of the complicated expressions of parameters $A_1$,  $A_2$, $B_1$, $B_2$, instead of directly using Eq~\ref{eq:ci-correction}, we use an alternative but equivalent bias correction for the confidence interval proposed by \cite{efron-better-ci}, the accelerated bias correction. The corrected confidence $\mathcal{I}''_1$ is 
\begin{align}\label{eq:ci-correction-abc}
    &\mathcal{I}''_1=(\hat{y}_{\mathrm{ABC},\frac{1+\alpha}{2}},\ \hat{y}_{\mathrm{ABC},1-\frac{1+\alpha}{2}}),
    \end{align}
with $\hat{y}_{\mathrm{ABC},\alpha}$ defined as
    \begin{align*}
    &\hat{y}_{\mathrm{ABC},\alpha}=\hat{L}^{-1}\left(\Phi\left[\hat{m}+(\hat{m}+z_{\alpha})\{1-\hat{a}(\hat{m}+z_{\alpha})\}^{-1}\right]\right),
\end{align*}
where $\hat{m}$ and $\hat{a}$ for $d$-dimensional smooth function of count functionals are
\begin{equation}\label{eq:ci-correction-abc-mhat}
    \hat{m}=\hat{L}^{-1}(\hat{T}_n)= n^{-1/2}\hat{p}_1(0),
    \end{equation}
    \begin{equation}\label{eq:ci-correction-abc-ahat}
    %\hat{a}=\frac{\hat{\sigma}^{-3}}{6n^{1/2}}\sum_{i=1}^d\sum_{j=1}^d\sum_{k=1}^d\hat{a}_i\hat{a}_j\hat{a}_k\hat{\lm}_{ijk}.%+O(n^{-1}).
     \hat{a}=n^{-1/2}\frac{1}{6} \left\{-(\hat{A}_2\hat{\sigma}^{-3}+\hat{B}_2)\right\}.
    \end{equation}
%and $A$ for $d$-dimensional smooth function of count functionals is 
%\begin{align}
%    \hat{A}=\frac{r^3}{n^{3/2}}\sum_{i=1}^d\sum_{j=1}^d\sum_{k=1}^da_ia_ja_k\bu_L^{(i)}\bu_L^{(j)}\bu_L^{(k)}+O\left(\frac{1}{n}\right).
%\end{align}
Calculation and proof of Eq~??? is provided in detail in Supplementary Section~\ref{sec:supp:sub-ci-abc}.  
\fi
\bk

==> hoeffding.tex <==

%
%BLAHBLAHBLAH
\section{The Hoeffding decomposition}
The Hoeffding decomposition, introduced in \citet{hoeffding1948}, is a key technical tool for studying the asymptotic properties of U-statistics.  In essence, a U-statistic may be represented as a sum of U-statistics of different orders.  Only the linear (order one) term is non-negligible; the order 2 term is also needed for higher-order correctness. The Hoeffding decomposition, however, generalizes far beyond U-statistics.  We will provide a more general treatment of the Hoeffding decomposition below, following \citet{Bentkus-edgeworth-symmetric}. This general decomposition will be used to derive a Hoeffding decomposition for the bootstrap statistic.

Let $X_1, \ldots, X_n$ be independent random variables and $\Omega = \{1, \ldots n\}$. For any $B \subset \Omega$ and a random variable $T = t(X_1, \ldots , X_n)$, let
\begin{align}
T_B = \mathbb{E}[T \ \mid  X_i \in B]
\end{align}
It may be verified that:
\begin{align*}
T_B = \sum_{C \subset B} (-1)^{|B| - |C|} T_C
\end{align*}
We also have the following inverse relationship:
\begin{align*}\mathbb{E}[T \ \mid  X_i \in C] = \sum_{B \subset C} T_B 
\end{align*}
which implies the Hoeffding decomposition:
\begin{align}
    T = \sum_{B \subset \Omega} T_B
\end{align}
In what follows, we will group terms by their cardinality, leading to a decomposition closely resembling the familiar decomposition for U-statistics.
\section{Proof of Lemma~\ref{lemma:hoeffding-bootstrap}}
\label{sec:supp:lemmaone}
\begin{proof}
In what follows, we will consider a projection of $T_{n,M}^*$ with respect to the random variables $ \w_1, \ldots \w_n$, conditional on $A$ and $X$. 

Recall that $\xi_i$ follows the Gaussian Product distribution. First, we may express $T_{n,M}^*$ as:
\begin{align*}
T_{n,M}^* = \frac{1}{{n \choose r}} \sum_{1 \leq i_1 < i_2 < \ldots i_r} \left(\xi_{i_1 \cdots i_r} - 1\right)  \cdot \left( H(A_{i_1, \ldots, i_r}^{(n)}) - \hat{T}_n \right)
\end{align*}
where $\xi_{i_1 \cdots i_r}$ denotes the product $\xi_{i_1} \times \cdots \times \xi_{i_r}$. It turns out that applying the Hoeffding decomposition directly to $T_{n,M}^*$ leads to tedious combinatorial calculations; following \citet{Bentkus-edgeworth-symmetric}, let $\Omega_r$ denote an $r$-tuple of $\{1, \ldots, n\}$.  For each summand, we will consider a Hoeffding representation with respect to $\Omega_r$.   Note that using the Hoeffing projection (also see~\cite{Bentkus-edgeworth-symmetric} section 2.8), 
\begin{align*}
    \prod_{1\leq i\leq r}\w_i-1=\sum_{k=1}^r\sum_{1\leq i_1<\dots< i_k\leq r} h_k(\w_{i_1},\dots,\w_{i_k}),
\end{align*}
where for $\Omega_k=\{1,\dots, k\}$,
\begin{align*}
    h_k(\w_{1},\dots,\w_{k})=\sum_{B\in \Omega_k}(-1)^{k-|B|}\E\left[\prod_{1\leq i\leq r}\w_i-1\mid B\right]
\end{align*}
Thus the first two terms are given by:
\begin{align*}
    h_1(\w_{1})&:=(\w_1-1)\\ h_2(\w_{1},\w_{2})&:=(\w_1\w_2-1)-(\w_1-1)-(\w_2-1)=(\w_1-1)(\w_2-1)
\end{align*}
In what follows, we will also denote $A^{(n)}_{i_1,\dots,i_r}$ by $A^{(n)}_S$, where $S=\{i_1,\dots, i_r\}$.
Let 
\begin{align}\label{eq:hhij}
    \hhij= \frac{1}{{n-2 \choose r-2}}\sum_{S,i,j\in S}H(A_S).
\end{align}
Thus $T_{n,M}^*$ can be written as follows:
\begin{align}\label{eq:hofftnm}
    T_{n,M}^* &= \frac{1}{{n \choose r}} \sum_{1 \leq i_1 < i_2 < \ldots < i_r} \left(\xi_{i_1 \cdots i_r} - 1\right)  \cdot \left( H(A_{i_1, \ldots, i_r}^{(n)}) - \hat{T}_n \right)\notag\\
    &=\frac{1}{{n \choose r}} \sum_{1 \leq i_1 < i_2 < \ldots < i_r}\sum_{k=1}^r\sum_{1\leq i_1<\dots< i_k\leq i_r} h_k(\w_{i_1},\dots,\w_{i_k})\cdot \left( H(A_{i_1, \ldots, i_r}^{(n)}) - \hat{T}_n \right)\notag\\
    &=\frac{1}{{n \choose r}} \sum_{k=1}^r \sum_{1\leq i_1<\dots< i_k\leq n} h_k(\w_{i_1},\dots,\w_{i_k})\cdot\sum_{S}  \left( H(A_S^{(n)}) - \hat{T}_n \right)1 (i_1,\dots, i_k\in S)\notag\\
    &=\frac{1}{{n \choose r}} \sum_{k=1}^r {n-k\choose r-k}\sum_{1\leq i_1<\dots< i_k\leq n}h_k(\w_{i_1},\dots,\w_{i_k}) \frac{\sum_{S}  \left( H(A_S^{(n)}) - \hat{T}_n \right)1 (i_1,\dots, i_k\in S)}{{n-k\choose r-k}}\notag\\
    &=\frac{r}{n}\sum_i (\xi_i-1)\gi+\frac{r(r-1)}{n(n-1)}\sum_{1\leq i<j\leq n} (\w_i-1)(\w_j-1)\underbrace{(\hat{H}_2(i,j)-\tnhat)}_{\tilde{g}_2(i,j)}+R_n
\end{align}


\iffalse
The first two terms of the decomposition are given by:
\begin{align*}
f_1(A_{i,i_2, \ldots, i_r}) &= \left(\xi_i - 1 \right) \cdot \left( H(A_{i,i_2, \ldots, i_r}^{(n)}) - \hat{T}_n \right) 
\\ f_2( A_{i,j,i_3, \ldots, i_r}) %&= \rd \left(\xi_i \cdot \xi_j - \w_i-\w_j +1 \right) \cdot \left( H(A_{i,j,i_3, \ldots, i_r}^{(n)}) - \hat{T}_n \right) \bk\\
&=\left(\xi_i \cdot \xi_j - 1 \right) \cdot \left( H(A_{i,j,i_3, \ldots, i_r}^{(n)}) - \hat{T}_n \right) - f_1(A_{i,i_2, \ldots, i_r}) - f_1(A_{j,i_2, \ldots, i_r})
\end{align*}
\rd
\begin{align*}
f_{1,i}(A_{S}) &= \left(\xi_i - 1 \right) \cdot \left( H(A_{S}^{(n)}) - \hat{T}_n \right) 1(i\in S)
\\ f_{2,i.j}( A_{S}) &= \rd \left(\xi_i \cdot \xi_j - \w_i-\w_j +1 \right) \cdot \left( H(A_{S}^{(n)}) - \hat{T}_n \right)1(i,j\in S) \bk\\
%&=\left(\xi_i \cdot \xi_j - 1 \right) \cdot \left( H(A_{i,j,i_3, \ldots, i_r}^{(n)}) - \hat{T}_n \right) - f_1(A_{i,i_2, \ldots, i_r}) - f_1(A_{j,i_2, \ldots, i_r})
\end{align*}
\bk
 Now, combining terms, we have that:
\begin{align*}
 T_{n,M}^* - \hat{T}_n &= \frac{1}{{n \choose r}} \sum_{\Omega_r \subset \Omega}  \left(\xi_{i_1 \cdots i_r} - 1\right)  \cdot \left( H(A_{i_1, \ldots, i_r}^{(n)}) - \hat{T}_n \right) 
 \\ &= \frac{r}{n} \sum_{i=1}^n (\xi_i - 1) \hat{g}_1(i)
 \\ & \ \ \ +\frac{r(r-1)}{n(n-1)}\sum_{i<j}(\w_i\w_j-1) \tilde{g}_2(i,j)-(\w_i-1) \cdot \hat{g}_1(i) - (\w_i-1) \cdot \hat{g}_1(j) + R_n
% \\ & = \frac{r}{n}\sum_{i=1}^n \sum_{ f_1(\xi_i; A_{i, i_2, \ldots, i_r}) + \frac{r(r-1)}{n(n-1)} \sum_{i < j} f_2(\xi_i, \xi_j; A_{i,j,i_3, \ldots, i_r}) +R_n 
 \end{align*}
 \fi
 Now, it remains to show that the remainder of $(T_{n,M}^* - \hat{T}_n)/\hat{\sigma}_n$ is $O(\delta(n,\rho_n,R))$, where:
 \begin{align*}
    \delta(n,\rho_n,R) =\begin{cases} 
      \frac{1}{n\rho_n} & \text{R is acyclic} \\
       \frac{1}{n\rho_n^{3/2}}& \text{R is cyclic} .
  \end{cases}
\end{align*}

 The residual $R_n$ is a sum of higher order Hoeffding projections, which are all uncorrelated. %
 Therefore, we see that the variance of the $u^{th}$ order term is $\dfrac{\sum_{1\leq i_1<i_2\dots<i_u}  \tilde{g}_u(i_1,i_2,\dots,i_u)^2}{\hat{\sigma}_n^2 {n\choose u}^2}$. We will now obtain expressions for $3\leq u\leq r$.
 %Therefore, we see that the variance of the third order term (the first one in the remainder) is $\dfrac{\sum_{ijk}  \hat{g}_3(i,j,k)^2}{\hat{\sigma}_n^2 {n\choose 3}} \times O(1/n^3)$.  By Markov inequality, it further suffices to show $\mathbb{E}[\hat{g}_3(i,j,k)^2\delta^2(n,\rho_n,R)/\hat{\sigma}_n^2  ] )$ is bounded.
 %Now, we have that:
 %\begin{align*}
 %\mathbb{E}[\tilde{g}_u(i,j,k)^2] \leq 2 \left( \mathrm{Var}(\hat{g}_3(i,j,k)) + \mathrm{Var}(\hat{T}_n) \right)
 %\end{align*}
 
 
 
%  We may reinterpret $\mathbb{E}[\hat{g}_3(i,j,k)^2$ as $\mathrm{Var}(\hat{g}_3(i,j,k))$.  To bound this term,    
 
%  Note that  $\hat{g}_3(i,j,k)^2=O_P(\rho_n^{3s-3})$ for cyclic and $O_P(\rho_n^{3s-2})$ for acyclic subgraphs. This is because, for any two nonoverlapping $S,T$ (not containing $\{i,j,k\}$)  of size $r-3$, there are potentially three edges common between the subgraphs induced by $S\cup \{i,j,k\}$ and  $S\cup \{i,j,k\}$ for a cyclic subgraph, and two for an acyclic one.
%  Thus we can show that the remainder is the same order as $O(\mathcal{M}(n,\rho_n,R))$.




% For each summand, since $\mathbb{E}[\w] = 1$, it is now clear that the conditional expectation with respect to a set $A$ is $0$ if  $\{i_1, \ldots i_r\} \cap A = \emptyset$.  We may collect summands with a nonempty intersection, leading to the expressions:
% \begin{align*}
%  T_{\{\xi_i\}} = \left(\xi_i - 1 \right) \cdot \frac{{n-1 \choose r-1}}{{n \choose r}} \cdot \left[\frac{1}{{n-1 \choose r-1}} \sum_{i, i_2 < \ldots < i_r, i_u \neq i } \left( H(A_{i, i_2, \ldots, i_r}^{(n)}) - \hat{T}_n \right)\right]     
% \end{align*}

% \begin{align*}
%  T_{\{\xi_i, \xi_j \}}  &= \left(\xi_i \cdot \xi_j + \xi_i + \xi_j - 1 \right) \cdot \frac{{n-2 \choose r-2}}{{n \choose r}} \cdot \left[\frac{1}{{n-2 \choose r-2}} \sum_{i,j i_3 < \ldots < i_r, i_u \neq i,j } \left( H(A_{i,j,i_3, \ldots, i_r}^{(n)}) - \hat{T}_n \right)\right]
%  \\  & \ \ \ + (\xi_i-1) \cdot T_{\xi_i} + (\xi_i-1) \cdot T_{\xi_j}
% \end{align*}



% For any set set $S$ of $r$ nodes, $S=\{i_{1}\dots i_{r}\}$, denote $\W_S= \prod_{i \in S} \w_i$.
% Conditioned on the graph $A$ and $X$, we see that the hoeffding projections of the weighted bootstrap statistic gives: %the $X$ observed as $x$, $\tnt$ and $\hat{H}(x_i)$ for each $i$ are all observed.  $\hat{H}(x_i)$ is defined as
% \begin{equation*}
%     \begin{split}
%      &\hi= \frac{1}{{n-1 \choose r-1}}\sum_{S,i\in S}H(A_S), \\
%      &\hhij= \frac{1}{{n-2 \choose r-2}}\sum_{S,i,j\in S}H(A_S).
% \end{split}
% \end{equation*}
% Recall the definition of $\gi$ and $\gj$ from the main paper. To remind the reader, we have:

% \begin{equation*}
%     \begin{split}
%      &\gi= \frac{1}{{n-1 \choose r-1}}\sum_{S,i\in S}(H(A_S)-\tnhat), \\
%      &\ggij= \frac{1}{{n-2 \choose r-2}}\sum_{S,i,j\in S}(H(A_S)-\tnhat).
% \end{split}
% \end{equation*}

% We are interested in the Hoeffding decomposition [\rd Put eqn number from main \bk] of the following quantity. Below we derive the Hoeffding decomposition.
% %We define weighted boostrap of count statistic as $\vnhat$. Conditioned on A, Standardized $\vnhat$ can be written as follows using $\W_S=1$.
% \begin{equation}\label{eq:wb-def-vn}
%     \begin{split}
%         \frac{\vnhat-\tnhat}{\hat{\sigma}_n}&=\frac{\sum_S \W_S (\hat{H}(A_S)-\tnhat)}{{n \choose r} \hat{\sigma}_n} = \frac{\sum_S (\W_S-1)(\hat{H}(A_S)-\tnhat)}{{n \choose r} \hat{\sigma}_n} \\
%         &=\frac{r}{n\hat{\sigma}_n} \sum_i f_1(\w_i) + \frac{r(r-1)}{n(n-1)\hat{\sigma}_n} \sum_{1\leq i<j \leq n} f_2(\w_i,\w_j) + \rd R_n \bk.
%     \end{split}
% \end{equation}

% We now derive the Hoeffding projections.

% Applying a Hoeffding decompsition to $\sum_S (\W_S-1)(\hat{H}(A_S)-\tnhat)/{n \choose r}$ above with respect to $\W$ yields

% \begin{equation*}
%     \begin{split}
%       & f_1(\w_i)= E[\hat{H}(X_S,\\W_S)\mid \w_i,x_i]; \\
%       & f_2(\w_i,w_j)=E[\hat{H}(X_S,\\W_S)\mid \w_i,x_i,\w_j,x_j].
%     \end{split}
% \end{equation*}
% Equivalently , $g_1(x_i)$ and $g_2(x_i,x_j)$ can be written as 
% \begin{equation}
% \begin{split}
%     f_1(\w_i)&=E[\W_S (\hat{H}(A_S)-\tnhat)\mid \w_i]= (\w_i-1)(\hi-\tnhat)=(\w_i-1)\gi;\notag\\
%     f_2(\w_i,\w_j)&=E[\W_S (\hat{H}(A_S)-\tnhat)\mid \w_i,\w_j] \notag\\
%     &=(\w_i\w_j-\w_i-\w_j+1)(\hhij-\tnhat)\notag\\
%     &=(\w_i\w_j-1)(\hhij-\tnhat)-(\w_i-1)(\hi-\tnhat)-(\w_j-1)(\hj-\tnhat),\label{eq:wb-hp}
% \end{split}
% \end{equation}

% \rd The residual $R_n$ is essentially a sum of higher order Hoeffding projections, which are all uncorrelated. Therefore, we see that the variance of the third order term (the first one in the remainder) is $\dfrac{\sum_{ijk}  \hat{g}_3(i,j,k)^2}{\hat{\sigma}_n^2 {n\choose 3}} \times O(1/n^3)$. Note that  $\hat{g}_3(i,j,k)^2=O_P(\rho_n^{3s-3})$ for cyclic and $O_P(\rho_n^{3s-2})$ for acyclic subgraphs. This is because, for any two nonoverlapping $S,T$ (not containing $\{i,j,k\}$)  of size $r-3$, there are potentially three edges common between the subgraphs induced by $S\cup \{i,j,k\}$ and  $S\cup \{i,j,k\}$ for a cyclic subgraph, and two for an acyclic one.
% Thus we can show that the remainder is the same order as $O(\mathcal{M}(n,\rho_n,R))$.


%\subsection{Edgeworth Expansion for Unweighted Boostrap}
% \section{\large{Edgeworth Expansion for Standardized Count Statistic}}
% In a size $n$ graph $\mathcal{G}_n$, define $\tnhat$ as normalized count statistic for a $r$-node $d$-edge subgraph $R$ with vertex set $V(R) $ and edge set $E(R)$.  For any set of $r$ nodes $S=\{X_{i_1},,,X_{i_r}\}$, denote
% \begin{equation*}
%     H(A_S)=  \prod_{(i_i,i_j)\in E(R)} A_{i_ii_j} ,
% \end{equation*}
% \begin{equation*}
%     h(X_{i_1},...,X_{i_r})=  \prod_{(i_i,i_j)\in E(R)} E(A_{i_ii_j}) =\prod_{(i_i,i_j)\in E(R)} \rho_n  w(X_{i_i},X_{i_j}) \wedge 1.
% \end{equation*}
% Then, $\tnhat$ can be written as 
% %Let $Iso(R)$ denote the class of graphs isomorphic to $R$, and $| Iso(R)|$ its cardinality. Then,
% %\begin{equation*}
% %\tnhat=\rho_n^{-d} \frac{1}{{n \choose p} \ |\mathrm{Iso}(R)| } \sum_{S \sim R} \mathbbm{1}(S = G_n[S])
% %\end{equation*}
% %Equivalently, we can also write $\tnhat$ as 

% \begin{equation*}
%     \tnhat= \frac{1}{{n \choose r}}\sum_{1\leq i_1<...<i_r\leq n} H(X_{i_1},,,X_{i_r}).
% \end{equation*}


% Let $T_n= E[\tnhat|\mathbf{X}]$ and $\theta=E[T_n]$. $T_n$ is a noiseless U-statistic with kernel function $h$. 
% \begin{equation*}
%      T_n= \frac{1}{{n \choose r}}\sum_{1\leq i_1<...<i_r\leq n} h(X_{i_1},,,X_{i_r}).
% \end{equation*}

% Define 
% \begin{equation*}
%     \begin{split}
%         & h_1(X_1)= E[h(X_1,X_2,,,X_r)\mid X_1=x_1];\\
%         & h_2(X_1,X_2)= E[h(X_1,X_2,,,X_r)\mid X_1=x_1,X_2=x_2].
%     \end{split}
% \end{equation*}
% Applying Hoeffding's decompsition of U-statistic \citep{hoeffding1992class} to $T_n$ yields 
% \begin{equation*}
%     T_n -\theta = \frac{r}{n}\sum_{i=1}^ng_1(X_i)+ \frac{r(r-1)}{n(n-1)}\sum_{1\leq i <j \leq n}g_2(X_i,X_j) + O_P(\rho_n^{d}n^{-1}),
% \end{equation*}
% where 
% \begin{equation}\label{eq:g1g2}
% \begin{split}
%     &g_1(X_i)= h_1(X_i)-\theta , \\
%     &g_2(X_i,X_j)= h_2(X_i,X_j) - \theta -g_1(X_1)-g_2(X_2) .
% \end{split}
% \end{equation}

% In addition, we define 
% \begin{align*}
%     \tau^2= \var(g_1(\mathbf{X})), \ \ \
%      \tilde{\tau_n} ^2= \frac{r^2}{n}\tau^2, \ \ \
%      \sigma_n^2 = \var(\tnt) .
% \end{align*}

% % U-stats hf decomp
% \rd I am removing $\tnhat$ because we don't use it in main paper and I think the shorthand may be a bit confusing  \bk


% % standardized form of $\tnhat$, denoting as $\tnt$,
% % \begin{equation*}
% %     \tnt = \frac{\tnhat - \mu_n}{\sigma_n}.
% % \end{equation*}
% \begin{theorem}\label{thm:ew-sd}
% % Edgeworth Expansion for $\tnt$. 

% Define \\
% \begin{equation*}
%     G_n(u)= \Phi(u)- \phi(u)\frac{(u^2-1)}{6n^{1/2}\tau^3}\{E[g_1^3(X_1)]+3(r-1)E[g_1(X_1)g_1(X_2)g_2(X_1,X_2)]\},
% \end{equation*}
% where $\Phi(u)$ and $\phi(x)$ denotes the CDF and PDF of standard Gaussian distribution. \rd For $\rho_n = O_P ((\log n)^{-1})$, and $\rho_n= \omega(n^{-1/2})$ for acyclic R and $\rho_n= \omega(n^{-1/r})$ for cyclic R.
% \bk  we have,
% \begin{equation*}
%     \sup_u \bigg{|} F_{\tnt}(u)-G_n(u)\bigg{|} = O(\mathcal{M}(n,\rho_n,R)).
% \end{equation*}
% \end{theorem}

Consider any term $\hat{g}_u(1,\dots,u)$. We will now bound $\E[\hat{g}_u(1,\dots,u)^2]$.
\begin{align*}
    \E[\hat{g}_u(1,\dots,u)^2]\leq 2(\var(\hat{g}_u(1,\dots,u))+\underbrace{\var(\tnhat)}_{O(\rho_n^{2s}/n)})
\end{align*}
The bound on the second term follows from~\cite{Bickel-Chen-Levina-method-of-moments} and will be smaller than that of the first term.
Let $\mathcal{S}_{r,u}$ denote all subsets of size $r-u$, not containing $1,\dots u$. For any subset $S\in \mathcal{S}_{r,u}$, also define, $S_u=S\cup \{1,\dots,u\}$.
For the first part, we have:
\begin{align*}
    \var(\hat{g}_u(1,\dots,u))=\frac{\sum_{S,T\in \mathcal{S}_{r,u}}\cov(H(A_{S_u}),H(A_{T_u}))}{{n-u\choose r-u}^2}
\end{align*}
Note that the dominating term here will indeed be the one where $|S\cap T|=0$. Number of such terms is ${n\choose 2r-u}$. Also the covariance of those terms will be $\rho_n^{2s-E(A_{1,\dots,u})}$, where $E(A_{1,\dots,u})$ denotes the intersection of the edgeset of $A_{1,\dots,u}$ and the subgraph we are counting. This number can be at most $u-1$ for acyclic $R$ and $u$ for cyclic $R$. For $|S\cap T|=k$, the number of terms is ${n\choose 2r-2u-k}$ and the exponent on $\rho_n$ is at most $2s-(u+k-1)$. Thus, for an acyclic subgraph, we have,
\begin{align*}
    \var(\hat{g}_u(1,\dots,u))&\leq \frac{\sum_{k=0}^r {n\choose 2r-2u-k}\rho_n^{2s-(u+k-1)}}{{n-u\choose r-u}^2}\\
    &\leq \sum_{k=0}^r n^{-k}\rho_n^{2s-(u+k-1)}=\rho_n^{2s-(u-1)}\left(1+\sum_{k>0}\frac{1}{(n\rho_n)^k}\right)
\end{align*}
The cyclic one is worse by a factor of $\rho_n$.
Thus the contribution of the $u^{th}$ element of the Hoeffding decomposition is 
\begin{align*}
    n\cdot \frac{\sum_{i_1,\dots, i_u} \hat{g}_u(i_1,\dots,i_u)^2}{{n\choose u}^2 \hat{\tau}_n^2}&=\begin{cases}O_P\left(\frac{1}{(n\rho_n)^{u-1}}\right)&\mbox{$R$ acyclic}\\
    O_P\left(\frac{\rho_n^{-1}}{(n\rho_n)^{u-1}}\right)&\mbox{$R$ cyclic}\end{cases}
\end{align*}

This shows that the third term contributes the most to $R_n$ in Eq~\ref{eq:hofftnm}.  By Markov's inequality, and the definition of $O_P(.)$ notation, it is easy to see that $R_n=O_P(\delta(n,\rho_n,R))$. 
\end{proof}


==> network_mb_jasa_to_arxiv (1)/cicoverage.tex <==
So far, we have proposed a family of bootstrapped methods for standardized count functionals of networks. Note that studentized statistics are typically preferred because they produce higher order correct confidence intervals. However it is well known~\citep{hall-bootstrap-edgeworth} that in many situations like correlation coefficients,  pivoting may not be suitable, because the variance estimate can be unstable. On the other hand, standardized bootstrap procedures produce first order correct confidence intervals. In this section, we show how to correct these intervals to get higher order coverage. \bk


From our proposed bootstrap, we construct a two-sided confidence interval with nominal coverage $\alpha$ $\mathcal{I}_1=\left(\hat{y}_{\frac{1-\alpha}{2}},\hat{y}_{\frac{1+\alpha}{2}}\right)$,
%\begin{align}\label{eq:cifirst}
 %   \mathcal{I}_1=\left(\hat{y}_{\frac{1-\alpha}{2}},\hat{y}_{\frac{1+\alpha}{2}}\right),
%\end{align}
where we define function $\hat{L}(t)=P(\hat{T}_n^* < t \mid  A,X)$ for bootstrap samples $\{\hat{T}^*_n\}$, and $\hat{y}_\alpha=\hat{L}^{-1}(\alpha)$.
Let $z_{\alpha}$ denote standard normal critical point at $\alpha$ where $\Phi(z_{\alpha})=\alpha$, then $\hat{y}_\alpha=\hat{L}^{-1}(\Phi(z_{\alpha}))$.
%Coverage error of a confidence interval is the difference of its true coverage and nominal coverage, $P(\theta \in \mathcal{I}_1)-\alpha$. %First-order correct CIs have coverage error of order $O(n^{-1/2})$, whereas second-order correct CIs have coverage error of $O(n^{-1})$. 
%A confidence interval is first-order correct if its coverage error is of order $O(n^{-1/2})$, but is second-order correct if its coverage error is of order $O(n^{-1})$. Alternatively, 
Equivalently, define $\hat{u}_{\alpha}$ as the critical point at $\alpha$ for standardized bootstrap sample $(\hat{T}^*_n-\hat{T}_n)/\hat{\sigma}_n$ distribution and $\hat{v}_{\alpha}$ as the critical point at $\alpha$ for studentized bootstrap sample $(\hat{T}^*_n-\hat{T}_n)/\hat{\sigma}^*_n$ distribution.
Standardized and studentized bootstrap CIs  $\mathcal{I}_1$ and  $\mathcal{I}_2$ can be written as 
\begin{align*}
    &\mathcal{I}_1=(\hat{T}_n+n^{-1/2}\hat{\sigma}_n\hat{u}_{\frac{1-\alpha}{2}},\hat{T}_n+n^{-1/2}\hat{\sigma}_n\hat{u}_{\frac{1+\alpha}{2}}) ,\\
    &\mathcal{I}_2=(\hat{T}_n+n^{-1/2}\hat{\sigma}_n\hat{v}_{\frac{1-\alpha}{2}},\hat{T}_n+n^{-1/2}\hat{\sigma}_n\hat{v}_{\frac{1+\alpha}{2}}).
\end{align*}

$\mathcal{I}_1$ and  $\mathcal{I}_2$ are bootstrap estimates of theoretical $\alpha$ coverage percentile CIs $\mathcal{J}_1$ and $\mathcal{J}_2$ respectively,
\begin{align*}
     &\mathcal{J}_1=(\hat{T}_n+n^{-1/2}\sigma_nu_{\frac{1-\alpha}{2}},\hat{T}_n+n^{-1/2}\sigma_nu_{\frac{1+\alpha}{2}}) ,\\
    &\mathcal{J}_2=(\hat{T}_n+n^{-1/2}\hat{\sigma}_n v_{\frac{1-\alpha}{2}},\hat{T}_n+n^{-1/2}\hat{\sigma}_n v_{\frac{1+\alpha}{2}}),
\end{align*}
where $u_{\alpha}$ is the critical point at $\alpha$ of the distribution for $(\hat{T}_n-T_n)/\sigma_n$ and $v_{\alpha}$  is the critical point at $\alpha$ of the distribution for $(\hat{T}_n-T_n)/\hat{\sigma}_n$.
Our standardized bootstrap confidence interval $\mathcal{I}_1$ is only first-order correct, as the end points of $\mathcal{I}_1$ differ from  $\mathcal{J}_1$ by $O(n^{-1})$ (or equivalently, they agree only to and including terms of order $O(n^{-1/2})$). In contrast, studentized bootstrap confidence interval $\mathcal{I}_2$ is second-order correct; the end points of $\mathcal{I}_2$ differs from  $\mathcal{J}_2$ by $O(n^{-3/2})$.   However, $\mathcal{I}_1$ can be shifted to be second-order correct as follows:% (also see~\cite{hall-bootstrap-edgeworth}). %\cite{hall-bootstrap-edgeworth} Section 3.10 gives an explicit form of shifting $\mathcal{I}_1$ to $\mathcal{I}'_1$ and $\mathcal{I}'_1$ is second-order correct. 
\begin{align}\label{eq:ci-correction}
    \mathcal{I}'_1 = \left(\hat{y}_{\frac{1-\alpha}{2}}+n^{-1}\hat{\sigma}\left\{\hat{p}_1(z_{\frac{1-\alpha}{2}})+\hat{q}_1(z_{\frac{1-\alpha}{2}})\right\},\  \hat{y}_{\frac{1+\alpha}{2}}+n^{-1}\hat{\sigma}\left\{\hat{p}_1(z_{\frac{1+\alpha}{2}})+\hat{q}_1(z_{\frac{1+\alpha}{2}})\right\} \right)
\end{align}
where for any $x \in \mathbb{R}$, $\hat{p}_1(x)$ and   $\hat{q}_1(x)$ are estimates for $p_1(x)$ and $q_1(x)$. $p_1(x)$ is polynomial coefficient of $n^{-1/2}\phi(x)$ in standardized Edgeworth Expansion $G_n(x)$ developed in Eq~\ref{eq:edgeworth-gn} and $q_1(x)$ is the polynomial in front of $n^{-1/2}\phi(x)$ in studentized Edgeworth Expansion $G_n'(x)$ developed in previous work. Therefore, we can write
\begin{align*}
    &\hat{p}_1(\mathit{z}_{\alpha})= \frac{(1-\mathit{z}_{\alpha}^2)}{6\hat{\tau}_n^3}\biggl[\mathbb{E}\{\hat{g}_1^3(X_1)\}+3(r-1)\mathbb{E}\{\hat{g}_1(X_1)\hat{g}_1(X_2)\hat{g}_2(X_1,X_2)\} \biggr], \\
    &\hat{q}_1(\mathit{z}_{\alpha})=\frac{1}{\hat{\tau}_n^3}\biggl[\frac{2\mathit{z}_{\alpha}^2+1}{6}\mathbb{E}\{\hat{g}_1^3(X_1)\}+\frac{r-1}{2}(\mathit{z}_{\alpha}^2+1)\mathbb{E}\{\hat{g}_1(X_1)\hat{g}_1(X_2)\hat{g}_2(X_1,X_2)\} \biggr].
\end{align*}

\rd 
Now, for smooth functions of conditional expectation of count functionals, we have derived $\sigma$ and $p_1(x)$ in Section~\ref{sec:smf}. % needed for correction.
We now present the form of $q_1(x)$ for the studentized version of this. Define the studentized functional $S_n'=n^{1/2}(f(\bu)-f(\bmu))/\hat{\sigma}$, where $\bu$ and $\bmu$ are defined as the conditional and unconditional expectations of the count statistics. We use this form to correct our confidence intervals.
\bk

The derivation of $q_1$ is much more complicated than deriving $p_1$, since one needs to append to $\bu$ more terms so that the variance of $f(\bu)$ can be written as a function of the elongated mean vector $E[\bu]$. For example, for estimating mean of i.i.d univariate random variables one will use a two dimensional vector $(x_1,x_2)$ with $x_1=X_i$ and $x_2=X_i^2$. for smooth functions of count  statistics the variance of the smooth function of $f(\bu)$ is $\sigma^2/n$, where $\sigma$ is given in Eq~\ref{eq:p1sigma}. In order to write this as a function of $\bmu$, we create the following mean vector.

\begin{equation*}
\begin{split}
   \cbu=\bigg{\{}\underbrace{\frac{\tnt{(1)}}{\rho_n^{s_1}},\ldots, \frac{\tnt{(d)}}{\rho_n^{s_d}}}_{d \text{ terms}},\underbrace{\frac{r_1r_2\sum_{i=1}^n\hat{h}_1^{(1)}(X_i)\hat{h}_1^{(2)}(X_i)}{n\rho_n^{s_1}\rho_n^{s_2}},\ldots,\frac{r_{d-1}r_d\sum_{i=1}^n\hat{h}_1^{(d-1)}(X_i)\hat{h}_1^{(d)}(X_i)}{n\rho_n^{s_1}\rho_n^{s_2}}}_{{d \choose 2} \text{ terms}},\\
   \underbrace{\frac{r_1^2\sum_{i=1}^n\hat{h}_1^{(1)}(X_i)^2}{n\rho_n^{2s_1}},\ldots,\frac{r_d^2\sum_{i=1}^n\hat{h}_1^{(d)}(X_i)^2}{n\rho_n^{2s_d}}}_{d \text{ terms}}\bigg{\}}, 
\end{split}
\end{equation*}
where $\hat{h}_1(X_i)$ is given by:
\begin{align*}
    \hat{h}_1(X_i)=\frac{1}{{n-1 \choose r-1}}\sum_{1\leq i_1<\ldots< i_r\leq n, i_1,\ldots,i_r \neq i } \hat{h}(X_i,X_{i_1},\ldots,X_{i_r}).
\end{align*}

Under similar conditions required to establish the Edgeworth expansion of Eq~\ref{eq:EW-SMF}, we have
 \begin{align*}
    P(S_n' < x) = \Phi(x) + n^{-1/2}q_1(x)\phi(x) + o\left(n^{-1/2}\right),
\end{align*}
\begin{align*}
    q_1(x)=-\{B_1+\frac{1}{6}B_2(x^2-1)\},
    \end{align*}
    where 
    \begin{align}
        B_1= A_1\sigma^{-1}-\frac{1}{2}\sigma^{-3}n\sum_{i=1}^{d'}\sum_{j=1}^{d'}a_ic_j\E\{(\cbu-\cbmu)^{(i)}(\cbu-\cbmu)^{(j)}\}.
    \end{align}
   % We provide the form of $B_1$ explicitly in Supplementary Section~ \ref{sec:supp:proof-smf-ew-stu-and-ci-abc}. 
   Note that the CDF of the studentized and standardized statistics match at $x=0$, i.e. $p_1(0)=q_1(0)$. Hence one can estimate $B_2$ if $A_1,A_2$, and $B_1$ are available.
    
    Estimating the moments in the above expression requires one to expand out the expression and we do this in detail in the Supplement Section~\ref{sec:supp:proof-smf-ew-stu-and-ci-abc}.
    
    
    In the following figures we compare the absolute deviation of the empirical Edgeworth expansion of the transitivity coefficient from the true distribution with that of the Gaussian approximation for the \smg graphon. It is easy to see that the Edgeworth expansion is much more accurate than the Gaussian approximation.
    
    \begin{figure}[h]
%\vskip 0.2in
\centering
%\text{no log}\\
\begin{tabular}{c}
    \includegraphics[width=  0.4\textwidth]{plots2/Smg-p1-error.pdf} 
     \includegraphics[width=  0.4\textwidth]{plots2/Smg-q1-error.pdf}
  %   \vspace{-2em}
     %  \includegraphics[trim=0em 1em 0em 5em, clip, width=  \textwidth]{plots/EW-MB-trans-nobar.pdf}
  %     \vspace{-1em}
    %\vspace{-4em}
%    \includegraphics[width=  0.8\textwidth,height=0.4\textwidth]{plots/EW-MB-twostars-nobar.pdf}\\
\end{tabular}
%\\\vspace{5mm}\text{taking log}\\
%\begin{tabular}{c}
%    \includegraphics[width=  0.4\textwidth]{plots2/sbm-triangles-log.pdf} 
%    \includegraphics[width=  0.4\textwidth]{plots2/ng2-triangles-log.pdf}\\
%    \includegraphics[width=  0.4\textwidth]{plots2/sbm-triangles-centerbytnhat-log.pdf}\includegraphics[width=  0.4\textwidth]{plots2/ng2-triangles-centerbytnhat-log.pdf}
  %   \vspace{-2em}
     %  \includegraphics[trim=0em 1em 0em 5em, clip, width=  \textwidth]{plots/EW-MB-trans-nobar.pdf}
  %     \vspace{-1em}
    %\vspace{-4em}
%    \includegraphics[width=  0.8\textwidth,height=0.4\textwidth]{plots/EW-MB-twostars-nobar.pdf}\\
%\end{tabular}
 \caption{\rd Standardized and studentized transitivity: Y axis is absolute error $|Fn(u) - F^*(u)|$ of CDFs, X axis is  X axis is $u$ $\in$ $[-3:3]$. Left is absolute error of standardized Edgeworth expansion to standardized truth compare to absolute error of N(0,1) to standardized truth. Right is absolute error of studentized Edgeworth expansion to studentized truth compared with absolute error of N(0,1) to studentized truth. }.
%\begin{center}
\label{fig:cdf-error}
\end{figure}
\rd
In the Supplement, we also provide a table for different statistics like linear combinations of triangle and two star densities, the product of triangle and two-star densities, the product of the squares of triangle and two-star densities. The general observation is that if the derivatives $a_i,a_{ij}$ have to be estimated from data, then the error of the empirical Edgeworth gets worse.
\bk
%The explicit form of $B_1$ and $B_2$ are provided in Supplementary Section~ \ref{sec:supp:proof-smf-ew-stu-and-ci-abc}. 
\iffalse
However, because of the complicated expressions of parameters $A_1$,  $A_2$, $B_1$, $B_2$, instead of directly using Eq~\ref{eq:ci-correction}, we use an alternative but equivalent bias correction for the confidence interval proposed by \cite{efron-better-ci}, the accelerated bias correction. The corrected confidence $\mathcal{I}''_1$ is 
\begin{align}\label{eq:ci-correction-abc}
    &\mathcal{I}''_1=(\hat{y}_{\mathrm{ABC},\frac{1+\alpha}{2}},\ \hat{y}_{\mathrm{ABC},1-\frac{1+\alpha}{2}}),
    \end{align}
with $\hat{y}_{\mathrm{ABC},\alpha}$ defined as
    \begin{align*}
    &\hat{y}_{\mathrm{ABC},\alpha}=\hat{L}^{-1}\left(\Phi\left[\hat{m}+(\hat{m}+z_{\alpha})\{1-\hat{a}(\hat{m}+z_{\alpha})\}^{-1}\right]\right),
\end{align*}
where $\hat{m}$ and $\hat{a}$ for $d$-dimensional smooth function of count functionals are
\begin{equation}\label{eq:ci-correction-abc-mhat}
    \hat{m}=\hat{L}^{-1}(\hat{T}_n)= n^{-1/2}\hat{p}_1(0),
    \end{equation}
    \begin{equation}\label{eq:ci-correction-abc-ahat}
    %\hat{a}=\frac{\hat{\sigma}^{-3}}{6n^{1/2}}\sum_{i=1}^d\sum_{j=1}^d\sum_{k=1}^d\hat{a}_i\hat{a}_j\hat{a}_k\hat{\lm}_{ijk}.%+O(n^{-1}).
     \hat{a}=n^{-1/2}\frac{1}{6} \left\{-(\hat{A}_2\hat{\sigma}^{-3}+\hat{B}_2)\right\}.
    \end{equation}
%and $A$ for $d$-dimensional smooth function of count functionals is 
%\begin{align}
%    \hat{A}=\frac{r^3}{n^{3/2}}\sum_{i=1}^d\sum_{j=1}^d\sum_{k=1}^da_ia_ja_k\bu_L^{(i)}\bu_L^{(j)}\bu_L^{(k)}+O\left(\frac{1}{n}\right).
%\end{align}
Calculation and proof of Eq~??? is provided in detail in Supplementary Section~\ref{sec:supp:sub-ci-abc}.  
\fi
\bk

==> network_mb_jasa_to_arxiv (1)/conc.tex <==
%\section{Conclusion}
%\rd In this paper we have proposed a new multiplicative bootstrap (\mbm) method, and its faster variants, which use additive (\mbl) and quadratic (\mbq) weights. We have established that $\mbm$ and $\mbq$ are both  higher-order correct under certain sparsity conditions. We have shown that the empirical Edgeworth expansion (\ew) is perhaps the fastest and most accurate way of estimating the CDF of a count statistic. However, deriving an \ew for more general functions of count functionals like transitivity requires intricate analysis, whereas resampling or subsampling methods automatically adapt to the underlying distribution. While we do not present theory for this, our simulations suggest that indeed, bootstrap-based methods can be  higher-order correct for smooth functions. Among competing methods, a close contender is the empirical graphon (\eg), which is orders of magnitude slower than our fast multiplier bootstrap \mbq.

% \rd
% In this paper, we focus on the multiplier bootstrap for inferring network count functionals. The bootstrap procedure perturbs a potential subgraph by the product of independent multiplier random variables.  We also present the linear and quadratic bootstrap, which can be seen as different orders of approximations of the Hoeffding decomposition of the statistic arising from the multiplier bootstrap. We show that the quadratic bootstrap is higher-order correct but slower whereas the linear bootstrap is first order correct but faster. As a side product of our analysis, we derive an empirical edgeworth expansion which has the lowest error for dense networks. Empirically, we show that for sparse degree regimes, the linear bootstrap in fact provides better accuracy since the higher-order correct methods directly or indirectly involve estimation of higher-order moments which may not be accurately estimated under sparsity. To truly harness the computational power of the linear bootstrap, we also present and analyze an approximate bootstrap method which uses randomized sketching algorithms for estimating local network counts which are used by the linear method. Finally, we derive the Edgeworth expansion for smooth funcitons of the conditional expectation of subgraph counts, and show that the Edgeworth expansion of our higher-order correct bootstrap methods  are suitably close to the former population counterpart.
% \bk
In this paper, we propose a family of multiplier bootstraps for network count functionals.  %Our multiplicative proposal involves perturbing a potential subgraph by the product of independent multiplier random variables.  
For large sparse graphs, we  present and analyze an approximate linear bootstrap method that uses randomized sketching algorithms for subgraph counting.  Our theoretical results establish a phase transition phenomena in which different computational regimes lead to limiting behavior. We also present the quadratic bootstrap, which is higher-order correct for moderately sparse graphs; therefore, this method offers a computationally feasible alternative for smaller graphs where accuracy is paramount. For the first time in the literature, we also derive Edgeworth expansions for smooth functions of counts.  %Empirically, we observe an interesting phenomenon in which the linear bootstrap, which is not higher-order correct in any regime, performs better than other methods for sparse graphs since the higher-order correct methods directly or indirectly involve estimation of higher-order moments that may not be accurately estimated under sparsity. 
Taken together, we establish the multiplier bootstrap as a user-friendly, automatic procedure that can be tailored to yield higher-order correctness or scalable and consistent inference.  
\bk

==> network_mb_jasa_to_arxiv (1)/exp4.tex <==
Here we provide simulated and real data examples demonstrating the effectiveness of our methods.
\subsection{Simulation study}
\label{sec:sim}
We consider two graphons in our simulation study. The first graphon we consider is a Stochastic Blockmodel (SBM), introduced by \cite{holland-sbm}. The SBM is a popular model for generating networks with community structure. The SBM may be parameterized by a $K \times K$ probability matrix $B$ and a membership probability vector $\pi$ that takes values in the probability simplex in $\mathbb{R}^K$. Let $Y_1, \ldots Y_n \in \{1, \ldots, K\}$ be random variables indicating the community membership of the corresponding node, with probability given by the entries of $\pi$. Under this model, we have that $P(A_{ij}^{(n)} = 1 \ \mid \ Y_i = u, Y_j = v) = \rho_n B_{uv}$.  In our simulations, we consider a two block SBM (\sbm) with $B_{ij}=0.6$ for $i=1,j=1$ and $0.2$ for the rest, with $\pi=(0.65, 0.35)$.
%
\iffalse
\begin{figure}\centering
\begin{tikzpicture}[zoomboxarray,  zoomboxarray inner gap=.5cm, zoomboxarray columns=1, zoomboxarray rows=1]
    \node [image node] { \includegraphics[width=0.4\textwidth]{plots2/sbm-triangles.pdf} };
   % \zoombox{0.175,0.9}
    \zoombox[magnification=2]{.15,.7}
   % \zoombox{0.15,0.3}
    %\zoombox[magnification=10]{0.86,0.35}
\end{tikzpicture}\\
\begin{tikzpicture}[zoomboxarray,  zoomboxarray inner gap=.5cm, zoomboxarray columns=1, zoomboxarray rows=1]
    \node [image node] { \includegraphics[width=0.4\textwidth]{plots2/sbm-triangles-centerbytnhat.pdf} };
   % \zoombox{0.175,0.9}
    \zoombox[magnification=2]{.15,.7}
   % \zoombox{0.15,0.3}
    %\zoombox[magnification=10]{0.86,0.35}
\end{tikzpicture}\\
\caption{\rd fill in \bk}
\end{figure}
\fi
We also do experiments on a smooth graphon model(\smg). For space considerations, additional experiments for the \sbm model and experimental results for the \smg model are deferred to Supplement Section~\ref{sec:addlexp}. %including  the $\sup$ of (absolute) difference of the bootstrap CDFs for two-star density and timing for four-cycles for this model are deferred to  Supplement Section~\ref{sec:addlexp}. \bk



 %We use the following as an approximation of the Kolmogorov distance between $F$ and $G$.
 %\begin{align*}
 %\text{err}(F,G)=\sup\limits_{x\in [-3,3]}|F(x)-G(x)|
 %\end{align*}  
 Define $\text{err}(F,G)$ as the maximum of $|F(x)-G(x)|$ over a grid on $[-3,3]$ with grid size $0.1$; this will serve as an approximation to the Kolmogorov distance between $F$ and $G$.  In order to study this error, we first need an estimate of the true CDF. \bk To this end, we conduct Monte Carlo simulations with $M$ samples generated from each model. Note that, since our goal is to show that the error is better than the Normal approximation, we need $M=\omega((n\rho_n)^2)$, which ensures that the error from the Monte Carlo samples is $o(1/n\rho_n)$.  To ease the computational burden, we perform simulations on small networks with $n=160$ nodes.  We generate $M=10^6$ Monte Carlo simulations, so that the higher-order correctness is not obscured by error from the simulations.   In addition to this, we also compare the coverage for different resampling methods in Figure~\ref{fig:coverage}, where we use $n=500$, since the true CDF does not have to be estimated. In this setting we estimate the true parameter of inferential interest from a 15000 node network. In the next subsection we show how to obtain higher-order correct confidence intervals.\bk

\subsection{Higher-order correct confidence intervals}
% So far, we have proposed a family of bootstrapped methods for standardized count functionals of networks.

%\rd In this paper, we have studied the properties of bootstrap methods for standardized count functionals of networks.  While our Edgeworth expansions establish that the standardized bootstrap is higher-order correct in the Kolmogorov norm, it is well known that corresponding confidence intervals do not offer refined accuracy over those formed from a Normal approximation; see \citet{hall-theoretical-comparison-bootstrap-ci}.  In contrast, studentized bootstraps produce higher-order correct confidence intervals. However it is also well-known that in many situations like correlation coefficients,  studentization may not be suitable because the variance estimate can be unstable ~\citep{hall-bootstrap-edgeworth}. In this section, we show how to correct standardized intervals to attain higher-order accuracy for coverage.  \bk

In this paper, we have studied the properties of bootstrap methods for standardized count functionals of networks.  While our Edgeworth expansions establish that the standardized bootstrap is higher-order correct in the Kolmogorov norm, in general that does not imply higher-order correct confidence intervals (see Chapter~3 page~93 of \citet{hall-theoretical-comparison-bootstrap-ci}). There are two approaches in the literature to deal with this issue, one is studentization and the other is using the bias-corrected standardized intervals.  While our theoretical results can be extended to studentized count functionals (see Remark \ref{remark:standardvsstudent}), it is well-known that for statistics such as correlation coefficients,  studentization may not be suitable because the variance estimate can be unstable ~\citep{hall-bootstrap-edgeworth}. 
Bias-corrected standardized CIs have been extensively investigated in other settings; see for example, \citet{efron-jackknife-resampling}, \citet{efron-better-ci}, and \citet{hall-theoretical-comparison-bootstrap-ci}. In this section, we show how to correct standardized intervals to attain higher-order accuracy for coverage.  \bk


% The (uncorrected) two-sided confidence interval for the standardized bootstrap \bk two-sided confidence interval with nominal coverage $\alpha$ is given by: $\mathcal{I}_1=\left(\hat{y}_{\frac{1-\alpha}{2}},\hat{y}_{\frac{1+\alpha}{2}}\right)$,
%%\begin{align}\label{eq:cifirst}
% %   \mathcal{I}_1=\left(\hat{y}_{\frac{1-\alpha}{2}},\hat{y}_{\frac{1+\alpha}{2}}\right),
%%\end{align}
%where we define function $\hat{L}(t)=P(\hat{T}_n^* < t \mid  A,X)$ for bootstrap samples $\{\hat{T}^*_n\}$ and $\hat{y}_\alpha=\hat{L}^{-1}(\alpha)$.
%Let $z_{\alpha}$ denote standard normal critical point at $\alpha$ where $\Phi(z_{\alpha})=\alpha$. %, then $\hat{y}_\alpha=\hat{L}^{-1}(\alpha)$.
%%Coverage error of a confidence interval is the difference of its true coverage and nominal coverage, $P(\theta \in \mathcal{I}_1)-\alpha$. %First-order correct CIs have coverage error of order $O(n^{-1/2})$, whereas second-order correct CIs have coverage error of $O(n^{-1})$. 
%%A confidence interval is first-order correct if its coverage error is of order $O(n^{-1/2})$, but is second-order correct if its coverage error is of order $O(n^{-1})$. Alternatively, 
%Equivalently, define $\hat{u}_{\alpha}$ as the critical point at $\alpha$ for standardized bootstrap sample $(\hat{T}^*_n-\hat{T}_n)/\hat{\sigma}_n$ distribution and $\hat{v}_{\alpha}$ as the critical point at $\alpha$ for studentized bootstrap sample $(\hat{T}^*_n-\hat{T}_n)/\hat{\sigma}^*_n$ distribution. The
% standardized  bootstrap CI $\mathcal{I}_1$  can be written as 
%\begin{align*}
%    &\mathcal{I}_1=(\hat{T}_n+n^{-1/2}\hat{\sigma}_n\hat{u}_{\frac{1-\alpha}{2}},\hat{T}_n+n^{-1/2}\hat{\sigma}_n\hat{u}_{\frac{1+\alpha}{2}}).
% %   &\mathcal{I}_2=(\hat{T}_n+n^{-1/2}\hat{\sigma}_n\hat{v}_{\frac{1-\alpha}{2}},\hat{T}_n+n^{-1/2}\hat{\sigma}_n\hat{v}_{\frac{1+\alpha}{2}}).
%\end{align*}
%Since the population version of $\mathcal I_1$ involves the true $\sigma_n$ instead of $\hat{\sigma}_n$, it follows that $\sigma_n - \hat{\sigma}_n$ is too large of a perturbation for higher-order correctness to hold.  


We define function $\hat{L}(t)=P(\hat{T}_n^* < t \mid  A,X)$ for bootstrap samples $\{\hat{T}^*_n\}$ and for nominal coverage $\alpha$. Let $z_{\alpha}$ denote the standard normal critical point, and let $\hat{y}_\alpha=\hat{L}^{-1}(\alpha)$. %In order to make the CI identical to the studentized CI (and thus be higher order correct), 
Our bias-corrected standardized CI is given as follows (see~\cite{hall-bootstrap-edgeworth} for more details):
\iffalse
%has to shift 
$\mathcal{I}_1$ and $\mathcal{I}_2$ are bootstrap estimates of theoretical $\alpha$ coverage percentile CIs $\mathcal{J}_1$ and $\mathcal{J}_2$ respectively,
\begin{align*}
     &\mathcal{J}_1=(\hat{T}_n+n^{-1/2}\sigma_nu_{\frac{1-\alpha}{2}},\hat{T}_n+n^{-1/2}\sigma_nu_{\frac{1+\alpha}{2}}) ,\\
    &\mathcal{J}_2=(\hat{T}_n+n^{-1/2}\hat{\sigma}_n v_{\frac{1-\alpha}{2}},\hat{T}_n+n^{-1/2}\hat{\sigma}_n v_{\frac{1+\alpha}{2}}),
\end{align*}
where $u_{\alpha}$ is the critical point at $\alpha$ of the distribution for $(\hat{T}_n-T_n)/\sigma_n$ and $v_{\alpha}$  is the critical point at $\alpha$ of the distribution for $(\hat{T}_n-T_n)/\hat{\sigma}_n$.
Our standardized bootstrap confidence interval $\mathcal{I}_1$ is only first-order correct, as the end points of $\mathcal{I}_1$ differ from  $\mathcal{J}_1$ by $O(n^{-1})$ (or equivalently, they agree only to and including terms of order $O(n^{-1/2})$). In contrast, studentized bootstrap confidence interval $\mathcal{I}_2$ is second-order correct; the end points of $\mathcal{I}_2$ differs from  $\mathcal{J}_2$ by $O(n^{-3/2})$. However, $\mathcal{I}_1$ can be shifted to be second-order correct as follows:% (also see~\cite{hall-bootstrap-edgeworth}). %\cite{hall-bootstrap-edgeworth} Section 3.10 gives an explicit form of shifting $\mathcal{I}_1$ to $\mathcal{I}'_1$ and $\mathcal{I}'_1$ is second-order correct. 
\fi
\begin{align}\label{eq:ci-correction}
    \mathcal{I}'_1 = \left(\hat{y}_{\frac{1-\alpha}{2}}+n^{-1}\hat{\sigma}_n\left\{\hat{p}_1(z_{\frac{1-\alpha}{2}})+\hat{q}_1(z_{\frac{1-\alpha}{2}})\right\},\  \hat{y}_{\frac{1+\alpha}{2}}+n^{-1}\hat{\sigma}_n\left\{\hat{p}_1(z_{\frac{1+\alpha}{2}})+\hat{q}_1(z_{\frac{1+\alpha}{2}})\right\} \right),
\end{align}
where for any $x \in \mathbb{R}$, $\hat{p}_1(x)$ and   $\hat{q}_1(x)$ are estimates for $p_1(x)$ and $q_1(x)$. Recall that $p_1(x)$ and $q_1(x)$ are polynomial coefficients of the second order term in the  Edgeworth expansions of the standardized and studentized statistic. % developed in Eq~\ref{eq:edgeworth-gn} and $q_1(x)$ is the polynomial in front of $n^{-1/2}\phi(x)$ in studentized Edgeworth Expansion $G_n'(x)$ developed in previous work. 


When the statistic is a count functional like the triangle or two-star density, then we already know the form of $p_1(x)$ and $q_1(x)$. For smooth functions of count statistics like the transitivity, we derive the standardized and studentized Edgeworth expansion for the smooth function of the corresponding U statistics in the Supplement Sections~\ref{sec:supp:sub-proof-smf-ew} and~\ref{sec:supp:proof-smf-ew-stu-and-ci} respectively.  We also show that the Edgeworth expansion of the bootstrapped smooth function converges to this population version in the Supplement Section~\ref{sec:supp:sub-proof-smf-bt-close-to-ew}. %\rd Qiao, please make sure these point to the smooth function EW and bootstrap convergence subsections \bk
\bk
\subsection{Competing methods}
We compare our algorithms with the following network resampling procedures. % discussed in Section \ref{sec:related-work}.  %In particular, we consider subsampling with subsample size $b_n = 0.5n$ (\sub), the empirical graphon with resample size $n$ (\eg), the latent space bootstrap (\ls), and the empirical Edgeworth expansion (\ew).  For the latent space bootstrap, we treat the latent dimension as known for \sbm \  and estimate the latent dimension for \smg \ using Universal Singular Value Thresholding (\usvt) procedure of \citet{chatterjee-usvt}. We provide a brief description of each algorithm below.

\textit{Empirical Graphon (\eg).} We draw $B$ size $n$ resamples $S_i^{*}$ with replacement from $1,\dots, n$.  We compute the count functional $\hat{T}_{n,i}^*$ on $A^{(n)}(S_i^*,S_i^*)$. We compute $\tnhat$ and $\hat{\sigma}_n^2$ on the whole graph. Now for triangles and two-stars we compute the CDF of $\{(\hat{T}_{n,i}^*-\tnhat)/\hat{\sigma}_n\}_{i=1}^B$. For functions of counts, we compute the function for each resampled graph, center using the function computed on the whole network.

\textit{Subsampling (\sub).} We draw $B$ size $b$ ($b=0.5n$) subsamples $S_i^{*}$ without replacement  from $1,\dots, n$ . We compute the count functional $\hat{T}_{b,i}^*$ on $A^{(n)}(S_i^*,S_i^*)$. We also compute $\tnhat$ and $\hat{\sigma}_n^2$ on the whole graph. We set $\hat{\sigma}_b^2=n/b\hat{\sigma}_n^2$. Now for triangles and two-stars we compute the CDF of $\{(\hat{T}_{b,i}^*-\tnhat)/\hat{\sigma}_b\}_{i=1}^B$. For functions of counts, we compute the function for each subsampled graph, center using the function computed on the whole network.

\newcommand{\bhx}{\hat{\boldsymbol{X}}}
\textit{Latent Space  (\ls).} We first estimate the latent variables $\hat{X}:=\{\hat{X}_1,\dots, \hat{X}_n\}$ from the given network. For \sbm, we use the true number of blocks. %whereas for smooth graphon \smg, we use the \usvt algorithm to estimate the number of latent variables. 
We compute $g_1(\hat{X}_i)$ for $i=1\dots n$, and then compute $T_n(\hat{X})=T_n(\hat{X}_1,\dots, \hat{X}_n)$. Now we simply use the additive variant of bootstrap $T_n(\hat{X})+\frac{r}{n}\sum_i (g_1(\hat{X}_i)-T_n(\hat{X}))$ (see~\cite{levin-levina-rdpg-bootstrap}). For triangles and two-stars, we normalize by the square root of $r^2/n\sum_i g_1(\hat{X}_i)^2$. For functions of counts, we center using the function computed on $\hat{X}$. 

%\rd add Kato : \\
%\bk


We compare the performance of the resampling methods for two-stars, triangles and a variant of the transitivity coefficient defined in Example 3 of \citet{Bhattacharyya-subsample-count-features}, which is essentially an appropriately defined ratio between triangles and two-stars. 


\subsection{Results}
 In Figure \ref{fig:cdf-error}, we plot the maximum of (absolute) difference of the bootstrap CDF $F_n^*$ over the $[-3,3]$ range  (\KL{$F_n$}{$F_n^*$}) for triangle density from the true CDF $F_n$ for sparsity parameter $\rho_n$ varying from $0.05$ to $1$.   We show the average of the expected difference over 30 independent runs along with error-bars. In this figure we see an interesting phenomenon. For sparse networks with $\rho_n\leq 0.2$, the linear method outperforms the higher-order correct methods. As the networks become denser, the higher-order correct methods start performing better. For $\rho_n\leq 0.2$, we also see that the empirical Edgeworth expansion performs worse than the linear bootstrap method.
 
 We also compare the bootstrap samples centered at the bootstrap mean (first row) with bootstrap samples centered at the subgraph density computed on the whole network. We see that the latest space method (LS) and approximate linear bootstrap method (\mblapx) behave differently under these two centerings, with LS performing much worse. This suggests that while both suffer from bias, LS suffers from it to a higher degree. For all parameter settings, we used $N=50\log n$. It is possible that increasing $N$ for sparser settings may lead to reduced bias of \mblapx.
 
 In Figure \ref{fig:coverage}, we show the coverage of  95\% bootstrap percentile CI with correction for triangles (left) and transitivity coefficient (right) of the \sbm model  in $\rho_n$ from $0.05$ to $1$. We simulate $200$ graphs for each $\rho_n$ from \sbm model, construct CI from bootstrap percentiles and correct the CI using Eq~\ref{eq:ci-correction}  for triangles and transitivity respectively.  For smooth functions, computing the bootstrap distribution is straightforward. One simply computes $u^*$ which is now a vector of bootstrapped triangles and two-star densities. Now a standardized bootstrap replicate is given by $\{f(u^*)-f(u)\}/\tdsigf$, where $u$ is the vector of triangles and two-star densities computed on the whole graph, and $\tdsigf$ is given by Eq~\ref{eq:sigmahatfemp}. For transitivity, $f(x,y)=3x/y$.
\begin{figure}[H]
\vspace{-5mm}
\centering
\begin{tikzpicture}[zoomboxarray,  zoomboxarray inner gap=.5cm, zoomboxarray columns=1, zoomboxarray rows=1]
    \node [image node] { \includegraphics[width=0.35\textwidth]{plots2/sbm-triangles.pdf}};
   % \zoombox{0.175,0.9}
    \zoombox[magnification=2]{.15,.7}
   % \zoombox{0.15,0.3}
    %\zoombox[magnification=10]{0.86,0.35}
\end{tikzpicture}
%\begin{tikzpicture}[zoomboxarray,
%zoomboxarray inner gap=.5cm, 
%zoomboxarray columns=1, 
%zoomboxarray rows=1]
%    \node [image node] { \includegraphics[width=0.35\textwidth]{plots2/ng2-triangles.pdf} };
   % \zoombox{0.175,0.9}
 %   \zoombox[magnification=2]{.15,.7}
   % \zoombox{0.15,0.3}
    %\zoombox[magnification=10]{0.86,0.35}
%\end{tikzpicture}\\
\begin{tikzpicture}[zoomboxarray,
zoomboxarray inner gap=.5cm, 
zoomboxarray columns=1, 
zoomboxarray rows=1]
    \node [image node] { \includegraphics[width=0.35\textwidth]{plots2/sbm-triangles-centerbytnhat.pdf} };
   % \zoombox{0.175,0.9}
    \zoombox[magnification=2]{.15,.7}
   % \zoombox{0.15,0.3}
    %\zoombox[magnification=10]{0.86,0.35}
\end{tikzpicture}\\
%\begin{tikzpicture}[zoomboxarray,
%zoomboxarray inner gap=.5cm, 
%zoomboxarray columns=1, 
%zoomboxarray rows=1]
%    \node [image node] { \includegraphics[width=0.35\textwidth]{plots2/ng2-triangles-centerbytnhat.pdf} };
   % \zoombox{0.175,0.9}
 %   \zoombox[magnification=2]{.15,.7}
   % \zoombox{0.15,0.3}
    %\zoombox[magnification=10]{0.86,0.35}
%\end{tikzpicture}
\vspace{-3mm}
\caption{We plot \KL{$F_n$}{$F_n^*$} ($Y$ axis) vs sparsity parameter $\rho_n$ ($X$ axis) for triangle density on networks generated from \sbm, where $F_n^*(t)$ corresponds to the appropriate resampling distribution. The first row is centered at bootstrap mean and normalized by variance estimation from each method $\hat{\sigma}_n$. The second row is centered by triangles density estimated on the whole graph (\mblapx is centered at approximate triangle density estimated from the whole graph) and normalized by $\hat{\sigma}_n$. %\rd Results for \smg are shown in the Supplement Section~\ref{sec:addlexp}.} \bk
}
\label{fig:cdf-error}
\end{figure}


\iffalse
\begin{figure}[!htb]
%\vskip 0.2in
\centering
%\text{no log}\\
\begin{tabular}{c}
    \includegraphics[width=  0.4\textwidth]{plots2/sbm-triangles.pdf} 
    \includegraphics[width=  0.4\textwidth]{plots2/ng2-triangles.pdf}\\
    \includegraphics[width=  0.4\textwidth]{plots2/sbm-triangles-centerbytnhat.pdf}\includegraphics[width=  0.4\textwidth]{plots2/ng2-triangles-centerbytnhat.pdf}
  %   \vspace{-2em}
     %  \includegraphics[trim=0em 1em 0em 5em, clip, width=  \textwidth]{plots/EW-MB-trans-nobar.pdf}
  %     \vspace{-1em}
    %\vspace{-4em}
%    \includegraphics[width=  0.8\textwidth,height=0.4\textwidth]{plots/EW-MB-twostars-nobar.pdf}\\
\end{tabular}
%\\\vspace{5mm}\text{taking log}\\
%\begin{tabular}{c}
%    \includegraphics[width=  0.4\textwidth]{plots2/sbm-triangles-log.pdf} 
%    \includegraphics[width=  0.4\textwidth]{plots2/ng2-triangles-log.pdf}\\
%    \includegraphics[width=  0.4\textwidth]{plots2/sbm-triangles-centerbytnhat-log.pdf}\includegraphics[width=  0.4\textwidth]{plots2/ng2-triangles-centerbytnhat-log.pdf}
  %   \vspace{-2em}
     %  \includegraphics[trim=0em 1em 0em 5em, clip, width=  \textwidth]{plots/EW-MB-trans-nobar.pdf}
  %     \vspace{-1em}
    %\vspace{-4em}
%    \includegraphics[width=  0.8\textwidth,height=0.4\textwidth]{plots/EW-MB-twostars-nobar.pdf}\\
%\end{tabular}
 \caption{We plot \KL{$F_n$}{$F_n^*$} \bk for triangle density for all methods on the $Y$ axis, where $F_n^*(t)$ corresponds to the appropriate resampling distribution. We vary the sparsity parameter $\rho_n$ on the $X$ axis. The networks in the left column are simulated from \sbm and those in the right column are simulated from \smg. The first row is centered at bootstrap mean and normalized by variance estimation from each method $\hat{\sigma}_n$  The second row is centered by triangles density estimated on the whole graph (\mblapx is centered at approximate triangle density estimated from the whole graph) and normalized by $\hat{\sigma}_n$.}
%\begin{center}
\label{fig:cdf-error}
\end{figure}
\fi 


\iffalse
\begin{figure}[!htb]
\centering
\begin{tabular}{cc}
     \includegraphics[width=  .4\textwidth]{plots2/sbm-trans.pdf}&\includegraphics[width=  .4\textwidth]{plots2/ng2-trans.pdf}\\
     \includegraphics[width=  .4\textwidth]{plots2/sbm-trans-centerbytnhat-ut2.pdf}&\includegraphics[width=  .4\textwidth]{plots2/ng2-trans-centerbytnhat-ut2.pdf}\\
     (A)&(B)
\end{tabular}
\rd \caption{We present $\log(\sup_{-3\leq u\leq 3}|F_n(u)-F_n^*(u)|)$ for the transitivity coefficient of the \sbm (A) and \smg (B) models with $\rho_n$ varying from $0.05$ to $1$. First row is centered by mean of bootstrap samples, normalized by true standard deviation. Second row is centered by transitivity estimated on the whole graph,(\mblapx centered at approximate transitivity estimation on the whole graph), normalized by true standard deviation.  Left Column is simulated from \sbm and right column is simulated from \smg.} %In the right panel, we present timing results for triangle frequencies for the \sbm (B) and \smg (D) models against sample size $n$. }
\label{fig:transitivity}
\end{figure}
\fi
\iffalse
\begin{figure}
\begin{tabular}{cc}
     \includegraphics[width=  .5\textwidth]{plots2/coverage-sbm-triangles.pdf}&\includegraphics[width=  .5\textwidth]{plots2/coverage-ng2-triangles.pdf}\\
     \includegraphics[width=  .5\textwidth]{plots2/coverage-sbm-trans.pdf}&\includegraphics[width=  .5\textwidth]{plots2/coverage-ng2-trans.pdf}\\
     (A)&(B)
\end{tabular}
\rd \caption{We present coverage of  95\% normal CI constructed from point estimate on the whole graph and bootstrap variance   for triangles and transitivity coefficient of the \sbm (A) and \smg (B) models in $\rho_n$ from $0.05$ to $1$. First row is row is for triangles and second row for transitivity. Left Column is simulated from \sbm and right column is simulated from \smg.} %In the right panel, we present timing results for triangle frequencies for the \sbm (B) and \smg (D) models against sample size $n$. }
\label{fig:coverage}
\end{figure}
%\rd being fixed\bk
\fi




\iffalse
\begin{figure}[!htb]
\begin{tabular}{cc}
     \includegraphics[trim=2em 2em 0em 0em, clip, width=  .5\textwidth]{plots2/correct-v-nocorrect-triangles-sbm.pdf}&\includegraphics[trim=2em 2em 0em 0em, clip,width=  .5\textwidth]{plots2/correct-v-nocorrect-triangles-ng2.pdf}\\
     \includegraphics[trim=2em 2em 0em 0em, clip,width=  .5\textwidth]{plots2/correct-v-nocorrect-trans-sbm.pdf}&\includegraphics[trim=2em 2em 0em 0em, clip,width=  .5\textwidth]{plots2/correct-v-nocorrect-trans-ng2.pdf}\\
    (A)&(B)
\end{tabular}
\rd \caption{We present coverage of  95\% bootstrap percentile CI with correction versus without correction  95\% bootstrap percentile CI coverage for MB-Q, SS and EG for triangles (top) and transitivity coefficient (bottom)  of the \sbm (A) and \smg (B) models. } %In the right panel, we present timing results for triangle frequencies for the \sbm (B) and \smg (D) models against sample size $n$. }
\label{fig:coverage2}
\end{figure}
\fi

  
 \begin{figure}[!htb]
%\begin{tabular}{cc}
     \includegraphics[trim=2em 2em 0em 0em, clip, width=  .5\textwidth]{plots2/corrected-triangles-sbm.pdf}%&\includegraphics[trim=2em 2em 0em 0em, clip,width=  .5\textwidth]{plots2/corrected-triangles-ng2.pdf}\\
     \includegraphics[trim=2em 2em 0em 0em, clip,width=  .5\textwidth]{plots2/corrected-trans-sbm-new.pdf}%&\includegraphics[trim=2em 2em 0em 0em, clip,width=  .5\textwidth]{plots2/corrected-trans-ng2-new.pdf}%\\
   % (A)&(B)
%\end{tabular}
\caption{We present coverage of  95\% bootstrap percentile CI with correction for triangles (left) and transitivity coefficient (right) of the \sbm model  with $\rho_n$ varying from $0.05$ to $1$. %Results for \smg model are shown in the Supplement Section~\ref{sec:addlexp}.
 } %In the right panel, we present timing results for triangle frequencies for the \sbm (B) and \smg (D) models against sample size $n$. }
\label{fig:coverage}
\end{figure}

 
 \bk %see that the approximate linear bootstrap % We see that the empirical Edgeworth expansion (\ew) has strong performance for both two-stars and triangles, outperforming all other methods.  

%Our proposed bootstrap procedures also exhibit strong performance on these functionals, but the advantage of using the bootstrap is most clear for transitivity (Figure \ref{fig:transitivity} (left panel)). For smooth functions of counts such as transitivity, analytical expressions for the Edgeworth expansion are much more difficult to attain; the bootstrap is more user-friendly since the general procedure remains the same.    

%The empirical graphon (\eg) also performs well and exhibits higher order correctness.  However, as previously mentioned, higher-order correctness to this point has only been established under a Cramer condition.  In contrast, the latent space bootstrap (\ls) and the linear bootstrap do not appear to be higher order correct, as suggested by our theory.  These two bootstrap procedures track each other closely, suggesting that estimating latent positions did not substantially affect performance for the graphons under consideration.  Subsampling had the worst performance; however, it is plausible that subsampling will perform better with a more principled choice of subsample size.

\iffalse
\begin{table}[h]
\centering
\begin{tabular}{ll|llllll}
\hline
                                         &     & \multicolumn{2}{c}{MB-Q} & \multicolumn{2}{c}{SS} & \multicolumn{2}{c}{EG} \\
                                         &     & w/ c       & w/o c       & w/ c      & w/o c      & w/ c      & w/o c      \\
\hline
\multicolumn{1}{c}{\multirow{3}{*}{\sbm}} & $\rho_n=0.2$ & \textbf{97.0}       & 99.5        & \textbf{97.5}      & 99.5       & 92.5      & 95.0       \\
\multicolumn{1}{c}{}                     & $\rho_n=0.6$ & \textbf{98.5}       & 90.0        & \textbf{97.5}      & 91.0       & \textbf{97.5}      & 82.0       \\
\multicolumn{1}{c}{}                     & $\rho_n=1$   & \textbf{95.0}       & 94.5        & \textbf{95.0}      & 94.0       & \textbf{95.0}      & 92.5       \\
\hline
\multirow{3}{*}{\smg}                     & $\rho_n=0.2$  & \textbf{95.0}       & 99.5        & \textbf{97.0}      & 99.5       & \textbf{91.5}      & 100.0      \\
                                         & $\rho_n=0.6$  & \textbf{97.0  }     & 91.5        & \textbf{96.5 }     & 91.0       & \textbf{97.0}      & 83.5       \\
                                         & $\rho_n=1$    & \textbf{94.5}       & 91.0        & \textbf{93.5}      & 91.0       & \textbf{94.0}      & 89.0    \\
\hline
\end{tabular}
\caption{We present coverage of  95\% bootstrap percentile CI with correction (w/ c) versus without correction (w/o c) for MB-Q, SS and EG for transitivity of the \sbm and \smg models. }
\label{tab:ci-trans-wcvnc}
\end{table}
\rd
\fi




%In Figure \ref{tab:ci-trans-wcvnc}, we show difference of  95\% Bootstrap Percentile CI the coverage with correction and without correction for MB-Q, SS and EG. Each of them are first-order correct before correction and second-order correct after. 

\subsection{Computation time}
In Figure \ref{fig:4cycle-timing}  we show logarithm of running time for 4-cycles count against growing $n$ for %\sbm and \smg models respectively. 
\sbm model.  We compare our approximate linear method \mblapx with \mblbts, which uses a randomized algorithm for approximating U-statistics proposed in Section~2.2 of~\cite{chen2019randomized}, for precomputation of the local network statistics. 
\begin{figure}[h]
%\begin{tabular}{cc}
\centering
    \includegraphics[width=  .4\textwidth]{plots2/runtime-sbm-fi.pdf} %&
     %\includegraphics[width=  .5\textwidth]{plots2/runtime-ng2-fi.pdf}\\
     %(A)&(B)
%\end{tabular}
\rd \caption{Logarithm of running time for  four-cycles in  \sbm  against sample size $n$.}
\label{fig:4cycle-timing}
\end{figure}
We see that among higher-order correct methods, \mbq offers strong computational performance, outperforming methods such as the \eg and \sub. We see that while \eg has comparable performance to \mbq, it requires recomputation of the count statistic for every bootstrap iteration, making it about $500$ times slower than \mbq for $n=500$ for four-cycle counting. \mbm is the slowest one we do not show here as the weights make symmetric counting shortcuts not as simple to apply. \ew is the fastest among higher-order correct methods, but it cannot be readily adapted for smooth functions of count statistics and is much slower compared to additive methods \ls, \mbl, \mblbts, \mblapx. The four additive methods, i.e. \ls, \mbl, \mblbts, \mblapx are the fastest four of all methods, but they are not higher-order accurate; among them \mblapx is the fastest method in all with our proposed approximate precomputation. The procedure \mblbts draws around $N(n-1)/(r-1)$ size $r-1$ subsets with replacement, whereas we draw $N$ permutations at random and then divide each into consecutive disjoint subsets of size $r-1$.   We observe that \mblapx appears to be faster empirically even if theoretically it has similar computational complexity as \mblbts. 
% Even though theoretically both have similar accuracy and similar speed, we believe that the with replacement sampling of subsets incurs additional computational burden. \bk
%We performed two sets of experiments, one on a stochastic block model (SBM) with B matrix ((0.6,0.2),(0.2,0.2)), and cluster probablity vector (0.65,0.35), and a smooth graphon (SM-G), with kernel function  $w(x_i,x_j)=(x_i^2+x_j^2)/3\times cos(1/(u^2+v^2))+0.15$. 
%We first simulate $10^6$ number of $n=160$ graphs from both of the graphons and calculated the triangle and two-star density from each graph to approximate the true CDF. 
% We then generate 30 graphs from each graphon, and perform empirical edgeworth, multiplier bootstrap with Gaussian Product multiplier ( N(0,1/2)$\times$ N(0,1/3) has first three central moments all as $1$.) We also compare to bootstrapping with latent space structure (LSS) \cite{levin2019bootstrapping} (with largest three eigenvalues for SBM and USVT for SM-G), empirical graphon (EG) \cite{green2017bootstrapping} and subsampling with $b=0.5n$. We conduct each bootstrap with $B=5000$. 
% From each method we have an estimated CDF. We take $\sup |\text{CDF(Est)} - \text{CDF(true)}|$. From 30 graphs we construct an estimate and error bar of $\sup |\text{CDF(Est)} - \text{CDF(true)}|$. 
 The simulation experiments are run on the Lonestar super computer (1252 Cray XC40 compute nodes, each with two 12-core Intel® Xeon® processing cores for a total of 30,048 compute cores) at the Texas Advance Computing Center. 


% \begin{figure}[t]
% %\vskip 0.2in
% \begin{tabular}{c}
%     \includegraphics[trim=0em 1em 0em 5em, clip, width=  \textwidth]{plots/EW-MB-triangles-nobar.pdf} \\
%   %   \vspace{-2em}
%      \includegraphics[trim=0em 1em 0em 5em, clip, width=  \textwidth]{plots/EW-MB-twostars-nobar.pdf}\\
% %     \includegraphics[trim=0em 1em 0em 5em, clip, width=  \textwidth]{plots/EW-MB-trans-nobar.pdf}
%   %     \vspace{-1em}
%     %\vspace{-4em}
% %    \includegraphics[width=  0.8\textwidth,height=0.4\textwidth]{/plots/EW-MB-twostars-nobar.pdf}\\
% \end{tabular}
%  \caption{Y axis has absolute error $|\mathbb{E}[F_n(u)]-G_n(u)|$ of CDFs for all methods. X axis is $u\in [-3:3]$. The two rows are for triangles and two-star from top to bottom. The left column is for SBM whereas the right column is for the smooth graphon (\smg).}
% %\begin{center}
% \end{figure}

% %\rd being fixed\bk
% \begin{figure*}[t]
% \begin{tabular}{cc}
%      \includegraphics[ trim=0em 1em 0em 5em, clip,width=  .5\textwidth]{plots/EW-MB-trans-nobar-sbm.pdf}&\includegraphics[ trim=0em 1em 0em 5em, clip,width=  .5\textwidth]{plots/time-tri-sbm.pdf} 
% \end{tabular}
% \caption{In the left panel, we present $\mathbb{E}|F_n(u)-F_n^*(u)|$ for the transitivity coefficient of the SBM model.  In the right panel, we present timing results for triangle frequencies for the SBM model. }
% \end{figure*}



% \begin{figure*}
% \vskip 0.2in
% \begin{center}
% \vspace{-0.5cm}
% \includegraphics[width=  0.32\textwidth,height=0.32\textwidth]{/plots/EW-MB-sup-tri.pdf}
% \includegraphics[width=  0.32\textwidth,height=0.32\textwidth]{plots/EW-MB-sup-ts.pdf}
% \includegraphics[width=  0.32\textwidth,height=0.32\textwidth]{plots/EW-MB-sup-trans.pdf}
% %\begin{footnotesize}
% %\begin{tabular} {p{0.8cm}p{2.6cm}p{2.6cm}p{2.6cm}p{2.6cm}}
% %     &(e) &(f) &(g) &(h) \\
% %\end{tabular}
% %\end{footnotesize}
% %\vspace{-0.5cm}
% \caption{Sup CDF Error and its 95\% CI over the grid of (-3,3) for different methods. Left:Triangle Densities; Middle: Two-star Densities; Right: Transitivity}
% \label{fig:cdf-grid}
% \end{center}
% \vskip -0.2in
%\end{figure*}


% \begin{table}[t]
% \caption{Average Calculation Time Spent on Estimating Triangle/two-star Density CDF Using Each Method Per Graph}
% 	\label{table:time}
% 	\vspace{-3mm}
% 	\begin{center}
% 	\small
% \begin{tabular}{llllllll}
% \toprule
%   \textbf{Triangles}  & EW          & MB-M     & MB-Q    & MB-L   & LS    & EG    & SS     \\
%   \hline
% SBM  & 0.0023 & 14.89 & 0.7418 & 0.5902 & 1.4593 & 3.6745 & 0.6399 \\
% SM-G & 0.0024 & 11.9845 & 0.9451 & 0.7903 & 1.5329 & 3.6772 & 0.6053 \\
% \bottomrule
% \toprule
%   \textbf{two-star}  & EW          & MB-M     & MB-Q    & MB-L    & LS    & EG    & SS     \\
% \hline
% SBM  &0.0027 & 7.4196 & 0.7453 & 0.5954 & 1.4312 & 3.8565 & 0.8048 \\
% \hline
% SM-G &0.0027 & 7.0410 &  0.7688 & 0.6288 & 1.2522 & 3.5436 & 0.7851\\
% \bottomrule
% \end{tabular}
% \normalsize
% \end{center}
% \end{table}
%\newpage


==> network_mb_jasa_to_arxiv (1)/hoeffding.tex <==

%
%BLAHBLAHBLAH
\section{The Hoeffding decomposition}
The Hoeffding decomposition, introduced in \citet{hoeffding1948}, is a key technical tool for studying the asymptotic properties of U-statistics.  In essence, a U-statistic may be represented as a sum of U-statistics of different orders.  Only the linear (order one) term is non-negligible; the order 2 term is also needed for higher-order correctness. The Hoeffding decomposition, however, generalizes far beyond U-statistics.  We will provide a more general treatment of the Hoeffding decomposition below, following \citet{Bentkus-edgeworth-symmetric}. This general decomposition will be used to derive a Hoeffding decomposition for the bootstrap statistic.

Let $X_1, \ldots, X_n$ be independent random variables and $\Omega = \{1, \ldots n\}$. For any $B \subset \Omega$ and a random variable $T = t(X_1, \ldots , X_n)$, let
\begin{align}
T_B = \mathbb{E}[T \ \mid  X_i \in B]
\end{align}
It may be verified that:
\begin{align*}
T_B = \sum_{C \subset B} (-1)^{|B| - |C|} T_C
\end{align*}
We also have the following inverse relationship:
\begin{align*}\mathbb{E}[T \ \mid  X_i \in C] = \sum_{B \subset C} T_B 
\end{align*}
which implies the Hoeffding decomposition:
\begin{align}
    T = \sum_{B \subset \Omega} T_B
\end{align}
In what follows, we will group terms by their cardinality, leading to a decomposition closely resembling the familiar decomposition for U-statistics.
\section{Proof of Lemma~\ref{lemma:hoeffding-bootstrap}}
\label{sec:supp:lemmaone}
\begin{proof}
In what follows, we will consider a projection of $T_{n,M}^*$ with respect to the random variables $ \w_1, \ldots \w_n$, conditional on $A$ and $X$. 

Recall that $\xi_i$ follows the Gaussian Product distribution. First, we may express $T_{n,M}^*$ as:
\begin{align*}
T_{n,M}^* = \frac{1}{{n \choose r}} \sum_{1 \leq i_1 < i_2 < \ldots i_r} \left(\xi_{i_1 \cdots i_r} - 1\right)  \cdot \left( H(A_{i_1, \ldots, i_r}^{(n)}) - \hat{T}_n \right)
\end{align*}
where $\xi_{i_1 \cdots i_r}$ denotes the product $\xi_{i_1} \times \cdots \times \xi_{i_r}$. It turns out that applying the Hoeffding decomposition directly to $T_{n,M}^*$ leads to tedious combinatorial calculations; following \citet{Bentkus-edgeworth-symmetric}, let $\Omega_r$ denote an $r$-tuple of $\{1, \ldots, n\}$.  For each summand, we will consider a Hoeffding representation with respect to $\Omega_r$.   Note that using the Hoeffing projection (also see~\cite{Bentkus-edgeworth-symmetric} section 2.8), 
\begin{align*}
    \prod_{1\leq i\leq r}\w_i-1=\sum_{k=1}^r\sum_{1\leq i_1<\dots< i_k\leq r} h_k(\w_{i_1},\dots,\w_{i_k}),
\end{align*}
where for $\Omega_k=\{1,\dots, k\}$,
\begin{align*}
    h_k(\w_{1},\dots,\w_{k})=\sum_{B\in \Omega_k}(-1)^{k-|B|}\E\left[\prod_{1\leq i\leq r}\w_i-1\mid B\right]
\end{align*}
Thus the first two terms are given by:
\begin{align*}
    h_1(\w_{1})&:=(\w_1-1)\\ h_2(\w_{1},\w_{2})&:=(\w_1\w_2-1)-(\w_1-1)-(\w_2-1)=(\w_1-1)(\w_2-1)
\end{align*}
In what follows, we will also denote $A^{(n)}_{i_1,\dots,i_r}$ by $A^{(n)}_S$, where $S=\{i_1,\dots, i_r\}$.
Let 
\begin{align}\label{eq:hhij}
    \hhij= \frac{1}{{n-2 \choose r-2}}\sum_{S,i,j\in S}H(A_S).
\end{align}
Thus $T_{n,M}^*$ can be written as follows:
\begin{align}\label{eq:hofftnm}
    T_{n,M}^* &= \frac{1}{{n \choose r}} \sum_{1 \leq i_1 < i_2 < \ldots < i_r} \left(\xi_{i_1 \cdots i_r} - 1\right)  \cdot \left( H(A_{i_1, \ldots, i_r}^{(n)}) - \hat{T}_n \right)\notag\\
    &=\frac{1}{{n \choose r}} \sum_{1 \leq i_1 < i_2 < \ldots < i_r}\sum_{k=1}^r\sum_{1\leq i_1<\dots< i_k\leq i_r} h_k(\w_{i_1},\dots,\w_{i_k})\cdot \left( H(A_{i_1, \ldots, i_r}^{(n)}) - \hat{T}_n \right)\notag\\
    &=\frac{1}{{n \choose r}} \sum_{k=1}^r \sum_{1\leq i_1<\dots< i_k\leq n} h_k(\w_{i_1},\dots,\w_{i_k})\cdot\sum_{S}  \left( H(A_S^{(n)}) - \hat{T}_n \right)1 (i_1,\dots, i_k\in S)\notag\\
    &=\frac{1}{{n \choose r}} \sum_{k=1}^r {n-k\choose r-k}\sum_{1\leq i_1<\dots< i_k\leq n}h_k(\w_{i_1},\dots,\w_{i_k}) \frac{\sum_{S}  \left( H(A_S^{(n)}) - \hat{T}_n \right)1 (i_1,\dots, i_k\in S)}{{n-k\choose r-k}}\notag\\
    &=\frac{r}{n}\sum_i (\xi_i-1)\gi+\frac{r(r-1)}{n(n-1)}\sum_{1\leq i<j\leq n} (\w_i-1)(\w_j-1)\underbrace{(\hat{H}_2(i,j)-\tnhat)}_{\tilde{g}_2(i,j)}+R_n
\end{align}


\iffalse
The first two terms of the decomposition are given by:
\begin{align*}
f_1(A_{i,i_2, \ldots, i_r}) &= \left(\xi_i - 1 \right) \cdot \left( H(A_{i,i_2, \ldots, i_r}^{(n)}) - \hat{T}_n \right) 
\\ f_2( A_{i,j,i_3, \ldots, i_r}) %&= \rd \left(\xi_i \cdot \xi_j - \w_i-\w_j +1 \right) \cdot \left( H(A_{i,j,i_3, \ldots, i_r}^{(n)}) - \hat{T}_n \right) \bk\\
&=\left(\xi_i \cdot \xi_j - 1 \right) \cdot \left( H(A_{i,j,i_3, \ldots, i_r}^{(n)}) - \hat{T}_n \right) - f_1(A_{i,i_2, \ldots, i_r}) - f_1(A_{j,i_2, \ldots, i_r})
\end{align*}
\rd
\begin{align*}
f_{1,i}(A_{S}) &= \left(\xi_i - 1 \right) \cdot \left( H(A_{S}^{(n)}) - \hat{T}_n \right) 1(i\in S)
\\ f_{2,i.j}( A_{S}) &= \rd \left(\xi_i \cdot \xi_j - \w_i-\w_j +1 \right) \cdot \left( H(A_{S}^{(n)}) - \hat{T}_n \right)1(i,j\in S) \bk\\
%&=\left(\xi_i \cdot \xi_j - 1 \right) \cdot \left( H(A_{i,j,i_3, \ldots, i_r}^{(n)}) - \hat{T}_n \right) - f_1(A_{i,i_2, \ldots, i_r}) - f_1(A_{j,i_2, \ldots, i_r})
\end{align*}
\bk
 Now, combining terms, we have that:
\begin{align*}
 T_{n,M}^* - \hat{T}_n &= \frac{1}{{n \choose r}} \sum_{\Omega_r \subset \Omega}  \left(\xi_{i_1 \cdots i_r} - 1\right)  \cdot \left( H(A_{i_1, \ldots, i_r}^{(n)}) - \hat{T}_n \right) 
 \\ &= \frac{r}{n} \sum_{i=1}^n (\xi_i - 1) \hat{g}_1(i)
 \\ & \ \ \ +\frac{r(r-1)}{n(n-1)}\sum_{i<j}(\w_i\w_j-1) \tilde{g}_2(i,j)-(\w_i-1) \cdot \hat{g}_1(i) - (\w_i-1) \cdot \hat{g}_1(j) + R_n
% \\ & = \frac{r}{n}\sum_{i=1}^n \sum_{ f_1(\xi_i; A_{i, i_2, \ldots, i_r}) + \frac{r(r-1)}{n(n-1)} \sum_{i < j} f_2(\xi_i, \xi_j; A_{i,j,i_3, \ldots, i_r}) +R_n 
 \end{align*}
 \fi
 Now, it remains to show that the remainder of $(T_{n,M}^* - \hat{T}_n)/\hat{\sigma}_n$ is $O(\delta(n,\rho_n,R))$, where:
 \begin{align*}
    \delta(n,\rho_n,R) =\begin{cases} 
      \frac{1}{n\rho_n} & \text{R is acyclic} \\
       \frac{1}{n\rho_n^{3/2}}& \text{R is cyclic} .
  \end{cases}
\end{align*}

 The residual $R_n$ is a sum of higher order Hoeffding projections, which are all uncorrelated. %
 Therefore, we see that the variance of the $u^{th}$ order term is $\dfrac{\sum_{1\leq i_1<i_2\dots<i_u}  \tilde{g}_u(i_1,i_2,\dots,i_u)^2}{\hat{\sigma}_n^2 {n\choose u}^2}$. We will now obtain expressions for $3\leq u\leq r$.
 %Therefore, we see that the variance of the third order term (the first one in the remainder) is $\dfrac{\sum_{ijk}  \hat{g}_3(i,j,k)^2}{\hat{\sigma}_n^2 {n\choose 3}} \times O(1/n^3)$.  By Markov inequality, it further suffices to show $\mathbb{E}[\hat{g}_3(i,j,k)^2\delta^2(n,\rho_n,R)/\hat{\sigma}_n^2  ] )$ is bounded.
 %Now, we have that:
 %\begin{align*}
 %\mathbb{E}[\tilde{g}_u(i,j,k)^2] \leq 2 \left( \mathrm{Var}(\hat{g}_3(i,j,k)) + \mathrm{Var}(\hat{T}_n) \right)
 %\end{align*}
 
 
 
%  We may reinterpret $\mathbb{E}[\hat{g}_3(i,j,k)^2$ as $\mathrm{Var}(\hat{g}_3(i,j,k))$.  To bound this term,    
 
%  Note that  $\hat{g}_3(i,j,k)^2=O_P(\rho_n^{3s-3})$ for cyclic and $O_P(\rho_n^{3s-2})$ for acyclic subgraphs. This is because, for any two nonoverlapping $S,T$ (not containing $\{i,j,k\}$)  of size $r-3$, there are potentially three edges common between the subgraphs induced by $S\cup \{i,j,k\}$ and  $S\cup \{i,j,k\}$ for a cyclic subgraph, and two for an acyclic one.
%  Thus we can show that the remainder is the same order as $O(\mathcal{M}(n,\rho_n,R))$.




% For each summand, since $\mathbb{E}[\w] = 1$, it is now clear that the conditional expectation with respect to a set $A$ is $0$ if  $\{i_1, \ldots i_r\} \cap A = \emptyset$.  We may collect summands with a nonempty intersection, leading to the expressions:
% \begin{align*}
%  T_{\{\xi_i\}} = \left(\xi_i - 1 \right) \cdot \frac{{n-1 \choose r-1}}{{n \choose r}} \cdot \left[\frac{1}{{n-1 \choose r-1}} \sum_{i, i_2 < \ldots < i_r, i_u \neq i } \left( H(A_{i, i_2, \ldots, i_r}^{(n)}) - \hat{T}_n \right)\right]     
% \end{align*}

% \begin{align*}
%  T_{\{\xi_i, \xi_j \}}  &= \left(\xi_i \cdot \xi_j + \xi_i + \xi_j - 1 \right) \cdot \frac{{n-2 \choose r-2}}{{n \choose r}} \cdot \left[\frac{1}{{n-2 \choose r-2}} \sum_{i,j i_3 < \ldots < i_r, i_u \neq i,j } \left( H(A_{i,j,i_3, \ldots, i_r}^{(n)}) - \hat{T}_n \right)\right]
%  \\  & \ \ \ + (\xi_i-1) \cdot T_{\xi_i} + (\xi_i-1) \cdot T_{\xi_j}
% \end{align*}



% For any set set $S$ of $r$ nodes, $S=\{i_{1}\dots i_{r}\}$, denote $\W_S= \prod_{i \in S} \w_i$.
% Conditioned on the graph $A$ and $X$, we see that the hoeffding projections of the weighted bootstrap statistic gives: %the $X$ observed as $x$, $\tnt$ and $\hat{H}(x_i)$ for each $i$ are all observed.  $\hat{H}(x_i)$ is defined as
% \begin{equation*}
%     \begin{split}
%      &\hi= \frac{1}{{n-1 \choose r-1}}\sum_{S,i\in S}H(A_S), \\
%      &\hhij= \frac{1}{{n-2 \choose r-2}}\sum_{S,i,j\in S}H(A_S).
% \end{split}
% \end{equation*}
% Recall the definition of $\gi$ and $\gj$ from the main paper. To remind the reader, we have:

% \begin{equation*}
%     \begin{split}
%      &\gi= \frac{1}{{n-1 \choose r-1}}\sum_{S,i\in S}(H(A_S)-\tnhat), \\
%      &\ggij= \frac{1}{{n-2 \choose r-2}}\sum_{S,i,j\in S}(H(A_S)-\tnhat).
% \end{split}
% \end{equation*}

% We are interested in the Hoeffding decomposition [\rd Put eqn number from main \bk] of the following quantity. Below we derive the Hoeffding decomposition.
% %We define weighted boostrap of count statistic as $\vnhat$. Conditioned on A, Standardized $\vnhat$ can be written as follows using $\W_S=1$.
% \begin{equation}\label{eq:wb-def-vn}
%     \begin{split}
%         \frac{\vnhat-\tnhat}{\hat{\sigma}_n}&=\frac{\sum_S \W_S (\hat{H}(A_S)-\tnhat)}{{n \choose r} \hat{\sigma}_n} = \frac{\sum_S (\W_S-1)(\hat{H}(A_S)-\tnhat)}{{n \choose r} \hat{\sigma}_n} \\
%         &=\frac{r}{n\hat{\sigma}_n} \sum_i f_1(\w_i) + \frac{r(r-1)}{n(n-1)\hat{\sigma}_n} \sum_{1\leq i<j \leq n} f_2(\w_i,\w_j) + \rd R_n \bk.
%     \end{split}
% \end{equation}

% We now derive the Hoeffding projections.

% Applying a Hoeffding decompsition to $\sum_S (\W_S-1)(\hat{H}(A_S)-\tnhat)/{n \choose r}$ above with respect to $\W$ yields

% \begin{equation*}
%     \begin{split}
%       & f_1(\w_i)= E[\hat{H}(X_S,\\W_S)\mid \w_i,x_i]; \\
%       & f_2(\w_i,w_j)=E[\hat{H}(X_S,\\W_S)\mid \w_i,x_i,\w_j,x_j].
%     \end{split}
% \end{equation*}
% Equivalently , $g_1(x_i)$ and $g_2(x_i,x_j)$ can be written as 
% \begin{equation}
% \begin{split}
%     f_1(\w_i)&=E[\W_S (\hat{H}(A_S)-\tnhat)\mid \w_i]= (\w_i-1)(\hi-\tnhat)=(\w_i-1)\gi;\notag\\
%     f_2(\w_i,\w_j)&=E[\W_S (\hat{H}(A_S)-\tnhat)\mid \w_i,\w_j] \notag\\
%     &=(\w_i\w_j-\w_i-\w_j+1)(\hhij-\tnhat)\notag\\
%     &=(\w_i\w_j-1)(\hhij-\tnhat)-(\w_i-1)(\hi-\tnhat)-(\w_j-1)(\hj-\tnhat),\label{eq:wb-hp}
% \end{split}
% \end{equation}

% \rd The residual $R_n$ is essentially a sum of higher order Hoeffding projections, which are all uncorrelated. Therefore, we see that the variance of the third order term (the first one in the remainder) is $\dfrac{\sum_{ijk}  \hat{g}_3(i,j,k)^2}{\hat{\sigma}_n^2 {n\choose 3}} \times O(1/n^3)$. Note that  $\hat{g}_3(i,j,k)^2=O_P(\rho_n^{3s-3})$ for cyclic and $O_P(\rho_n^{3s-2})$ for acyclic subgraphs. This is because, for any two nonoverlapping $S,T$ (not containing $\{i,j,k\}$)  of size $r-3$, there are potentially three edges common between the subgraphs induced by $S\cup \{i,j,k\}$ and  $S\cup \{i,j,k\}$ for a cyclic subgraph, and two for an acyclic one.
% Thus we can show that the remainder is the same order as $O(\mathcal{M}(n,\rho_n,R))$.


%\subsection{Edgeworth Expansion for Unweighted Boostrap}
% \section{\large{Edgeworth Expansion for Standardized Count Statistic}}
% In a size $n$ graph $\mathcal{G}_n$, define $\tnhat$ as normalized count statistic for a $r$-node $d$-edge subgraph $R$ with vertex set $V(R) $ and edge set $E(R)$.  For any set of $r$ nodes $S=\{X_{i_1},,,X_{i_r}\}$, denote
% \begin{equation*}
%     H(A_S)=  \prod_{(i_i,i_j)\in E(R)} A_{i_ii_j} ,
% \end{equation*}
% \begin{equation*}
%     h(X_{i_1},...,X_{i_r})=  \prod_{(i_i,i_j)\in E(R)} E(A_{i_ii_j}) =\prod_{(i_i,i_j)\in E(R)} \rho_n  w(X_{i_i},X_{i_j}) \wedge 1.
% \end{equation*}
% Then, $\tnhat$ can be written as 
% %Let $Iso(R)$ denote the class of graphs isomorphic to $R$, and $| Iso(R)|$ its cardinality. Then,
% %\begin{equation*}
% %\tnhat=\rho_n^{-d} \frac{1}{{n \choose p} \ |\mathrm{Iso}(R)| } \sum_{S \sim R} \mathbbm{1}(S = G_n[S])
% %\end{equation*}
% %Equivalently, we can also write $\tnhat$ as 

% \begin{equation*}
%     \tnhat= \frac{1}{{n \choose r}}\sum_{1\leq i_1<...<i_r\leq n} H(X_{i_1},,,X_{i_r}).
% \end{equation*}


% Let $T_n= E[\tnhat|\mathbf{X}]$ and $\theta=E[T_n]$. $T_n$ is a noiseless U-statistic with kernel function $h$. 
% \begin{equation*}
%      T_n= \frac{1}{{n \choose r}}\sum_{1\leq i_1<...<i_r\leq n} h(X_{i_1},,,X_{i_r}).
% \end{equation*}

% Define 
% \begin{equation*}
%     \begin{split}
%         & h_1(X_1)= E[h(X_1,X_2,,,X_r)\mid X_1=x_1];\\
%         & h_2(X_1,X_2)= E[h(X_1,X_2,,,X_r)\mid X_1=x_1,X_2=x_2].
%     \end{split}
% \end{equation*}
% Applying Hoeffding's decompsition of U-statistic \citep{hoeffding1992class} to $T_n$ yields 
% \begin{equation*}
%     T_n -\theta = \frac{r}{n}\sum_{i=1}^ng_1(X_i)+ \frac{r(r-1)}{n(n-1)}\sum_{1\leq i <j \leq n}g_2(X_i,X_j) + O_P(\rho_n^{d}n^{-1}),
% \end{equation*}
% where 
% \begin{equation}\label{eq:g1g2}
% \begin{split}
%     &g_1(X_i)= h_1(X_i)-\theta , \\
%     &g_2(X_i,X_j)= h_2(X_i,X_j) - \theta -g_1(X_1)-g_2(X_2) .
% \end{split}
% \end{equation}

% In addition, we define 
% \begin{align*}
%     \tau^2= \var(g_1(\mathbf{X})), \ \ \
%      \tilde{\tau_n} ^2= \frac{r^2}{n}\tau^2, \ \ \
%      \sigma_n^2 = \var(\tnt) .
% \end{align*}

% % U-stats hf decomp
% \rd I am removing $\tnhat$ because we don't use it in main paper and I think the shorthand may be a bit confusing  \bk


% % standardized form of $\tnhat$, denoting as $\tnt$,
% % \begin{equation*}
% %     \tnt = \frac{\tnhat - \mu_n}{\sigma_n}.
% % \end{equation*}
% \begin{theorem}\label{thm:ew-sd}
% % Edgeworth Expansion for $\tnt$. 

% Define \\
% \begin{equation*}
%     G_n(u)= \Phi(u)- \phi(u)\frac{(u^2-1)}{6n^{1/2}\tau^3}\{E[g_1^3(X_1)]+3(r-1)E[g_1(X_1)g_1(X_2)g_2(X_1,X_2)]\},
% \end{equation*}
% where $\Phi(u)$ and $\phi(x)$ denotes the CDF and PDF of standard Gaussian distribution. \rd For $\rho_n = O_P ((\log n)^{-1})$, and $\rho_n= \omega(n^{-1/2})$ for acyclic R and $\rho_n= \omega(n^{-1/r})$ for cyclic R.
% \bk  we have,
% \begin{equation*}
%     \sup_u \bigg{|} F_{\tnt}(u)-G_n(u)\bigg{|} = O(\mathcal{M}(n,\rho_n,R)).
% \end{equation*}
% \end{theorem}

Consider any term $\hat{g}_u(1,\dots,u)$. We will now bound $\E[\hat{g}_u(1,\dots,u)^2]$.
\begin{align*}
    \E[\hat{g}_u(1,\dots,u)^2]\leq 2(\var(\hat{g}_u(1,\dots,u))+\underbrace{\var(\tnhat)}_{O(\rho_n^{2s}/n)})
\end{align*}
The bound on the second term follows from~\cite{Bickel-Chen-Levina-method-of-moments} and will be smaller than that of the first term.
Let $\mathcal{S}_{r,u}$ denote all subsets of size $r-u$, not containing $1,\dots u$. For any subset $S\in \mathcal{S}_{r,u}$, also define, $S_u=S\cup \{1,\dots,u\}$.
For the first part, we have:
\begin{align*}
    \var(\hat{g}_u(1,\dots,u))=\frac{\sum_{S,T\in \mathcal{S}_{r,u}}\cov(H(A_{S_u}),H(A_{T_u}))}{{n-u\choose r-u}^2}
\end{align*}
Note that the dominating term here will indeed be the one where $|S\cap T|=0$. Number of such terms is ${n\choose 2r-u}$. Also the covariance of those terms will be $\rho_n^{2s-E(A_{1,\dots,u})}$, where $E(A_{1,\dots,u})$ denotes the intersection of the edgeset of $A_{1,\dots,u}$ and the subgraph we are counting. This number can be at most $u-1$ for acyclic $R$ and $u$ for cyclic $R$. For $|S\cap T|=k$, the number of terms is ${n\choose 2r-2u-k}$ and the exponent on $\rho_n$ is at most $2s-(u+k-1)$. Thus, for an acyclic subgraph, we have,
\begin{align*}
    \var(\hat{g}_u(1,\dots,u))&\leq \frac{\sum_{k=0}^r {n\choose 2r-2u-k}\rho_n^{2s-(u+k-1)}}{{n-u\choose r-u}^2}\\
    &\leq \sum_{k=0}^r n^{-k}\rho_n^{2s-(u+k-1)}=\rho_n^{2s-(u-1)}\left(1+\sum_{k>0}\frac{1}{(n\rho_n)^k}\right)
\end{align*}
The cyclic one is worse by a factor of $\rho_n$.
Thus the contribution of the $u^{th}$ element of the Hoeffding decomposition is 
\begin{align*}
    n\cdot \frac{\sum_{i_1,\dots, i_u} \hat{g}_u(i_1,\dots,i_u)^2}{{n\choose u}^2 \hat{\tau}_n^2}&=\begin{cases}O_P\left(\frac{1}{(n\rho_n)^{u-1}}\right)&\mbox{$R$ acyclic}\\
    O_P\left(\frac{\rho_n^{-1}}{(n\rho_n)^{u-1}}\right)&\mbox{$R$ cyclic}\end{cases}
\end{align*}

This shows that the third term contributes the most to $R_n$ in Eq~\ref{eq:hofftnm}.  By Markov's inequality, and the definition of $O_P(.)$ notation, it is easy to see that $R_n=O_P(\delta(n,\rho_n,R))$. 
\end{proof}


==> network_mb_jasa_to_arxiv (1)/intro.tex <==


% Network data is ubiquitous. The internet is a giant, directed network of webpages
% pointing to other webpages. 




% Facebook is an undirected network built via friendships between users. The ecological web is a directed network of different species with edges specified by ‘who-eats-whom’ relationships. The protein-protein interaction networks are undirected networks consisting of pairs of bait-prey proteins which bind to each other during coaffinity purification experiments arising in mass spectrometry analysis. Brain networks are built using different measures of association between regions of interest in the human brain. 
%Network data, which represents complex relationships between different entities, have become ubiquitous in many fields. 
%Starting from 

%Commented for brevity
%Network data has become ubiquitous in a broad range of real-world applications, ranging from social networks such as Twitter and Facebook to biological networks such as protein-protein interaction networks and brain networks.
% The ecological web is a directed network of different species with edges specified by ‘who-eats-whom’ relationships.
%Protein-protein interaction networks are undirected networks consisting of pairs of bait-prey proteins that bind to each other during coaffinity purification experiments arising in mass spectrometry analysis. Finally, brain networks represent association between regions of interest in the brain.

% Since network data are now widespread, there is a growing need for computationally efficient and statistically valid procedures for analyzing such data.  Recently, several inference procedures for network data have been proposed; we postpone a detailed discussion of related work to Section blah.  In the present work, we consider the problem of developing fast and accurate bootstrap procedures for count functionals of networks.
Count functionals play a pivotal role in the analysis of network data.  In biological networks, it is believed that certain subgraphs  may  represent functional subunits within the larger system \citep{milo-network-motifs,chen-yuan-protein-protein-interaction-network,daudin-exceptionality-motifs,kim2014}.  In social networks, the frequency of triangles provides information about the likelihood of mutual friendships \citep{newman-collaboration-network,meyers-social-network-twitter,ugander-facebook-graph}. At a more theoretical level, count functionals may be viewed as network analogs of the moments of a random variable. Thus, a method of moments approach may be used to estimate the underlying model under suitable conditions~\citep{Bickel-Chen-Levina-method-of-moments}.  %Furthermore, the convergence of graph sequences (at least dense sequences) may be stated in terms of the convergence of a collection of subgraph frequencies \citep{borgs-convergence-dense-graphons-1}.

%Given their practical and theoretical importance, quantifying the uncertainty of count functionals is naturally of substantial interest. One may use the limiting normal distribution~\citep{Bickel-Chen-Levina-method-of-moments} for inference, but estimating parameters of the limiting normal for smooth functions of counts like the transitivity (suitably normalized ratio of triangles and two stars) requires calculation of the variance which can be cumbersome for a practitioner. Bootstrap presents a user friendly alternative, where one replaces complex calculations by computer simulations.

% Such estimates may be used to construct confidence intervals for underlying parameters and conduct two-sample tests between two networks.
While real-world networks share many qualitative features (see e.g. \citet{newman-structure-networks}), they often vary substantially in terms of size, given by the number of vertices in the network, and sparsity level, given by the number of edges relative to the number of vertices. For networks of small to moderate size, inferential methods that are highly accurate are advantageous; for sparse, massive networks, one needs to simultaneously consider computational tractability. %In this paper consistency are highly desirable.

%Given their practical and theoretical importance, quantifying the uncertainty of count functionals is naturally of substantial interest. 
To meet these diverse needs in real-world applications with user-friendly computational tools, we develop a new family of bootstrap procedures for uncertainty estimation of count functionals of networks. Our methods range from a very fast approximate linear bootstrap to a fast quadratic bootstrap procedure that offers improved accuracy for moderately sparse networks. Both procedures may be viewed as approximations\footnote{More precisely, the linear and quadratic bootstraps may be viewed as first and second-order terms of a Hoeffding decomposition for the multiplier bootstrap, respectively.} to a multiplier bootstrap method in which each potential subgraph in the network is perturbed by the product of independent multiplier random variables. This multiplier bootstrap is closely related to a bootstrap method for U-statistics (see for example, \citet{bose-chatterjee-u-stats-resampling}). Under the sparse graphon model (see Section \ref{sec:sparse-graphon}), subgraph counts may be viewed as U-statistics perturbed by asymptotically negligible noise, allowing the adaptation of bootstrap methods for U-statistics to the network setting.

One of the main theoretical contributions of our paper is that we establish the statistical properties of a computationally efficient randomized approximation for computing local subgraph counts.   This  approximation alleviates the main computational bottleneck for our linear bootstrap procedure. By invoking these results in our analysis of the bootstrap, we characterize the relationship between the sparsity level of the graph and the degree of randomization allowed to achieve either asymptotically efficient confidence intervals or the less ambitious aim of consistent inference via vanishing confidence intervals.
  % Our approximation method may also be used to scale up the first-order correct Normal approximation.
 In the worst case, counting a local subgraph of size $r$ (e.g. number of r-cycles a node is involved in) in a $n$ node network has a computation complexity of $O(n^{r-1})$. In contrast, our methods can be used to reduce this time substantially depending on the nature of the subgraph and sparsity level; for triangles for example, the computational complexity of our approximation is $O(Nn^2 \rho_n\log(n\rho_n))$, where $N$ is the number of random permutations and $\rho_n$ is the probability of an edge.
\bk

While randomized linear bootstrap is more scalable, it does not yield higher-order correctness, which can be achieved with certain methods for sufficiently dense graphs (see~\citet{zhang-xia-network-edgeworth}). As the second theoretical contribution of our paper, we propose the quadratic bootstrap and establish conditions under which it is higher order correct. % derive (uniform) Edgeworth expansions for the quadratic bootstrap. %Higher-order correctness is one theoretical advantage the quadratic bootstrap possesses compared to a Normal approximation~\citep{hall-bootstrap-edgeworth}. %Edgeworth expansions may be viewed as a refinement of the Normal approximation that accounts for skewness; an excellent treatment of this topic in the IID setting is given by \citet{hall-bootstrap-edgeworth}. 
To this end, we establish an Edgeworth expansion for the quadratic bootstrap and show that it is close to the Edgeworth expansion of the sampling distribution. %Thus, we  establish that the bootstrap is higher-order correct under certain sparsity conditions. 
%Therefore, the quadratic bootstrap offers a faster convergence rate in the Kolmogorov distance than the Berry-Esseen bound.  
We bypass the typical Cram\'{e}r's condition required by~\cite{zhang-xia-network-edgeworth} in their analysis of existing bootstrap methods by considering a continuous multiplier that matches the first three moments of the data. It is well-known that continuous random variables satisfy Cram\'{e}r's condition. %We derive our Edgeworth expansion for the bootstrap using tools developed for order two U-statistics~\citep{wang-jing-weighted-bootstrap-u-statistics}. 


%Edgeworth expansions for network moments were first studied by~\citet{zhang-xia-network-edgeworth}.  The authors show that the network noise has a smoothing effect that allows them to bypass the typical Cram\'{e}r condition, which is restrictive in the network setting.  
%We bypass the typical Cram\'{e}r' condition for the bootstrap, using a continuous multiplier that matches the first three moments of the data. It is well-known that continuous random variables satisfy Cram\'{e}r's condition. We derive our Edgeworth expansion for the bootstrap using tools developed for order two U-statistics~\citep{wang-jing-weighted-bootstrap-u-statistics}.  %It turns out that network noise, particularly when the graph is sparse, causes certain terms related to our Edgeworth expansion to blow up. While the details are technical, we show that a valid Edgeworth expansion is still possible, with the sparsity level directly affecting the convergence rate.

 
% In contrast to \citet{zhang-xia-network-edgeworth}, we consider Edgeworth expansions for standardized count statistics rather than studentized versions. While both expansions yield higher-order-correctness in the Kolmogorov metric, it is well-known that studentized bootstraps offer improved accuracy for confidence intervals while standardized bootstrap intervals do not; see \citet{hall-comparison-bootstrap}.  However, it is also known that these issues may be remedied by bias corrections, including the ABC method of \citet{efron-better-ci}.  Furthermore, confidence intervals of the standardized bootstrap are transformation invariant, which is a desirable property.  As another theoretical contribution, we derive correction terms for standardized count-statistics, yielding higher-order correct confidence intervals.  In contrast to previous work, our analysis also extends to smooth functions of counts such as transitivity, which are widely studied in applications.            

% Edgeworth expansions of studentized network moments were first studied by~\citet{zhang-xia-network-edgeworth}.  The authors show that the network noise has a ``smoothing" effect that allows them to bypass the typical Cramer condition, which is restrictive in the network setting.  We also bypass the Cramer condition for the bootstrap, but by using a different approach.  We choose a continuous multiplier that matches the first three moments of the data; it is well-known that continuous random variables satisfy Cramer's condition. To derive our Edgeworth expansion for the bootstrap, we also build upon results from ~\citet{wang-jing-weighted-bootstrap-u-statistics}  for order two U-statistics.  It turns out that network noise, particularly when the graph is sparse, causes certain terms related to our Edgeworth expansion to blow up. While the details are technical, we show that a valid Edgeworth expansion is still possible, with the sparsity level directly affecting the convergence rate.  

%\bl
%On the other hand, the linear bootstrap is not higher-order correct in any sparsity regime as it only aims to approximate the leading term of the Hoeffding decomposition. However for sparser networks, \rd simulations suggest that \bk the linear bootstrap outperforms the higher-order correct variants in terms of accuracy.  In essence, the extra terms in the quadratic bootstrap cannot be estimated accurately enough for sparse graphs and consequently these terms hurt more than they help in sparse regimes. %As discussed previously, we propose speeding up the  linear  bootstrap further by randomizing the precomputation of count functionals.  \rd Surprisingly, we show that randomization does not adversely affect coverage of the resulting intervals.  Randomization does affect the width of the confidence intervals (power for hypothesis testing), but for massive graphs, trading off accuracy for improved computation may be highly desirable. 
\bk
% By randomizing to an extent that is appropriate for the sparsity level of the network, we sacrifice very little statistical performance for vastly reduced computation.  Thus, the approximate linear bootstrap is well-suited for scalable inference on large, sparse graphs. 


% We show that degree of randomization allowed depends on the sparsity level of the graph.  If this sparsity condition is satisfied, in some sense we pay only minimal penalties in terms of accuracy for vastly improved computation.               

% Our proposal is also related to a two-step bootstrap procedure for count functionals proposed by \citet{levin-levina-rdpg-bootstrap}, which involves estimating the latent positions with the adjacency spectral embedding in the first step (see, for example, \citet{athreya-rdpg-survey}) and resampling the corresponding U-statistic with the estimated positions in the second step. However, for this estimation, the underlying network model's rank is required to be known and finite.  While it may be possible to relax this assumption, the procedure likely performs worse with an estimated rank.

% In contrast, our bootstrap procedure involves directly multiplying each potential subgraph in the network by a multiplier random variable. Applying the multiplier directly mimics the data generating process and we do not have to estimate the latent positions.  Furthermore, \citet{levin-levina-rdpg-bootstrap} consider only consider a linear bootstrap procedure, which does not offer improved accuracy for moderately sparse networks.




%  Edgeworth expansions of studentized network moments were first studied by~\citet{zhang-xia-network-edgeworth}.  The authors show that the network noise has a ``smoothing" effect that allows them to bypass the typical Cramer condition, which is restrictive in the network setting.  We also bypass the Cramer condition for the bootstrap, but by using a different approach.  We choose a continuous multiplier that matches the first three moments of the data; it is well-known that continuous random variables satisfy Cramer's condition. To derive our Edgeworth expansion for the bootstrap, we also build upon results from ~\citet{wang-jing-weighted-bootstrap-u-statistics}  for order two U-statistics.  It turns out that network noise, particularly when the graph is sparse, causes certain terms related to our Edgeworth expansion to blow up. While the details are technical, we show that a valid Edgeworth expansion is still possible, with the sparsity level directly affecting the convergence rate.




\bk  

% In other settings, the bootstrap introduced by~\citet{efron-jackkknife-bootstrap}, is a powerful inferential tool that operates on the principle of resampling the data to gauge variability.




% Under the sparse graphon model (see Section \ref{sec:sparse-graphon}), a count functional may be viewed as a U-statistic that is perturbed by asymptotically negligible Bernoulli noise. Viewing a count statistic as a (perturbed) U-statistic allows the adaptation of bootstrap methods for U-statistics (see, for example, \citet{bose-chatterjee-u-stats-resampling}) to network data.

% In particular our bootstrap procedure involves directly multiplying each potential subgraph in the network by a multiplier random variable. Applying the multiplier directly mimics the data generating process and we do not have to estimate the latent positions. We show that our multiplier bootstrap is higher-order correct under appropriate sparsity conditions.



% Recently, \citet{levin-levina-rdpg-bootstrap} proposed a two-step bootstrap procedure for count functionals that involves estimating the latent positions with the adjacency spectral embedding (see, for example, \citet{athreya-rdpg-survey}) in the first step and resampling the corresponding U-statistic with the estimated positions in the second step.  However, for this estimation, the underlying network model's rank is required to be known and finite.  While it may be possible to relax this assumption, the procedure likely performs worse with an estimated rank.

% In contrast, our bootstrap procedure involves directly multiplying each potential subgraph in the network by a multiplier random variable. Applying the multiplier directly mimics the data generating process and we do not have to estimate the latent positions. We show that our multiplier bootstrap is higher-order correct under appropriate sparsity conditions.





% Since this higher-order correct bootstrap is computationally expensive, we propose linear and quadratic approximations to the multiplier bootstrap, which correspond to the first and second-order H\'{a}jek projections of the U-statistic, respectively. Using only the linear term of the Hoeffding projection was also considered in ~\citet{levin-levina-rdpg-bootstrap}.  The linear approximation sacrifices higher-order accuracy at the cost of faster computation. In contrast, the quadratic multiplier may be viewed as a computationally efficient approximation to our multiplicative procedure that retains higher-order correctness under the same conditions. 






% Our observation is also in agreement with previous work on Edgeworth expansions for U-statistics \citep{Bentkus-edgeworth-symmetric,maesono-edgeworth-expansion-u-statistics,lai-symmetric-edgeworth}, which suggests that the bootstrap must preserve the first two terms of the Hoeffding decomposition for higher-order correctness. 


% In contrast to the higher-order correct procedures, the linear bootstrap requires estimating the coefficients of the quadratic term in the Hoeffding decomposition. These coefficients are scaled and centered local count statistics, like the number of subgraphs two nodes are involved in. While this leads to the loss of higher-order accuracy for dense degree regimes, for sparse networks, we observe an interesting phenomenon; in this case, the linear bootstrap outperforms the higher-order correct variants in terms of accuracy. Computationally, all multiplier bootstrap procedures require the precomputation of local and global count statistics. We present a randomized algorithm to compute these count statistics using a randomized algorithm in linear time.

%  Edgeworth expansions of studentized network moments were first studied by~\citet{zhang-xia-network-edgeworth}.  The authors show that the network noise has a ``smoothing" effect that allows them to bypass the typical Cramer condition, which is restrictive in the network setting.  We also bypass the Cramer condition for the bootstrap, but by using a different approach.  We choose a continuous multiplier that matches the first three moments of the data; it is well-known that continuous random variables satisfy Cramer's condition. To derive our Edgeworth expansion for the bootstrap, we also build upon results from ~\citet{wang-jing-weighted-bootstrap-u-statistics}  for order two U-statistics.  It turns out that network noise, particularly when the graph is sparse, causes certain terms related to our Edgeworth expansion to blow up. While the details are technical, we show that a valid Edgeworth expansion is still possible, with the sparsity level directly affecting the convergence rate.   
 
 
%This estimation step also complicates the theoretical analysis of their procedure.

% For certain functionals, the bootstrap is not only consistent but also higher-order correct \citep{singh-bootstrap-accuracy,hall-bootstrap-ci, lai-symmetric-edgeworth, wang-jing-weighted-bootstrap-u-statistics}, meaning that the bootstrap distribution converges to the true sampling distribution at a rate faster than the rate from the associated Berry-Esseen bound (i.e. error of normal approximation) under certain conditions. The key technical apparatus for establishing higher-order correctness is the Edgeworth expansion (see e.g. \citet{hall-bootstrap-edgeworth}), which may be viewed as a refinement of the Normal approximation that corrects for higher moments. 








% There has been much evidence that in presence of neurological disorders, including Alzheimer's disease, attention deficit hyperactivity disorder, autism spectrum disorder etc~\cite{Hedden2009, Tomasi2012, Rudie2013}, the connectivity network changes in comparison to that of a healthy brain. This leads to a natural statistical question, given two networks, can one two a two sample test to see if both are generated from the same underlying (unobserved) population? Existing work~\cite{kim2014} often summarize a network via a set of features and carry out a two sample test on that. Another line of work~\cite{durante2018} proposes fully parametric models and obtain testing procedures under those models. 

% In contrast, an important statistical direction would be to design a fully non-parametric two sample test. The main predicament of course, is that the nodes in a network are dependent, and hence one cannot use traditional techniques like bootstrap~\cite{efron-jackkknife-bootstrap}, subsampling~\cite{politis1994}, or related methods to obtain distributions of different statistics and compare those distributions. 

% In this respect, quantifying the variability of subgraph counts is paramount, as such estimates are needed for hypothesis testing and confidence intervals.  Recently, several procedures have been proposed for quantifying the uncertainty of subgraph frequencies; we will postpone a detailed discussion of this growing literature to the related work section.

% Generally speaking, the bootstrap, introduced by \citet{efron-jackkknife-bootstrap}, is a powerful inference tool. For certain functionals, the bootstrap is not only consistent but also higher-order correct \citep{singh-bootstrap-accuracy,hall-bootstrap-ci, lai-symmetric-edgeworth, wang-jing-weighted-bootstrap-u-statistics}, meaning that the bootstrap distribution converges to the true sampling distribution at a rate faster than the rate from the associated Berry-Esseen bound (i.e. error of normal approximation) under certain conditions. The key technical apparatus for establishing higher-order correctness is the Edgeworth expansion (see e.g. \citet{hall-bootstrap-edgeworth}), which may be viewed as a refinement of the Normal approximation that corrects for higher moments. 

% Recently \citet{zhang-xia-network-edgeworth} have derived network variants of the Edgeworth expansion for a class of count functionals introduced in \citet{Bickel-Chen-Levina-method-of-moments}.  Typically, Edgeworth expansions require that the distribution of interest is non-lattice. Intuitively, a lattice distribution's support is on equidistant points, for example,  (see~\cite{feller-vol-2} page 539). This  would rule out important classes of models such as the stochastic block models with equal sized blocks \citep{holland-sbm}, where the underlying latent positions are basically $k$ equidistant points in $[0,1]$. However, the aforementioned authors show that network noise has a smoothing effect, allowing accurate Edgeworth expansions even for lattice distributions under a mild sparsity condition.  Their work also shows that network resampling procedures like~\citep{Bhattacharyya-subsample-count-features,green-shalizi-network-bootstrap} also exhibit higher order correctness under mild conditions. However, these methods are either computationally intensive, or need careful tuning of hyperparameters. 

% In the present work, we introduce a new class of multiplier bootstraps for count functionals of networks.  Our procedure uses the fact that a count functional may be viewed as a U-statistic that is perturbed by asymptotically negligible Bernoulli noise. 

% This allows us to represent the network moments by their Hoeffding projection~\citep{hoeffding1948}, which is obtained by taking sequential projections of the U-statistic on the space of linear functions of $k$ tuples of random variables, $k\geq 1$. The first term in this sequence is the celebrated Hajek projection, which is used to show normal convergence of U-statistics. 

% Viewing a count statistic as a U-statistic naturally allows one to adapt the well studied sampling methods~\citep{bose-chatterjee-u-stats-resampling} for U statistics for networks. Recently, ~\citet{levin-levina-rdpg-bootstrap} proposed to directly estimate latent positions for a broad class of random graph models, and did inference for the count functional by bootstrapping a (conventional) U-statistic with estimated latent positions.  However, for this estimation, the rank of the underlying network model is required to be known and finite.  While it may be possible to relax this assumption, it is also likely that the procedure performs worse with an estimated rank.  In any case, this estimation step complicates the theoretical analysis of their procedure.

 %The sampling procedure is different from that in~\citep{chen2019randomized}

%, we build upon the recent work of 
              


% Furthermore, we explore in more detail the choice of random variable used for the multiplier.  In other settings, it is well-known that to attain higher order accuracy, the multiplier random variable should be chosen so that the bootstrap version of the functional matches the first three moments of the data \citep{liu-non-iid-bootstrap, mammen-wild-bootstrap, wang-jing-weighted-bootstrap-u-statistics}.

%Edgeworth expansions for U-statistics \citep{Bentkus-edgeworth-symmetric,maesono-edgeworth-expansion-u-statistics} also suggest that the bootstrap must preserve the first two terms of the Hoeffding decomposition of a U-statistic. Additive weights, discussed in \citet{bose-chatterjee-u-stats-resampling} and implemented in \citet{levin-levina-rdpg-bootstrap}, have strong computational properties, but it appears that they only approximate the leading term of the Hoeffding decomposition.  We show that two alternative forms for the weights, multiplicative and quadratic, achieve higher order correctness. In fact, the quadratic multiplier may be viewed as a computationally efficient approximation to the multiplicative multiplier that retains higher order correctness and may be preferable in many cases. 

% Since we establish an Edgeworth expansion for the statistic in question, we may also consider a procedure that involves plugging in estimated moments, leading to an ``empirical Edgeworth'' expansion. While such a procedure has its advantages of being fast and accurate, for smooth functions of counts, it is not straightforward to establish the corresponding Edgeworth expansion. However our experiments suggest that our bootstrap procedures may also be higher order consistent for these functionals.  

 In addition to obtaining Edgeworth expansions for count statistics, we also obtain Edgeworth expansions for smooth functions of U-statistics. We show that, under suitable sparsity assumptions, the cumulative distribution function of smooth functions arising from the quadratic bootstrap match this asymptotic expansion and are therefore higher-order correct. In this setting, obtaining analytical expressions for Edgeworth expansions are cumbersome, whereas the bootstrap is automatic and user-friendly.  
 % , since the general procedure remains the same.    

We will now provide a roadmap for the rest of the paper.  In Section~\ref{sec:related-work}, we discuss related work, focusing on the emerging area of resampling methods for network data.  The problem setting and our bootstrap proposal is introduced in Section~\ref{sec:setup}.  In Section~\ref{sec:main}, we present our main results, which establish higher-order correctness for our bootstrap procedures.  In Section~\ref{sec:exp}, we present experiments on both simulations and real data, which show that our procedures exhibit strong finite-sample performance in various settings.  %Finally, in Section~\ref{sec:realdata}, we use our bootstrap methods to compare real-world networks. % representing the voting similarities of U.S. Congress from 1949 to 2012. \rd We also use our method to compare networks for different page categories in Facebook data. \bk

==> network_mb_jasa_to_arxiv (1)/main_results_2.tex <==
% Before stating our theorems, we present some mild assumptions, similar to those in previous work.  In what follows, recall $\tau_n^2=\var[\E\{h(X_S)\mid X_1\}]$ denote the asymptotic variance of the  U-statistic.

% %\rd Fix later \bk 
 


% The first condition is a standard non-degeneracy assumption for U-statistics.   The second is a nontrivial sparsity assumption that we require for higher-order correctness.
 
 
  \subsection{Theoretical guarantees for approximate linear bootstrap}
 In this section, we show that the linear bootstrap statistic using the approximate moments in Eq~\ref{eq:define-h1-tilde} is indeed first-order correct under appropriate sparsity conditions as long as $N$ is large enough.  In this section, we make the following assumptions:
  % For theorem~\ref{thm:boot-linear-apx}, we will use the following assumption:
 \begin{assumption}\label{ass:linear}
  \begin{enumerate}
      \item[(a)] $\tau_n/\rho_n^s\geq c>0$, for some constant $c$.
    \item[(b)] $0<w(u,v)<C$, for some constant $C$.
  \end{enumerate}
 \end{assumption}
 The first condition is a standard non-degeneracy assumption for U-statistics.  Boundedness of the graphon is also a common assumption; this assumption can be relaxed at the cost of longer proofs.  % Our overall strategy follows \citet{chen2019randomized}.  
 In what follows, let:
\begin{align}\label{eq:def-sigmatildeAX}
\tilde{\sigma}^2_{|A,X}:= \mathrm{Var}(\tilde{T}_n - \hat{T}_n \ | \ A, X), \ \ \ \tilde{\sigma}_n^2 := E(\tilde{\sigma}^2_{|A,X})
\end{align}
% Recall from Equation~\ref{eq:def-sigmatildeAX} that $\noisesdax^2 = \var(\tilde{T}_n - \hat{T}_n \ | \ A,X)$ and $\noisesd^2 = E(\noisesdax^2)$.%, and $\nu_n^2 = \noisesd^2 + \sigma_n^2$. 
Our first result is a central limit theorem for approximate count statistics.  We show that, so long as $N \gg 1/n^2 \rho_n^s$, the appropriately scaled and centered count functional converges in distribution to a standard Normal.  This threshold ensures that the random conditional variance $\tilde{\sigma}^2_{|A,X}$ concentrates appropriately around its expectation $\tilde{\sigma}_n^2$.  Furthermore, our theorem below establishes two computation/sparsity regimes. When $N \gg 1/n \rho_n^s$, the limiting variance corresponds to the limiting variance of $\hat{T}_n$, given by $\sigma_n^2$, whereas when $1/n^2 \rho_n^s \ll  N \ll 1/n \rho_n^s$, the limiting variance is dominated by $ \tilde{\sigma}_n^2$, which captures the the effect of randomization.  The main technical difficulty is establishing appropriate concentration of $\tilde{\sigma}^2_{|A,X}$ when $N$ is small; our proof involves delicate combinatorial analysis and exploiting the degeneracy of an appropriate U-statistic.  See Supplement S2 for details. 
 \begin{theorem}\label{thm:clt-approx}
 Suppose that $\rho_n \rightarrow 0$ and either $R$ is acyclic and $n \rho_n \rightarrow \infty$ or $R$ is a simple cycle and $n^{r-1} \rho_n^r \rightarrow \infty$.  Moreover, suppose that $N \gg 1/n^2\rho_n^s$.  
 \begin{enumerate}
\item[(a)] (Variance of approximate count statistic $\tilde{T}_n$) 
\begin{align*}
\var(\tilde{T}_n) = 
\tilde{\sigma}_n^2 + \sigma_n^2, \text{ \ where \ } \sigma_n^2 = \Theta\left( \frac{\rho_n^{2s}}{n} \right) \text{ \ and \ } \tilde{\sigma}_n^2 = \Theta\left( \frac{\rho_n^{s}}{Nn^2} \right)
\end{align*}
Consequently, when $N\gg \frac{1}{n\rho_n^s}$, $\var(\tilde{T}_n)/\sigma_n^2\rightarrow 1$ and when $\frac{1}{n^2\rho_n^s}\ll N\ll \frac{1}{n\rho_n^s}$, 
$\var(\tilde{T}_n)/\tilde{\sigma}_n^2\rightarrow 1$.
\item[(b)] (CLT for approximate count statistic $\tilde{T}_n$)
 \begin{align*}
 \sup_{u} \left| P\left( \frac{\tilde{T}_n - \theta_n}{ \sqrt{\noisesd^2 + \sigma_n^2}} \leq u  \right) - \Phi(u)    \right| \rightarrow 0
 \end{align*}
 \end{enumerate}
 \end{theorem}
 
 Our next result establishes the consistency of our bootstrap procedure under appropriate conditions.  For a broad range of computational regimes, ranging from $1/n^2 \rho_n^s \ll N \ll 1/n \rho_n^s$ to $N \gg 1/n \rho_n^s$, we show that bootstrap consistently approximates the distribution of $\tilde{T}_n$. In the regime $N \gg 1/n \rho_n^s$, the bootstrap is $\sqrt{n}$-consistent whereas in the other aforementioned regime, the bootstrap offers faster computation while still providing vanishing confidence intervals.   Our proof here again involves combinatorial analysis and tight bounds for appropriate higher-order moments; see Supplement S2 for details. \bk
 
 \begin{theorem}\label{thm:boot-linear-apx}
%%%%%%%%% The commented out part below is already stated in Theorem 6 now %%%%%%%%%%


%Let the variance of the bootstrap estimator be given by
%\begin{align*}
%\bootsd^2 := \dfrac{c_n^2}{n^2}\sum_{i=1}^n (\tilde{H}_1(i) - \tilde{T}_n)^2.
%\end{align*}
%where $c_n=r$ when $Nn\rho_n^s\gg 1$ and $c_n=1$ otherwise. We have that if $ N = \omega(1/n \rho_n)$ or $N= \omega(1/n \rho_n), N=o(\omega(1/n \rho_n) $ 
%\begin{align*}
%\frac{\bootsd}{\nu_n} \xrightarrow{P} 1    
%\end{align*}
%Moreover,
Suppose that $\rho_n \rightarrow 0$, $r \geq 2$ and either $R$ is acyclic and $n \rho_n \rightarrow \infty$ or $R$ is a simple cycle and $n^{r-1} \rho_n^{r} \rightarrow \infty$. Let $\mathcal{R}$ denote the independent random variables determining the random permutations chosen with replacement.
\begin{enumerate}
    \item[(a)] When $1/n^2\rho_n^s\ll N\ll 1/n\rho_n^s$, we have $\var(\tilde{T}_{n,L}^*|A,X,\mathcal{R})/\tilde{\sigma}_n^2\stackrel{P}{\rightarrow} 1$. In contrast, when $ N\gg 1/n\rho_n^s$, we have $\var(\tilde{T}_{n,L}^*|A,X,\mathcal{R})/\sigma_n^2\stackrel{P}{\rightarrow} 1$.

\item [(b)]
When $1/n^2\rho_n^s\ll N\ll 1/n\rho_n^s$ or $N\gg 1/n\rho_n^s$, we have 
\begin{align*}
\sup_{u} |P( \tilde{T}_{n,L}^* - \tilde{T}_n   \leq u) - P( \tilde{T}_n - \theta_n   \leq u)     | \xrightarrow{P} 0.    
\end{align*}
\end{enumerate}
\end{theorem}

\begin{remark}

     As seen in Theorem~\ref{thm:clt-approx}, $N=\Theta(1/n\rho_n^s)$ is where a phase transition occurs. When $N$ is a smaller (or larger) order than this threshold, the variance of the bootstrapped statistic $\tilde{T}_{n,L}^*$ converges to variance of the approximate count statistic $\tilde{T}_n$. However, at the point of the phase transition, the bootstrap variance does not match the variance of the approximate count statistic.  In some sense, this is unavoidable since U-statistics and averages of independent random variables have fundamentally different structure owing to the dependence of U-statistics; thus, one cannot mimic the structure of both components with this approach simultaneously. From a practical standpoint, this is not a problem since the user can choose $N$ to be either in the smaller or larger order regimes.  Moreover, at the boundary, one can always opt for a conservative estimate of the variance.      
     
    %  because the sparsity level is estimable and based on this estimate and computational constraints, 
    %  the user can choose $N$ to be either in the smaller or larger order regimes. 
     
    %  This is not surprising because the U-statistic underlying the count statistics has an additional factor of $r$ which is not there in a sum of independent random variables.
    
 \end{remark}
 
 
%  \rd Our theorem below is the first in the literature to establish a rate of convergence for inferential methods in the sparse regime, where $ \rho_n = \omega(1/n)$ for acyclic graphs.  \bk %We establish the theorem for $\ttnl$ and conditions on $N$ below. 

% \begin{theorem}\label{thm: apprx-linear-bootstrap}
% Suppose  Assumption~\ref{ass:linear} is satisfied,  
%  the weights $\w_1,\dots,\w_n$ are generated from a distribution such that $\E[\xi_1] = 1$, $\E[(\xi_1-1)^2] = 1$,  $\E[(\xi_1-1)^3] < \infty$.  Further assume that  $\rho_n =\omega(1/n) $ when $R$ is acyclic or  $\rho_n=\omega(n^{-1/r})$ when $R$ is cyclic. Then,   %$n^{s-1} \rho_n^s \rightarrow \infty $ and $R$ is a $r$-cycle.   Then,  \bk 
%  \begin{enumerate}
%  \item[(a)] The standardized bootstrap distribution converges at the Berry-Esseen rate to a standard Normal: 
% %\rd If $N\geq \max(1,\rho^{-s}k/n)$, then,
% \begin{align}\label{eq:BE-approx}
%   \sup_{u \in R} \bigg{|}P^*\bb{\frac{\ttnl-\tilde{T}_n}{\{\var(\ttnl \mid A,X)\}^{1/2}}\leq u} -\Phi(u)\bigg{|}=  O_P\left(n^{-1/2}\right),
% \end{align}
% where $P^*(\cdot)$ denotes the conditional measure conditioned on $A$ and $X$.

% \rd 
% Propose to change (a) to 
% \item[(a)]  Let $\tilde{\sigma}_n^2 = \var(\tilde{T}_n - \theta_n)$.  For any $N >0$, the following form of bootstrap consistency holds:
% \begin{align}\label{eq:BE-approx}
%     &\sup_{t\in R}\bigg{|}P^*\left(\frac{\ttnl-\Tilde{T}_n}{\tilde{\sigma}_n }\leq t\right)-P\left(\frac{\tilde{T}_n-\theta_n}{\tilde{\sigma}_n}\leq t\right)\bigg{|} \xrightarrow{P} 0
%     % \\&= O_P({n^{-1/2}}) + O_P\left(\frac{1}{n\rho_n}\right)+O_P\left(\frac{1}{Nn\rho_n^s} \right) + 
%     % O(\mathcal{M}(n,\rho_n,R))+O_P\left(\frac{1}{n^{1/2}\rho_n^{3s}}\right) \nonumber.
% \end{align}
% where $P^*(\cdot)$ denotes the conditional measure conditioned on $A$ and $X$
% Moreover, $\tilde{\sigma}_n$ satisfies:  
% \begin{align}
% \tilde{\sigma}_n = O\left(\sqrt{\frac{\rho_n^{2s}}{n}}\right) + O\left(\sqrt{\frac{\rho_n^s}{Nn}}\right)
% \end{align}

% \bk
% % \item[(b)] For $N = \Omega(\rho_n^{-s+1})$, the Kolmogorov distance between bootstrap distribution and sampling distribution satisfies:
% % \begin{align*}
% %     \sup_{u \in R} \bigg{|}P^*\bb{\frac{\ttnl-\tilde{T}_n}{r\{\var(\ttnl-\tilde{T}_n\mid A,X)\}^{1/2}}\leq u} - P\left(\frac{\hat{T}_n - \theta_n}{\sigma_n} \leq u \right) \bigg{|} = O_P((n\rho_n)^{-1/2})
% % \end{align*}
% \item[(b)]  When $N \gg \rho_n^{-s}/n$, consistency with respect to the distribution of $\hat{T}_n - \theta$ holds:
% \begin{align}\label{eq:BE-approx-2}
%     &\sup_{t\in R}\bigg{|}P^*\left(\frac{\ttnl-\Tilde{T}_n}{\sigma_n }\leq t\right)-P\left(\frac{\hat{T}_n-\theta_n}{\sigma_n}\leq t\right)\bigg{|} \xrightarrow{P} 0
%     % \\&= O_P({n^{-1/2}}) + O_P\left(\frac{1}{n\rho_n}\right)+O_P\left(\frac{1}{Nn\rho_n^s} \right) + 
%     % O(\mathcal{M}(n,\rho_n,R))+O_P\left(\frac{1}{n^{1/2}\rho_n^{3s}}\right) \nonumber.
% \end{align}    






% % The variance of $\ttnl$ satisfies:
% % %$1-1/\log^\epsilon(n)$, %\rd for $N>\frac{k}{n\rho^s}$,\bk
% % \begin{align}\label{eq:approx-var}
% % % \frac{\var(\ttnl-\tilde{T}_n\mid A,X)}{n\rho^{2s}}=\frac{\tau_n^2}{\rho^{2s}}\left(1+O_P\left(\frac{1}{n\rho_n}\right)\right)+(\log n)^{\epsilon}O\left(\frac{r}{Nn\rho^s} \right).
% %  \frac{ \ \var(\ttnl \mid A,X)}{\sigma_n^2}=1+O_P\left(\frac{1}{n\rho_n}\right)+O_P\left(\frac{1}{Nn\rho_n^s} \right).
% % \end{align}



% % \item[(c)] If $\ttnl$ in Eq \ref{eq:BE-approx} is replaced by the \rd $\cfbl$\bk \bl (was $T_{n,L}$ here before, wrong notation as Refree 1 pointed out, un-approximated linear bootstrap should be $\cfbl$ as Eq~\ref{eq:cfbl}) \bk  computed without approximate moments and $\tilde{T}_n$ is replaced by $\hat{T}_n$, then Eq \ref{eq:BE-approx} holds. We also have:
% % \begin{align}\label{eq:linear-var}
% % % \frac{\var(\ttnl-\tilde{T}_n\mid A,X)}{n\rho^{2s}}=\frac{\tau_n^2}{\rho^{2s}}\left(1+O_P\left(\frac{1}{n\rho_n}\right)\right)+(\log n)^{\epsilon}O\left(\frac{r}{Nn\rho^s} \right).
% % %  \frac{\ \var(\cfbl\mid A,X)}{\sigma_n^2}=1+O_P\left(\frac{1}{n\rho_n}\right).
% % \end{align}


% \end{enumerate}


\begin{remark}
    % Theorem~\ref{thm:boot-linear-apx} establishes that the distribution of approximate linear bootstrap converges to a normal distribution.
    % It is natural to wonder what value is added by the linear method to a direct normal approximation. The advantage is two-fold. 
     The advantage of the fast linear bootstrap over a direct Normal approximation is that it is automatic and more user-friendly.
     Estimating parameters of the limiting normal for count statistics using estimated sparsity parameter or smooth functions of counts such as the transitivity (suitably normalized ratio of triangles and two stars) requires additional analytic calculations which can be cumbersome for a practitioner. The bootstrap presents a user-friendly alternative, where one replaces burdensome calculations by computer simulations.  However, our analysis also sheds light on the properties of a Normal approximation using approximate count statistics. Therefore, the approximate moment computation proposed in this section can be also used to estimate the limiting variance in both the small and large $N$ setting.  
     
    %  approximate moment computation proposed in this section can be also used to estimate the limiting variance in both the small and large $N$ setting. %Overall, our analysis also provides insight into the limiting variance of the normal distribution in the low $N$ setting, since there the limiting variance is dominated by that arising from the noise.
\end{remark}
% \textbf{
% Referee's words:
% Even though the authors, in Theorem 2, show that the standardized
% bootstrap distribution of the (approximate) linear bootstrap statistics
% converges at the Berry-Esseen rate to a standard Normal, the
% advantages of the (approximate) linear bootstrap method over the
% Normal approximation is still not clear. Maybe, the author needs to
% show the difference of (approximate) linear bootstrap method and the
% method of Normal approximation. Only in this way can the advantage
% of (approximate) linear bootstrap method be shown more clearly.
% }
% Furthermore,  we have, \rd with probability at least $1-o(1)$,
% %$1-1/\log^\epsilon(n)$, %\rd for $N>\frac{k}{n\rho^s}$,\bk
% \begin{align}\label{eq:approx-var}
% % \frac{\var(\ttnl-\tilde{T}_n\mid A,X)}{n\rho^{2s}}=\frac{\tau_n^2}{\rho^{2s}}\left(1+O_P\left(\frac{1}{n\rho_n}\right)\right)+(\log n)^{\epsilon}O\left(\frac{r}{Nn\rho^s} \right).
%  \frac{\var(\ttnl-\tilde{T}_n\mid A,X)/n}{\tau_n^2}=1+O_P\left(\frac{1}{n\rho_n}\right)+\tilde{O}\left(\frac{r}{Nn\rho^s} \right).
% \end{align}
% If $\ttnl$ in Eq \ref{eq:BE-approx} is replaced by the $T_{n,L}$ computed without approximate moments, and $\tilde{T}_n$ is replaced by $\hat{T}_n$, then Eq \ref{eq:BE-approx} holds, and  with probability $1-o(1)$, we also have:
% \begin{align}\label{eq:linear-var}
% % \frac{\var(\ttnl-\tilde{T}_n\mid A,X)}{n\rho^{2s}}=\frac{\tau_n^2}{\rho^{2s}}\left(1+O_P\left(\frac{1}{n\rho_n}\right)\right)+(\log n)^{\epsilon}O\left(\frac{r}{Nn\rho^s} \right).
%  \frac{\var(T_{n,L}^*-\hat{T}_n\mid A,X)/n}{\tau_n^2}=1+O_P\left(\frac{1}{n\rho_n}\right).
% \end{align}

%\end{theorem}

\begin{remark}[Comparison to existing work on approximating $U$- statistics]
	In~\cite{chen2019randomized}, the authors draw $\omega(n)$ subsets of size $r$ from all ${n\choose r}$ subsets with replacement to estimate an incomplete $U$-statistic. The total number of subsets
	we examine for approximating a local count statistic is also $\omega(n)$. Comparing our Theorem~\ref{thm:boot-linear-apx} with their result shows that both
	methods require similar computation to achieve consistency. However, practically, drawing $Nn/r$ subsamples with replacement seems to be slower than drawing a $N$ permutations
	and then dividing each into disjoint subsets (see Fig~\ref{fig:4cycle-timing}). While they also consider the effect of randomization on the Gaussian approximation, our results take into account the sparsity level, and require delicate and novel combinatorial analysis.
	\end{remark}

%\rd Change remark 2 and remark 3 \bk
\begin{remark}[Approximation quality]
%In the above theorem,  if  $Nn/r = \omega(\rho_n^{-s})$, then the ratio of the variance of the linear bootstrap statistic and that of the count statistic in question converges in probability to one. This shows that for sparse networks we need larger number of random permutations to estimate the moments. \rd 
%Recall from Eq~\ref{eq:def-sigmatildeAX} that $\tilde{\sigma}_{\mid A,X}$ denotes $\var(\ttnl \mid A,X)$. 
Let $\hat{\nu}_n^2$ denote $\var(\ttnl \mid A,X,\mathcal{R})$.
The standardized  bootstrap CI with coverage $\alpha$ constructed from the approximated linear bootstrap $\ttnl$ can be written as $$\bb{\frac{\tilde{T}_n-\hat{\nu}_nz_{\frac{1-\alpha}{2}}}{\rho_n^s},\ \ \frac{\tilde{T}_n-\hat{\nu}_nz_{\frac{1+\alpha}{2}}}{\rho_n^s}}$$ where $z_{\frac{1-\alpha}{2}}$ and $z_{\frac{1+\alpha}{2}}$ are the $\frac{1-\alpha}{2}$ and $\frac{1+\alpha}{2}$ quantiles from the standard normal distributions.
%When $N\gg 1/n\rho_n^s$, Theorem~\ref{thm:boot-linear-apx} states that $\var(\ttnl \mid A,X,\mathcal{R})=\Theta(\rho_n^{2s}/n)$, and hence the CI width goes to zero. 
When $1/n^2\rho_n^s\ll N\ll 1/n\rho_n^s$, Theorem~\ref{thm:boot-linear-apx} states that $\var(\ttnl \mid A,X,\mathcal{R})=\Theta(\rho_n^{s}/nN)$ and hence the CI width vanishes, thus leading to consistent estimation of the parameter of inferential interest. 
%For the width of the confidence interval to converge in probability to $0$ as $n \xrightarrow[]{} \infty$, we need $\tilde{\sigma}_{\mid A,X}/\rho_n^s \ll 1$, which is achieved when $N >> \frac{1}{n^2\rho_n^s}$. 
For estimated $\rho_n$ these intervals can be established using a delta method approach.\bk %\rd Experimentally, we saw that a constant times logarithm of $n$ permutations suffice. \bk
%$O\left(\frac{r}{Nn\rho^s} \right)=o(1)$. Since $\tau_n=\Theta(\rho^s)$, we have, under the condition that  $N >> \rho^{-s}r/n$, $\frac{\var(\ttnl-\tdu\mid A,X)}{n}$ converges in probability to $\tau_n^2$.
\end{remark}
%Similar to \cite{zhang-xia-network-edgeworth}, we also define an empirical edgeworth expansion, in particular $\gnhat$ in Eq \ref{eq:gnhat}. 

\begin{remark}[Broader Sparsity Regime]\label{rem:apx}
Theorem~\ref{thm:boot-linear-apx} suggests that the linear bootstrap with a suitably large $N$ gives a consistent estimate of variance under much weaker conditions on sparsity than that needed for establishing higher order correctness (Theorem~\ref{thm:mbq-firstorder} and Corollary~\ref{thm:mbm-firstorder}).  It should be noted that the arguments in \cite{zhang-xia-network-edgeworth} require $\rho_n = \omega(1/\sqrt{n})$ for acyclic graphs and therefore, their convergence rates for empirical Edgeworth expansions do not hold in sparser regimes.  \bk
\end{remark}


\bk
%Finally, we conclude this section with a note on smooth function of counts. %While we do not establish an Edgeworth expansion for smooth functions, we show that under suitable assumptions,  the conditional CDF of the quadratic multiplier bootstraps is a higher order correct approximation of the CDF of the  smooth function of the conditional expectation of the count statistics.
% \rd 
% \begin{remark}
% Confidence intervals converge at rate
% \end{remark}
% \bk
 
 
%\citet{zhang-xia-network-edgeworth} establish an Edgeworth expansion for count functionals with an estimated variance. 
\subsection{Results on higher-order correct bootstrap procedures}
Below, we establish an Edgeworth expansion normalized by the true standard deviation, which is more appropriate for our purposes.  Since estimating the variance leads to a non-negligible perturbation, the polynomials in our expansion differ from those established by \cite{zhang-xia-network-edgeworth}.  All proofs and details are deferred to Supplement Section \ref{sec:suppprop3} and Section \ref{sec:suppthm23}. \bk In what follows, let $F_n(u)$ denote the CDF of $\hat{T}_n$ and $G_n(u)$ denote the Edgeworth expansion of interest, given by:

%
\begin{equation}\label{eq:edgeworth-gn}
    G_n(u)= \Phi(u)- \phi(u)\frac{(u^2-1)}{6n^{1/2}\tau_n^3}\biggl[E\{g_1^3(X_1)\}+3(r-1)E\{g_1(X_1)g_1(X_2)g_2(X_1,X_2)\} \biggr].
\end{equation}

Furthermore, recall $\tau_n^2=\var[\E\{h(X_S)\mid X_1\}]$ denotes the asymptotic variance of the  U-statistic.  Throughout this section, we will impose the following condition:

 \begin{assumption}\label{ass:sparse}
  For acyclic $R$, $\rho_n = \omega(n^{-1/2})$ and for cyclic $R$,  $\rho_n = \omega(n^{-1/r})$.
 \end{assumption}
 
\iffalse
\begin{assumption}\label{ass:sparse}
 We assume the following:
 \begin{enumerate}
     \item[(a)] $\tau_n/\rho_n^s\geq c>0$, for some constant $c$.
     \item[(b)] For acyclic $R$, $\rho_n = \omega(n^{-1/2})$ and for cyclic $R$,  $\rho_n = \omega(n^{-1/r})$
     % \item $0<w(u,v)<C$, for some constant $C$.
 \end{enumerate}
\end{assumption}
\fi
  The above is a nontrivial sparsity assumption that we require for higher-order correctness.
We have the following result:
\bk 

\begin{proposition} 
\label{prop:ew}%[Edgeworth Expansion for Count Functionals] 
Let $G_n$ be the Edgeworth expansion defined in Eq \ref{eq:edgeworth-gn} and let $R$ be a fixed subgraph. Suppose that Assumptions \ref{ass:linear} and \ref{ass:sparse} hold.  Further suppose that $\rho_n=O(1/\log n)$ or Cram\'{e}r's condition holds, i.e. $\limsup_{t\rightarrow \infty} \left|\E\left\{e^{itg_1(X_1)/\tau_n}\right\}\right|<1$ then we have,
\begin{align}
\sup_u \left| F_{n}(u) - G_n(u) \right| = O(\mathcal{M}(n, \rho_n , R))
\end{align}
where $F_{n}$ is the cumulative distribution function of $\frac{\hat{T}_n-\theta_n}{\sigma_n}$ and 
\begin{align}
\label{eq:M-def}
\mathcal{M}(n,\rho_n,R) = \begin{cases} 
      \frac{1}{n\rho_n} & \text{R is acyclic} \\
       \frac{1}{n\rho_n^{r/2}} & \text{R is cyclic} 
  \end{cases}
\end{align}
\end{proposition}

Now, we will state our bootstrap approximation results.  
We will first show that conditioned on the network, and latent variables, the CDF of \mbq matches the asymptotic expansion in Eq \ref{eq:edgeworth-gn}, where the true moments are replaced by their empirical versions. In what follows, let $\hat{E}_n(\cdot)$ denote the expectation operator with respect to the empirical measure of $A$ and $X$. Define
 \begin{equation}\label{eq:gnhat}
   % \gnhat(u) = \Phi(u) -\frac{(u^2-1)\phi(u)}{6n^{1/2}\hat{\tau}_n^3}\left[ \text{ \stackon[-6pt]{$g_1^3$}{\vstretch{1}{\hstretch{2.0}{\widehat{\phantom{\;}}}}}}+ 3(r-1) \text{\ \stackon[-8pt]{$g_1(i)g_1(j)g_2(i,j)$}{\vstretch{1.5}{\hstretch{9.0}{\widehat{\phantom{\;}}}}}}\ \right],
%\widehat{g_1(i)g_1(j)g_2(i,j)})\right]
 \gnhat(u) = \Phi(u) -\frac{(u^2-1)\phi(u)}{6n^{1/2}\widehat{\tau}_n^3}\left[\widehat{E}_n\left\{g_1(i)^3\right\}+ 3(r-1) \widehat{E}_n\{g_1(i)g_1(j)g_2(i,j)\} \right],
 \end{equation}
where we have:
 \begin{equation}\label{eq:empmoment}
 \begin{split}
  %  &\hat{\tau}_n^2=\sum_i \frac{\hat{g}_1(i)^2}{n}, \bk \quad
  &\widehat{E}_n\left\{g_1(i)^3\right\} = \frac{1}{n}\sum_{i=1}^n \gi^3, \\
    &\widehat{E}_n\{ g_1(i)g_1(j)g_2(i,j) \}=\frac{1}{{n \choose 2}}\sum_{1 \leq i<j\leq n}\tilde{g}_2(i,j)\gi\gj. %\rd \times \frac{n}{n-1}\bk.
 \end{split}
 \end{equation}
\begin{theorem}\label{thm:mbq-firstorder}
If  Assumptions \ref{ass:linear} and \ref{ass:sparse} are satisfied, 
 the weights $\w_1,\dots,\w_n$ are generated from a non-lattice distribution (see \cite{feller-vol-2} page 539) such that $\E[\xi_1] = 1$, $\E[(\xi_1-1)^2] = 1$,  $\E[(\xi_1-1)^3] = 1$, then 
%  with probability tending to one, we have,
$$\sup_u\left|P^*\left(\frac{\cfbq-\tnhat}{\shat} \leq u \right)-\gnhat(u)\right|= o_P(n^{-1/2})  + O_P\left(\frac{\log n}{n^{2/3}\rho_n}\right),$$
where $P^*(\cdot)$ denotes the conditional probability of event $(\cdot)$ conditioned on $A$ and $X$.

\end{theorem}
%\begin{proofsketch}
%
%\end{proofsketch}


\begin{remark}
	\label{remark:standardvsstudent}
	While the above theorem is for standardized bootstraps, our proof may be adapted to yield an analogous statement for bootstraps studentized by a variance estimator inspired by the Delta Method.  In essence, the studentized bootstrap may also be expressed as a weighted U-statistic and a negligible remainder term, allowing the use of similar proof techniques.    
\end{remark}

\begin{remark}
	While \cite{zhang-xia-network-edgeworth} establish higher-order correctness under milder sparsity conditions for subsampling and the empirical graphon, our result here does not require Cram\'{e}r's condition for $g_1(X_i)$, which is an important feature for network applications.  Our simulation study suggests that our rate here can be improved, but we leave this to future work. \bk
\end{remark}

Combining Theorem \ref{thm:mbq-firstorder} with the Hoeffding decomposition in Eq \ref{eq:boot-hoeff}, we obtain the corollary below for the multiplicative bootstrap.  Since the remainder term in the Hoeffding decomposition concentrates slowly for well-connected subgraphs of sparser networks, we impose additional assumptions on the subgraph to maintain the rate from the previous theorem. 
% The argument involves using a smoothing argument using the error term in Eq \ref{eq:boot-hoeff}.
\begin{corollary}\label{thm:mbm-firstorder}
Suppose Assumption \ref{ass:linear} is satisfied and either R is acyclic and $\rho_n = \omega(1/\sqrt{n})$ or R is a simple cycle and $\rho_n = \omega(n^{-1/r})$.  Further suppose that the weights $\w_1,\dots,\w_n$ are generated from a non-lattice distribution with such that $\E(\xi_1) = 1$, $\E\{(\xi_1-1)^2\} = 1$,  $\E\{(\xi_1-1)^3\} = 1$, then, %\rd should we state $\hat{\sigma}_n=r\hat{\tau}_n/n^{1/2}$? or is it clear enough from Eq(4), PS: Eq 4 is numbered but not labeled nor cited \bk
% with probability tending to one,
% we have,
% $$\sup_u\left|P^*\left(\frac{\cfbm-\tnhat}{\shat}\right)-\gnhat(u)\right|= o(n^{-1/2})  + O\left(\frac{\log n}{n^{2/3}\rho_n}\right),$$

$$\sup_u\left|P^*\left(\frac{\cfbm-\tnhat}{\shat} \leq u \right)-\gnhat(u)\right|= o_P(n^{-1/2})  + O_P\left(\frac{\log n}{n^{2/3}\rho_n}\right),$$


% $$\sup_u\left|P^*\left(\frac{\cfbm-\tnhat}{\shat}\right)-\gnhat(u)\right|= o(n^{-1/2})  + O\left(\frac{\log n}{n^{2/3}\rho_n}\right),$$
where $P^*(\cdot)$ denotes the conditional probability of event $(\cdot)$ conditioned on $A$ and $X$ and $\hat{\sigma}_n=r\hat{\tau}_n/n^{1/2}$.
\end{corollary}
%\rd now have to show $\gnhat$ converges to $G_n$. \bk

% \begin{remark}
% The above theorems show that \mbq and \mbm are both higher-order correct. Note that, for acyclic subgraphs, our rate is not as sharp as the rate in Proposition \ref{prop:ew}. We believe this can be tightened and leave this for future work. We also want to point out that while the normal approximation of count statistic yields $O(n^{-1/2}\rho_n^{-1/2})$ error (see \cite{Bickel-Chen-Levina-method-of-moments}), as long as $\rho_n\gg (\log n)^2/n^{1/3}$,  our error term is of smaller order than $O(n^{-1/2}\rho_n^{-1/2})$.
% \end{remark}


% \rd
% %\begin{remark}
% 	Note that Corollary~\ref{thm:mbm-firstorder} holds for acyclic subgraphs and simple cycles since for these graphs the remainder term of the Hoeffding decomposition of 	the multiplier bootstrap statistic is bounded. However the quadratic bootstrap only uses the first two terms of the Hoeffding decomposition, and thus Theorem~\ref{thm:mbq-firstorder} holds for acyclic and cyclic subgraphs, where the later includes any subgraph which has at least one cycle. 
% %	\end{remark}
% \bk
% Note that if we did not have Bernoulli noise, the proof of Theorems \ref{thm:mbq-firstorder} and \ref{thm:mbm-firstorder} would have been a direct consequence of results from \citep{wang-jing-weighted-bootstrap-u-statistics}, which establishes higher order correctness of weighted bootstrap.

The proof of Theorem \ref{thm:mbq-firstorder} build upon results from \citet{wang-jing-weighted-bootstrap-u-statistics}\bk, which establish higher-order correctness of the weighted bootstrap for order-2 U-statistics.  However, certain terms that appear as constants in their work blow up when perturbed by sparse network noise. To deal with this issue, we control various terms unique to the network setting and use different arguments to control the overall error rate.  

Similar to \cite{zhang-xia-network-edgeworth}, we now consider an empirical Edgeworth expansion in which the expected quantities of interest are estimated.
%As in \cite{zhang-xia-network-edgeworth}, it is also possible to consider an empirical Edgeworth expansion in which the expectations of interest are estimated.  We state a result for this procedure below:
 % Finally, the Edgeworth expansion provides  a way to do empirical Edgeworth expansions as below.
% and make the rate significantly worse.
% To remedy this, we had to keep track of the constants and use different arguments to control the overall error rate.
% We have deferred the proofs to Supplement Section \ref{sec:supp:thm34}.
%\rd fix later \bk
 %\subsection{Empirical Edgeworth Expansions}
   % Since $\E\{g_2(X_1,X_2)g_1(X_1)g_1(X_2)\}=\E[\E\{h(X_S)-\theta_n\mid X_1,X_2\}g_1(X_1)g_1(X_2)]$, we also have:
   \begin{lemma}\label{lem:convEW}
Under the assumptions in Assumption \ref{ass:linear} and \ref{ass:sparse}, we have 
% (see Supplement Section \ref{sec:suppthm23} for the proof):
\begin{align*}
    \sup_u|\gnhat(u)-F_n(u)|= O_P(\mzx)
\end{align*}
\end{lemma}
 The lemma above suggests that the empirical Edgeworth expansion achieves a better rate than the bootstrap procedures considered.  In the experimental section, we see that the empirical Edgeworth expansion (\ew) in fact achieves the smallest error when the network is dense enough. 
  % We call this method the empirical Edgeworth 
  % While experimentally we see that the empirical Edgeworth corrections have the lowest error in the higher average degree regime,
  However, for smooth functions of counts, it is cumbersome to derive such expansions and the bootstrap emerges as a strong practical alternative that offers improved accuracy over a Normal approximation in certain regimes.       \bk
   %one can show that, if Assumption \ref{ass:sparse} is satisfied, then with high probability, $$\sup_u |\gnhat(u)-G_n(u)|=O(\mathcal{M}(n, \rho_n , R)).$$

 %Since the proof is similar to \cite{zhang-xia-network-edgeworth}, 
% The proof is deferred to the Supplement Section \ref{sec:suppthm23} .
 
 % This leads to a natural question: why not use the empirical Edgeworth expansion to estimate the sampling distribution of the statistic $\cfhat$. We show that, indeed, this 
 % \rd The above result  \bk
 
% \iffalse
\subsection{Smooth functions of count statistics}\label{sec:smf}
%Consider a smooth function $g$ of $d$ count statistics for subgraphs with $r_1,\dots,r_d$ nodes and $s_1,\dots,s_d$ edges. Let $\bu$ denote the vector of conditional expectation of the respective count statistics. Define $S_n=n^{1/2}(f(\bu)-f(\bmu))/\sigma$.  Let $u^*$ be bootstrapped vector of scaled count functionals  $\{\frac{\cfbq{(1)}}{\rho^{s_1}},\ldots, \frac{\cfbq{(d)}}{\rho^{s_d}}\}$.

% In this section, we study Edgeworth expansions for the bootstrap for smooth functions of count frequencies. 
In network science, the transitivity coefficient, which may be defined as a smooth function of triangles and two-stars, is commonly used to quantify how much nodes in the network cluster together. Given the importance of such functions in applications, accurate inference for these parameters is naturally of substantial interest. Our results in this section establish the quadratic and multiplicative bootstraps as  accurate and user-friendly methods for smooth functions of counts that sidestep the cumbersome computation of gradients and moments required by empirical Edgeworth expansions.

%\rd Our theorem below is the first result in the literature for Edgeworth expansions of smooth functions of count statistics.  In fact, to the best of our knowledge, Edgeworth expansions for smooth functions of U-statistics were not derived previously.  \bk
To the best of our knowledge, below we provide the first result on Edgeworth expansions for smooth functions of U-statistics.  It turns out that arguments to derive Edgeworth expansions for smooth functions of IID means such as those in \citet{hall-bootstrap-edgeworth} depend heavily on the properties of cumulants of independent random variables and require multivariate Edgeworth expansions, complicating extensions even to U-statistics.  In contrast, we adapt flexible Edgeworth expansion results of \citet{jing2010unified} to approximate non-negligible terms arising from a Taylor approximation of the smooth functional.

To state our result, we need to introduce some additional notation.   Let $\bu$ denote a d-dimensional vector of count functionals, let $\bu^*$ be a vector of corresponding bootstrap statistics generated by either the multiplier bootstrap $\hat{T}_{n,M}^*$ or the the quadratic bootstrap $\hat{T}_{n,Q}^*$.  Furthermore, let $f: \mathbb{R}^d \mapsto \mathbb{R}$ denote the function of interest.  
% ; in the latter case, one may ignore an additional negligible term that arises from approximating a U-statistic by the first two terms of the Hoeffding decomposition.   
Consider the following smooth function of bootstrapped count frequencies:
\begin{align}
\label{eq-snstar}
S_n^*=n^{1/2}\{f(\bu^*)-f(\bu)\}/\tdsigf
\end{align}
 where  $\tdsigf$ is used to standardize the bootstrap version and will be defined shortly.  The standard Delta Method involves a first-order Taylor expansion; to attain higher-order correctness, we need to consider a second-order expansion.  We use the following notation to denote the derivatives of interest  evaluated at the expectation $E(\bu) = \bmu$: 
 \begin{align}%\label{eq:EW-SMF-aij}
\label{eq:ai}
  &  a_i=\frac{\partial f(\bxx)}{\partial \bxx^{(i)}}\bigg{|}_{\bxx=\bmu}, \ 
    a_{ij}=\frac{\partial^2 f(\bxx)}{\partial \bxx^{(i)}\partial \bxx^{(j)}}\bigg{|}_{\bxx=\bmu},
\end{align}
Define corresponding gradients for the bootstrap evaluated at the count functional $\bu$:
\begin{align}
\label{eq-ahat}
%\label{eq:EW-SMF-aij}
  &  \hat{a}_i=\frac{\partial f(\bxx)}{\partial \bxx^{(i)}}\bigg{|}_{\bxx=\bu}, \ 
    \hat{a}_{ij}=\frac{\partial^2 f(\bxx)}{\partial \bxx^{(i)}\partial \bxx^{(j)}}\bigg{|}_{\bxx=\bu}.
\end{align}
% These derivatives may be viewed as perturbations of the derivatives evaluated at the expectation $E(\bu) = \bmu$:
% Define the following empirical analogues of the moments of interest:
% %
% \begin{align*}
%     \tilde{\lm}_{i_1,\ldots,i_j}&=\frac{1}{n}\sum_{l=1}^n\left(r_{i_1}\frac{\hat{g}_1^{(i_1)}(l)}{\rho_n^{s_{i_1}}}\right)\ldots \left(r_{i_d}\frac{\hat{g}_1^{(i_d)}(l)}{\rho_n^{s_{i_d}}}\right)
% \end{align*}
Define the asymptotic variance of the smooth function as: %\rd $\lm_{ij}$ not defined \bk
\begin{align}
\label{eq:sigmaf}
\sigf^2&=\sum_{i=1}^d\sum_{j=1}^da_ia_j E \left(\frac{r_{i}\hat{g}_1^{(i)}(l)}{\rho_n^{s_{i}}}\frac{r_{j}\hat{g}_1^{(j)}(l)}{\rho_n^{s_{j}}}\right).
\end{align}
and define the empirical analogue of the asymptotic variance as:
\begin{align}\label{eq:sigmahatfemp}
\tdsigf^{2}&=\sum_{i=1}^d\sum_{j=1}^d\hat{a}_i\hat{a}_j \widehat{E}_n \left(\frac{r_{i}\hat{g}_1^{(i)}(l)}{\rho_n^{s_{i}}} \frac{r_{j}\hat{g}_1^{(j)}(l)}{\rho_n^{s_{j}}}\right).
\end{align}

  We are now ready to state our Edgeworth expansion for the smooth function of the bootstrapped statistics. For simplicity, we state the Edgeworth expansion for $u^*$ resulting from the quadratic bootstrap procedure \mbq. A similar result holds for \mbm, albeit under stronger conditions on the subgraph like those imposed in Corollary~\ref{thm:mbm-firstorder}. 

\begin{theorem}
\label{thm:boot_smooth}
%  Define $S_n^*=n^{1/2}(f(\bu^*)-f(\bu))/\tdsigf$, Use $P^*$ to denote probability given $A$ and $X$. Under the same condition of Proposition~\ref{prop:smooth-pop}, 
Suppose that $\sigf>0$, the function $f$ has three continuous derivatives in a neighborhood of $\bmu$ and suppose that the weights $\w_1,\dots,\w_n$ are generated from a non-lattice distribution such that $\E(\xi_1) = 1$, $\E\{(\xi_1-1)^2\} = 1$,  $\E\{(\xi_1-1)^3\} = 1$.  Further suppose that Assumptions \ref{ass:linear} and \ref{ass:sparse} are satisfied. Then, we have:
 \begin{align}\label{eq:smf-bt-ew}
    P^*(S_n^* \leq x) = \Phi(x) + n^{-1/2}\phi(x)\{\tilde{A}_1\tdsigf^{-1}+\frac{1}{6}\tilde{A}_2\tdsigf^{-3}(x^2-1)\} + O_P\left(\frac{\log n}{n^{2/3}\rho_n}\right).
\end{align}
where:
 \begin{align*}
% \tdsigf^{2}&=\sum_{i=1}^d\sum_{j=1}^d\hat{a}_i\hat{a}_j\tilde{\lm}_{ij},\\
\tilde{A}_1=& \ \frac{1}{2}\sum_{i=1}^d\sum_{j=1}^d\hat{a}_{ij} \widehat{E}_n \left(\frac{r_{i}\hat{g}_1^{(i)}(l)}{\rho_n^{s_{i}}} \frac{r_{j}\hat{g}_1^{(j)}(l)}{\rho_n^{s_{j}}}\right),\\
    \tilde{A}_2=& \ \sum_{i=1}^d\sum_{j=1}^d\sum_{k=1}^d \hat{a}_i \hat{a}_j\hat{a}_k \widehat{E}_n \left(\frac{r_{i}\hat{g}_1^{(i)}(l)}{\rho_n^{s_{i}}} \frac{r_{j}\hat{g}_1^{(j)}(l)}{\rho_n^{s_{j}}} \frac{r_{k}\hat{g}_1^{(k)}(l)}{\rho_n^{s_{k}}}\right)
    \\ + & \ 3 \ \sum_{i=1}^d\sum_{j=1}^d\sum_{k=1}^d\sum_{t=1}^{d}\hat{a}_i\hat{a}_j\hat{a}_{kt} \widehat{E}_n \left(\frac{r_{i}\hat{g}_1^{(i)}(l)}{\rho_n^{s_{i}}} \frac{r_{k}\hat{g}_1^{(k)}(l)}{\rho_n^{s_{k}}}\right) \widehat{E}_n \left(\frac{r_{j}\hat{g}_1^{(j)}(l)}{\rho_n^{s_{j}}} \frac{r_{j}\hat{g}_1^{(t)}(l)}{\rho_n^{s_{t}}}\right)
    \\ + & \ 3 \ \sum_{i=1}^d\sum_{j=1}^d\sum_{k=1}^d \hat{a}_i\hat{a}_j\hat{a}_k \widehat{E}_n\left( \frac{r_i \hat{g}_1^{(i)}(l)}{\rho_n^{s_i}} \frac{r_j \hat{g}_1^{(j)}(m)}{\rho_n^{s_j}} \frac{r_k(r_k-1) \tilde{g}_2^{(k)}(l,m)}{\rho_n^{s_k}} \right).
\end{align*}
\end{theorem}
In the Supplementary Material, we derive Edgeworth expansions for smooth functions of U-statistics corresponding to the non-negligible component of the count functional in Proposition~\ref{prop:smooth-pop} and show that our bootstrap version of the Edgeworth expansion is close to this expansion in Proposition~\ref{prop:smf-bt-ew-close}. To derive Edgeworth expansions for the U-statistic, we impose a non-lattice condition; however, it is likely that this assumption can be removed for count functionals if a smoothing argument used in \cite{zhang-xia-network-edgeworth} is adapted.  
\bk
% but have not been studied previously, even for U-statistics, to the best of our knowledge.  For smooth functions, we derive Edgeworth expansions for the standardized bootstrap and show that they are very close to Edgeworth expansions of the U-statistic (signal) component of the count functional.
% , assuming that a multivariate Edgeworth expansion exists. The results of~\cite{zhang-xia-network-edgeworth} strongly suggest that smooth functions of counts have the same Edgeworth expansion as the U-statistic component, but rigorously establishing this fact would involve long derivations using similar smoothing arguments and is left to future work.
% \bk
% \rd
% So far, we have established the Edgeworth expansion for count statistics and shown that our bootstrap methods match this expansion. The results of~\cite{zhang-xia-network-edgeworth} and our Proposition~\ref{prop:ew} are strongly suggestive of the fact that the Edgeworth expansion of smooth function of count statistics should match that of their respective conditional expectations. However, even the form of the Edgeworth expansion of the smooth function of the conditional expectation is not known. So in this section and the next, we derive the form of the polynomials for standardized and studentized variants of smooth functions of the conditional expectation, assuming that there exists such an expansion. Our experiments suggest that indeed, the Edgeworth expansions match the true distribution of the smooth function of count statistics. 
% We also show that  the bootstrapped version of $S_n$ converges to this expansion conditioned on the network. 
% In this section we derive the form of the Edgeworth expansion for the CDF of $S_n$, and show that that the bootstrapped version converges to this expansion conditioned on the network. 
% Deriving the form of the Edgeworth expansion requires computing derivatives of the function by hand and estimating moments. In contrast, the quadratic and multiplier bootstrap methods are easier to implement and automatically lead to a higher order correct approximation of the conditional CDF. 
% Consider a smooth function $g$ of $d$ count statistics for subgraphs with $r_1,\dots,r_d$ nodes and $s_1,\dots,s_d$ edges. Let $\bu$ denote the vector of conditional expectation of the respective count statistics. Define $S_n=n^{1/2}(f(\bu)-f(\bmu))/\sigma$.  Let $u^*$ be bootstrapped vector of scaled count functionals  $\{\frac{\cfbq{(1)}}{\rho^{s_1}},\ldots, \frac{\cfbq{(d)}}{\rho^{s_d}}\}$.
% \bk
% To be concrete, using this one can do inference for transitivity by using $f(x,y)=x/y$ where $x$ and $y$ are the bootstrapped triangle and edge densities respectively.
% \bl
% Suppose that the  multivariate U-statistic $T_n$ admits a Edgeworth expansion of the form:
% \begin{align}\label{eq:EW-SMF}
%     P\{n^{1/2}(T_n - \mu) \in R \}=  P_1(\mathcal{R}) + n^{-1/2} P_2(\mathcal{R}) + o(n^{-1/2})
% \end{align}
% uniformly for sets $\mathcal{R}$ satisfying:
% \begin{align*}
% \sup_{R \in \mathcal{R}} \int_{(\partial R)^\eta } \exp\left(\frac{1}{2} \|x\|^2 \right) = O(\eta)   
% \end{align*}
% for signed measures $P_j(\mathcal{R})$. The form given above is standard for multivariate Edgeworth expansions; see \citet{hall-bootstrap-edgeworth} and \citet{bhattacharya-rao-normal-asymptotic}.  Under the assumption of such an expansion, results for smooth functions follow due to arguments in \citet{hall-bootstrap-edgeworth}; what remains is to derive cumulants of the smooth function. 
% % and if the cumulants of $S_n$ can be expanded using a power series, as is true in many cases of practical interest \citep{hall-bootstrap-edgeworth},
% then one can derive the exact form of the polynomial $p_1$ as shown below.
%  First define:
% \begin{align}\label{eq:EW-SMF-aij}
%   &  a_i=\frac{\partial f(\bu)}{\partial \bu^{(i)}}\bigg{|}_{\bu=\bmu}, \ 
%     a_{ij}=\frac{\partial^2 f(\bu)}{\partial \bu^{(i)}\partial \bu^{(j)}}\bigg{|}_{\bu=\bmu},
% \end{align}
% \begin{align}\label{eq:EW-SMF-lambda}
% & \lm_{i_1,\ldots,i_j}=E\left\{\left(\frac{r_{i_1}g_1^{(i_1)}(X_l)}{\rho^{s_{i_1}}}\right)\ldots\left(\frac{r_{i_d}g_1^{(i_d)}(X_l)}{\rho^{s_{i_d}}}\right)\right\}.
% \end{align}
% \begin{align}\label{eq:EW-SMF-p1}
%     p_1(x)=-\{A_1\sigma^{-1}+\frac{1}{6}A_2\sigma^{-3}(x^2-1)\},
% \end{align}
% where $\sigma^2$, $A_1$ and $A_2$ are
% \begin{align}
% \sigma^2&=\sum_{i=1}^d\sum_{j=1}^da_ia_j\lm_{ij},\notag\\
% A_1&=\frac{1}{2}\sum_{i=1}^d\sum_{j=1}^da_{ij}\lm_{ij},\notag\\
%     A_2&=\sum_{i=1}^d\sum_{j=1}^d\sum_{k=1}^d a_i a_ja_k \lm_{ijk}+3\sum_{i=1}^d\sum_{j=1}^d\sum_{k=1}^d\sum_{t=1}^{d}a_ia_ja_{kt}\lm_{ik}\lm_{jt}\notag\\ &+ \frac{3r_ir_jr_k(r_k-1)}{\rho^{s_i}\rho^{s_j}\rho^{s_k}}\sum_{i=1}^d\sum_{j=1}^d\sum_{k=1}^d a_ia_ja_k E\left\{g_1^{(i)}(X_{i_1})g_1^{(j)}(X_{i_2})g_2^{(k)}(X_{i_1},X_{i_2})\right\} .\label{eq:p1sigma}
% \end{align}
% %We show that conditioned on $A$ and $X$, the Edgeworth expansion of the smooth function of $\bu^{*}$ converges to $P(S_n<x)$. 
% \rd The interesting observation about the above form, is that, this is similar to functions of sums of independent random variables~\citep{hall-bootstrap-edgeworth}. Our analysis uses the linear and quadratic terms in the Hoeffding decomposition of the conditional expectation.
% \bk
% For the bootstrapped quantity, one can show (see the Supplement Section~\ref{sec:supp:sub-proof-smf-bt}) that the CDF of $S_n^*=n^{1/2}(f(\bu^*)-f(\bu))/\tilde{\sigma}$, where $\tilde{\sigma}$ is obtained by the plug-in principle using $\hat{g}_1$ for $g_1$ and empirical moments for $\mu$ in Eqs \ref{eq:EW-SMF-p1} and \ref{eq:p1sigma}. This can be found in the Supplement Section~\ref{sec:supp:sub-proof-smf-bt}. 
% Define 
% \begin{align*}
% \tilde{\sigma}^{2}&=\sum_{i=1}^d\sum_{j=1}^d\hat{a}_i\hat{a}_j\tilde{\lm}_{ij},
% \end{align*}
% where
% \begin{align*}
%  &\hat{a}_i=\frac{\partial f(\bu)}{\partial u^{(i)}}\bigg{|}_{\bu=\hat{\bu}}, \ 
%     \hat{a}_{ij}=\frac{\partial^2 f(\bu)}{\partial u^{(i)}\partial u^{(j)}}\bigg{|}_{\bu=\hat{\bu}},\\
%     &\tilde{\lm}_{ij}=E^*\left\{\left[r_{i}\left(\frac{\hat{g}_1^{(i)}(X_l)V_l}{\rho^{s_{i}}}-\hat{\bu}^{(i)}\right)\right]\left[r_{j}\left(\frac{\hat{g}_1^{(j)}(X_l)V_l}{\rho^{s_{j}}}-\hat{\bu}^{(j)}\right)\right]\right\}.
% \end{align*}
% Under the above assumption of $g$, applying similar technique that used to prove Theorem \ref{thm:smf-ew}, we arrive at the following Theorem.
% %\begin{equation*}
% %    n^{1/2}(g(\bu^*)-g(\bhatu))=n^{-1/2}<\bu^*_L,\nabla g(\bhatu)> + \frac{1}{n^{3/2}}\left(<\bu^*_Q,\nabla g(\bhatu)>+\frac{1}{2}\bu_L^{*T} H(\bhatu)\bu_L^*\right)+O\left(\frac{1}{n}\right).
% %\end{equation*}
% \begin{proposition}
% % \label{thm:smf-bt}
% Define $S_n^*=n^{1/2}(f(\bu^*)-f(\bu))/\tilde{\sigma}$. Under the condition that the function $f$ has three continuous derivatives in a neighbourhood of $\bmu$,  we have
% \begin{align*}
%     P^*(S_n^*<x)%= \Phi(x) + n^{-1/2}p_1^*(x)\phi(x) + o(n^{-1/2})
%     =P(S_n<x) +o_P\left(n^{-1/2}\right).
% \end{align*}
% \end{proposition}
% \bk
% \begin{figure}[H]
% %\vskip 0.2in
% \centering
% \vspace{-5mm}
%     \includegraphics[trim=0mm 3mm 0mm 10mm,width=  0.7\textwidth]{plots2/ew-trans-test.pdf} 
%       %   \vspace{-2em}
    % %     \includegraphics[trim=0em 1em 0em 5em, clip, width=  \textwidth]{plots/EW-MB-trans-nobar.pdf}
%   %     \vspace{-1em}
%     %\vspace{-4em}
% %    \includegraphics[width=  0.8\textwidth,height=0.4\textwidth]{plots/EW-MB-twostars-nobar.pdf}\\
%  \caption{We present $E|F_n(x)-F^*_n(x)|$ for the transitivity coefficient of the \sbm
%  $n=160$, $\rho=1$ graphs, where EW is calculated using Eq \ref{eq:EW-SMF} and MB-M, MB-Q, MB-L are calculated as Algorithm 1 but normalized by true standard deviation}.
% %\begin{center}
% \label{fig:cdf-error}
% \end{figure}

==> network_mb_jasa_to_arxiv (1)/problem_setup.tex <==
\subsection{The sparse graphon model}
\label{sec:sparse-graphon}
Let $\{A^{(n)}\}_{n \in \mathbb{N}}$ denote a sequence of $n \times n$ binary adjacency matrices and let $w:[0,1]^2 \mapsto \mathbb{R}$ be a symmetric measurable function such that $\int_0^1 \int_0^1 w(u,v) \ du \ dv = 1$ and $ w(u,v) \leq C$ for some $1 \leq C < \infty$.  We assume that $A^{(n)}$ is generated by the following model:
%
\begin{align}
\label{eq:sparse-graphon-model}
A_{ij}^{(n)} = A_{ji}^{(n)} \sim \mathrm{Bernoulli}(\rho_n w(X_i, X_j))
\end{align}
%
where $X_i, X_j \sim \mathrm{Unif}[0,1]$, $\rho_n \rightarrow 0$, and $A_{ii}^{(n)} = 0$.  While closely related models were considered by \citet{bollobas-inhomogenous-graphs}, \citet{hoff-raftery-handcock-latent-space-model}, and \citet{borgs-lp-part-one} this particular parameterization was introduced by  \citet{Bickel-Chen-on-modularity}. We will refer to (\ref{eq:sparse-graphon-model}) as the sparse graphon model.  Sparse graphons are a very rich class of models, subsuming many widely used models, including stochastic block models and their variants \citep{holland-sbm, karrer-newman-dcsbm, airoldi-mmsb}, and  (generalized) random dot product graphs \citep{young-schneiderman-rdpg, generalized-rdpg}.  More generally, sparse graphons are natural models for graphs that exhibit vertex exchangeability; the functional form is motivated by representation theorems for exchangeable arrays established by \citet{aldous-representation-array} and \citet{hoover-exchangeability}.  The parameter $\rho_n = P(A_{ij} = 1)$ determines the sparsity level of the sequence $\{ A^{(n)} \}_{n \in \mathbb{N}}$.  Many real world graphs are thought to be sparse, with $o(n^2)$ edges; $\rho_n \rightarrow 0$ is needed for graphs generated by (\ref{eq:sparse-graphon-model}) to exhibit this behavior. 

While boundedness of the graphon is a common assumption in the statistics literature (see, for example, the review article by \citet{gao-ma-minimax-network-analysis}), it should be noted that unbounded graphons are known to be more expressive.  As noted by \citet{borgs-lp-part-one}, unboundedness allows graphs that exhibit power-law degree distributions, a property that bounded graphons fail to capture. For mathematical expedience, in the present article, we focus on the bounded case, but we believe that our analysis may be extended to sufficiently light-tailed unbounded graphons as well. We use standard asymptotic notations such as $O()$,$o()$ and $\omega()$ throughout the paper. 

\subsection{Count functionals}
Now we will introduce notation related to our functional of interest. 
%\citet{Bickel-Chen-Levina-method-of-moments} and \citet{zhang-xia-network-edgeworth} use different notation to express count functionals, but since we are interested in establishing Edgeworth expansions for the bootstrap, we will adopt the notation of the latter authors for ease of comparison.  Let $R$ denote the adjacency matrix of a subgraph of interest, which contains $r$ vertices and $s$ edges.
Let $R$ denote the adjacency matrix of a subgraph of interest, with $r$ vertices and $s$ edges. Let $A_{i_1, \ldots, i_r}^{(n)}$ denote the adjacency matrix formed by the node subset $\{i_1, \ldots, i_r\}$ and for each such $r$-tuple, define the following function: 
%
\begin{align*}
H(A_{i_1, \ldots, i_r}^{(n)}) := \mathbbm{1}(A_{i_1, \ldots, i_r}^{(n)} \cong R)
\end{align*}
where we say that $A_{i_1, \ldots, i_r}^{(n)} \cong R$ if there exists a permutation function $\pi$ such that $A_{\pi(i_1), \ldots, \pi(i_r)} = R$.  Our count functional, which we denote $\hat{T}_n(R)$, or $\hat{T}_n$ when there is no ambiguity, is formed by averaging over all $r$-tuples in the graph.
%and normalizing by $\rho_n^s$ to ensure that our functional converges to an informative non-zero quantity:
%\begin{align}
%\hat{T}_n := \frac{1}{{n \choose r} \rho_n^{s}} \sum_{1 \leq i_1 < i_2 < \ldots < i_r \leq n} H(A_{i_1, \ldots, i_r}^{(n)}) 
%\end{align}
\begin{align}\label{eq:cf}
\cfhat := \frac{1}{{n \choose r} } \sum_{1 \leq i_1 < i_2 < \ldots < i_r \leq n} H(A_{i_1, \ldots, i_r}^{(n)}) 
\end{align}
%Now let $V(Q) \subset \{1, \ldots n\}$ denote the vertex set associated with a graph $Q$ and $E(Q) \subset V(Q) \times V(Q)$ the corresponding vertex set.  Furthermore, let $\overline{E(Q)}$ denote the complement of $E(Q)$ given the universal set $V(Q) \times V(Q)$. 
Let $h(X_{i_1}, \ldots X_{i_r})$ denote the conditional expectation of $H(A_{i_1, \ldots, i_r}^{(n)})$.
%Define the following kernel:
%\rd shouldn't there be a $\rho^s$ here? \bk
%\begin{align}
%\begin{split}
%h_n(X_{i_1}, \ldots X_{i_r}) :&= \E\{ H(A_{i_1, \ldots, i_r}^{(n)}) \mid X_{i_1}, \ldots, X_{i_r}\}
%\\ &= \sum_{Q \sim R, V(Q) = \{i_1, \ldots i_r\} } \prod_{(i,j) \in E(Q)} \rho_n w(X_i, X_j) \prod_{(i,j) \in \overline{E(Q)}} \left\{1 -\rho_n w(X_i, X_j)\right\}
%\end{split}
%\end{align}
%For readability, we will suppress the $n$ in $h_n$ in what follows. 
Now, define the following (conventional) U-statistic:
\begin{align*}
T_n := \frac{1}{{n \choose r}} \sum_{1 \leq i_1 < i_2 < \ldots < i_r \leq n} h(X_{i_1}, \ldots X_{i_r})
\end{align*}
 For notational convenience we will refer to $h(X_{i_1}, \ldots, X_{i_r})$ by $h(X_S)$, where $S$ is the subset $\{i_1,\dots, i_r\}$.  Denote $\theta_n:=\E\{h(X_S)\}$. We see that $\theta_n/\rho_n^s\rightarrow\mu$. This can be thought of as a normalized subgraph density that we want to infer. The normalization by $\rho_n^s$ is to ensure that our functional converges to an informative non-zero quantity.

  By a central limit theorem for U-statistics \citep{hoeffding1948}, it can be shown that $(T_n - \theta_n)/\sigma_n$ is asymptotically Gaussian.  Here we have:
  \begin{align}\label{eq:taun}
      \tau_n^2=\var[\E\{h(X_S)\mid X_1\}],\ \  \  \sigma_n^2=r^2\tau_n^2/n
  \end{align}
 % $\sigma_n^2=r^2\tau_n^2/n$, and $\tau_n^2=\var[\E\{h(X_S)\mid X_1\}]$ . 
 Furthermore, \citet{Bickel-Chen-Levina-method-of-moments} show that, 
%   for acyclic graphs and $p$-cycles, under the condition $n \rho_n \rightarrow \infty$,
  $( \cfhat - T_n)/\sigma_n = o_P(1)$  under mild sparsity conditions for a wide range of subgraphs.   Thus, we may view $(\cfhat - \theta_n)/\sigma_n = (\cfhat- T_n)/\sigma_n + (T_n - \theta_n)/\sigma_n$ as a U-statistic perturbed by asymptotically negligible noise.

\subsection{Preliminaries of proposed bootstrap procedures}
\label{subsec:proposed-bootstrap}
In order to estimate the subgraph density, we will consider the following multiplier bootstrap procedures. In what follows let $\w_1, \ldots \w_n$ be i.i.d. continuous random variables with mean $\mu = 1$ and central moments $\mu_2 =1$, and $\mu_3 =1$.  An example of such a random variable is the product $Z$ of two independent Normal random variables $X$ and $Y,$ defined below: %a product of the independent Normal distributions $X \sim N(1,1/2)$ and $Y \sim N(1, 1/3)$. We will refer to distribution as the \texttt{Gaussian Product} distribution.
\begin{align}\label{eq:gaussproduct}
    X\sim N(1,1/2) \qquad Y\sim N(1,1/3) \qquad Z=XY
\end{align}



Let $\w_{i_1 \cdots i_r}$ denote $\w_{i_1} \times \ldots \times \w_{i_r}$ and define the following multiplicative bootstrap:
%\rd Add Tn-hat to the LHS \bk
%\rd change notations? \bk
\begin{align}
\label{eq:multiplicative-bootstrap}
\cfbm = \cfhat+ \frac{1}{{n\choose r}} \sum_{1 \leq i_1 < i_2 < \ldots i_r} \xi_{i_1 \cdots i_r}  \cdot \left\{ H(A_{i_1, \ldots, i_r}^{(n)}) - \cfhat \right\}
\end{align}

Our multiplicative bootstrap is motivated by Hoeffding's decomposition (see Supplement Section~\ref{sec:supp:lemmaone}).  The first two terms of the decomposition for $T_n - \theta_n$ are given by:
\begin{align*}
g_1(X_i) &= E\{h(X_i, X_{i_2} \ldots X_{i_r}) \mid X_i\} - \theta_n 
%\\ g_2(X_i, X_j) &= \mathbb{E}[h(X_i, X_j, X_{i_3} \ldots X_{i_r}) \mid X_i, X_j] - g_1(X_i) - g_1(X_j)  - \theta_n,
\\ g_2(X_i, X_j) &= E\{h(X_i, X_j, X_{i_3} \ldots X_{i_r}) \mid X_i, X_j\} -g_1(X_i)-g_1(X_j) - \theta_n,
\end{align*}
leading to the representation:
\begin{align}\label{eq:hoeffding-noiseless}
T_n - \theta_n = \frac{r}{n}\sum_{i=1}^n g_1(X_i) + \frac{r(r-1)}{n(n-1)} \sum_{i < j}  g_2(X_i,X_j)  + o_p\left(\frac{\rho_n^s}{n}\right) 
\end{align}
Similarly, conditional on the data, it can be shown that we have the following bootstrap analog. Let:
\begin{align}
\hat{g}_1(i) &= \frac{1}{{n-1 \choose r-1 }} \sum_{1 \leq i_2 < \ldots i_r \leq n, i_u \neq i } \bigl\{H(A_{i,i_2, \ldots i_r}) - \cfhat \bigr\}\label{eq:g1hat}
\\ \tilde{g}_2(i,j) &= \frac{1}{{n-2 \choose r-2 }} \sum_{1 \leq i_3 < \ldots i_r \leq n, i_u \neq i,i_u \neq j }  \bigl\{H(A_{i,i_2, \ldots i_r}) - \cfhat \bigr\}   \\
\hat{g}_2(i,j)&=\tilde{g}_2(i,j)-\hat{g}_1(i) -\hat{g}_1(j) \label{eq:g2hat}
\end{align}
Furthermore, Eq~\ref{eq:g1hat} can be used to standardize the bootstrap replicates using the following estimate of $\tau_n$ (Eq~\ref{eq:taun}):
\begin{align}\label{eq:tauhat}
\hat{\tau}_n^2=\sum_i \frac{\hat{g}_1(i)^2}{n}
\end{align}
%Before providing the Hoeffding decomposition for our bootstrap statistic, we first give a short discussion on the Hoeffding decomposition.
%\input{arxiv-version/hoeffding.tex}
We now present the Hoeffding decomposition for our bootstrap statistic. The proof is deferred to the Supplement Section~\ref{sec:supp:lemmaone}.


% It turns out that the Hoeffding decomposition for $\hat{T}_n - \theta_n$ has the same form a noiseless U-statistic.  Define the terms:
% \begin{align*}
% g_1(X_i) &= \mathbb{E}[h(X_i, X_{i_2} \ldots X_{i_r}) \mid X_i] - \theta_n 
% \\ g_2(X_i, X_j) &= \mathbb{E}[h(X_i, X_j, X_{i_3} \ldots X_{i_r}) \mid X_i, X_j] - g_1(X_i) - g_1(X_j)  - \theta_n
% \end{align*}
% The Hoeffding decomposition for $\hat{T}_n - \theta_n$ may be written as:
% \begin{align*}
% T_n - \theta_n = \frac{r}{n}\sum_{i=1}^n g_1(X_i) + \frac{r(r-1)}{n(n-1)} \sum_{i < j} g_2(X_i,X_j) + O_P\left(\frac{1}{n}\right) 
% \end{align*}

%We will now establish the Hoeffding decomposition for our bootstrapped functional below.  


 \begin{lemma}
 \label{lemma:hoeffding-bootstrap}
  We have the following decomposition: 
  \begin{align}\label{eq:boot-hoeff}
 \begin{split}
 \cfbm - \cfhat &= \frac{r}{n}\sum_{i=1}^n (\w_i-1) \cdot \hat{g}_1(i)  + \frac{r(r-1)}{n(n-1)}\sum_{i<j } \ (\w_i \ \w_j - \w_i-\w_j+1) \cdot \tilde{g}_2(i,j)    
 \\ & \ \ \ \ \ +  O_P\left(\rho_n^sn^{-1/2}\delta(n,\rho_n,R) \right),
 \end{split}
 \end{align}
% %
 where $\delta(n,\rho_n,R)$ is defined as follows: 
 
 % $(n\rho_n)^{-1}$ if $R$ is acyclic, and $\left(n\rho_n^{3/2}\right)^{-1}$ if $R$ is cyclic. %is defined as:
 $\begin{aligned}
     \delta(n,\rho_n,R) =\begin{cases} 
       \dfrac{1}{n\rho_n} & \text{R is acyclic} \\
       \dfrac{1}{n\rho_n^{3/2}} & \text{R is a simple cycle} .
  \end{cases}
\end{aligned}$
 \end{lemma}
 
 \iffalse
\begin{align}
\begin{split}
\hat{U}_{n, \w}^M - \hat{U}_n &= \frac{r}{n}\sum_{i=1}^n (\w_i-1) \cdot \hat{g}_1(i)  + \frac{r(r-1)}{n(n-1)}\sum_{i<j } \ (\w_i \ \w_j - 1) \cdot \hat{g}_2(i,j)  
\\ & \ \ \ - (\w_i-1) \cdot \hat{g}_1(i) - (\w_i-1) \cdot \hat{g}_1(j)   + \rd O_P(\delta(n,\rho_n,R)),
\end{split}
\end{align}
where $\delta(n,\rho_n,R)$ is defined as:
\begin{equation*}
    \delta(n,\rho_n,R) =\begin{cases} 
      \frac{1}{n\rho_n} & \text{R is acyclic} \\
       \frac{1}{n\rho_n^{3/2}}& \text{R is acyclic} 
  \end{cases}
\end{equation*}

\fi
Although the quadratic term in the above expansion may seem different from Eq~\ref{eq:hoeffding-noiseless}, Some manipulation yields that $\sum_{i<j }( \ \w_i \ \w_j - \w_i-\w_j+1) \cdot \tilde{g}_2(i,j)  $ is equivalent to $\sum_{i<j}(\w_i\w_j-1) \tilde{g}_2(i,j)-(\w_i-1) \cdot \hat{g}_1(i) - (\w_i-1) \cdot \hat{g}_1(j)$, which is similar to the corresponding term in the Hoeffding decomposition of the U statistic (see Eq~\ref{eq:hoeffding-noiseless}).

Viewing $\hat{g}_1(i)$ and $\hat{g}_2(i,j)$ as estimates of $g_1(X_i)$ and $g_2(X_i, X_j)$, respectively, it is clear that that our weighted bootstrap version encapsulates important information about $\cfhat - \theta_n$. The above decomposition also suggests that one may approximate the non-negligible terms more directly.  Ignoring the remainder term, we arrive at the linear and quadratic bootstrap estimates:
\iffalse
\begin{align}
\begin{split}
\hat{U}_{n, \w}^Q &= \hat{U}_n +  \frac{r}{n}\sum_{i=1}^n (\w_i-1) \cdot \hat{g}_1(i)  + \frac{r(r-1)}{n(n-1)}\sum_{i<j }\left( \ (\w_i \ \w_j - 1) \cdot \hat{g}_2(i,j)  
\right.\\ & \left.\ \ \ - (\w_i-1) \cdot \hat{g}_1(i) - (\w_i-1) \cdot \hat{g}_1(j)\right)
\end{split}
\end{align}
\fi
\begin{align}
%\begin{split}
\cfbl &= \cfhat +  \frac{r}{n}\sum_{i=1}^n (\w_i-1) \cdot \hat{g}_1(i)   \label{eq:cfbl}\\ \cfbq &= \cfbl+ \frac{r(r-1)}{n(n-1)}\sum_{i<j } \ (\w_i \ \w_j - \w_i-\w_j+1) \cdot \tilde{g}_2(i,j). \label{eq:cfbq} %\cfhat +  \frac{r}{n}\sum_{i=1}^n (\w_i-1) \cdot \hat{g}_1(i)  + \frac{r(r-1)}{n(n-1)}\sum_{i<j } \ (\w_i \ \w_j - \w_i-\w_j+1) \cdot \tilde{g}_2(i,j)  
%\right.\\ & \left.\ \ \ - (\w_i-1) \cdot \hat{g}_1(i) - (\w_i-1) \cdot \hat{g}_1(j)\right)
%\end{split}
\end{align}
% \rd

% \bk

Now that we have introduced the main concepts, we are ready to present the  our bootstrap procedures. We first present the results on our fast linear bootstrap method.
%and a fast randomized algorithm for precomputation of moments needed for the linear bootstrap procedure. 
\bk
\section{Proposed algorithms}\label{sec:proposed-alg}
In this section, we present a fast linear bootstrap method using Eq~\ref{eq:cfbl}. Recall that the multiplicative bootstrap requires to precompute $\cfhat$ and $\hat{g}_1(i)$ for all $i$. This computation is $O(n^r)$ in the worst case. In addition to this, the computation complexity for MB-L is $O(Bn)$. Therefore, in what follows, our goal is to reduce the precomputation time. 


\subsection{Fast linear bootstrap}\label{subsec:fast-linear-boot}
We propose a randomized approximation for $\cfhat$ and $\hat{g}_1(i)$. The main idea is that an average over all size $r$ subset can be written as an average over $n!$ permutations (see~\cite{hoeffding1948,subsampling-sparse-graphons}). 
For any $i \in \{1,\ldots,n\}$, denote the set of all subsets of size $r-1$ taken from  $\{1,\ldots,i-1,i+1,\ldots n\}$ as $\si$. %Denote $\{X_{i_{2}},\ldots ,X_{i_{r}} \}$ for $S=\{i_2,\ldots i_r\}  \in \mathbb{S}_{-i}$  as $X_s$.  
Denote  $H(A_{i,i_2, \ldots i_r})$ for $S=\{i_2, \ldots i_r\}  \in \mathbb{S}\{-i\}$ as $\hsxi$. 
Denote 
\begin{align*}
    %H_1(i)%= \frac{1}{{n-1 \choose r-1 }} \sum_{1 \leq i_2 < \ldots i_r \leq n, i_u \neq i } H(A_{i,i_2,\ldots i_r}) 
     &\hoi = \frac{1}{{n-1 \choose r-1 }} \sum_{S \in \mathbb{S}\{-i\}} \hsxi.%\\
   % & h_1(i)= \frac{1}{{n-1 \choose r-1 }} \sum_{s \in S\{-i\}} \shsxi.
\end{align*}
%we know 
%\rd
%\begin{align*}
%   & E\hoi= E(h_s(X)\mid X_i). \\
 %  & E(\hoi-\theta)^2=Var(h_s(X)\mid X_i).
%\end{align*}
\bk 

One can also write $H_1(i)$ as follows:
\begin{align*}
    H_1(i)=\frac{1}{(n-1)!}\sum_{\pi} H_\pi(i).
\end{align*}
Here $H_\pi(i)=\frac{\sum_{S\in\mathbb{S}_{\pi} }\hsxi}{\frac{n-1}{r-1}},$ where $\mathbb{S}_{\pi}$ denotes the set of all disjoint subsets  $\{\pi_{(i-1)(r-1)+1},\dots, \pi_{i(r-1)}\}$, $i=1,\dots, \frac{n-1}{r-1}$ obtained from permutation $\pi$. 
Now let  $\pi_j$ be a permutation picked with replacement and uniformly at random from the set of all permutations of $\{1,\dots,n\}\setminus i$. 

Our randomized algorithm makes use of this structure and draws $j=1,\ldots,N$ independent permutations $\pi_j$. %$\xpi \sim Bernoulli(p)$, let $\pimi$ denote all the permutations of $\{1,\ldots,i-1,i+1,\ldots n\}$.
%Let $\mathbb{S}_{\pi}$ denote the set of all disjoint subsets  $\{\pi_{(i-1)(k-1)+1},\dots, \pi_{i(k-1)}\}$, $i=1,\dots, \frac{n-1}{k-1}$ obtained from permutation $\pi$.  %We have $\sum_ {\pi \in \pimi} \xpi = \tilde{N}$ and $E\left(\sum_{\pi \in \pimi}\xpi\right)=N$.\bk  
\iffalse
We write
\begin{align}\label{eq:define-tnl-tilde}
  \ttnl  =  \Tilde{T}_n + \frac{r}{n}\sum_{i=1}^n (\xi_i-1)(\tdh(i)-\tdu),
\end{align}
\fi
We compute
\begin{equation}\label{eq:define-h1-tilde}
%&\tdh(i)=\frac{\sum_{\pi \in \pimi}\xpi\hpi(i)}{\sum_{\pi \in \pimi}\xpi},\\
\tdh(i)=\frac{\sum_{j} H_{\pi_j}(i)}{N},\qquad \tdu=\frac{1}{n}\sum_{i=1}^n\tdh(i).
\end{equation}
\iffalse
\begin{equation*}
\hpi(i)=\frac{\sum_{S\in\mathbb{S}_{\pi} }\hsxi}{\frac{n-1}{k-1}},
\end{equation*}
\begin{equation}\label{eq:define-tn-tilde}
\tdu=\frac{1}{n}\sum_{i=1}^n\tdh(i)
\end{equation}
\fi

To calculate $\tdh(i)$, for each $i$, we permute the node set excluding $i$ for $N$ times and for each of these permutations $\pi$ we check the disjoint set $\mathbb{S}_{\pi}$ for count functionals.  Thus, the complexity for calculating $\tdh(i)$ is now $O\left(N\frac{n}{r}\right)$. From $\{\tdh(i)_{i=1}^n\}$, $\tdu$ is calculated from their mean and $\tilde{\tau}_n$ is defined as
\begin{align}\label{eq:define-taun-tilde}
    \tilde{\tau}_n^2= \frac{\sum_{i=1}^n\{\tdh(i)-\tdu\}^2}{n^2}.
\end{align}
The linear bootstrap uses $\tilde{T}_{n,L}$ by plugging in $\tilde{g}_1(i)=\tilde{H}_1(i)-\tilde{T}_n$ and $\tilde{T}_n$ in Eq~\ref{eq:cfbl}.
\begin{align}\label{eq:define-tnl-tilde}
  \ttnl  =  \Tilde{T}_n + \frac{c_n}{n}\sum_{i=1}^n (\xi_i-1)\{\tdh(i)-\tdu\},
\end{align}
where $c_n=r$ when $Nn\rho_n^s\gg 1$ and $c_n=1$ otherwise.


\begin{remark}
As we show in Theorem~\ref{thm:clt-approx}, the variance of the approximate count statistic consists of the true limiting variance of the underlying U-statistic and the noise variance. When  $N= \Theta(1/n\rho_n^s)$, there is a phase transition from the case where the noise variance dominates to one where the signal variance dominates. The factor $c_n$ helps match the two variances before and after this phase transition. 
\end{remark}

We denote the bootstrap based on Eq~\ref{eq:define-tnl-tilde} by \mblapx and explicitly provide the algorithm in the Supplement (see Algorithm~\ref{alg:apx}). 

\iffalse
% \paragraph{Difference from previous work}
\begin{remark}
In~\cite{chen2019randomized}, the authors draw $\omega(N)$ subsets of size $r$ without replacement to estimate an incomplete $U$ statistic. The total number of subsets we examine is also $Nn/r$. Comparing our Theorem~\ref{thm: apprx-linear-bootstrap} with their result shows that both methods require $\omega(n)$ computation to achieve consistency. However, practically, drawing $Nn/r$ subsamples without replacement is slower than drawing a $N$ permutations and then scanning over each to look at disjoint subsets (see Fig~\ref{fig:4cycle-timing}). 
\end{remark}
\fi

\begin{remark}\label{remark:sparsity}
We can adapt the computation of \mblapx to exploit the sparsity in networks. Take for example the simple case of triangles. Instead of scanning over a given permutation of $n-1$ nodes to calculate $\tdh(i)$ for node $i$ (see Eq~\ref{eq:define-h1-tilde}), we can ``sample'' the positions of the neighbors of $i$ in a random permutation, and then check for consecutive neighbors among these positions, thus reducing the computation from $O(n)$ per permutation to $O(n\rho_n\log(n\rho_n))$.  This idea can be extended to other subgraphs as well. We provide details of this approach for counting triangles, two stars and three paths in the Supplement Section~\ref{sec:suppalgapx}. For large sparse graphs (with about 50,000 nodes and 750,000 edges) our approach computes three paths in about 850 seconds, where brute force counting did not finish in a day (see Section~\ref{sec:realdata}). This method reduces the complexity of approximating count statistics to $O(n^2N\rho_n\log(n\rho_n))$, while brute force counting for a three-path can be as large as $O(n^4)$ and become too slow and impractical for large sparse networks. 
\end{remark}


%for simple count statistics such as triangles, V-stars and three-paths, we use an equivalent method as we sample index of $i$'s neighbours in the permuted sequence and only check the disjoint subsets including the neighbours in the permutation. \color{blue}{The full algorithms are shown in Supplement Section~\ref{sec:suppalgapx}.} \rd This method reduces the complexity of approximating count statistics to $O(n^2N\rho\log(n\rho))$, while brute force counting for a three-path can be as large as $O(n^4)$ and become too slow and impractical for large sparse networks. 
\bk



\subsection{Higher-order correct bootstrap procedures}
In this section, we present our proposed quadratic, and multiplicative algorithms (\mbq, and \mbm). The detailed pseudocode can be found in the Supplement (Algorithm~\ref{alg:ho} in Section~\ref{sec:suppalgapx}).

For a given network, we first compute $\cfhat$ and $\hat{\tau}_n$ (see Eqs~\ref{eq:cf},~\ref{eq:tauhat}).
For each algorithm, we generate $B$ samples of $n$ weights $\{\w^{(j)}_i,i=1,\dots, n\}_{j=1}^B$ from the \texttt{Gaussian Product} distribution (see beginning of Section~\ref{subsec:proposed-bootstrap}). For each of these, \mbm, \mbq, and \mbl respectively values $\cfbm,\cfbq$ and $\cfbl$. From the $B$ values one then constructs the CDF of the statistic in question, after shifting and normalizing it appropriately. %(Y^{*}-\cfhat)/n^{1/2}\hat{\tau}_n$, where $Y^{*}$ is $\cfbm,\cfbq$ or $\cfbl$. 
While we divide by $\frac{r}{n^{1/2}}\hat{\tau}_n$, our statistic is not studentized, yielding a different expansion from previous work. Conditioned on the data, $\hat{\tau}_n$ is constant for the bootstrap samples.


Note that \mbm is computationally expensive since it involves computing the expression in Eq~\ref{eq:multiplicative-bootstrap} for each sample of the bootstrap. The worst-case complexity of evaluating all ${n\choose r}$ subsets of nodes is $n^r$. For $B$ bootstrap samples, the worst-case timing of \mbm will be $B n^r$. In comparison, for \mbl and \mbq, we can precompute the $\hat{g}_1(i)$ and $\hat{g}_2(i,j)$ values in $O(n^r)$ time. After that, the time per bootstrap sample is linear for \mbl and quadratic for \mbq. Thus worst-case computational complexity for a dense network for \mbm, \mbq, and \mbl is $O(Bn^r)$, $Bn^2$ and $Bn$ respectively, \textit{excluding} precomputation time (O($n^r$) in the worst case). In contrast, the approximate linear bootstrap is much faster (see Section~\ref{subsec:fast-linear-boot}).
% In contrast, the approximate linear bootstrap algorithm \mblapx takes O($Nn/r$) computation for each $\tilde{H}_1(i),i\leq n$. Note that we can easily parallelize this step. With $C$ cores, that will lead to a computational cost of $Nn^2/rC$.%As we mention in Remark~\ref{rem:apx}, experimentally, we see that $N=C\log n$ is enough.
% So the total computation including precomputation is $O(Nn^2)$, where precomputation for all other methods can be $O(n^r)$ in the worst case. \bk

%\rd Fix later\bk
%\subsection{Algorithm for functions of count functionals}
 %In this section, we explicitly provide the algorithm for the multiplicative bootstrap \bl for smooth functions of counts.  Other versions are analogous. Consider a function of $m$ count functionals $f(\theta_n^{(1)},\dots,\theta_n^{(m)})$. We first compute $u=f(\hat{\theta}_n^{1},\dots,\hat{\theta}_n^{m})$ from the whole graph. Then we  standardize with an  estimate of the variance (see Eq~\ref{eq:sigmahatf}). Call this $\hat{\sigma}_f$. For $i\in\{1,\dots, B\}$, draw $\{\w_1^{(i)},\dots,\w_n^{(i)}\}_{i=1}^B$ samples from the Gaussian Product distribution. Now, for each of these samples, compute the bootstrap estimate of the $m$ count functionals $u^*=\{\cfbm(\theta_n^{(1)}),\dots, \cfbm(\theta_n^{(m)})\}$. \rd Why Gaussian Multipliers?????? \bk

 % Again, $\hat{S}_n$ is a constant conditioned on the data, making this to be different from Studentized statistics. 
 % For the truth, we simply computed the CDF of a statistic normalized using the variance across all different runs. The experimental results suggest that indeed our multiplicative and quadratic procedures achieve higher order accuracy. 

% \rd
% \mbm is computationally expensive and since it involves computing the expression in Eq~\ref{eq:multiplicative-bootstrap} for each sample of the weighted bootstrap. For example, the worst-case complexity of evaluating all ${n\choose r}$ subsets of nodes is $n^r$. For $B$ bootstrap samples, the worst-case timing of \mbm will be $B n^r$. In comparison, for \mbl and \mbq, we can precompute the $\hat{g}_1(i)$ and $\hat{g}_2(i,j)$ values in $O(n^r)$ time. After that, the time per bootstrap sample is linear for \mbl and quadratic for \mbq. Thus worst-case computational complexity for a dense network for \mbm, \mbq, and \mbl is $O(Bn^r)$, $Bn^2$ and $Bn$ respectively, \textit{excluding} precomputation time (which is O($n^r$) in the worst case).\bk

% \subsection{Edgeworth Expansions \rd [shorten]}
% We will now introduce some notation needed to define Edgeworth expansions and higher-order correctness.  Let $\Phi(t)$ and $\phi(t)$ denote the CDF and PDF of a standard Normal distribution, respectively, \rd and $F_{\hat{T}_n}(t)$ denote the CDF of $\hat{T}_n$.  In Proposition 1, under some conditions, we show that, for the Edgeworth expansion $G_n(t)$: \bk
% \begin{align*}
% \norm{F_{\hat{T}_n}(t) - G_n(t)}_\infty = o(n^{-1/2}\rd \rho_n^{-1/2})
% \end{align*}
% where for $\tau_n^2=\var(E[h(X_S)\mid X_1])$, $G_n(t)$ is given by:
% \begin{equation}\label{eq:edgeworth-gn}
%     G_n(t)= \Phi(t)- \phi(t)\frac{(t^2-1)}{6n^{1/2}\tau_n^3}\biggl\{\mathbb{E}[g_1^3(X_1)]+3(r-1)\mathbb{E}[g_1(X_1)g_1(X_2)g_2(X_1,X_2)] \biggr\}.
% \end{equation}
% As previously discussed, $G_n(t)$ provides a refinement of the Berry-Esseen theorem, which gives an error bound $O(1/n^{1/2})$ for a Normal approximation.  In the next section, we will show that the same Edgeworth expansion applies to the bootstrap distribution, which would imply higher order correctness since:
% \begin{align*}
% F_{n}(u) - F_{n,M}^*(u)\leq \norm{F_{n}(u)  - G_n(u) } _\infty + \norm{G_n(u) -  F_{n,M}^*(u)  }_\infty
% \end{align*}

% \rd Define $F_n $ and $F_{n,M}^*(u)$\bk








% The Hoeffding decomposition (see the Supplementary Material for details) suggests that we may in fact approximate the distribution of $U_n - \theta_n$ more directly. Define the terms:
% \begin{align*}
% \hat{g}_1(i) &= \frac{1}{{n-1 \choose r-1 }} \sum_{1 \leq i_2 < \ldots i_r \leq n, i_u \neq i } \bigr(\bigl(H(A_{i,i_2,i_3 \ldots i_r}) - \hat{U}_n \bigr) 
% \\ \hat{g}_2(i,j) &= \frac{1}{{n-2 \choose r-2 }} \sum_{1 \leq i_3 < \ldots i_r \leq n, i_u \neq i,i_u \neq j }  \bigl(H(A_{i,i_2,i_3 \ldots i_r}) - \hat{U}_n \bigr)    
% \end{align*}
% The quadratic multiplier bootstrap is given by:
% \begin{align}
% \begin{split}
% \hat{U}_{n, \w}^Q &= \hat{T}_n +  \frac{r}{n}\sum_{i=1}^n (\w_i-1) \cdot \hat{g}_1(i)  + \frac{r(r-1)}{n(n-1)}\sum_{i<j } \ (\w_i \ \w_j - 1) \cdot \hat{g}_2(i,j)  
% \\ & \ \ \ - (\w_i-1) \cdot \hat{g}_1(i) - (\w_i-1) \cdot \hat{g}_1(j)
% \end{split}
% \end{align}
% The Hoeffding decomposition implies that the variance of our bootstrap functionals is largely determined by the variance of a sum of independent random variables.  Define:  
% \begin{align*}
% \sigma_{boot}^2 = \frac{r^2}{n}\sum_{i=1}^n \hat{g}_1^2(i), \ \ \ \hat{T}_n^M = \frac{ \hat{U}_{n,\w}^M -\hat{U}_n}{\sigma_{boot}}, \ \ \ \hat{T}_n^Q = \frac{ \hat{U}_{n,\w}^Q -\hat{U}_n}{\sigma_{boot}}   
% \end{align*}




% \begin{align*}
% g_1(X_i) &= \mathbb{E}[h(X_i, X_{i_2} \ldots X_{i_r}) \mid X_i] - \theta_n 
% \\ g_2(X_i, X_j) &= \mathbb{E}[h(X_i, X_j, X_{i_3} \ldots X_{i_r}) \mid X_i, X_j] - g_1(X_i) - g_1(X_j)  - \theta_n
% \end{align*}





% Our multiplicative bootstrap is motivated by Hoeffding's decomposition, which we describe below, following Section 4 of \citet{Bentkus-edgeworth-symmetric}.  Let $X_1, \ldots, X_n$ be independent random variables and $\Omega = \{1, \ldots n\}$. For any $A \subset \Omega$ and a random variable $T$, let $T_A = \mathbb{E}[T \mid  X_i \in A]$.  It may be verified that $T_A = \sum_{B \subset A} (-1)^{|A| - |B|} T_B $. We also have the inverse relationship $\mathbb{E}[T \mid X_i \in B] = \sum_{A \subset B} T_A  $, which implies the Hoeffding decomposition:
% \begin{align}
%     T = \sum_{A \subset \Omega} T_A
% \end{align}
% It turns out that the Hoeffding decomposition for $\hat{T}_n - \theta_n$ has the same form a noiseless U-statistic.  Define the terms:
% \begin{align*}
% g_1(X_i) &= \mathbb{E}[h(X_i, X_{i_2} \ldots X_{i_r}) \mid X_i] - \theta_n 
% \\ g_2(X_i, X_j) &= \mathbb{E}[h(X_i, X_j, X_{i_3} \ldots X_{i_r}) \mid X_i, X_j] - g_1(X_i) - g_1(X_j)  - \theta_n
% \end{align*}
% The Hoeffding decomposition for $\hat{T}_n - \theta_n$ may be written as:
% \begin{align*}
% T_n - \theta_n = \frac{r}{n}\sum_{i=1}^n g_1(X_i) + \frac{r(r-1)}{n(n-1)} \sum_{i < j} g_2(X_i,X_j) + O_p\left(\frac{1}{n}\right) 
% \end{align*}

% Conditioning on  $X_1, \ldots X_n$, we may also define a Hoeffding decomposition for $\hat{T}_{n, \xi}^M$ with respect to $\w_1, \ldots \w_n$.  Let:
% %
% \begin{align*}
% \hat{g}_1(i) &= \frac{1}{{n-1 \choose r-1 }} \sum_{1 \leq i_2 < \ldots i_r \leq n, i_u \neq i } \bigr(\bigl(H(A_{i,i_2,\ldots i_r}) - \hat{T_n} \bigr) 
% \\ \hat{g}_2(i,j) &= \frac{1}{{n-2 \choose r-2 }} \sum_{1 \leq i_3 < \ldots i_r \leq n, i_u \neq i,i_u \neq j }  \bigl(H(A_{i,i_2, \ldots i_r}) - \hat{T_n} \bigr)    
% \end{align*}
% %
% We have the following decomposition:
% \begin{align}
% \begin{split}
% \hat{T}_{n, \w}^M - \hat{T}_n &= \frac{r}{n}\sum_{i=1}^n (\w_i-1) \cdot \hat{g}_1(i)  + \frac{r(r-1)}{n(n-1)}\sum_{i<j } \ (\w_i \ \w_j - 1) \cdot \hat{g}_2(i,j)  
% \\ & \ \ \ - (\w_i-1) \cdot \hat{g}_1(i) - (\w_i-1) \cdot \hat{g}_1(j)   + O_P(1/n)
% \end{split}
% \end{align}
% Viewing $\hat{g}_1(X_i)$ and $\hat{g}_2(X_i,X_j)$ as estimates of $g_1(X_i)$ and $g_2(X_i, X_j)$, respectively , it is clear that that our weighted bootstrap version encapsulates important information about $T_n - \theta_n$.  The above decomposition also suggests that one may approximate the non-negligible terms more directly.  Ignoring the remainder term, we arrive at the quadratic bootstrap:
% \begin{align}
%  \hat{T}_{n,\xi}^Q =    
% \end{align}





% Our quadratic multiplier bootstrap may be viewed as an approximation to the multiplicative multiplier that only considers the first two terms in the Hoeffding decomposition; see the Supplementary Material for details.

% Define the following terms:
% \begin{align}

% \end{align}





==> network_mb_jasa_to_arxiv (1)/realdata.tex <==
\subsection{Real data application}
\label{sec:realdata}
%In this section, we apply our algorithms to compare networks representing the voting similarities of U.S. Congress.
%\begin{figure}[!htb]
%	\centering
%	\includegraphics[width= \textwidth]{plots2/house-threshold-illustration.png}
%	\caption{Threshold for forming edges between congress members calculated from histograms of same-party (SP) and cross-party (CP) agreements, illustrated with example of 81st Congress and 109th Congress}
%	\label{fig:votethreshold}
%\end{figure}
%We use roll call vote data from the U.S. House of Representatives~\citep{voteview} from 1949 (commencement of the 81$^{st}$ Congress) to 2012 (adjournment of 112$^{nd}$ Congress). Each Congress forms a network of representatives (nodes).  An edge between a node pair is formed when the number of agreements, i.e. number of times they both vote \textit{yay} or \textit{nay}  exceeds a threshold computed by~\citep{andris2015votethreshold} of this congress. The threshold is computed by constructing histograms of same-party pairs’ number of agreements and cross-party pair’s number of agreements and using the intersection point of the two histograms as the threshold. We will denote same-party by \texttt{SP} and cross-party by \texttt{CP}. For example, the threshold value is $124$ for $81$st Congress and $766$ for $109^{th}$ Congress as illustrated in Figure~\ref{fig:votethreshold}.
%%Now we have a vote record network formed between members for each Congress. 
%For each network, we calculate the normalized cross-party edge density and cross-party triangle density, and perform our bootstrap methods on these quantities.  We construct 95\%  second-order corrected Confidence Intervals from  the MB-Q method and present the CIs over $81$st to $112$nd Congress.  Note that the CIs are adjusted by Bonferonni Correction where  $\alpha=1-0.05/32$ for $32$ experiment congresses. 
%
%In Figure~\ref{fig:voteCI}, we can see a significant decrease in cross party edge densities and cross party triangle densities over the years,  suggesting a trend of decreasing bipartisan agreement.
%\begin{figure}[!htb]
%    \centering
%    \includegraphics[width=0.45\textwidth]{plots2/house-year-mb-cped-bc-quantile-mblinqua.pdf}
%    \includegraphics[width=0.45\textwidth]{plots2/house-year-mb-cptri-bc-quantile-mblinqua.pdf}
%    \caption{Bonferroni-adjusted 95\% second-order corrected CI for cross party edge density (left) and cross party triangle density (right) from 1949 (commencement of the 81st Congress) to 2012 (adjournment of 112nd Congress).}
%    \label{fig:voteCI}
%\end{figure}
%
%%\iffalse
%%\rd REMOVE?
%%We also present here the average timing for $32$ congresses each method takes.
%%%\begin{figure}[H]
%    %\centering
% %   \includegraphics[width=0.47\textwidth]{plots2/runtime-cped.pdf}
% %   \includegraphics[width=0.47\textwidth]{plots2/runtime-cptri.pdf}
% %   \caption{Time in seconds for each method takes on average for $32$ congresses, on cross-party edge density (Left) and cross-party triangle density (Right).}
%  %  \label{fig:votetiming}
%%\end{figure}
%
%%\fi
%%\rd
%%To further illustrate our approximated linear bootstrap algorithm on large sparse networks, we apply \mblapx on Facebook page network dataset. %In the first example, we use the Facebook college network data from \cite{nr}. We compare three college pairs, Yale and Harvard, Duke and Wake Forest University (WFU), Auburn and UGA. Yale and Harvard are both Ivy League colleges; Duke and Wake Forest are both large universities in North Carolina; Auburn and UGA are both large public land-grant research university in the South.  We compare each pair using \mblapx constructed $90\%$ CI of triangles, two-stars and three-paths. Figure~\ref{fig:fb-colleges} shows that triangles can significantly separate all three pairs. Harvard has significantly more normalized counts of triangles compared to Yale, and so does Duke to its comparison Wake Forest, and UGA to Auburn. \sout{Table~\ref{tab:fb-colleges-summary} summarizes the size, edge density and time cost for each network and count statistic.}\bl The size of the networks in this study ranges from around $5000$ to $25000$, edge density ranges from $0.004$ to $0.011$. For example, for UGA of size $24389$ and edge density $0.004$, our approximate three-path calculation takes $18$min $23$s (in total 1103 s) while brute force counting does not finish in $24$ hours. 
%
%
%%\begin{figure}
% %   \centering
%   %    \scriptsize
%   % \begin{tabular}{ccc}
%   % \includegraphics[width=0.3\textwidth]{plots2/Bonf-Colleges_wUGA_CI_tri.pdf}
%  %  &\includegraphics[width=0.3\textwidth]{plots2/Bonf-Colleges_wUGA_CI_vstar.pdf}
%   % &\includegraphics[width=0.3\textwidth]{plots2/Bonf-Colleges_wUGA_CI_3path.pdf}\\
%   % Triangles & two-stars & Three-paths \\
%   % \end{tabular}
%   % \caption{Bonferroni-adjusted $90\%$ CI for three pairs of college comparison with triangles, two-stars and three-path using \mblapx algorithm.}
%    %\label{fig:fb-colleges}
%%\end{figure}
%\iffalse
%\begin{table}[h]
%\scriptsize
%\centering
%\begin{tabular}{|l|c|c|c|c|c|}
%\hline
%        & \multicolumn{1}{l|}{Size} & \multicolumn{1}{l|}{Edge Density} & \multicolumn{1}{l|}{Time Cost (Triangles)} & \multicolumn{1}{l|}{Time Cost (two-stars)} & \multicolumn{1}{l|}{Time Cost (Three-paths)} \\ \hline
%Yale    & 8578                      & 0.011                              & 27.88s                                     & 53.71s                                   & 288.64s                                      \\ \hline
%Harvard & 15126                     & 0.007                              & 62.39s                                     & 134.64s                                  & 691.29s                                      \\ \hline
%Duke    & 9895                      & 0.010                              & 35.18s                                     & 68.10s                                   & 360.51s                                      \\ \hline
%WFU     & 5372                      & 0.019                              & 17.66s                                     & 32.66s                                   & 173.56s                                      \\ \hline
%Auburn  & 18448                     & 0.005                              & 76.81s                                     & 176.90s                                  & 830.76s                                      \\ \hline
%UGA     & 24389                     & 0.004                              & 100.80s                                    & 237.14s                                  & 1103.07s                                     \\ \hline
%\end{tabular}
%\caption{Summaries of size, edge density and time cost for each network and count statistics in the Facebook colleges dataset.}
%\label{tab:fb-colleges-summary}
%
%\boxed{\bl Summarize \ the \ table! }
%\end{table}
%\fi
To illustrate our approximated linear bootstrap algorithm on large sparse networks, we apply \mblapx (with the speedup for sparse graphs discussed in Remark~\ref{remark:sparsity}) on the Facebook page network dataset from \cite{rozemberczki2019gemsec}. Each network represents blue verified Facebook pages of different categories. Nodes represent the pages and edges are mutual likes among them. We compare the categories of athletes, politicians and artists also using \mblapx constructed $90\%$ CIs using triangles, two-stars and three-paths. Figure~\ref{fig:fb-pages} shows that both three-paths and two-stars can separate all three pairs of the networks:  athletes vs politicians, athletes vs artists, politicians vs artists, while three-paths provide more clearly separate CIs than two-stars. Three-paths and two-stars are significantly more prevalent in the network of artists compared to athletes and politicians. The sizes of the networks in this example range from around $5000$ to $50000$, whereas the edge densities range from $0.0006$ to $0.0024$. For example, for the artist network ($50515$ nodes, edge density is $0.0006$), our approximate three-path calculation takes around $14$ minutes  while brute force counting does not finish in $24$ hours. See detailed description in Supplement Section~\ref{sec:addlexp}. \bk

\begin{figure}
    \centering
        \scriptsize
    \begin{tabular}{ccc}
    \includegraphics[width=0.3\textwidth]{plots2/New2BonfCo_FB_CI_3grp_tri.pdf}
    &\includegraphics[width=0.3\textwidth]{plots2/New2BonfCo_FB_CI_3grp_vstar.pdf}
    &\includegraphics[width=0.3\textwidth]{plots2/New2BonfCo_FB_CI_3grp_3path.pdf}\\
    Triangles & Two-stars & Three-paths \\
    \end{tabular}
    \caption{Bonferroni-adjusted $90\%$ CI for three categories of Facebook pages with triangles, two-stars and three-path using \mblapx algorithm.}
    \label{fig:fb-pages}
\end{figure}

We also compare networks representing the voting similarities of U.S. Congress, which we defer to the Supplement Section~\ref{sec:addlexp} for space constraints.
%---- move to section 4.1 -----

%Note that in \mblapx, instead of doing full permutations of all $n-1$ nodes to calculate $\tdh(i)$ for node $i$ as described in Eq~\ref{eq:define-h1-tilde}, for simple count statistics such as triangles, two-stars and three-paths, we use an equivalent method as we sample index of $i$'s neighbours in the permuted sequence and only check the disjoint subsets including the neighbours in the permutation. \color{blue}{The full algorithms are shown in Supplementary Section~\ref{sec:suppalgapx}.} \rd This method reduces the complexity of approximating count statistics to $O(n^2N\rho\log(n\rho))$, while brute force counting for a three-path can be as large as $O(n^4)$ and become too slow and impractical for the two facebook examples shown above. 


\bk



==> network_mb_jasa_to_arxiv (1)/related_work.tex <==
%Several resampling procedures have recently been proposed for count functionals.  
The first theoretical result for resampling network data was attained by~\citet{Bhattacharyya-subsample-count-features}.  Their subsampling proposals involve expressing the variance of a count functional in terms of other count functionals and estimating the non-negligible terms through subsampling.  \citet{subsampling-sparse-graphons} show that it is also possible to conduct inference using quantiles of the subsampling distribution as in~\citet{politis-romano-subsampling-minimal-assumptions}.   \citet{green-shalizi-network-bootstrap} propose a bootstrap based on the empirical graphon.  \citet{network-jackknife-theory} establish the validity of the network jackknife for count functionals. 

  \citet{levin-levina-rdpg-bootstrap} study a two-step procedure that is closely related to our linear bootstrap procedure. The above authors propose estimating the latent positions with the adjacency spectral embedding in the first step (see, for example, \citet{athreya-rdpg-survey}) and resampling the corresponding U-statistic with the estimated positions in the second step. They derive theoretical results under the assumption that the rank of the random dot product graph model is known and finite.  In contrast, our procedures do not impose assumptions on the spectral properties of the underlying graphon. \bk

% In contrast, our bootstrap procedure involves directly multiplying each potential subgraph in the network by a multiplier random variable. Applying the multiplier directly mimics the data generating process and we do not have to estimate the latent positions.  Furthermore, \citet{levin-levina-rdpg-bootstrap} consider only consider a linear bootstrap procedure, which does not offer improved accuracy for moderately sparse networks.
% \citet{levin-levina-rdpg-bootstrap} study a network bootstrap closely related to our proposal


% with one of the main differences being the estimation of latent positions.
% \citet{network-jackknife-theory} establish the validity of the network jackknife for count functionals. 

~\citet{zhang-xia-network-edgeworth} establish conditions under which the empirical graphon bootstrap exhibits higher-order correctness.  For establishing higher-order correctness for resampling methods studied in this work, Cram\'{e}r's condition is required, which is restrictive for network models.  %The jackknife is also considered as a variance estimator for an empirical Edgeworth expansion in \rd\citet{zhang-xia-network-edgeworth}\bk.  
In contrast, their empirical Edgeworth expansion proposal does not require Cram\'{e}r's condition. %which has been considered in other settings (see, for example, \citet{putter-vanzwet-empirical-edgeworth} and \citet{maesono-edgeworth-expansion-u-statistics}), involves studentizing by a variance estimate and plugging in estimated moments into an Edgeworth expansion.  
%In our work, we show that even for smooth functions, our proposed bootstrap procedures exhibit higher-order correctness. Multiplier bootstraps can handle functions of subgraph counts more easily than empirical Edgeworth corrections.   %While computationally more demanding, work in other settings suggests that the bootstrap may have some favorable properties over empirical Edgeworth expansions (see, for example, \citet{hall-bootstrap-vs-edgeworth}).  
% However, the empirical Edgeworth expansion assumes the existence of a valid Edgeworth expansion, which requires non-trivial sparsity and integrability conditions.  In contrast, the bootstrap adapts to the regularity of the problem, yielding higher order correctness when these conditions are met and still offering strong performance otherwise. 
On the mathematical side, the analysis of our multiplier bootstrap involves Edgeworth expansions for weighted sums. %Analyzing these non identically distributed random variables leads to error rates which are less sharp than existing work. % we see that multiplier bootstraps can handle functions of subgraph counts more easily than empirical Edgeworth corrections.  
% The generality of the Lindeberg-Feller central limit theorem suggests that going from independent and identically distributed sequences to independent but non-identically distributed sequences poses no essential difficulty for establishing weak convergence.  However, for Edgeworth expansions, 
Prior work (c.f. \citet{bai-zhao-independent-edgeworth} and \citet{liu-non-iid-bootstrap}) suggests that establishing sharp rates of convergence for the independent but non-identically distributed sequences is more difficult, with the above references establishing a  $o(n^{-1/2})$ error bound instead of the $O(n^{-1})$ bound for i.i.d. sequences.  Therefore, it is not surprising that our quadratic bootstrap proposal, while offering improved performance over first-order correct methods, does not quite match the rate of the empirical Edgeworth expansions studied by \citet{zhang-xia-network-edgeworth}.   

% We believe that this is the reason for not matching the same error rate as previous work. %Edgeworth expansions for multiplier bootstraps of (degree 2) U-statistics are also considered in~\citet{wang-jing-weighted-bootstrap-u-statistics}.

From the computational standpoint, \citet{chen2019randomized} presented a randomized algorithm to estimate high-dimensional U-statistics from a subsample of subsets from the set of all subsets of a given size. We propose a different sampling method that exploits the structure of U-statistics and draws random permutations instead of subsets. Empirically, we show that this method provides faster computation over subset sampling.








==> network_mb_jasa_to_arxiv (1)/supplementary_body.tex <==
% \documentclass[11pt]{article}
% \usepackage{amsmath,amssymb,amsthm}
% \usepackage{amsmath,amssymb,amsthm}
% \usepackage{stackengine}
% \usepackage{scalerel}

% \usepackage{xr}
% \externaldocument{network_mb}




% \usepackage[table]{xcolor}
% \usepackage{bbm}
% \usepackage[utf8]{inputenc}
%  \usepackage[english]{babel}
%  \usepackage{nameref,zref-xr}
 
%  \usepackage{natbib}
%  \bibliographystyle{plainnat}
%  %\usepackage[numbers]{natbib}
% % \zxrsetup{toltxlabel}
% % \zexternaldocument*{ms_arxiv}
% %\zexternaldocument*{network_jackknife.tex}
% %\renewcommand{\thesubsection}{\Alph{subsection}}
% %\renewcommand{\theequation}{\Alph{equation}}
% %\renewcommand{\thesection}{A.\arabic{section}}
% %\renewcommand{\thesubsection}{A.\arabic{subsection}}
% %\renewcommand{\theequation}{A.\arabic{equation}}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{Remark}{Remark}[section]
% \newtheorem{Proof}{Proof}[section]
% \newtheorem{corollary}{Corollary}[theorem]
% \newtheorem{lemma}[theorem]{Lemma}
% \newcommand{\rd}{\color{red}}
% \newcommand{\bk}{\color{black}}
% \newcommand{\bl}{\color{blue}}

% \newcommand{\shat}{\hat{\sigma}_n}
% \newcommand{\m}{\delta}
% \newcommand{\w}{\xi}
% \newcommand{\W}{\xi}
% \newcommand{\dnm}{\Delta_n(m)}
% \newcommand{\tnas}{T_{n,1}^{*}}
% \newcommand{\tnbs}{T_{n,2}^{*}}

% \newcommand{\gi}{\hat{g}_1(i)}
% \newcommand{\gj}{\hat{g}_1(j)}
% \newcommand{\ggij}{\hat{g}_2(i,j)}

% \newcommand{\hi}{\hat{H}_1(i)}
% \newcommand{\hj}{\hat{H}_1(j)}
% \newcommand{\hhij }{\hat{H}_2(i,j)}
% \newcommand{\hij }{h_2(X_i,X_j)}



% \newcommand{\cov}{\mathrm{cov}}
% \newcommand{\var}{\mathrm{Var}}

% \newcommand{\tnt}{\Tilde{T}_n}
% \newcommand{\tnhat}{\hat{T}_n}
% \newcommand{\vnhat}{\hat{V}_n}


% \usepackage[utf8]{inputenc}
% \usepackage[english]{babel}
%  \newcommand{\E}{E}
% \newcommand{\gnhat}{\hat{G}_n}


% \section{On the Hoeffding Decomposition}

%\appendix
\newcommand{\bcom}{ \kappa_n }
\newcommand{\lfn}{ l_{5,n} \bk}
%\newcommand{\bb}[1]{\left(#1\right)}
%\section{Proof of Lemma \ref{lemma:hoeffding-bootstrap}(Hoeffding Decomposition for Bootstrapped Count Functional)}

%\section*{Appendix}
%In this supplement we provide proofs of Lemmas and main theorems in the paper.


%
%BLAHBLAHBLAH

%%%% Detailed code is in last section, section 9 %%%%%%%%%%%%%%%

\section{Proof of Lemma~\ref{lemma:hoeffding-bootstrap}}
\label{sec:supp:lemmaone}
% \begin{proof}\normalfont
In what follows, we will consider a projection of $T_{n,M}^*$ with respect to the random variables $ \w_1, \ldots \w_n$, conditional on $A$ and $X$. 

Recall that $\xi_i$ follows the Gaussian Product distribution. First, we may express $T_{n,M}^*$ as:
\begin{align*}
T_{n,M}^* = \frac{1}{{n \choose r}} \sum_{1 \leq i_1 < i_2 < \ldots i_r} \left(\xi_{i_1 \cdots i_r} - 1\right)  \cdot \left\{ H(A_{i_1, \ldots, i_r}^{(n)}) - \hat{T}_n \right\}
\end{align*}
where $\xi_{i_1 \cdots i_r}$ denotes the product $\xi_{i_1} \times \cdots \times \xi_{i_r}$. It turns out that applying the Hoeffding decomposition directly to $T_{n,M}^*$ leads to tedious combinatorial calculations; following \citet{Bentkus-edgeworth-symmetric}, let $\Omega_r$ denote an $r$-tuple of $\{1, \ldots, n\}$.  For each summand, we will consider a Hoeffding representation with respect to $\Omega_r$.   Note that using the Hoeffding projection (also see~\cite{Bentkus-edgeworth-symmetric} section 2.8), 
\begin{align*}
    \prod_{1\leq i\leq r}\w_i-1=\sum_{k=1}^r\sum_{1\leq i_1<\dots< i_k\leq r} h_k(\w_{i_1},\dots,\w_{i_k}),
\end{align*}
where for $\Omega_k=\{1,\dots, k\}$,
\begin{align*}
    h_k(\w_{1},\dots,\w_{k})=\sum_{B\in \Omega_k}(-1)^{k-|B|}\E\left\{\prod_{1\leq i\leq r}\w_i-1\mid B\right\}
\end{align*}
Thus the first two terms are given by:
\begin{align*}
    h_1(\w_{1})&:=(\w_1-1)\\ h_2(\w_{1},\w_{2})&:=(\w_1\w_2-1)-(\w_1-1)-(\w_2-1)=(\w_1-1)(\w_2-1)
\end{align*}
In what follows, we will also denote $A^{(n)}_{i_1,\dots,i_r}$ by $A^{(n)}_S$, where $S=\{i_1,\dots, i_r\}$.
Let 
\begin{align}\label{eq:hhij}
    &\hhij= \frac{1}{{n-2 \choose r-2}}\sum_{S \ | \ i,j\in S}H(A_S),\\
    & \hat{H}_u(i_1,\ldots,i_u)=\frac{1}{{n-u \choose r-u}}\sum_{S \ | \ i_1,\ldots,i_u \in S}H(A_S) \notag.
\end{align}
Thus $T_{n,M}^*$ can be written as follows:
\begin{align}\label{eq:hofftnm}
    T_{n,M}^* &= \frac{1}{{n \choose r}} \sum_{1 \leq i_1 < i_2 < \ldots < i_r} \left(\xi_{i_1 \cdots i_r} - 1\right)  \cdot \left\{ H(A_{i_1, \ldots, i_r}^{(n)}) - \hat{T}_n \right\}\notag\\
    &=\frac{1}{{n \choose r}} \sum_{1 \leq i_1 < i_2 < \ldots < i_r}\sum_{k=1}^r\sum_{1\leq i_1<\dots< i_k\leq i_r} h_k(\w_{i_1},\dots,\w_{i_k})\cdot \left\{ H(A_{i_1, \ldots, i_r}^{(n)}) - \hat{T}_n \right\}\notag\\
    &=\frac{1}{{n \choose r}} \sum_{k=1}^r \sum_{1\leq i_1<\dots< i_k\leq n} h_k(\w_{i_1},\dots,\w_{i_k})\cdot\sum_{S}  \left\{ H(A_S^{(n)}) - \hat{T}_n \right\}1 (i_1,\dots, i_k\in S)\notag\\
    &=\frac{1}{{n \choose r}} \sum_{k=1}^r {n-k\choose r-k}\sum_{1\leq i_1<\dots< i_k\leq n}h_k(\w_{i_1},\dots,\w_{i_k}) \frac{\sum_{S}  \left\{ H(A_S^{(n)}) - \hat{T}_n \right\}1 (i_1,\dots, i_k\in S)}{{n-k\choose r-k}}\notag\\
    &=\frac{r}{n}\sum_i (\xi_i-1)\gi+\frac{r(r-1)}{n(n-1)}\sum_{1\leq i<j\leq n} (\w_i-1)(\w_j-1)\underbrace{\{\hat{H}_2(i,j)-\tnhat\}}_{\tilde{g}_2(i,j)}+R_n
\end{align}


\iffalse
The first two terms of the decomposition are given by:
\begin{align*}
f_1(A_{i,i_2, \ldots, i_r}) &= \left(\xi_i - 1 \right) \cdot \left( H(A_{i,i_2, \ldots, i_r}^{(n)}) - \hat{T}_n \right) 
\\ f_2( A_{i,j,i_3, \ldots, i_r}) %&= \rd \left(\xi_i \cdot \xi_j - \w_i-\w_j +1 \right) \cdot \left( H(A_{i,j,i_3, \ldots, i_r}^{(n)}) - \hat{T}_n \right) \bk\\
&=\left(\xi_i \cdot \xi_j - 1 \right) \cdot \left( H(A_{i,j,i_3, \ldots, i_r}^{(n)}) - \hat{T}_n \right) - f_1(A_{i,i_2, \ldots, i_r}) - f_1(A_{j,i_2, \ldots, i_r})
\end{align*}

\begin{align*}
f_{1,i}(A_{S}) &= \left(\xi_i - 1 \right) \cdot \left( H(A_{S}^{(n)}) - \hat{T}_n \right) 1(i\in S)
\\ f_{2,i.j}( A_{S}) &=  \left(\xi_i \cdot \xi_j - \w_i-\w_j +1 \right) \cdot \left( H(A_{S}^{(n)}) - \hat{T}_n \right)1(i,j\in S) \bk\\
%&=\left(\xi_i \cdot \xi_j - 1 \right) \cdot \left( H(A_{i,j,i_3, \ldots, i_r}^{(n)}) - \hat{T}_n \right) - f_1(A_{i,i_2, \ldots, i_r}) - f_1(A_{j,i_2, \ldots, i_r})
\end{align*}
\bk
 Now, combining terms, we have that:
\begin{align*}
 T_{n,M}^* - \hat{T}_n &= \frac{1}{{n \choose r}} \sum_{\Omega_r \subset \Omega}  \left(\xi_{i_1 \cdots i_r} - 1\right)  \cdot \left( H(A_{i_1, \ldots, i_r}^{(n)}) - \hat{T}_n \right) 
 \\ &= \frac{r}{n} \sum_{i=1}^n (\xi_i - 1) \hat{g}_1(i)
 \\ & \ \ \ +\frac{r(r-1)}{n(n-1)}\sum_{i<j}(\w_i\w_j-1) \tilde{g}_2(i,j)-(\w_i-1) \cdot \hat{g}_1(i) - (\w_i-1) \cdot \hat{g}_1(j) + R_n
% \\ & = \frac{r}{n}\sum_{i=1}^n \sum_{ f_1(\xi_i; A_{i, i_2, \ldots, i_r}) + \frac{r(r-1)}{n(n-1)} \sum_{i < j} f_2(\xi_i, \xi_j; A_{i,j,i_3, \ldots, i_r}) +R_n 
 \end{align*}
 \fi
 Now, it remains to show that the remainder of $(T_{n,M}^* - \hat{T}_n)/\hat{\sigma}_n$ is $O(\delta(n,\rho_n,R))$, where:
 \begin{align*}
    \delta(n,\rho_n,R) =\begin{cases} 
      \frac{1}{n\rho_n} & \text{R is acyclic} \\
       \frac{1}{n\rho_n^{3/2}}& \text{R is a simple cycle} .
  \end{cases}
\end{align*}



 The residual $R_n$ is a sum of higher order Hoeffding projections, which are all uncorrelated. %
 Therefore, we see that the variance of the $u^{th}$ order term is $\dfrac{\sum_{1\leq i_1<i_2\dots<i_u}  \tilde{g}_u(i_1,\dots,i_u)^2}{\hat{\sigma}_n^2 {n\choose u}^2}$. We will now obtain expressions for $3\leq u\leq r$.
 %Therefore, we see that the variance of the third order term (the first one in the remainder) is $\dfrac{\sum_{ijk}  \hat{g}_3(i,j,k)^2}{\hat{\sigma}_n^2 {n\choose 3}} \times O(1/n^3)$.  By Markov inequality, it further suffices to show $\E[\hat{g}_3(i,j,k)^2\delta^2(n,\rho_n,R)/\hat{\sigma}_n^2  ] )$ is bounded.
 %Now, we have that:
 %\begin{align*}
 %\E[\tilde{g}_u(i,j,k)^2] \leq 2 \left( \mathrm{Var}(\hat{g}_3(i,j,k)) + \mathrm{Var}(\hat{T}_n) \right)
 %\end{align*}
 
 
 
%  We may reinterpret $\E[\hat{g}_3(i,j,k)^2$ as $\mathrm{Var}(\hat{g}_3(i,j,k))$.  To bound this term,    
 
%  Note that  $\hat{g}_3(i,j,k)^2=O_P(\rho_n^{3s-3})$ for cyclic and $O_P(\rho_n^{3s-2})$ for acyclic subgraphs. This is because, for any two nonoverlapping $S,T$ (not containing $\{i,j,k\}$)  of size $r-3$, there are potentially three edges common between the subgraphs induced by $S\cup \{i,j,k\}$ and  $S\cup \{i,j,k\}$ for a cyclic subgraph, and two for an acyclic one.
%  Thus we can show that the remainder is the same order as $O(\mathcal{M}(n,\rho_n,R))$.




% For each summand, since $\E[\w] = 1$, it is now clear that the conditional expectation with respect to a set $A$ is $0$ if  $\{i_1, \ldots i_r\} \cap A = \emptyset$.  We may collect summands with a nonempty intersection, leading to the expressions:
% \begin{align*}
%  T_{\{\xi_i\}} = \left(\xi_i - 1 \right) \cdot \frac{{n-1 \choose r-1}}{{n \choose r}} \cdot \left[\frac{1}{{n-1 \choose r-1}} \sum_{i, i_2 < \ldots < i_r, i_u \neq i } \left( H(A_{i, i_2, \ldots, i_r}^{(n)}) - \hat{T}_n \right)\right]     
% \end{align*}

% \begin{align*}
%  T_{\{\xi_i, \xi_j \}}  &= \left(\xi_i \cdot \xi_j + \xi_i + \xi_j - 1 \right) \cdot \frac{{n-2 \choose r-2}}{{n \choose r}} \cdot \left[\frac{1}{{n-2 \choose r-2}} \sum_{i,j i_3 < \ldots < i_r, i_u \neq i,j } \left( H(A_{i,j,i_3, \ldots, i_r}^{(n)}) - \hat{T}_n \right)\right]
%  \\  & \ \ \ + (\xi_i-1) \cdot T_{\xi_i} + (\xi_i-1) \cdot T_{\xi_j}
% \end{align*}



% For any set set $S$ of $r$ nodes, $S=\{i_{1}\dots i_{r}\}$, denote $\W_S= \prod_{i \in S} \w_i$.
% Conditioned on the graph $A$ and $X$, we see that the hoeffding projections of the weighted bootstrap statistic gives: %the $X$ observed as $x$, $\tnt$ and $\hat{H}(x_i)$ for each $i$ are all observed.  $\hat{H}(x_i)$ is defined as
% \begin{equation*}
%     \begin{split}
%      &\hi= \frac{1}{{n-1 \choose r-1}}\sum_{S,i\in S}H(A_S), \\
%      &\hhij= \frac{1}{{n-2 \choose r-2}}\sum_{S,i,j\in S}H(A_S).
% \end{split}
% \end{equation*}
% Recall the definition of $\gi$ and $\gj$ from the main paper. To remind the reader, we have:

% \begin{equation*}
%     \begin{split}
%      &\gi= \frac{1}{{n-1 \choose r-1}}\sum_{S,i\in S}(H(A_S)-\tnhat), \\
%      &\ggij= \frac{1}{{n-2 \choose r-2}}\sum_{S,i,j\in S}(H(A_S)-\tnhat).
% \end{split}
% \end{equation*}

% We are interested in the Hoeffding decomposition [\rd Put eqn number from main \bk] of the following quantity. Below we derive the Hoeffding decomposition.
% %We define weighted boostrap of count statistic as $\vnhat$. Conditioned on A, Standardized $\vnhat$ can be written as follows using $\W_S=1$.
% \begin{equation}\label{eq:wb-def-vn}
%     \begin{split}
%         \frac{\vnhat-\tnhat}{\hat{\sigma}_n}&=\frac{\sum_S \W_S (\hat{H}(A_S)-\tnhat)}{{n \choose r} \hat{\sigma}_n} = \frac{\sum_S (\W_S-1)(\hat{H}(A_S)-\tnhat)}{{n \choose r} \hat{\sigma}_n} \\
%         &=\frac{r}{n\hat{\sigma}_n} \sum_i f_1(\w_i) + \frac{r(r-1)}{n(n-1)\hat{\sigma}_n} \sum_{1\leq i<j \leq n} f_2(\w_i,\w_j) + \rd R_n \bk.
%     \end{split}
% \end{equation}

% We now derive the Hoeffding projections.

% Applying a Hoeffding decompsition to $\sum_S (\W_S-1)(\hat{H}(A_S)-\tnhat)/{n \choose r}$ above with respect to $\W$ yields

% \begin{equation*}
%     \begin{split}
%       & f_1(\w_i)= E[\hat{H}(X_S,\\W_S)\mid\w_i,x_i]; \\
%       & f_2(\w_i,w_j)=E[\hat{H}(X_S,\\W_S)\mid\w_i,x_i,\w_j,x_j].
%     \end{split}
% \end{equation*}
% Equivalently , $g_1(x_i)$ and $g_2(x_i,x_j)$ can be written as 
% \begin{equation}
% \begin{split}
%     f_1(\w_i)&=E[\W_S (\hat{H}(A_S)-\tnhat)\mid\w_i]= (\w_i-1)(\hi-\tnhat)=(\w_i-1)\gi;\notag\\
%     f_2(\w_i,\w_j)&=E[\W_S (\hat{H}(A_S)-\tnhat)\mid\w_i,\w_j] \notag\\
%     &=(\w_i\w_j-\w_i-\w_j+1)(\hhij-\tnhat)\notag\\
%     &=(\w_i\w_j-1)(\hhij-\tnhat)-(\w_i-1)(\hi-\tnhat)-(\w_j-1)(\hj-\tnhat),\label{eq:wb-hp}
% \end{split}
% \end{equation}

% \rd The residual $R_n$ is essentially a sum of higher order Hoeffding projections, which are all uncorrelated. Therefore, we see that the variance of the third order term (the first one in the remainder) is $\dfrac{\sum_{ijk}  \hat{g}_3(i,j,k)^2}{\hat{\sigma}_n^2 {n\choose 3}} \times O(1/n^3)$. Note that  $\hat{g}_3(i,j,k)^2=O_P(\rho_n^{3s-3})$ for cyclic and $O_P(\rho_n^{3s-2})$ for acyclic subgraphs. This is because, for any two nonoverlapping $S,T$ (not containing $\{i,j,k\}$)  of size $r-3$, there are potentially three edges common between the subgraphs induced by $S\cup \{i,j,k\}$ and  $S\cup \{i,j,k\}$ for a cyclic subgraph, and two for an acyclic one.
% Thus we can show that the remainder is the same order as $O(\mathcal{M}(n,\rho_n,R))$.


%\subsection{Edgeworth Expansion for Unweighted Boostrap}
% \section{\large{Edgeworth Expansion for Standardized Count Statistic}}
% In a size $n$ graph $\mathcal{G}_n$, define $\tnhat$ as normalized count statistic for a $r$-node $d$-edge subgraph $R$ with vertex set $V(R) $ and edge set $E(R)$.  For any set of $r$ nodes $S=\{X_{i_1},,,X_{i_r}\}$, denote
% \begin{equation*}
%     H(A_S)=  \prod_{(i_i,i_j)\in E(R)} A_{i_ii_j} ,
% \end{equation*}
% \begin{equation*}
%     h(X_{i_1},...,X_{i_r})=  \prod_{(i_i,i_j)\in E(R)} E(A_{i_ii_j}) =\prod_{(i_i,i_j)\in E(R)} \rho_n  w(X_{i_i},X_{i_j}) \wedge 1.
% \end{equation*}
% Then, $\tnhat$ can be written as 
% %Let $Iso(R)$ denote the class of graphs isomorphic to $R$, and $\mid Iso(R)\mid$ its cardinality. Then,
% %\begin{equation*}
% %\tnhat=\rho_n^{-d} \frac{1}{{n \choose p} \ |\mathrm{Iso}(R)| } \sum_{S \sim R} \mathbbm{1}(S = G_n[S])
% %\end{equation*}
% %Equivalently, we can also write $\tnhat$ as 

% \begin{equation*}
%     \tnhat= \frac{1}{{n \choose r}}\sum_{1\leq i_1<...<i_r\leq n} H(X_{i_1},,,X_{i_r}).
% \end{equation*}


% Let $T_n= E[\tnhat|\mathbf{X}]$ and $\theta=E[T_n]$. $T_n$ is a noiseless U-statistic with kernel function $h$. 
% \begin{equation*}
%      T_n= \frac{1}{{n \choose r}}\sum_{1\leq i_1<...<i_r\leq n} h(X_{i_1},,,X_{i_r}).
% \end{equation*}

% Define 
% \begin{equation*}
%     \begin{split}
%         & h_1(X_1)= E[h(X_1,X_2,,,X_r)\midX_1=x_1];\\
%         & h_2(X_1,X_2)= E[h(X_1,X_2,,,X_r)\midX_1=x_1,X_2=x_2].
%     \end{split}
% \end{equation*}
% Applying Hoeffding's decompsition of U-statistic \citep{hoeffding1992class} to $T_n$ yields 
% \begin{equation*}
%     T_n -\theta = \frac{r}{n}\sum_{i=1}^ng_1(X_i)+ \frac{r(r-1)}{n(n-1)}\sum_{1\leq i <j \leq n}g_2(X_i,X_j) + O_P(\rho_n^{d}n^{-1}),
% \end{equation*}
% where 
% \begin{equation}\label{eq:g1g2}
% \begin{split}
%     &g_1(X_i)= h_1(X_i)-\theta , \\
%     &g_2(X_i,X_j)= h_2(X_i,X_j) - \theta -g_1(X_1)-g_2(X_2) .
% \end{split}
% \end{equation}

% In addition, we define 
% \begin{align*}
%     \tau^2= \var(g_1(\mathbf{X})), \ \ \
%      \tilde{\tau_n} ^2= \frac{r^2}{n}\tau^2, \ \ \
%      \sigma_n^2 = \var(\tnt) .
% \end{align*}

% % U-stats hf decomp
% \rd I am removing $\tnhat$ because we don't use it in main paper and I think the shorthand may be a bit confusing  \bk


% % standardized form of $\tnhat$, denoting as $\tnt$,
% % \begin{equation*}
% %     \tnt = \frac{\tnhat - \mu_n}{\sigma_n}.
% % \end{equation*}
% \begin{theorem}\label{thm:ew-sd}
% % Edgeworth Expansion for $\tnt$. 

% Define \\
% \begin{equation*}
%     G_n(u)= \Phi(u)- \phi(u)\frac{(u^2-1)}{6n^{1/2}\tau^3}\{E[g_1^3(X_1)]+3(r-1)E[g_1(X_1)g_1(X_2)g_2(X_1,X_2)]\},
% \end{equation*}
% where $\Phi(u)$ and $\phi(x)$ denotes the CDF and PDF of standard Gaussian distribution. \rd For $\rho_n = O_P ((\log n)^{-1})$, and $\rho= \omega(n^{-1/2})$ for acyclic R and $\rho= \omega(n^{-1/r})$ for cyclic R.
% \bk  we have,
% \begin{equation*}
%     \sup_u  \bigg{|} F_{\tnt}(u)-G_n(u) \bigg{|} = O(\mathcal{M}(n,\rho_n,R)).
% \end{equation*}
% \end{theorem}

Consider any term $\tilde{g}_u(1,\dots,u)$. We will now bound $\E\{\tilde{g}_u(1,\dots,u)^2\}$.
\begin{align*}
    \E\{\tilde{g}_u(1,\dots,u)^2\}\leq 2[\var\{\hat{H}_u(1,\dots,u)\}+\underbrace{\var(\tnhat)}_{O(\rho_n^{2s}/n)}]
\end{align*}
The bound on the second term follows from~\cite{Bickel-Chen-Levina-method-of-moments} and will be smaller than that of the first term.
Let $\mathcal{S}_{r,u}$ denote all subsets of size $r-u$, not containing $1,\dots u$. For any subset $S\in \mathcal{S}_{r,u}$, also define, $S_u=S\cup \{1,\dots,u\}$.
For the first part, we have:
\begin{align*}
    \var\{\hat{H}_u(1,\dots,u)\}=\frac{\sum_{S,T\in \mathcal{S}_{r,u}}\cov\{H(A_{S_u}),H(A_{T_u})\}}{{n-u\choose r-u}^2}
\end{align*}
Note that the dominating term here will indeed be the one where $|S\cap T| =0$. The number of such terms is ${n\choose 2r-u}$. Also the covariance of those terms will be $\rho_n^{2s-E(A_{1,\dots,u})}$, where $E(A_{1,\dots,u})$ denotes the intersection of the edgeset of $A_{1,\dots,u}$ and the subgraph we are counting. This number can be at most $u-1$ for acyclic $R$ and $u$ for a simple cycle $R$. For $|S\cap T|=k$, the number of terms is ${n\choose 2r-2u-k}$ and the exponent on $\rho_n$ is at most $2s-(u+k-1)$. Thus, for an acyclic subgraph, we have,
\begin{align*}
    \var\{\hat{H}_u(1,\dots,u)\}&\leq \frac{\sum_{k=0}^r {n\choose 2r-2u-k}\rho_n^{2s-(u+k-1)}}{{n-u\choose r-u}^2}\\
    &\leq \sum_{k=0}^r n^{-k}\rho_n^{2s-(u+k-1)}=\rho_n^{2s-(u-1)}\left(1+\sum_{k>0}\frac{1}{(n\rho_n)^k}\right)
\end{align*}
The cyclic one is worse by a factor of $\rho_n$.
Thus the contribution of the $u^{th}$ element of the Hoeffding decomposition is 
\begin{align*}
    n\cdot \frac{\sum_{i_1,\dots, i_u} \tilde{g}_u(i_1,\dots,i_u)^2}{{n\choose u}^2 \hat{\tau}_n^2}&=\begin{cases}O_P\left(\frac{1}{(n\rho_n)^{u-1}}\right)&\mbox{$R$ acyclic}\\
    O_P\left(\frac{\rho_n^{-1}}{(n\rho_n)^{u-1}}\right)&\mbox{$R$ a simple cycle}\end{cases}
\end{align*}

This shows that the third term contributes the most to $R_n$ in Eq~\ref{eq:hofftnm}.  By Markov's inequality, and the definition of $O_P(.)$ notation, it is easy to see that $R_n=O_P(\delta(n,\rho_n,R))$. 
% \end{proof}



\section{Proof of Theorems~\ref{thm:clt-approx} and~\ref{thm:boot-linear-apx}}\label{sec:sup:proof-be}
%\rd Note: Moving CLT before bootstrap
%\bk
To establish the central limit theorem, we will need the following intermediary result, which establishes  that the conditional variance concentrates around its expectation.  In what follows, let:
\begin{align}\label{eq:def-sigmatildeAX}
\tilde{\sigma}^2_{|A,X}:= \mathrm{Var}(\tilde{T}_n - \hat{T}_n \ | \ A, X), \ \ \ \tilde{\sigma}_n^2 := E(\tilde{\sigma}^2_{|A,X})
\end{align}

\begin{theorem}\label{thm:clt-var-conc}
% \rd Define $\tilde{\sigma}_{|A,X}^2$ and $\tilde{\sigma}^2$. \bk
Suppose that $\rho_n \rightarrow 0$, $n \rho_n \rightarrow \infty$, $R$ is acyclic or a simple cycle, and $r \geq 2$.  Then the following holds:
\begin{align*}
\frac{\tilde{\sigma}_{|A,X}^2}{\tilde{\sigma}_n^2} \xrightarrow{P} 1    
\end{align*}
\end{theorem}
\begin{proof}
By Chebychev's inequality, it suffices to show that $\var(\tilde{\sigma}_{|A,X}^2)/\tilde{\sigma}_n^4 \rightarrow 0$.  We start by lower bounding the expectation $\tilde{\sigma}_n^2$.  Observe that:  
%
\begin{align}
\begin{split}
E(\var( \tilde{H}_1(i) - H_1(i) \ | \ A,X)) &=  \frac{1}{N} \left\{ \frac{1}{(n-1)!}\sum_{\pi} E(H_\pi - \theta_i)^2 - E(H_1(i) - \theta_i)^2 \right\} 
\\ &= \frac{1}{N}\{ E( \var( H_\pi) \ | \ X_i) - E( \var( H_1(i) \ | \ X_i))\}
\\ &= \Theta\left( \frac{\rho_n^s}{Nn} \right) - O\left(\frac{\rho_n^{2s}}{Nn}\right)
\end{split}
\end{align}

Therefore,
\begin{align*}
E\{\var(\tilde{T}_n - \hat{T}_n \ | \ A,X)\} = \frac{1}{n^2} \sum_{i=1}^n E\{\var(\tilde{H}_1(i) - H_1(i) \ | \ A,X )\} = \Theta\left( \frac{\rho_n^s}{Nn^2} \right)
\end{align*}

Now, we analyze $\var(\tilde{\sigma}_{|A,X}^2)$. Let $\theta_n^{(i)} = \mathbb{E}[H_\pi(i) \ | \ X_i]$. We have that:
\begin{align*}
\tilde{\sigma}^2_{|A,X} &= \frac{1}{n^2 N} \sum_{i=1}^n \frac{1}{(n-1)!} \sum_{\pi} \{ H_\pi(i) - H_1(i)\}^2   
\\ &= \underbrace{\frac{1}{n^2 N} \sum_{i=1}^n \frac{1}{(n-1)!} \sum_{\pi} \{ H_\pi(i) - \cei \}^2}_{P_1} - \underbrace{\frac{1}{n^2 N} \sum_{i=1}^n \{ H_1(i)- \cei) \}^2}_{P_2} %
% \\ &= \underbrace{\frac{1}{n^2 N} \sum_{i=1}^n \frac{1}{(n-1)!} \sum_{\pi} H_\pi(i) ^2}_{P_1} - \underbrace{\frac{1}{n^2 N} \sum_{i=1}^n H_1(i) ^2}_{P_2}
\end{align*}
% 
% To show that $\tilde{\sigma}_{|A,X}/\tilde{\sigma} \xrightarrow{P} 1$, by Chebychev's inequality, it suffices to show that 
% $\var{(P_1)},\var{(P_2)} = o( \tilde{\sigma}^4)$.
% 
For $P_1$, we further expand the sum into two parts, consisting of squared terms and cross terms:
\begin{align*}
% P_1 =& \underbrace{\frac{(r-1)^2}{n^2(n-1)^2N} \sum_{i=1}^n \frac{1}{(n-1)!}\sum_\pi \sum_{S \in \mathbb{S}_\pi} H(A_{S \cup i})^2}_{P_{1,1}} \\ + \ & \ \underbrace{\frac{(r-1)^2}{n^2(n-1)^2N} \sum_{i=1}^n \frac{1}{(n-1)!} \sum_\pi \sum_{S \not= T, S,T \in \mathbb{S}_\pi}  H(A_{S \cup i}) H(A_{T \cup i})}_{P_{1,2}}
P_1 =& \underbrace{\frac{(r-1)^2}{n^2(n-1)^2N} \sum_{i=1}^n \frac{1}{(n-1)!}\sum_\pi \sum_{S \in \mathbb{S}_\pi} \{H(A_{S \cup i}) - \theta_n^{(i)}\}^2}_{P_{1,1}} \\ + \ & \ \underbrace{\frac{(r-1)^2}{n^2(n-1)^2N} \sum_{i=1}^n \frac{1}{(n-1)!} \sum_\pi \sum_{S \not= T, S,T \in \mathbb{S}_\pi} \{ H(A_{S \cup i}) - \cei\} \cdot \{ H(A_{T \cup i}) - \cei\}}_{P_{1,2}}
\end{align*}






% We will start by bounding $E(\var(H_\pi - \theta_i)^2 \ | \ X_i)$.  Expanding the square, we have that:

% \begin{align*}
% E((H_\pi(i) - \theta_n^{(i)})^2 \ | \ X_i) &= \frac{(r-1)^2}{(n-1)^2} \sum_{S,T \in \mathbb{S}_\pi}  E\left[\{H(A_{S \cup i}) -\theta_n^{(i)}\} \cdot \{ H(A_{T \cup i}) -\theta_n^{(i)} \} \ | \ X_i \right]  
% \\ &= \frac{(r-1)}{(n-1)} \var( H(A_{S \cup i}) \ | \ X_i) \leq \rho_n
% \end{align*}
For $P_{1,1}$, observe that $H(A_{S \cup i})^2 = H(A_{S \cup i})$. Distributing the square and re-writing each term as (weighted) U-statistics, we have that, for some constants $c_1,c_2,c_3$ depending only on $r$, 
\begin{align*}
P_{1,1} = \frac{1}{n^3 N} \left[ \frac{c_1}{{n \choose r}} \sum_{|S| = r} H(A_S) -  \frac{2c_2}{{n \choose r}} \sum_{|S|=r} \left(\frac{1}{r}\sum_{i \in S} \theta_n^{(i)}\right) H(A_S) + \frac{c_3}{n} \sum_{i=1}^n (\theta_n^{(i)})^2  \right]
\end{align*}

It can readily be seen that first summand dominates; therefore, $\var(P_{1,1}) = O( \rho_n^{2s}/n^7N^2  )$.

We proceed to bounding $\var(P_{1,2})$.  For a given node i, observe that each subset $S \cup T$ appears in $O(n^2 (n-1-2(r-1))!=O(n^2 (n-2r+1)!$ %$O(n^2 \times (n-2r-3)!)$ 
permutations.  We may now define a new kernel corresponding with $2r-1$ nodes on the entire graph; thus, for some $c$ depending only on $r$,
\begin{align*}
P_{1,2} =   \frac{c}{Nn{n \choose 2r-1}}\sum_{|K| = 2r-1  } \frac{1}{2r-1}\sum_{S \cup T = K, i \in S \cap T }[H(A_S) - \theta_n^{(i)}] \cdot [H(A_T) -\theta_n^{(i)}]    
\end{align*}
Using Lemma~\ref{lem:p12} we see that
\begin{align*}
\var(P_{1,2})=O\left( \frac{\rho_n^{4s}}{N^2n^4} \right)+O\left( \frac{\rho_n^{4s-2}}{N^2n^5} \right) + O\left( \frac{\rho_n^{2s}}{N^2n^{2r+1}} \right)
\end{align*}
%Since $S$ and $T$ only share a node, we have that $\var(P_{1,2}) = O( \rho_n^{4s}/n^6N^2)$



% \begin{align*}
    
% \end{align*}

% Observe that:
% \begin{align*}
% & \ E \biggl[ \frac{1}{(n-1)!} \sum_\pi \underbrace{\frac{(r-1)^2}{(n-1)^2}\sum_{S \not= T, S,T \in \mathbb{S}_\pi} \{ H(A_{S \cup i}) - \cei \} \cdot \{ H(A_{T \cup i}) - \cei \}}_{P_{1,2,i,\pi}} \ | \ X_i \biggr] \\ 
% & =   \frac{(r-1)^2}{(n-1)^2} \sum_{S,T \in \mathbb{S}_\pi}  E\left[\{H(A_{S \cup i}) -\cei \} \ | \ X_i \right] \cdot E\left[\{ H(A_{T \cup i}) - \cei \} \ | \ X_i \right]  = 0
% \end{align*}

% For $E\{\var(P_{1,2,i,\pi} \ | \ X_i)\}$, observe that there are $O(n^2)$ variance terms upper bounded by $ C\rho_n^{2s}/n^4$ for some $C >0$.  Observe that the that the terms are uncorrelated since two products can share at most on subset and even in this case:
% \begin{align*}
% & \cov( \{ H(A_{S \cup i}) - \cei \} \cdot \{ H(A_{T \cup i}) - \cei \}, \{ H(A_{S \cup i}) - \cei\} \cdot \{ H(A_{R \cup i}) -  \cei \}     \ | \ X_i)
% \\ = & E[ E[\{ H(A_{S \cup i}) - \cei\}^2 \ | \ X_i] \cdot E[\{ H(A_{T \cup i}) - \cei\} \ | \ X_i] \cdot E[\{ H(A_{R \cup i}) - \theta_n^{(i)}\} \ | \ X_i] \ ]
% \\  & -  (E[ E[\{ H(A_{S \cup i}) - \cei \} \  | \ X_i] \cdot E[\{ H(A_{T \cup i}) - \cei\} \  | \ X_i]]^2 = 0
% \end{align*}

% the conditional covariance is zero if the terms do not share a subset. Therefore, there are $O(n^3)$ covariance terms, with covariance upper bounded by $C \rho_n^{2s}/n^4$.  Therefore, $\var(P_{1,2,i,\pi}) = O(\rho_n^{2s}/n)$.
% Now, observe that the variance of an average is upper bounded by the maximum variance.  Therefore, $\var(P_{1,2}) = O(\rho_n^{2s}/(n^4 N^2))$.    

% Since $E(H_\pi - \theta_i \ | X_i) = 0$, we have that $\var( H_\pi - \theta_i ) = \var(H_\pi - \theta_i \ | \ X_i)$.  

% Now expanding the square, $P_{1,1}$ may be written as:
% \begin{align*}
% P_{1,1} &= \frac{(r-1)}{n^2(n-1)N} \left( \hat{T}_n - \frac{2}{{n \choose r} } \sum_{1 \leq i_1 < \ldots < i_r \leq n}  \frac{\{\theta^{(i_1)} + \ldots + \theta^{(i_r)}\}}{r}  H(A_{i_1, \ldots, i_r}^{(n)}) + \frac{1}{n} \sum_{i=1}^n (\theta_n^{(i)})^2 \right)
% \\ &= P_{1,1,1} + P_{1,1,2} + P_{1,1,3}, \text{ say}.  
% \end{align*}
% We can immediately deduce that $\var(P_{1,1,1}) = O( \rho_n^{2s}/n^7N^2)$ and $\var(P_{1,1,3}) = O( \rho_n^{4s}/n^7N^2)$.  For the middle term, consider the decomposition:

% \begin{align*}
% \ & \  \frac{1}{{n \choose r} } \sum_{1 \leq i_1 < \ldots < i_r \leq n}  \frac{\{\theta^{(i_1)} + \ldots + \theta^{(i_r)}\}}{r}  H(A_{i_1, \ldots, i_r}^{(n)}) - E\left[\frac{\{\theta^{(i_1)} + \ldots + \theta^{(i_r)}\}}{r} H(X_{i_1}, \ldots X_{i_r}) \right] \\ 
% = & \ 
% \frac{1}{{n \choose r} } \sum_{1 \leq i_1 < \ldots < i_r \leq n}  \frac{\{\theta^{(i_1)} + \ldots + \theta^{(i_r)}\}}{r}  [H(A_{i_1, \ldots, i_r}^{(n)}) - h(X_1, \ldots X_r)] 
% \\ \ & + \frac{1}{{n \choose r} } \sum_{1 \leq i_1 < \ldots < i_r \leq n} \frac{\{\theta^{(i_1)} + \ldots + \theta^{(i_r)}\}}{r} h(X_1, \ldots X_r) - E\left[\frac{\{\theta^{(i_1)} + \ldots + \theta^{(i_r)}\}}{r} h(X_1, \ldots X_r) \right]
% \end{align*}
% The variance of the second term is $O(\rho_n^{4s}/n)$ since it is a U-statistic.  For the variance of the first term, we may condition on $X_1, \ldots X_n$ and use analogous arguments Theorem 1 of \citet{Bickel-Chen-Levina-method-of-moments} to conclude that this term is $o(\rho_n^{4s}/n)$.

For $P_2$, we again expand the square and consider squared and cross terms:
\begin{align*}
P_2 =& \underbrace{\frac{1}{n^2N}\sum_{i=1}^n \frac{1}{{n-1 \choose r-1}^2}\sum_{S \in \mathbb{S}\{-i\}} \{H(A_{S \cup i}) -\cei\}^2}_{P_{2,1}}   \\ + & \underbrace{\frac{1}{n^2N} \sum_{i=1}^n \frac{1}{{n-1 \choose r-1}^2}\sum_{S \neq T, S,T \in \mathbb{S}\{-i\}} \{H(A_{S \cup i}) -\cei\} \cdot \{ H(A_{T \cup i}) - \cei \} }_{P_{2,2}}
% P_2 =& \underbrace{\frac{1}{n^2N}\sum_{i=1}^n \frac{1}{{n-1 \choose r-1}^2}\sum_{S \in \mathbb{S}\{-i\}} \{H(A_{S \cup i}) - \cei\}^2}_{P_{2,1}}   \\ + & \frac{1}{n^2N} \sum_{i=1}^n \underbrace{\frac{1}{{n-1 \choose r-1}^2}\sum_{S \neq T, S,Y \in \mathbb{S}\{-i\}} \{H(A_{S \cup i}) - \theta_n^{(i)}\} \cdot \{H(A_{T \cup i}) - \cei \}}_{P_{2,2,i}} 
\end{align*}
For $P_{2,1}$, we immediately have that, for $c_1,c_2,c_3$ depending only on $r$,
\begin{align*}
P_{2,1} = \frac{1}{ N n^r}  \left[\frac{c_1}{{n \choose r}} \sum_{|S| = r} H(A_S) - \frac{2c_2}{{n \choose r}} \sum_{|S|=r} \left(\frac{1}{r}\sum_{i \in S} \theta_n^{(i)}\right) H(A_S) + \frac{c_3}{n} \sum_{i=1}^n (\theta_n^{(i)})^2\right]   
\end{align*}
    Therefore, $\var(P_{2,1}) = O(\rho_n^{2s}/n^{2r+1}N^2)$.  

Finally using Lemma~\ref{lem:p12},
\begin{align*}
    \var(P_{2,2})=O\bb{\frac{1}{N^2}\bb{\frac{\rho_n^{2s}}{n^7}+\frac{\rho_n^{2s}}{n^{2r+1}}+\frac{\rho_n^{4s}}{n^4}+\frac{\rho_n^{4s-2}}{n^5}}}
\end{align*}
Now, putting everything together, we see that $\var( \tilde{\sigma}_{|A,X}^2) = o\left( \frac{\rho_n^{2s}}{N^2n^4} \right)$ and thus the result follows.
\end{proof}

Below, we state and prove lemmas that establish the order of the cross-terms that may be written as noisy U-statistics. Let:
\begin{align*}
\hat{U}_n^{(k)} = \frac{1}{n^k} \frac{1}{{n \choose 2r-k} }\sum_{K :|K| = 2r-k } \ \sum_{ \substack{S,T : \ S \cup T = K, \\|S| = r,\ |T| = r }} \ \sum_{i \in S \cap T} \{H(A_S) - \cei\} \cdot \{(H(A_T) - \cei \}  
\end{align*}
We have the following lemma:
\begin{lemma}
\label{lem:p12}
Suppose that $n \rho_n \rightarrow \infty$ and $S$ is acyclic or a simple cycle with $r \geq 2$. Then, for any $k \in \{1, \ldots, r-1 \}$,
\begin{align*}
\var(U_n^{(k)}) = O\left( \frac{\rho_n^{4s}}{n^4} \right)+O\left( \frac{\rho_n^{4s-2}}{n^5} \right) +  O\left( \frac{\rho_n^{2s}}{n^{2r+1}} \right)
\end{align*}

\end{lemma}

\begin{proof}
We again argue by law of iterated variance.  Observe that the conditional expectation given $X_1, \ldots, X_n$ is a (noiseless) U-statistic, with kernel of the order $\rho_n^{4s-2k+2}$.  Therefore, for $k>1$,
\begin{align*}
\var\{E(U_{n}^{(k)} | X_1, \ldots X_n) \} &= O\left(\frac{\rho_n^{4s-2k+2}}{n^{2k+1}} \right)
\\ &= O\left(\frac{\rho_n^{4s-2} }{n^5} \right)
\end{align*}
For $k=1$, we use the fact that the corresponding kernel is degenerate of order 1.  To see this, first note that the expectation is 0 since:
\begin{align*}
E[ E[\{H(A_S) - \cei \} \ | \ X_i] \cdot E[\{H(A_T) - \cei \} \ | \ X_i] = 0   
\end{align*}
 Moreover, for any $j \in K$, the conditional expectation is 0. Without loss of generality, suppose $j \in S$ and $j \neq i$; the $i=j$ calculation is analogous to the expectation one above.  Then,
 \begin{align*}
  & E[\{H(A_S) - \cei\} \cdot \{(H(A_T) - \cei \} \ | \ X_j] 
 \\ = & \  E[E[\{H(A_S) - \cei\} \cdot \{H(A_T) - \cei \} \ | \ X_i,X_j] \ | \ X_i] 
 \\ = & \  E[E[\{H(A_S) - \cei\} \ | \ X_i,X_j] \cdot E[\{H(A_T) - \cei \} \ | \ X_i] \ | \ X_i] = 0   
 \end{align*}
 Therefore, the Hayek projection is 0, and the variance satisfies:
 \begin{align*}
\var\{E(U_{n}^{(1)} | X_1, \ldots X_n) \} = O\left(\frac{\rho_n^{4s}}{n^4} \right)
 \end{align*}
 %
 Now for the conditional expectation of the variance, we further split  the variance of a sum into variance and covariance components.  Observe that that the variance of the product $\{H(A_S) - \cei\} \cdot \{(H(A_T) - \cei \}$ conditional on $X_1, \ldots X_n$ is dominated by the variance of the term $H(A_S)H(A_T)$, which is Bernoulli(p) with $p = O( \rho_n^{2s-k+1})$.  Thus, for $k \geq 1$, the contribution of these terms is $O( \rho_n^{2s}/n^{r+1})$.  Now for the covariance, for all $k \geq 1$, by Lemma  \ref{lemma-cov-order}, the contribution of these terms is upper bounded by $O\left(\frac{\rho_n^{4s}}{n^4} \right) + O\left(\frac{\rho_n^{4s-2}}{n^5} \right)$.  The result follows.

 \end{proof}
 
 Now we state and prove a result on the order of the conditional covariance terms, which was used in the previous lemma.   
 \begin{lemma}
 \label{lemma-cov-order}
Suppose that $n \rho_n \rightarrow \infty$ and $S$ is acyclic or a simple cycle with $r \geq 2$. Then, for any $k \in \{1, \ldots, r-1 \}$, \bk
 \begin{align*}
   & \frac{1}{n^{4r}}\sum_{i,j}\sum_{\substack{S\neq T, S,T\in \mathbb{S}\{-i\}\\S'\neq T', S',T'\in \mathbb{S}\{-j\}}} E\bb{(H(A_{S\cup i})-\cei)(H(A_{T\cup i})-\cei)(H(A_{S'\cup j})-\theta^{(j)})(H(A_{T'\cup j})-\theta^{(j)})}
 \\ & = O\left(\frac{\rho_n^{4s}}{n^4} \right) + O\left(\frac{\rho_n^{4s-2}}{n^5} \right)  
\end{align*}
 \end{lemma}
 \begin{proof}
%  For computing the expectation of the conditional variance, we upper bound as follows: %$E\var (P_{2,2}|X)$
% %upper bounded by:
% \begin{align*}
%     \frac{1}{n^{4r}}\sum_{i,j}\sum_{\substack{S\neq T, S,T\in \mathbb{S}\{-i\}\\S'\neq T', S',T'\in \mathbb{S}\{-j\}}} E\bb{(H(A_{S\cup i})-\cei)(H(A_{T\cup i})-\cei)(H(A_{S'\cup j})-\theta^{(j)})(H(A_{T'\cup j})-\theta^{(j)})}
% \end{align*}


%Another term which has $S\cap T=S'\cap T'$, contributes $n^{4r-3k}\rho_n^{4s-k+1}$ leading to $\rho_n^{4s+1}/(n\rho_n)^kn^{2k}$.
%We will consider two different strategies for $k=1$ and $k >1$; for the former, we use degeneracy of the corresponding U-statistic kernel to get a sharper bound.

% For $k >1$, we further break up $P_{2,2}$ as follows:
% \begin{align*}
%   \sum_{k>1} \frac{U_k}{Nn^k} &= \sum_{k>1}  \frac{1}{Nn^k {n \choose 2r-k }} \sum_{|K| = 2r-k} \frac{1}{2r-k} \sum_{S \cup T= K} H(A_S)H(A_T)  
%  \\ & \ \ + \sum_{k>1}  \frac{1}{Nn^k {n \choose 2r-k }} \sum_{|K| = 2r-k} \frac{1}{2r-k} \sum_{S \cup T= K}   \left\{ \sum_{ i \in S \cap T} \cei \right\} \cdot H(A_S)
%   \\ & \ \ + \sum_{k>1}  \frac{1}{Nn^k {n \choose 2r-k }} \sum_{|K| = 2r-k} \frac{1}{2r-k} \sum_{S \cup T= K}   \left\{ \sum_{ i \in S \cap T} \cei \right\} \cdot H(A_T)
%   \\ & \ \ + \sum_{k>1}  \frac{1}{Nn^k} \frac{1}{n}\sum_{i=1}^n (\cei)^2 = P_{2,2,1}+ P_{2,2,2} + P_{2,2,3} + P_{2,2,4}, \text{ say.} 
%   \end{align*}
%  Now for $P_{2,2,1}$, we use law of iterated variance.  For the variance of the conditional expectation given $X$, observe that the resulting expectation is a U-statistic; therefore the contribution of the the $k$th term to the variance is $O(\rho_n^{4s-2k}/N^2n^{2k+1})$, which is upper bounded by $O(\rho_n^{2s+4}/N^2n^5)$.  
 
%  Now, for the expectation of the variance conditional on $X$, we consider the contribution of conditional variance and covariance terms for some fixed $k >1$.  For the contribution of the covariance terms, suppose that $|S \cap T| = k$, $|S' \cap T'| = k$, and that $(S \cup T) \cap (S' \cup T') =q$ for $q \geq 2$.  There are $O(n^{4r-2k-q})$ such terms, with conditional covariance upper bounded by $C\rho_n^{4s-2k-q}$ for some $C>0$; therefore the conditional covariance is $O(  \rho_n^{4s-2k}/(N^2n^{2k}(n\rho_n)^q)$, which is further upper bounded by $O(\rho_n^{2s+4}/(N^2 n^4))$. 
%  $|(S \cup T) \cap (S' \cup T')|=q$ for some $q \geq 2$, which implies that the subgraphs corresponding to $S \cup T$ and $S' \cup T'$ share at most $q$ edges. 
%  Observe that there at most $O(n^{4r-2k-q_1-q_2+d})$ such vertex sets, with covariance conditional on $X$ is upper bounded by $\rho_n^{4s-2k -q_1 -q_2 + }$; therefore, the covariance is $O( \rho_n^{4s-2k}/(N^2 n^{2k}(n\rho_n)^{2q}))$, which is further upper bounded by $O( \rho_n^{2s+2}/ N^2 n^4)$. 
 
% Purna's stab at the above para.
 
 Consider four subsets $S,T,S',T'$. There are 3 types of intersections. The first type are nodes \textit{only} in the intersection of a pair of subsets, and between six pairs. We will denote the size of  these intersections by $k_i,i\in[6]$. We will denote by $K$ the sum of $k_i's$. The second are nodes only in triple wise intersections with sizes $j_i,i\in[4]$. The total of these numbers is $J$. Finally there are nodes in the intersection between all four, whose size will be denoted by $J$. Note that for any given configuration of the sets (translating to a configuration of these numbers), there are a total of $n^{4r-(K+2L+3J)}$ nodes. This is because every node in the pairwise intersection gets counted twice. Those in three-way intersections get counted thrice and those in the four-way intersection get counted thrice. Finally note that there are a total of $K+L+J$ nodes such that each node belongs to some intersection (call this $I$). In order to find the number of edges, note that this intersection can be represented as four sets, which are $I\cap S,I\cap T$ etc. For each of these intersections, since we are allowing simple cycles or acyclic graphs,  note that we can have $|I\cup S|-1(|I\cup S|>0)$ edges. Thus the the total number of edges can be at most $|I|-1$ edges in the intersection. So the contribution of these numbers is
 $$\frac{n^{4r-(K+2L+3J)}\rho_n^{4s-(K+L+J-1)}}{n^{4r}}=\frac{\rho_n^{4s+1}}{(n\rho_n)^{K+L+J}n^{L+2J}}$$
 Now we consider some cases of configuration before summing over all $K,L,J$. We first note that all cases with $K\leq 3,L=0,J=0$ are zero. 
 For $K=4,L=0,J=0$, the only possible case that contributes to the covariance is the one with $k_i=1,i\leq 4$. This contributes $\rho_n^{4s}/n^{4}$. Similarly note that if we have $K=5$, the contribution comes from $k_1=1,k_2=1,k_3=1,k_4=2$ which has contribution $\rho_n^{4s-1}/n^5$ and so on. Thus the terms contribute $\sum_{i\geq 0}\rho_n^{4s-i}/n^{4+i}=O\bb{\rho_n^{4s}/n^4}$. 
  We also consider the case where $K= 1,L= 2,J= 1$, this will contribute $\frac{\rho_n^{4s-1}}{n^5}$.
 Now we consider the case with $K= 2,L= 0,J= 1$. These terms will contribute $ \frac{\rho_n^{4s-2}}{n^5}$. In fact for $K=2,L\geq 1,J\geq 1$, we will have a contribution of
 \begin{align*}
     \frac{\rho_n^{4s+1}}{(n\rho_n)^4n^3}=\frac{\rho_n^{4s-2}}{(n\rho_n)n^6}
 \end{align*}
 
 Now we consider the terms of the form $K\geq 3,L\geq 0, J\geq 1$. These terms contribute:
 \begin{align*}
     \frac{\rho_n^{4s+1}}{(n\rho_n)^{4}n^{2}}=\frac{\rho_n^{4s-2}}{(n\rho_n)n^{5}}
 \end{align*}
 
Consider $C_{k,\ell,j}$ the covariance contribution for sets with $K=k,L=\ell,J=j$.  Putting everything together, we have:
 \begin{align*}
     \sum_{k,\ell,j\geq 0}C_{k,\ell,j}&=
     \sum_{k< 4, \ell=j=0}C_{k,\ell,j}+\sum_{k\geq 4, \ell=j=0}C_{k,\ell,j}+\sum_{k=1,\ell=2,j=0}C_{k,\ell,j}+\sum_{k=2, \ell=0,j= 1}C_{k,\ell,j}\\
     &\qquad +\sum_{k=2, \ell\geq 1,j\geq 1}C_{k,\ell,j}+\sum_{k\geq 3, \ell\geq 0,j\geq 1}C_{k,\ell,j}\\
     &=0+O\bb{\frac{\rho_n^{4s}}{n^4}}+ O\bb{\frac{\rho_n^{4s-1}}{n^5}}+ O\bb{\frac{\rho_n^{4s-2}}{n^5}}.
 \end{align*}
 \end{proof}
 Now, we establish a CLT for the approximate count functional.  Our overall strategy is follows \citet{chen2019randomized}.  Recall from Equation~\ref{eq:def-sigmatildeAX} that $\noisesdax^2 = \var(\tilde{T}_n - \hat{T}_n \ | \ A,X)$ and $\noisesd^2 = E(\noisesdax^2)$.%, and $\nu_n^2 = \noisesd^2 + \sigma_n^2$.    
 \begin{theorem}
 Suppose that $\rho_n \rightarrow 0$ and either $R$ is acyclic and $n \rho_n \rightarrow \infty$ or $R$ is a simple cycle and $n^{r-1} \rho_n^r \rightarrow \infty$.  Moreover, suppose that $N \gg 1/n^2\rho_n^s$.  Then,
 \begin{align*}
 \sup_{t \in \mathcal{R}} \left| P\left( \frac{\tilde{T}_n - \theta_n}{ \sqrt{\noisesd^2 + \sigma_n^2}} \leq t  \right) - \Phi(t)    \right| \rightarrow 0
 \end{align*}
 
 \end{theorem}
 
\begin{proof}
 Let $Z \sim N(0,1)$ be independent of $A,X$ and $t' = \sqrt{\noisesd^2 + \sigma_n^2} \cdot t$.
%  In addition, let $\noisesdax^2 = \var(\tilde{T}_n - \hat{T}_n \ | \ A,X)$ and $\noisesd^2 = E(\noisesdax^2)$.   
 We may further reduce the problem to establishing central limit theorems for the randomization and signal components separately as follows:

% We start by conditioning on $A,X$ and establishing a Gaussian approximation for the noise.  Let $\noisesdax = \var(\tilde{T}_n - \hat{T}_n \ | \ A,X)$ and rearranging $\tilde{T}_n - \theta = \tilde{T}_n - \hat{T}_n + \hat{T}_n - \theta$ we have:
\begin{align*}
& \ \sup_{t \in \mathcal{R}} \left| P\left( \frac{\tilde{T}_n - \theta_n}{ \sqrt{\noisesd^2 + \sigma_n^2} } \leq t  \right) - \Phi(t)    \right|
\\ \leq & \  \sup_{t' \in \mathcal{R}} \left|P\left( \frac{\tilde{T}_n - \hat{T}_n}{\noisesdax } \leq \frac{t'-(\hat{T}_n - \theta_n)}{\noisesdax}  \right) -\Phi\left(\frac{t'-(\hat{T}_n - \theta_n)}{\noisesd} \right) \right| 
\\ + & \ \sup_{t' \in \mathcal{R}} \left| P\left(\frac{(\hat{T}_n - \theta_n) + \noisesd Z}{\sigma_n} \leq \frac{t^\prime}{\sigma_n} \right) - \Phi\left(\frac{t'}{\sqrt{\noisesd^2 + \sigma_n^2}} \right)   \right| = I +II 
\end{align*}
To show $I \rightarrow 0$, observe that:
\begin{align*}
I  \leq & \   E \left\{ \ \sup_{t' \in \mathcal{R}} \left|P\left( \frac{\tilde{T}_n - \hat{T}_n}{\noisesdax } \leq \frac{t'-(\hat{T}_n - \theta_n)}{\noisesdax} \ \biggr\rvert \  A,X  \right) -\Phi\left(\frac{t'-(\hat{T}_n - \theta_n)}{\noisesdax} \ \biggr\rvert \  A,X \right) \right| \ \right\}
 \\ + & E \left\{ \ \sup_{t' \in \mathcal{R}} \left| \Phi\left(\frac{t'-(\hat{T}_n - \theta_n)}{\noisesdax} \ \biggr\rvert \  A,X \right) - \Phi\left(\frac{t'-(\hat{T}_n - \theta_n)}{\noisesd} \ \biggr\rvert \  A,X \right)  \right| \ \right\} = I_a + I_b
\end{align*}

For $I_a$, the Berry-Esseen Theorem implies that if:
\begin{align}
\label{eq:conditional-berry-esseen-condition}
\frac{\frac{1}{n^3}\sum_{i=1}^n\E\left(|\tilde{H}_1(i) - H_1(i) |^3\ | \ A,X \right)}{\noisesdax^{3/2}} \xrightarrow{P} 0,
\end{align}
then:
\begin{align*}
\sup_{t' \in \mathcal{R}} \left|P\left( \frac{\tilde{T}_n - \hat{T}_n}{\noisesdax } \leq \frac{t'-(\hat{T}_n - \theta_n)}{\noisesdax} \ \biggr\rvert \ A, X  \right) -\Phi\left(\frac{t'-(\hat{T}_n - \theta_n)}{\noisesdax} \ \biggr\rvert \ A,X \right) \right| \xrightarrow{P} 0     
\end{align*}
By Theorem \ref{thm:clt-var-conc}, $\frac{\noisesdax^2}{\noisesd^2} \xrightarrow{P} 1$,
where $\noisesd^2 = \Theta\left( \frac{\rho_n^s}{Nn^2} \right)$.
%
Moreover, by Lemma \ref{lemma:third-moment-randomized}, we have that:
\begin{align*}
 \frac{1}{n^3}\sum_{i=1}^n\E\left(|\tilde{H}_1(i) - H_1(i) |^3\ | \ A,X \right)= O_P\left( \frac{\rho_n^s}{n^4N^2} \right) + O_P\left(\frac{\rho_n^{3s/2}}{N^{3/2}n^{7/2}} \right)   
\end{align*}
Therefore, under the condition $N \gg 1/n^2 \rho_n^s $, Eq \ref{eq:conditional-berry-esseen-condition} holds and thus the expectation in converges to zero since the Kolmogorov distance is bounded.  Furthermore, we have that:
%
\begin{align*}
\sup_{t' \in \mathcal{R}} \left|\Phi\left(\frac{t'-(\hat{T}_n - \theta_n)}{\noisesdax} \ \biggr\rvert \ A,X \right) - \Phi\left(\frac{t'-(\hat{T}_n - \theta_n)}{\noisesd} \ \biggr\rvert \ A,X \right)  \right| \xrightarrow{P} 0   
\end{align*}
Therefore by similar reasoning $I_b \rightarrow 0$.
Now for $II$, for some $Z'$ independent of $Z$, by Theorem 1 of \citet{Bickel-Chen-Levina-method-of-moments} and P{\'o}lya's theorem:
% Proposition~\ref{prop:ew} (proof in Section~\ref{sec:suppprop3}), 
\begin{align*}
II & \leq E \left\{\sup_{t' \in \mathcal{R}} \left| P\left(\frac{(\hat{T}_n - \theta_n)}{\sigma_n} \leq \frac{t^\prime - \noisesd Z}{\sigma_n} \ \biggr\rvert \ Z=z \right) - P\left(Z^\prime \leq \frac{t^\prime - \noisesd Z}{\sigma_n} \ \biggr\rvert \ Z=z \right) \right| \right\} \rightarrow 0
% \Phi\left(\{t-(\hat{T}_n - \theta)\}/\noisesd \right)  & = P\left( \noisesd Z + (T_n - \theta) \leq  t    \right)
% \\ &= E\left\{P\left( \frac{T_n - \theta}{\sigma_n} \leq \frac{t + \tilde{\sigma}_n Z}{\sigma_n} \ \biggr\rvert \ Z=z \right) \right\}
% \\ &= P( \tilde{\sigma}_n Z + \sigma_n Z^\prime \leq t) + o(1)
\end{align*}
To conclude the proof, observe that:
\begin{align*}
P\left(Z^\prime \leq \frac{t^\prime - \noisesd Z}{\sigma_n} \right)
= P(\sigma_n Z^\prime + \noisesd Z \leq t') = \Phi\left( \frac{t'}{\sqrt{\noisesd^2 +\sigma_n^2}}  \right)
\end{align*}
\end{proof}

% Moreover, for any $j \in K$, the conditional expectation satisfies:
% \begin{align*}
% E[\{H(A_S) - \cei\} \cdot \{(H(A_T) - \cei \} \ | \ X_j] = E[\{H(A_S) - \cei\} \cdot \{(H(A_T) - \cei \} \ | \ X_j]  
% \end{align*}
% , observe that the Hayek projection is 0 since $E[\{H(A_S) - \cei \} \cdot \{H(A_T) - \cei \}] = 0$ and moreover, for any $j \in K$,
% \begin{align*}
% E[\{H(A_S) - \cei\} \cdot \{(H(A_T) - \cei \} \ | \ X_j] 
% &= 
% \end{align*}
% \begin{align*}
    
% \end{align*}


% We use different strategies for $k=1$ and $k>1$.  For $k=1$, we exploit the fact that the corresponding noiseless U-statistic is degenerate and thus the variance is smaller order.    





% \begin{lemma}\label{lem:p12}
% If $n \rho_n \rightarrow \infty$ and $S$ is acyclic or a simple cycle with $r \geq 2$, we have:
% \begin{align*}
% \var(U_n^{(1)}) = O\left( \frac{\rho_n^{4s}}{n^4} \right)+O\left( \frac{\rho_n^{4s-2}}{n^5} \right) +  O\left( \frac{\rho_n^{2s}}{n^{2r+1}} \right)
% \end{align*}
% \end{lemma}
% \begin{proof}
% \begin{align*}
% \frac{1}{Nn{n \choose 2r-1}}\sum_{|K| = 2r-1, \  } \frac{1}{2r-1}\sum_{S \cup T = K, i \in S \cap T }[H(A_S) - \theta_n^{(i)}] \cdot [H(A_T) -\theta_n^{(i)}]
% \end{align*}

% Observe that the inner two sums may be written as:
% \begin{align*}
% & \ \sum_{S \cup T = K, i \in S \cap T }[H(A_S) - \theta_n^{(i)}] \cdot [H(A_T) -\theta_n^{(i)}] \\ =& \  \sum_{S \cup T = K }[H(A_S) - h(X_S)] \cdot [H(A_T) - h(X_T) ] + \sum_{S \cup T = K, i \in S \cap T }[H(A_S) - h(X_S)] \cdot [h(X_T) - \theta_n^{(i)} ] 
% \\  &+ \sum_{S \cup T = K, i \in S \cap T }[h(A_S) - \theta_n^{(i)}] \cdot [H(A_T) -h(X_T) ]  + \sum_{S \cup T = K, i \in S \cap T }[h(A_S) - \theta_n^{(i)}] \cdot [h(X_T) - \theta_n^{(i)}] 
% \\ =& \ V_{1,K} + V_{2,K} + V_{3,K} + V_{4,K}, \ \text{say}.  
% \end{align*}
% So that:
% \begin{align*}
% U_n^{(1)}&
% \frac{1}{Nn{n \choose 2r-1}}\sum_{|K| = 2r-1, \  } \frac{1}{2r-1}\sum_{S \cup T = K, i \in S \cap T }\{H(A_S) - \theta_n^{(i)}\} \cdot \{H(A_T) -\theta_n^{(i)}\} \\ 
% = \frac{1}{n{n \choose 2r-1}} \sum_{|K| = 2r-1} V_{1,K} + \frac{1}{n{n \choose 2r-1}} \sum_{|K| = 2r-1} V_{2,K} + \frac{1}{n{n \choose 2r-1}} \sum_{|K| = 2r-1} V_{3,K} + \frac{1}{n{n \choose 2r-1}} \sum_{|K| = 2r-1} V_{4,K}
% \\ &= V_1 + V_2 + V_3 + V_4, \text{ say}. 
% \end{align*}
%
% We start by bounding $\var(V_1)$.  Since $A_S$ and $A_T$ share no edges, we have that:
% \begin{align*}
% \var(V_{1,K})&\leq  E(\var(V_{1,K} |X_i)) =   E\{\var(H_S | X_i) \  \var(H_T | X_i)\} 
% \\ &= O( \rho_n^{2s})
% \end{align*}
% where above we used the fact that the variance of an average is upper bounded by the largest variance, which is simply the variance of any one of the terms since they are identically distributed.

% Therefore, the contribution of the variance terms of the form $\var(V_{1,K})$ to $\var(V_1)$ is $O(\rho_n^{2s}/n^{2r-1}n^2N^2)$
% Now for the contributions of the covariance terms to $V_{1}$,  it is immediately clear that the covariance is 0 if $(S,T)$ and $(S^\prime, T^\prime)$ are disjoint or share only a root node $i$.  

% When the pairs share 3 nodes and an edge, the covariance is 0.  To see this, without loss of generality, assume that $S$ and $S^\prime$ share two nodes and an edge and $T$ and $T^\prime$ only share the root $i$.  Then,
% 
% that share 3 nodes (including a common root i) and an edge is 0.  To see this, without loss of generality, assume that $S$ and $S^\prime$ share two nodes and an edge and $T$ and $T^\prime$ only share the root $i$.  Then,
% \begin{align*}
% &\cov([H( A_S) - h(A_S)] \cdot [H( A_T) - h(A_T)], [H( A_{S^\prime}) - h(A_{S^\prime})] \cdot [H( A_{T^\prime}) - h(A_{T^\prime})]) 
% \\ = & \  E\{E( [H( A_S) - h(A_S)] \cdot [H( A_{S^\prime}) - h(A_{S^\prime})] \ | \ X_1) \cdot  E([H( A_T) - h(A_T)] \cdot [H( A_{T^\prime}) - h(A_{T^\prime})] \ | \ X_1)\} = 0 
% \end{align*}
% Now, consider the case where $(S,T)$ and $(S^\prime, T^\prime)$ share $4$ nodes, but are centered at different vertices.  Without loss of generality, suppose $S, S^\prime$ share node $k$, $T, T^\prime$ share node $l$, $(S,T)$ share node $i$, and $(S^\prime, T^\prime)$ shared node $j$.   Again, the covariance is zero by law of iterated covariance on the conditioning set $X_i, X_j,X_k,X_l$.  The asymmetric case where $S$ and $S^\prime$ share 3 nodes and $T$ and $T^\prime$ share one node is analogous. 

% Thus, the dominant term is the case where $S$ and $S^\prime$ and $T$ and $T^\prime$ both share 2 nodes and an edge. There are $O(n^{4r-5})$ such terms, each with covariance upper bounded by $C\rho_n^{4s-2}$ for some $C >0$.  \bl Therefore, the contribution of such terms to the variance is $\rho_n^{4s-2}/N^2 n^4$. [Purna: is this not $\rho_n^{4s-2}/N^2 n^5$]\rd 

% We now bound $\var(V_2)$ and $\var(V_3)$.  By law of iterated variance,
% $\var(V_2) = E(\var(V_2 \ | X)$.  Observe that there are $O(n^{2r-1})$ variance terms of the order $\rho_n^{3s}$; therefore the total contribution is $O(\rho_n^{3s}/N^2 n^2 n^{2r-1})$. For the covariance terms, the leading term we have that $S$ and $S'$ and $T$ and $T'$ each share two vertices, with one also sharing an edge.  There are again $O(n^{4r-5})$ terms, where the conditional covariance is bounded by $C\rho_n^{2s-1}$ and the expectation component is $O(\rho_n^{2s-1})$.  Therefore, the total contribution of covariance terms is $O(\rho_n^{4s-2}/N^2n^5)$.  The variance for $V_3$ is analogous. 

% Finally for $V_4$, observe that the kernel is degenerate of order 1. Therefore, $\var(V_4) = O(\rho_n^{4s}/N^2n^4)$.  
% \end{proof}


% \begin{proof}\normalfont
\iffalse
For any $i \in \{1,\ldots,n\}$, denote the set of all subsets of size $r-1$ taken from  $\{1,\ldots,i-1,i+1,\ldots n\}$ as $\si$. %Denote $\{X_{i_{2}},\ldots ,X_{i_{r}} \}$ for $S=\{i_2,i_3 \ldots i_r\}  \in \mathbb{S}_{-i}$  as $X_s$.  
Denote  $H(A_{i,i_2, \ldots, i_r})$ for $S=\{i_2,\ldots, i_r\}  \in \mathbb{S}\{-i\}$ as $\hsxi$. 
Denote 
\begin{align*}
    %H_1(i)%= \frac{1}{{n-1 \choose r-1 }} \sum_{1 \leq i_2 < \ldots i_r \leq n, i_u \neq i } H(A_{i,i_2,i_3 \ldots i_r}) 
     &\hoi = \frac{1}{{n-1 \choose r-1 }} \sum_{S \in \mathbb{S}\{-i\}} \hsxi.%\\
   % & h_1(i)= \frac{1}{{n-1 \choose r-1 }} \sum_{s \in S\{-i\}} \shsxi.
\end{align*}
%we know 
%\rd
%\begin{align*}
%   & E\hoi= E(h_s(X)|X_i). \\
 %  & E(\hoi-\theta)^2=Var(h_s(X)\mid X_i).
%\end{align*}

Now let  $\pi_j$ be a permutation picked with replacement and uniformly at random from the set of all permutations of $\{1,\dots,n\}\setminus i$.  We have $j=1,\ldots,N$ independent permutations $\pi_j$. %$\xpi \sim Bernoulli(p)$, let $\pimi$ denote all the permutations of $\{1,\ldots,i-1,i+1,\ldots n\}$.
Let $\mathbb{S}_{\pi}$ denote the set of all disjoint subsets  $\{\pi_{(i-1)(r-1)+1},\dots, \pi_{i(r-1)}\}$, $i=1,\dots, \frac{n-1}{r-1}$ obtained from permutation $\pi$.  %We have $\sum_ {\pi \in \pimi} \xpi = \tilde{N}$ and $E\left(\sum_{\pi \in \pimi}\xpi\right)=N$.\bk  
We write
\begin{align*}
  \ttnl - \Tilde{T}_n = \frac{r}{n}\sum_{i=1}^n (\xi_i-1)\{\tdh(i)-\tdu\},
\end{align*}
where
\begin{align*}
%&\tdh(i)=\frac{\sum_{\pi \in \pimi}\xpi\hpi(i)}{\sum_{\pi \in \pimi}\xpi},\\
&  \tdh(i)=\frac{\sum_{j} H_{\pi_j}(i)}{N},\\
&\hpi(i)=\frac{\sum_{S\in\mathbb{S}_{\pi} }\hsxi}{\frac{n-1}{r-1}},\\
&\tdu=\frac{1}{n}\sum_{i=1}^n\tdh(i).
\end{align*}
\fi
%$\tdh(i)$ is an estimator for $\hoi$, with $\xpi \sim Bernoulli(p)$ and $\sum_ {\pi \in \pimi} \xpi = \hat{N}$ and $E\left(\sum_{\pi \in \pimi}\xpi\right)=N$.

%Given $A$ and $X$, $(\tdh(i)-\tdu)$ are observed constants,
%\begin{align*}
%  Q_n = \frac{r}{n}\sum_{i=1}^n (\xi_i-1)(\tdh(i)-\tdu).
%\end{align*}
% Note that
% \begin{align*}
% \var (\ttnl - \Tilde{T}_n|A,X)=\frac{r^2}{n^2}\sum_i \tilde{\sigma}_{n,i}^2
% \end{align*}

% \rd
% \begin{proposition}[The Old Theorem 2(a)]
%  If $Nn\rho_n^s\gg 1$, we have:%the standardized bootstrap distribution converges at the Berry-Esseen rate to a standard Normal:
% %\rd If $N\geq \max(1,\rho^{-s}k/n)$, then,
% \begin{align}\label{eq:BE-approx}
%   \sup_{u \in R} \bigg{|}P^*\bb{\frac{\ttnl-\tilde{T}_n}{\{\var(\ttnl \mid A,X)\}^{1/2}}\leq u} -\Phi(u)\bigg{|}=  O_P\left(n^{-1/2}\right),
 %  &\sup_{u \in R} \bigg{|}P^*\bb{\frac{\sqrt{n}(\ttnl-\tilde{T}_n)}{r\tau_n}\leq u|A,X} -P\bb{\frac{\sqrt{n}(\hat{T}_n-\theta_n)}{r\tau_n}\leq u}\bigg{|}\\&= 
  % O_P({n^{-1/2}}) + O_P\left(\frac{1}{n\rho_n}\right)+O_P\left(\frac{1}{Nn\rho_n^s} \right) + 
  %  O(\mathcal{M}(n,\rho_n,R))+O_P\left(\frac{1}{n^{1/2}\rho_n^{3s}}\right).
%O_P\left(n^{-1/2}+|\bootsd-r\tau_n|\right),
% \end{align}
% where $P^*(\cdot)$ denotes the conditional measure conditioned on $A$ and $X$

% \end{proposition}

\bk



% \textit{Proof of Theorem~\ref{thm: apprx-linear-bootstrap} (a):}

% Let $Y_i$ denote $(\xi_i-1)\{\tdh(i)-\tdu\}$. %$(\tdh(i)-\Tilde{U})$ is constant given $A$ and $X$. Thus, 
%  Conditioned on $A$ and $X$,  $\tdh(i)-\tdu$ are observed constants,  $Y_i$ are independent but not identically distributed with variance $\tdsigi^2$. \bk
% \begin{align*}
%   &\tdsigi^2= \var[(\xi_i-1)\{\tdh(i)-\tdu\}
%     \mid  A, X] =E[
%     \{\tdh(i)-\tdu\}^2\mid  A, X]
%   % & E\tdsigi^2=E[\{\tdh(i)-\tdu\}^2].
% \end{align*}

% Applying Berry-Esseen theorem to $  \ttnl - \Tilde{T}_n $ conditioned on $A$ and $X$, we have
% \begin{align*}%\label{eq:BE-for-Q}
%   &\sup_{u \in R}  \bigg{|}P^*\left(\frac{  \ttnl - \Tilde{T}_n }{\sqrt{\var(\ttnl - \Tilde{T}_n|A,X)}} \leq u \right)-\Phi(u) \bigg{|}\\
%   &=\sup_{u \in R}  \bigg{|}P^*\left(\frac{ \sum_i Y_i}{\sqrt{\sum_i \tilde{\sigma}_{n,i}^2}} \leq u \right)-\Phi(u) \bigg{|}\\
%   &\leq C_1\left(\sum_{i=1}^n(\tdsigi^2)\right)^{-3/2}\sum_{i=1}^n\tilde{\gamma}_i=:C_1\psi_N,
% \end{align*}
%where $\psi_N=\left(\sum_{i=1}^n(\tdsigi^2)\right)^{-3/2}\sum_{i=1}^n\gamma_i$, and  $\gamma_i=E\{|Y_i|^3\mid A,X\}$. \bk
% where 
% $\tilde{\gamma}_i=E\{|\tdh(i)-\tdu|^3\mid A,X\}$.


% \rd [THIS IS NOT APPLICABLE]
% From Lemma~\ref{lem:proveconv},
% we have%we have  $\gamma_i < \infty$ and 


%Plug in what we have in C.5 
% \begin{align}\label{eq:BE-order-of-gamma}
%     P\left(\frac{\sum_i \gamma_i/\rho_n^{3s}}{n}\leq c\right)&\rightarrow 1,
% \end{align}
% for some positive constant $c$. 
% \bk

% Now in order to bound  $\psi_N$, we need to bound $E\tdsigi^2$. We decompose $\tdsigi^2$ into 


% \begin{align}\label{eq:tildah1-decomp}
%   \tdsigi^2&= E\left[(\tdh(i)-\tdu)^2\mid A,X\right]\nonumber\\%=E[E[(\tdsh(i)-\Tilde{u})^2\mid A,X]]
%   % =E(\tdh(i)-H_1(i)+H_1(i)-\tnhat -(\tdu-\tnhat))^2 \nonumber\\
%   &= \E\bbb{\{\tdh(i)-H_1(i)\}^2\mid A,X} + (H_1(i)-\tnhat)^2  + \E\bbb{(\tdu-\tnhat)^2\mid A,X} \nonumber\\
%     &+ 2\E[\{\tdh(i)-H_1(i)\}\{H_1(i)-\tnhat)\}\mid A,X]
%     -2 \E[(H_1(i)-\tnhat)(\tdu-\tnhat)\mid A,X]\nonumber\\ &-2\E[\{\tdh(i)-H_1(i)\}(\tdu-\tnhat)\mid A,X]
% \end{align}

% It is easy to see that the first two cross terms are zero. As for the third, 
% the law of iterated expectation gives:
% \begin{align*}
%     &\E[\{\tdh(i)-H_1(i)\}(\tdu-\tnhat)]\mid A,X]
% %   % &= \frac{1}{n}\sum_{j \neq i}E[E[\{\tdh(i)-H_1(i)\}\tdh(j)\mid  A,X]] + \frac{1}{n} E[E[\tdh(i)^2\mid A,X]] - E\left[\frac{1}{n}H_1(i)^2\right] \\
%     =  \frac{1}{n} \var \{\tdh(i)\mid A,X\}.%E[E[\tdh(i)^2\mid A,X]] - E\left[\frac{1}{n}H_1(i)^2\right]=\frac{1}{n}\frac{1-p}{N\frac{n-1}{k-1}}E(\hsxi)^2. %\frac{1}{n}(p^2-1)E(h_1^2(i)) 
%     %\bl  \text{or should it be}\frac{1}{n}E(\frac{N}{\hat{N}}-1)^2E(h_1^2(i))
% \end{align*}
%The last line comes from similar argument as Eq~\ref{eq:BE-h1td-h1}. \\

%For the first term of Eq~\ref{eq:tildah1-decomp}, from Lemma~\ref{lem:proveconv-mean} \bl (Lemma C.5 in Appendix)\bk, we have
%\rd
%\begin{align*}
 %   \E(H_1(i)-\tnhat)^2= \Theta(\rho^{2s}). \bk%\var[E(h(X)\mid X_1)]
%\end{align*}
\bk
% Now we calculate the second term in Eq~\ref{eq:tildah1-decomp},
% \begin{align*}
%     \E\left\{(\tdu-\tnhat)^2\mid A,X\right\}= \E\left\{ \left[\frac{1}{n}\sum_{i=1}^n\{\tdh(i)-H_1(i)\}\right]^2 \mid A,X\right\}=\frac{\sum_{i=1}^n\var\{\tdh(i)\mid A,X)\}}{n^2}.
% \end{align*}



% We also have,
% \begin{align*}
%      E\left[\{\tdh(i)-H_1(i)\}^2\mid A,X\right]=\var\{\tdh(i)\mid A,X)\}.
% \end{align*}
% \bk


% Collecting all terms in Eq~\ref{eq:tildah1-decomp}, we have
% \begin{align}\label{eq:BE-esigma}
%   \tdsigi^2&=\left(1-\frac{2}{n}\right)\var\{\tdh(i)\mid A,X\}+\frac{\sum_{i=1}^n\var\{\tdh(i)\mid A,X)\}}{n^2}
%   +\hat{g}_1(i)^2.
  % &=\Theta\left(\rho^{2s}+\max\left(\frac{\rho^{2s}}{N},\frac{k\rho^{s}}{Nn} \right)\right)\\
  % &=\left(\rho^{2s}\max\left\{1,\frac{1}{N\frac{n}{k}\rho_n^s}\right\}\right)
% \end{align}

\begin{lemma}
\label{lemma:third-moment-randomized}
\begin{align*}
E|\tilde{H}_1(i) - H_1(i)|^3  = O\left( \frac{\rho_n^s}{n^2 N^2} \right) + O\left(\frac{\rho_n^{3s/2}}{N^{3/2}n^{3/2}} \right) 
\end{align*}
\end{lemma}

\begin{proof}
By Rosenthal's inequality, for some constant $C_1$ and $C_2$, we have 
\begin{align*}
    E\left(|\tilde{H}_1(i)-H_1(i)|^{3} \ \bigr \rvert \ A,X\right) &\leq \underbrace{\frac{C_1}{N^2} E[|H_\pi(i)-H_1(i)|^3|A,X]}_{I}\\ &+ \underbrace{\frac{C_2}{N^{3/2}}\left( E[(H_\pi(i)-H_1(i))^2|A,X]\right)^{3/2}}_{II}.
\end{align*}
Now, let $\cei = E[H(A_{S \cup i}) \ | \ X_i]$ and observe that $E|H_1(i) - \cei|^c \leq E|H(A_{S \cup i}) - \cei|^c$ for $c\geq 1$ via Jensen's inequality.  Moreover, conditionally on $X_i$, note that for $S \in  \mathbb{S}_\pi$,  $H(A_{S \cup i})$ are mutually independent since their node sets are disjoint.  Now for $I$, we use Rosenthal again to bound the third absolute moment of the Bernoulli sum:
% 
% we use Rosenthal's inequality again to bound $E[|H(A_{S \cup i})-H_1(i)|^3|A,X]$:
\begin{align*}
    E(|H_\pi(i)-H_1(i)|^3|) &\leq \frac{Cr^3}{n^3}\frac{1}{(n-1)!} \sum_{\pi}E\left[E\left(\bigr|\sum_{S\in \mathbb{S}_\pi} H(A_{S\cup i})-\cei\bigr|^3 \biggr \rvert \ X_i\right)\right]
    \\ & \leq  \frac{C_1}{n^2} E|H(A_{S \cup i}) -\cei|^3 +  \frac{C_2}{n^{3/2}} \left\{E(H(A_{S \cup i}) -\cei)^2\right\}^{3/2}
    \\ &= O\left( \frac{\rho_n^{s}}{n^2} \right) + O\left( \frac{\rho_n^{3s/2}}{n^{3/2}} \right)
    % \\ &+  \frac{C_2r^3}{n^3}\frac{1}{(n-1)!} \su\left(\sum_{S\in S_\pi}E[(H(A_{S\cup i})-H_1(i))^2|A,X]\right)^{3/2}
    % & \leq c'_1\frac{\rho_n^s}{n^2} + c'_2 \frac{(n\rho_n^s)^{3/2}}{n^3}.
\end{align*}
Now for $II$, 
\iffalse%since $w$ is bounded above, we have that:
%\begin{align*}
%E(II) \leq \frac{C \rho_n^{3/2}}{n^{3/2}N^{3/2}}    
%\end{align*}
\begin{align}\label{eq:EY2}
    &E\bb{E\bbb{\bb{H_{\pi}(i)-H_1(i)}^2|A,X}}^{3/2}= E\bb{\frac{1}{(n-1)!}\sum_\pi \bb{H_{\pi}(i)-H_1(i)}^2}^{3/2} \nonumber \\ 
    & = E\bb{\frac{1}{(n-1)!}\sum_\pi (H_{\pi}(i)-\cei)^2-(H_1(i)-\cei)^2}^{3/2} \nonumber\\
    & \leq E\bb{\frac{1}{(n-1)!}\sum_\pi (H_{\pi}(i)-\cei)^2}^{3/2} \nonumber\\
    &\leq  E\bigg{(}\frac{1}{n^2(n-1)!}\sum_{\pi}\bigg{(}\sum_{S\in\mathcal{S}_\pi(i)} \bb{H(A_{S\cup i})-\cei}^2 \nonumber\\&+\sum_{\stackrel{S\cap T=\phi}{S,T\in\mathcal{S}_\pi(i)}} (H(A_{S\cup i})-\cei)(H(A_{T\cup i})-\cei)\bigg{)}\bigg{)}^{3/2} \nonumber \\
    &\leq E\bb{\frac{2 H_1(i) + 2 {\cei}^2}{n}+C'H'_1(i)}^{3/2} = O\bb{\frac{\rho_n^{3s/2}}{n^{3/2}}}+O\bb{\frac{\rho_n^{3s-3/2}}{n^{3/2}}},
\end{align}
where the last step comes from the fact that $H'_1(i)$ is a mean zero U statistic and following the inequalities for $L^p$ norm, we have
\begin{align*}
    E(H_1'(i)^{3/2}|X_i) \leq  \left(E(H_1'(i)^{2}|X_i)\right)^{3/4}, 
\end{align*}
and the RHS follows from
\begin{align*}
  E(H_1'(i)^{2}|X_i)&=\frac{C}{
  n^{4(r-1)}}  \sum_{\substack{S\cap T=\phi\\S'\cap T'=\phi}}E\bbb{\prod_{J \in \{S,T,S',T'\}}(H(A_{J\cup i})-\cei)\bigg{|}X_i}\\
  &=O\bb{\frac{\rho_n^{4s-2}}{n^2}},
\end{align*}
dominated by $|S\cap S'|=1$ and $|T\cap T'|=1$.

Note now in Eq~\ref{eq:EY2}, since $s\geq 1$, $\frac{\rho_n^{3s/2}}{n^{3/2}} \geq \frac{\rho_n^{3s-3/2}}{n^{3/2}}$. Eq~\ref{eq:EY2} is dominated by first term $\frac{\rho_n^{3s/2}}{n^{3/2}}$.
\fi
using the bound in Lemma~\ref{lem:rosenthal:V11} Eq. \ref{eq:rosenthal-var-term}, along with the fact that $\|X\|_{3/2} \leq \|X\|_{2}$, we have for some constant $C$,
\begin{align*}
E(II) \leq \frac{C \rho_n^{3/2}}{n^{3/2}N^{3/2}}.    
\end{align*}

The result follows.
\end{proof}






\iffalse
\pp
Since the first two terms in Eq~\ref{eq:BE-esigma} is always positive, $\sum_i \tdsigi^2\geq n\hat{\tau}_n^2$.   Thus, $\sum_i \tdsigi^2\geq n\rho_n^{2s}$. 

Now we compute $\tilde{\gamma}_i^3$. Observe that,
\begin{align}\label{eq:tildah1-decomp}
   \sum_i\tilde\gamma_i^3&\leq C\left(\sum_iE\left[|\tilde{H}_1(i)-H_1(i)|^3|A,X\right]+\sum_i|H_1(i)-\tnhat|^3+\sum_iE[|\tnhat-\tilde{T}_n|^3|A,X]\right)
\end{align}

Note that for the last term in Eq~\ref{eq:tildah1-decomp}, using Jensen's inequality for convex function $f(x)=|x|^3$, for some constant $C_0$
\begin{align*}
    \sum_iE[|\tnhat-\tilde{T}_n|^3|A,X]&\leq n\times\frac{1}{n}\sum_iE[|\tilde{H}_1(i)-\tnhat|^3|A,X]\\&\leq C_0\left(\sum_iE\left[|\tilde{H}_1(i)-H_1(i)|^3|A,X\right]+\sum_i|H_1(i)-\tnhat|^3\right),
\end{align*}
which are just the first two terms in Eq~\ref{eq:tildah1-decomp}. So now we bound the first two terms in Eq~\ref{eq:tildah1-decomp}.

From Lemma~\ref{lem:proveconv}, we have with probability going to one, the second term in the above equation $\sum_i|H_1(i)-\tnhat|^3\leq cn\rho_n^{3s}$, for some constant $c$.

Now we look at the first term in Eq~\ref{eq:tildah1-decomp}. Using Rosenthal's inequality, for some constant $C_1$ and $C_2$, we have 
\begin{align*}
    \sum_iE\left[|\tilde{H}_1(i)-H_1(i)|^{3}|A,X\right] &\leq \underbrace{C_1\left(\sum_i\frac{1}{N^3}\sum_\pi E[|H_\pi(i)-H_1(i)|^3|A,X]\right)}_{Y_1}\\ &+ \underbrace{C_2\left(\sum_i\frac{1}{N^3}\left(\sum_\pi E[(H_\pi(i)-H_1(i))^2|A,X]\right)^{3/2}\right)}_{Y_2}.
\end{align*}

\iffalse
Now to bound $Y_1$, we use Rosenthal's inequality again to bound $E[|H_\pi(i)-H_1(i)|^3|A,X]$. For some constant $c_1$,$c_2$, and $c'_1$,$c'_2$,
\begin{align*}
    E[|H_\pi(i)-H_1(i)|^3|A,X] &\leq c_1 \frac{r^3}{n^3}\sum_{S \in S_\pi}E[|H(A_{S\cup i})-H_1(i)|^3|A,X] \\ &+ c_2 \frac{r^3}{n^3}\left(\sum_{S\in S_\pi}E[(H(A_{S\cup i})-H_1(i))^2|A,X]\right)^{3/2}\\
    & \leq c'_1\frac{\rho_n^s}{n^2} + c'_2 \frac{(n\rho_n^s)^{3/2}}{n^3}.
\end{align*}
As long as $n\rho_n^s \ll 1$, we have $\frac{\rho_n^s}{n^2} \gg \frac{(n\rho_n^s)^{3/2}}{n^3}$.
\fi 

Now, we bound $E(Y_1)$. Let $\cei = E[H(A_{S \cup i}) \ | \ X_i]$ and observe that $E|H_1(i) - \cei|^c \leq E|H(A_{S \cup i}) - \cei|^c$ for $c\geq 1$ via Jensen's inequality.  Moreover, conditionally on $X_i$, note that for $S \in  \mathbb{S}_\pi$,  $H(A_{S \cup i})$ are mutually independent since their node sets are disjoint.  Now for $Y_1$, we use Rosenthal again to bound the third absolute moment of the Bernoulli sum:
% 
% we use Rosenthal's inequality again to bound $E[|H(A_{S \cup i})-H_1(i)|^3|A,X]$:
\begin{align*}
    E(|H_\pi(i)-H_1(i)|^3|) &\leq \frac{Cr^3}{n^3}\frac{1}{(n-1)!} \sum_{\pi}E\left[E\left(\bigr|\sum_{S\in \mathbb{S}_\pi} H(A_{S\cup i})-\cei\bigr|^3 \biggr \rvert \ X_i\right)\right]
    \\ & \leq  \frac{C_1}{n^2} E|H(A_{S \cup i}) -\cei|^3 +  \frac{C_2}{n^{3/2}} E[E(H(A_{S \cup i}) -\cei)^2|X_i)^{3/2}]
    \\ &= O\left( \frac{\rho_n^{s}}{n^2} \right) + O\left( \frac{\rho_n^{3s/2}}{n^{3/2}} \right)
    % \\ &+  \frac{C_2r^3}{n^3}\frac{1}{(n-1)!} \su\left(\sum_{S\in S_\pi}E[(H(A_{S\cup i})-H_1(i))^2|A,X]\right)^{3/2}
    % & \leq c'_1\frac{\rho_n^s}{n^2} + c'_2 \frac{(n\rho_n^s)^{3/2}}{n^3}.
\end{align*}
%As long as $n\rho_n^s \ll 1$, we have $\frac{\rho_n^s}{n^2} \gg \frac{\rho_n^{3s/2}}{n^{3/2}}$.

Now, to bound $E(Y_2)$, 
\begin{align}\label{eq:EY2}
    &E\bb{E\bbb{\bb{H_{\pi}(i)-H_1(i)}^2|A,X}}^{3/2}= E\bb{\frac{1}{(n-1)!}\sum_\pi \bb{H_{\pi}(i)-H_1(i)}^2}^{3/2} \nonumber \\ 
    & = E\bb{\frac{1}{(n-1)!}\sum_\pi (H_{\pi}(i)-\cei)^2-(H_1(i)-\cei)^2}^{3/2} \nonumber\\
    & \leq E\bb{\frac{1}{(n-1)!}\sum_\pi (H_{\pi}(i)-\cei)^2}^{3/2} \nonumber\\
    &\leq  E\bb{\frac{1}{n^2(n-1)!}\sum_{\pi}\bb{\sum_{S\in\mathcal{S}_\pi(i)} \bb{H(A_{S\cup i})-\cei}^2+\sum_{\stackrel{S\cap T=\phi}{S,T\in\mathcal{S}_\pi(i)}} (H(A_{S\cup i})-\cei)(H(A_{T\cup i})-\cei)}}^{3/2} \nonumber \\
    &\leq E\bb{\frac{2 H_1(i) + 2 {\cei}^2}{n}+C'H'_1(i)}^{3/2} = O\bb{\frac{\rho_n^{3s/2}}{n^{3/2}}}+O\bb{\frac{\rho_n^{3s-3/2}}{n^{3/2}}},
\end{align}
where the last step comes from the fact that $H'_1(i)$ is a mean zero U statistic and following the inequalities for $L^p$ norm, we have
\begin{align*}
    E(H_1'(i)^{3/2}|X_i) \leq  \left(E(H_1'(i)^{2}|X_i)\right)^{3/4}, 
\end{align*}
and the RHS follows from
\begin{align*}
  E(H_1'(i)^{2}|X_i)&=\frac{C}{
  n^{4(r-1)}}  \sum_{\substack{S\cap T=\phi\\S'\cap T'=\phi}}E\bbb{\prod_{J \in \{S,T,S',T'\}}(H(A_{J\cup i})-\cei)\bigg{|}X_i}\\
  &=O\bb{\frac{\rho_n^{4s-2}}{n^2}},
\end{align*}
dominated by $|S\cap S'|=1$ and $|T\cap T'|=1$.

Note now in Eq~\ref{eq:EY2}, since $s\geq 1$, $\frac{\rho_n^{3s/2}}{n^{3/2}} > \frac{\rho_n^{3s-3/2}}{n^{3/2}}$. Eq~\ref{eq:EY2} is dominated by first term $\frac{\rho_n^{3s/2}}{n^{3/2}}$.


Therefore, combining $E(Y_1)$ and $E(Y_2)$, we have, for some constant $C_1$ and $C_2$, 
\begin{align*}
    E\left(\sum_iE\left[|\tilde{H}_1(i)-H_1(i)|^{3}|A,X\right]\right) &\leq C_1 \frac{nN}{N^3}\times \left(\frac{\rho_n^s}{n^2}+\frac{\rho_n^{3s/2}}{n^{3/2}}\right)+ C_2\frac{n\rho_n^{3s/2}}{N^{3/2}n^{3/2}}\\&= C_1 \frac{\rho_n^s}{nN^2}+C_1\frac{\rho_n^{3s/2}}{N^2n^{1/2}}+C_2\frac{\rho_n^{3s/2}}{N^{3/2}n^{1/2}}.
\end{align*}

Note that we always have $\frac{\rho_n^{3s/2}}{N^{2}n^{1/2}} \ll \frac{\rho_n^{3s/2}}{N^{3/2}n^{1/2}}$, and  $\frac{\rho_n^s}{nN^2} \ll \frac{\rho_n^{3s/2}}{N^{3/2}n^{1/2}}$ if $N\gg \frac{1}{n\rho_n^s}$. So as long as $N\gg \frac{1}{n\rho_n^s}$, the dominating term is $\frac{\rho_n^{3s/2}}{N^{3/2}n^{1/2}}$.


Thus, combining all terms in Eq~\ref{eq:tildah1-decomp} in expectation, for some constant $C_3$ and $C_4$, under the condition that  $N\gg \frac{1}{n\rho_n^s}$, we have 
\begin{align*}
    E\left(\sum_i\gamma_i^3\right) \leq C_3\frac{\rho_n^{3s/2}}{n^{1/2}N^{3/2}} + C_4n\rho_n^{3s}.  
\end{align*}

By Markov inequality, for constant $c$,with probability at least $1-1/c$, $\sum_i\gamma_i^3$ is bounded by $cE\left(\sum_i\gamma_i^3\right)$.

Recall that $\sum_i \tdsigi^2\geq n\rho_n^{2s}$, we are ready to present an upper bound for $\psi_N$,
\begin{align}\label{eq:BE-order-of-psi}
    \psi_N = \frac{\sum_{i=1}^n\gamma_i^3}{(\sum_{i=1}^n\tdsigi^2)^{3/2}} \leq \frac{ C_3\frac{\rho_n^{3s/2}}{n^{1/2}N^{3/2}} + C_4n\rho_n^{3s}}{(n\rho_n^{2s})^{3/2}}= O_P\left(\frac{1}{N^{3/2}n^{2}\rho_n^{3s/2}}\right)+O_P(n^{-1/2}).
\end{align}

Note that  $\frac{1}{N^{3/2}n^{2}\rho_n^{3s/2}}\ll\frac{1}{n^{1/2}}$ under the same condition that $N\gg\frac{1}{n\rho_n^s}$.
%Combining Eq~\ref{eq:BE-order-of-gamma} and $\hat{\tau}_n^2=\Theta(\rho_n^{2s})\bb{1+O_P(1/n\rho_n)+ O_P(n^{-1/2})}$ (Lemma~\ref{lem:moments-z/x}), we have: 
%\begin{align}\label{eq:BE-order-of-psi}
%    \psi_N = \frac{\sum_{i=1}^n\gamma_i^3}{(\sum_{i=1}^n\tdsigi^2)^{3/2}} %= O_p\left(\frac{n\rho_n^{3s}}{n^{3/2}\left(\rho_n^{2s}\max\left\{1,\frac{1}{N\frac{n}{k}\rho_n^s}\right\}\right)^{3/2}}\right)
 %   = O_P\left(n^{-1/2}\right).
%\end{align}




 %Conditional on $A$ and $X$, we have:%with $\tdsigi^2=E[(\tdh(i)-\Tilde{U})^2\mid  A, X]$, we have
 Thus we have, under the condition that  $N\gg\frac{1}{n\rho_n^s}$,
\begin{align}\label{eq:BE-for-Q-2}
   \sup_{u \in R}  \bigg{|}P\bb{\frac{n^{1/2}(\ttnl-\tdu)}{r\sqrt{\sum_{i=1}^n\tdsigi^2}}\leq u \mid A,X} -\Phi(u) \bigg{|}= O_P\left(n^{-1/2}\right).
\end{align} 


\bk

\fi

%Thus we have proof of Theorem~\ref{thm: apprx-linear-bootstrap} a).

%\rd ----------------------------------------------------------- \\
% To calculate $\var (\ttnl - \Tilde{T}_n|A,X)$, old 1 b) \bk 

% \textit{Proof of Theorem~\ref{thm: apprx-linear-bootstrap} (b):}
% Note that
% \begin{align*}
% \var (\ttnl - \Tilde{T}_n|A,X)=\frac{r^2}{n^2}\sum_i \tilde{\sigma}_{n,i}^2
% \end{align*}

% Using Lemma~\ref{lem:E-perm-to-subset} we have the following result for its expectation.
% \begin{align*}
% \E\left[\var\{\tdh(i)\mid A,X)\}\right]
% &=\Theta\left(\frac{r\rho_n^{s}}{Nn}\right).
% \end{align*}
%\begin{align*}
%   \E\bbb{\var\{\tdh(i)\mid A,X)\}}&= (1-p)\frac{\rd\var(\hsxi)\bk}{N\frac{n-1}{k-1}}+\frac{\theta^2(1-p) }{N}\\
%    &=\Theta\left(\max\left(\frac{\rho_n^{2s}}{N},\frac{k\rho_n^{s}}{Nn} \right)\right),
%\end{align*}
%since
%\rd
%\begin{align*}
%    \var(\hsxi)=\var(E\hsxi\mid X)+E\var(\hsxi\mid X)=\Theta(\rho_n^s).
%\end{align*}
%--------------------------------------------------------------------------------------------------------

% % \bk
% % Let $\zeta_n:=\frac{r\rho_n^{s}}{Nn} $. 
% % Using Markov's inequality, we have:
% % \begin{align*}
% %     P\bb{\sum_i \var\{\tdh(i)\mid A,X)\}\geq n\zeta_n\log^{\epsilon} n}&\leq (\log n)^{-\epsilon}.
% %     %&\leq \frac{\log n}{N}\max\bb{1,\frac{k\rho_n^{-s}}{n}}
% % \end{align*}
% % \bk

% % So
% % we have, with probability at least $1-1/\log(n)^\epsilon$,
% Now it follows from Eq~\ref{eq:BE-esigma} that:
% % \begin{align}\label{eq:BE-order-of-esigma}
% % \frac{\sum_i \tdsigi^2}{n}=\hat{\tau}_n^2 + (\log n)^\epsilon O\left(\frac{r\rho_n^{s}}{Nn} \right).
% % \end{align}
% \begin{align}\label{eq:BE-order-of-esigma}
% \frac{\sum_i \tdsigi^2}{n}=\hat{\tau}_n^2 +  O_P\left(\frac{r\rho_n^{s}}{Nn} \right).
% \end{align}

% Using Lemma~\ref{lem:moments-z/x} (a), it follows that $\hat{\tau}_n^2/\tau_n^2=1+O_P(1/n\rho_n)+O_P(n^{-1/2})$, thus we have 
% variance of $\ttnl$ satisfies Theorem~\ref{thm: apprx-linear-bootstrap} (b):
% \begin{align}\label{eq:approx-var-2}
%  \frac{ \ \var(\ttnl \mid A,X)}{\sigma_n^2}=1+O_P\left(\frac{1}{n\rho_n}\right)+O_P(n^{-1/2})+O_P\left(\frac{1}{Nn\rho_n^s} \right).
% \end{align}


%\rd --- For the new Theorem~\ref{thm: apprx-linear-bootstrap}(a)---\bk

% In what follows , let %the variance of the bootstrap estimator be given by
% %\begin{align*}
% $\bcom^2 := \dfrac{1}{n^2}\sum_{i=1}^n (\tilde{H}_1(i) - \tilde{T}_n)^2$ denote the sample variance corresponding to the randomization.  

\begin{theorem}\label{lem:bootvarconc}
Suppose that $\rho_n \rightarrow 0$, $r \geq 2$ and either $R$ is acyclic and $n \rho_n \rightarrow \infty$ or $R$ is a simple cycle and $n^{r-1} \rho_n^{r} \rightarrow \infty$. 
%\end{align*}
%where $c_n=r^2$ when $Nn\rho_n^s\gg 1$ and $c_n=1$ otherwise.
% When either $N \gg 1/n^2 \rho_n^s$, $\left.\bcom^2\right/E\bcom^2\stackrel{P}{\rightarrow}1
% $. 
\bk
Let $\kappa_n^2=\frac{1}{n^2}\sum_{i=1}^n (\tilde{H}_1(i) - \tilde{T}_n)^2$. When $N \gg 1/n^2 \rho_n^s$, we have that:
\begin{align*}
 %\frac{\hat{\nu}_n^2 }{\nu_n^2} \xrightarrow{P} 1    
  %\frac{\kappa_n^2 }{E\kappa_n^2} \xrightarrow{P} 1. 
  \frac{\kappa_n^2 }{\tilde{\sigma}_n^2+\sigma_n^2/r^2} \xrightarrow{P} 1. 
\end{align*}
% \begin{proof}
Furthermore, when $Nn\rho_n^s\gg 1$, $r^2(\tilde{\sigma}_n^2+\sigma_n^2/r^2)/\sigma_n^2\rightarrow 1$, whereas, when $Nn^2\rho_n^s\gg 1\gg Nn\rho_n^s$, $(\tilde{\sigma}_n^2+\sigma_n^2/r^2)/\tilde{\sigma}_n^2\rightarrow 1$. %$nE\bcom^2/\tau_n^2\rightarrow 1$, whereas, when $Nn^2\rho_n^s\gg 1\gg Nn\rho_n^s$, $nE\bcom^2/\var(\tilde{H}_1(i)-H_1(i)))\rightarrow 1$.\bk
\end{theorem}


\begin{proof}
First, observe that the variance of the bootstrap is given by:
\begin{align}\label{eq:def-vnhat}
\bootsd^2 = \frac{c_n^2}{n^2}\sum_{i=1}^n (\tilde{H}_1(i) - \tilde{T}_n)^2  = c_n^2\bcom^2   
\end{align}

We start by lower bounding the expectation. We can decompose the expectation as:
\begin{align*}
E\left\{\frac{1}{n^2} \sum_{i=1}^n(\tilde{H}_1(i) - \tilde{T}_n)^2 \right\} &=
\frac{1}{n^2}\sum_{i=1}^n E(\tilde{H}_1(i)) - \theta_n)^2  - \frac{1}{n}E (\tilde{T}_n - \theta_n)^2
\\ &=  \frac{1-1/n}{n} \cdot \var(\tilde{H}_1(i)) - \frac{ 2}{n}\cov( \tilde{H}_1(i), \tilde{H}_1(j))  
\end{align*}
For the covariance term, by law of iterated covariance,
\begin{align*}
\cov( \tilde{H}_1(i), \tilde{H}_1(j)) = \cov( H_1(i), H_1(j)) = O\left( \frac{\rho_n^{2s}}{(n \rho_n)n }\right)     
\end{align*}

For the variance term, we have that:
\begin{align*}
\var(\tilde{H}_1(i)) &=  \var(H_1(i) - \theta_n) + E\bbb{ \var(\tilde{H}_1(i) - H_1(i)) \ | A,X \ } \\
&= \tau_n^2\bb{1+O\bb{\frac{1}{n\rho_n}}} + \Theta\left( \frac{\rho_n^s}{Nn} \right)    
\end{align*}
where the latter bound follows from:
\begin{align*}
E(\var( \tilde{H}_1(i) - H_1(i) \ | \ A,X)) &=  \frac{1}{N} \left\{ \frac{1}{(n-1)!}\sum_{\pi} E(H_\pi - \theta_i)^2 - E(H_1(i) - \theta_i)^2 \right\} 
\\ &= \frac{1}{N}\{ E( \var( H_\pi) \ | \ X_i) - E( \var( H_1(i) \ | \ X_i))\}
\\ &= \Theta\left( \frac{\rho_n^s}{Nn} \right) - O\left(\frac{\rho_n^{2s}}{Nn}\right)
\end{align*}

Therefore,
\begin{align}\label{eq:Ekn2}
E\left\{\frac{1}{n^2} \sum_{i=1}^n(\tilde{H}_1(i) - \tilde{T}_n)^2 \right\} &= \frac{\sigma_n^2}{r^2}\bb{1+O\bb{\frac{1}{n\rho_n}}} + \Theta\left(\frac{\rho_n^s}{Nn^2}\right)
\end{align}

Now we will establish concentration.  Observe that:
\begin{align*}
 \frac{1}{n} \left\{\frac{1}{n}\sum_{i=1}^n(\tilde{H}_1(i) - \tilde{T}_n)^2 \right\} &= 
 \underbrace{\frac{1}{n} \left\{ \frac{1}{n}\sum_{i=1}^n (\tilde{H}_1(i) - H_1(i))^2 - (\tilde{T}_n - \hat{T}_n)^2 \right\}}_{V_1} 
 \\ &+ \underbrace{\frac{1}{n} \left\{ \frac{1}{n} \sum_{i=1}^n (H_1(i) - \theta_n)^2 - (\hat{T}_n-\theta_n)^2 \right\} }_{V_2}
 \\ &+ \underbrace{\frac{2}{n} \left[\frac{1}{n}\sum_{i=1}^n \{\tilde{H}_1(i) - H_1(i)\} \cdot \{ H_1(i) - \theta_n\} - \{\tilde{T}_n - \hat{T}_n\} \cdot \{ \hat{T}_n - \theta_n\} \right] }_{V_3}
\end{align*}
%\bl{[checked - agree]}
%\rd
Note that,
\begin{align}\label{eq:EV1}
    E\bbb{V_1}=\frac{1}{n}E\bbb{\var(\tilde{H}_1(i)|A,X)}\bb{1-\frac{1}{n}}=\tilde{\sigma}_n^2(1-1/n)
\end{align}
\bk
Observe that we may interpret $V_1$ and $V_2$ as sample variances and $V_3$ as a covariance term. We will first bound the variance of $V_2$ and $V_3$.

 For $V_2$, we apply results from \citet{zhang-xia-network-edgeworth}. Let:
\begin{align*}
V_2^\prime = \frac{1}{n^2}\sum_{i=1}^n \left\{ \frac{1}{{n-1 \choose r-1}}\sum_{S} h(X_{S \cup i}) - T_n  \right\}^2   
\end{align*}

% \rd 
% First we need $V_2^\prime/n$ to match. So $V_2$ is ZX's $\hat{S}_n^2$ (our $\hat{\sigma}_n^2$) and $V_2'$ is ZX's $\hat{\sigma}_n^2$ (we dont call it anything). 
% \bk

% Since $\hat{\sigma}_n^2/\nu_n \leq 1, \sigma_n^2/\hat{\sigma}_n^2 \leq 1 $ have that:
% \begin{align*}
% \ & \  P\left( \frac{|V_2 - E(V_2)|}{\nu_n} > \epsilon/3  \right)
% \\  \leq & \ P\left( \frac{|V_2 -V_2'|}{\sigma_n^2} > \epsilon/9  \right) + P\left( \frac{|V_2' - \sigma_n^2|}{\sigma_n^2} > \epsilon/9  \right) + \mathbbm{1}\left( \left| \frac{\hat{\sigma}_n^2 }{\sigma_n^2} - 1 \right| > \epsilon/9 \right)
% \\ = & \ P( \hat{\delta}_n > \epsilon/9 ) + P\left( \delta_n > \epsilon/9  \right) + \mathbbm{1}( \left| \hat{\sigma}_n^2/\sigma_n^2 - 1 \right| > \epsilon/9 ) , \text{say.}
% \end{align*}

%Since $\hat{\sigma}_n^2/\nu_n \leq 1, \sigma_n^2/\hat{\sigma}_n^2 \leq 1 $ have that:
%\rd When $N \gg 1/n\rho_n^s$ and thus $c_n = r^2$, we have: \bk
\begin{align}\label{eq:varv2}
\  \  P\left( \frac{|r^2V_2 - \sigma_n^2|}{\sigma_n^2} > \epsilon/3  \right)
 \leq & \ P\left( \frac{r^2|V_2 -V_2'|}{\sigma_n^2} > \epsilon/6  \right) + P\left( \frac{|r^2V_2' - \sigma_n^2|}{\sigma_n^2} > \epsilon/6  \right)% + \mathbbm{1}\left( \left| \frac{\hat{\sigma}_n^2 }{\sigma_n^2} - 1 \right| > \epsilon/9 \right)
%\\ = & \ P( \hat{\delta}_n > \epsilon/9 ) + P\left( \delta_n > \epsilon/9  \right) + \mathbbm{1}( \left| \hat{\sigma}_n^2/\sigma_n^2 - 1 \right| > \epsilon/9 ) , \text{say.}
\end{align}

By Lemma $3$c) of the above reference, the first term on the R.H.S of the above equation is $O_P(1/n\rho_n)$ and thus goes to zero.  For the second term, Lemma 3d) of the above reference implies that it is $ O_P(1/\sqrt{n})$; thus the second term goes to zero.  %The last term goes to zero since the variance of the noisy U-statistic converges to that of the noiseless one.   
 When $  1/n^2\rho_n^s \ll N \ll 1/n\rho_n^s$, we have that $\sigma_n^2/\nu_n^2 \rightarrow 0$, thus $V_2/\nu_n^2 \xrightarrow{P} 0$ and $V_1$ dominates.  \bk

% Thus we have:
% \begin{align}
%     \label{eq:V2}
%     V_2=o_P\bb{\frac{\rho_n^{2s}}{n}}
% \end{align}

 For $V_3$, observe that, $E(V_3|A,X) = 0$.  For $E\bbb{\var(V_3 |A,X)}$, rewriting the sample covariance, we have that
\begin{align}
\label{eq:v3-bound}
\var(V_3 |A,X) & \leq  \frac{2}{n^4} \sum_{i=1}^n \{(H_1(i) - \theta_n)^2 + (\hat{T}_n - \theta_n)^2\}  \cdot \var(\tilde{H}_1(i) - H_1(i) \ | \ A,X) 
% \\ + &  \frac{1}{n^4} \sum_{i=1}^n (H_1(i) - \theta)^2 \cdot \var(\tilde{H}_1(i) - H_1(i) \ | \ A,X) 
% \\ & \leq \frac{C}{n^4} \sum_{i=1}^n \var(\tilde{H}_1(i) - H_1(i) \ | \ A,X)  
\end{align}
Now define:
\begin{align*}
% & \frac{1}{n^4} \sum_{i=1}^n \{(H_1(i) - \theta)^2\}  \cdot \var(\tilde{H}_1(i) - H_1(i) \ | \ A,X) 
% 
\alpha_{i,1} &= \frac{1}{n^{2r-2}} \sum_{S}\{H(A_{S \cup i}) - \theta_n\}^2 \\ 
\alpha_{i,2} &= \frac{1}{n^{2r-2}} \sum_{S,T}\{H(A_{S \cup i}) - \theta_n\}  \{H(A_{T \cup i}) - \theta_n\}  \\
\beta_{i,1} &= \frac{1}{n^{r+1}} \sum_{S'}\{H(A_{S' \cup i}) - \cei\}^2 \\
\beta_{i,2} &= \frac{1}{n^{2r-1}} \sum_{S',T' : S' \cap T' = \emptyset}\{H(A_{S' \cup i}) - \cei\} \{H(A_{T' \cup i}) - \cei\}  \\ 
\end{align*}
It follows that, for some $C>0$,
\begin{align*}
&\frac{1}{n^4N}\sum_{i=1}^n\{(H_1(i) - \theta_n)^2  \cdot \var(\tilde{H}_1(i) - H_1(i) \ | \ A,X) \\
&\leq \frac{C}{Nn^4} \sum_{i=1}^n (\alpha_{i,1}\beta_{i,1} + \alpha_{i,1}\beta_{i,2} + \alpha_{i,2}\beta_{i,1} + \alpha_{i,2}\beta_{i,2})     
\end{align*}
For $\mathbb{E}[\alpha_{i,1}\beta_{i,1}]$, the leading term is when the node sets are disjoint (other than $i$); there are $O(n^{2r-2})$ such nodes and thus the contribution is $O(\rho_n^{2s}/n^{r+1})$. For $E[\alpha_{i,1}\beta_{i,2}]$, observe that the product is nonzero only if $|S\cap S^\prime|\ge 1$ and $|S\cap T^\prime|\ge 1$. Therefore, for the dominant term, there are $O(n^{3r-5})$ terms with a total contribution $O(\rho_n^{3s-2}/n^{r+2})$.  For $E[\alpha_{i,2}\beta_{i,1}]$, the dominant term is when $S,S^\prime,$ and $T^\prime$ disjoint; in this case the contribution is $O(\rho_n^{3s}/n^2)$.  Finally for $E[\alpha_{i,2}\beta_{i,2}]$, note that $S \cup T$ must share at least two nodes with $S^\prime \cup T^\prime$; there are $O(n^{4r-6})$ such terms and thus the dominant term is $O(\rho_n^{4s-2}/n^3)$. 
% ; there are $O(n^{2r-3})$ such nodes; therefore this term is $O(\rho_n^{2s-1}/n^{r+2})$. 

Now, the second term follows similar reasoning, but we elaborate further on the bound below for completeness. Let:
\begin{align*}
\alpha_{i,1}' &= \frac{1}{n^{2r}} \sum_{S}\{H(A_{S}) - \theta_n\}^2 \\ 
\alpha_{i,2}' &= \frac{1}{n^{2r}} \sum_{S,T}\{H(A_{S}) - \theta_n\}  \{H(A_{T}) - \theta_n\} 
\end{align*}
Then, for the second term in Eq \ref{eq:v3-bound}:
\begin{align*}
\frac{1}{n^4N}\sum_{i=1}^n\{(\hat{T}_n - \theta_n)^2  \cdot \var(\tilde{H}_1(i) - H_1(i) \ | \ A,X) \leq \frac{C}{Nn^4} \sum_{i=1}^n (\alpha_{i,1}'\beta_{i,1} + \alpha_{i,1}'\beta_{i,2} + \alpha_{i,2}'\beta_{i,1} + \alpha_{i,2}'\beta_{i,2})     
\end{align*}    

By analogous reasoning, $E[\alpha_{i,1}'\beta_{i,1}] = O(\rho_n^{2s}/n^{r+2})$, $E[\alpha_{i,1}'\beta_{i,2}] = O(\rho_n^{3s-2}/n^{r+3})$, $E[\alpha_{i,2}'\beta_{i,1}] = %O(\rho_n^{3s}/n^{2})$, \bl
O(\rho_n^{3s}/n^{3})$, $E[\alpha_{i,2}'\beta_{i,2}] = O(\rho_n^{4s-2}/n^{5})$.

Therefore,
\begin{align}
\var(V_3)=E\{\var(V_3|A,X)\} &= O\left( \frac{\rho_n^{2s}}{N n^{r+4}} \right) + O\left( \frac{\rho_n^{3s-2}}{N n^{r+5}}\right) + O\left( \frac{\rho_n^{3s}}{Nn^5} \right)+ O\left( \frac{\rho_n^{4s-2}}{Nn^6} \right)  \notag\\
&=O\bb{\frac{\rho_n^{2s}}{Nn^{r+4}}}+O\bb{\frac{\rho_n^{3s}}{Nn^5}}\label{eq:varv3}
\end{align}
\bk
%\rd Purna: check normalization here When $N = \omega(1/n^2 \rho_n^s)$, it follows that $E\{\var(V_3|A,X)\}/(\rho_n^{4s}/n^2) \rightarrow 0$.  






Now for $V_1$, by law of iterated variance, it suffices to bound $\var( E(V_1 \ | \ A,X))$ and $E(\var(V_1 \ | \ A,X))$.  

For the former, using Theorem~\ref{thm:clt-var-conc}, we have that:
\begin{align*}
\var\bb{E(V_1 \ | \ A,X)} &= \var\bb{\frac{1-1/n}{n^2}\sum_{i=1}^n\var(\tilde{H}_1(i) \ | A,X)}  = (1-1/n)^2\var\bb{\tilde{\sigma}_{|A,X}^2}=o\bb{\frac{\rho_n^{2s}}{N^2n^4}}
\end{align*}

%Note: Our calculation for concentration of $\tilde{T}_n - \hat{T}_n$ can be used here.



    Now for $E(\var(V_1 | A,X)$, let $V_{1,1} := \frac{1}{n^2} \sum_{i=1}^n\{\tilde{H}_1(i) - H_1(i))\}^2$, let $V_{1,2}:=\frac{1}{n}(\tilde{T}_n-\hat{T}_n)^2$. %(Plug in Purna's bound for k=2 and Robert's bound for k=1 here).



% we have by independence and Rosenthal's inequality,
% \begin{align*}
% \var(V_{1,1} | A,X) &= \frac{1}{n^4} \sum_{i=1}^n \var( (\tilde{H}_{1}(i) - H_1(i))^2 \ | \ A,X)  
% \\ & \leq \frac{1}{n^4} \sum_{i=1}^n \left[  \frac{C_1}{N^3(n-1)!} \sum_{\pi} \{H_\pi(i) - H_1(i)\}^4 + \frac{C_2}{N^2} \left(\frac{1}{(n-1)!}\sum_{\pi} \{H_\pi(i) - H_1(i)\}^2\right)^2 \right]
% \\ &= V_{1,1,1} + V_{1,1,2}, \text{ say.} 
% \end{align*}
% Now, for $E(V_{1,1,1})$, we have that:
% \begin{align*}
% E(V_{1,1,1}) &\leq \frac{C}{n^3N^3} \{ E(H_{\pi}(i) - \theta_n^{(i)})^4 + E(H_1(i) - \theta_n^{(i)})^4 \}
% \\ &= O\left( \frac{\rho_n^s}{n^5N^3}  \right)
% \end{align*}



% We consider two different regimes:
% $N \gg \rho_n^{-s}/n$, $N \ll \rho_n^{-s}/n$.  As an intermediate lemma, we will establish concentration for the following statistic calculated on all subsets:
% %
% \begin{align*}
% \frac{1}{n^2}\sum_{i=1}^n (H_1(i) - \hat{T}_n)^2
% \end{align*}

Note that,
\begin{align}\label{eq:V11-decomp}
      %\var\bb{\frac{1}{n^2}\sum_i \bb{\tilde{H}_1(i)-H_1(i)}^2|A,X}
      %\var\bb{\frac{1}{n^2}\sum_i \bb{\tilde{H}_1(i)-H_1(i)}^2|A,X}
      \var\bb{V_{1,1}|A,X}&=\frac{1}{n^4} \sum_i \var\bbb{\bb{\tilde{H}_1(i)-H_1(i)}^2|A,X}\notag\\
      &\leq \frac{1}{n^4} \sum_i E\bbb{\bb{\tilde{H}_1(i)-H_1(i)}^4|A,X}
    %  &=\frac{1}{N^2n^4}\sum_{i=1}^n\sum_{j=1}^N \var\bbb{\bb{\tilde{H}_{\pi_j}(i)-H_1(i)}^2|A,X}\\
  %    &\leq \frac{1}{N^2n^4}\sum_{i=1}^n\sum_{j=1}^N E\bbb{\bb{\tilde{H}_{\pi_j}(i)-H_1(i)}^4|A,X}\\
\end{align}
% \begin{align}
%     &\var\bbb{\left(\tilde{H}_1(i)-H_1(i)\right)^2|A,X}
%     \leq E\bbb{\bb{\tilde{H}_1(i)-H_1(i)}^4|A,X}\notag
%   %  &\leq \frac{1}{N^4}\bb{C_1\sum_{j=1}^N E\bbb{\bb{H_{\pi_j}(i)-H_1(i)}^4|A,X}+C_2\bb{\sum_{j=1}^N E\bbb{\bb{H_{\pi_j}(i)-H_1(i)}^2|A,X}}^2}\label{eq:varh1}
% \end{align}

Thus, using Lemma~\ref{lem:rosenthal:V11},
\begin{align*}
    E\bbb{\var\bb{\frac{1}{n^2}\sum_i \bb{\tilde{H}_1(i)-H_1(i)}^2|A,X}}\leq \frac{\rho_n^s}{n^6N^3}\bb{1+N n\rho_n^s}
\end{align*}


For $E(\var(V_{1,2})|A,X)$, note that, using Jensen's inequality,
\begin{align*}
    %E\bb{\var(V_{1,2}|A,X}\leq E V_{1,2}^2\leq \frac{1}{n^3}\sum_i E(\tilde{H}_1(i)-H_1(i))^4
    \var(V_{1,2}|A,X)&=\frac{1}{n^6}\var\bbb{\bb{\sum_i (\tilde{H}_1(i)-H_1(i))^2+\sum_{i\neq j}(\tilde{H}_1(i)-H_1(i))(\tilde{H}_1(j)-H_1(j))}|A,X}\\
    &\leq \frac{1}{n^6}\var\bbb{\sum_i (\tilde{H}_1(i)-H_1(i))^2|A,X}\\
    &+\frac{1}{n^6}\var\bb{\sum_{i\neq j}(\tilde{H}_1(i)-H_1(i))(\tilde{H}_1(j)-H_1(j))|A,X}
\end{align*}
We have the first part. For the second part, we see that:
\begin{align*}
    &\frac{1}{n^6}\var\bb{\sum_{i\neq j}(\tilde{H}_1(i)-H_1(i))(\tilde{H}_1(j)-H_1(j))|A,X}\\
    &=\frac{1}{n^6}\sum_{i\neq j}\var\bb{(\tilde{H}_1(i)-H_1(i))(\tilde{H}_1(j)-H_1(j))|A,X}\\
    &=\frac{1}{n^6}\sum_{i\neq j}E\bb{(\tilde{H}_1(i)-H_1(i))^2|A,X}E\bb{(\tilde{H}_1(j)-H_1(j))^2|A,X}\\
    &\leq \frac{1}{n^6} \bb{\sum_i E\bb{(\tilde{H}_1(i)-H_1(i))^2|A,X}}^2\\
    &\leq \frac{1}{n^6} \bb{\sum_i \var(\tilde{H}_1(i)|A,X)}^2
    \\&=\frac{1}{n^2}\var(\tilde{\sigma}_{|A,X}^2)+\frac{1}{n^6} \bb{\sum_i E(\tilde{H}_1(i)-H_1(i))^2}^2\\
    &\stackrel{(i)}{=}\frac{1}{n^2}o_P\bb{\frac{\rho_n^{2s}}{N^2n^4}}+\frac{1}{n^4}\bb{\frac{\rho_n^s}{nN}}^2=O\bb{\frac{\rho_n^{2s}}{n^6N^2}},
\end{align*}



%Then, we have $\var(\kappa_n^2)=\var(V_1+V_2+V_3)$, why do we need this in bracket here? \bl
%Now we compute the variance of the expectation. 
%In order to do this, we note that the conditional expectation is the same as the bootstrap variance. Thus, using Theorem~\ref{thm:clt-var-conc}, we have:
%Thus, the variance of the above is given by Lemma~\ref{}.
%\begin{align*}
    %\var\bb{E\bbb{\frac{1}{n^2}\sum_i \bb{\tilde{H}_1(i)-H_1(i)}^2|A,X}}&=\var(\tilde{\sigma}_{|A,X}^2)=o_P\bb{\frac{\rho_n^{2s}}{N^2n^4}}
    %O\bb{\frac{1}{N^2}\bb{\frac{\rho_n^{2s}}{n^7}+\frac{\rho_n^{2s}}{n^{2r+1}}+\frac{\rho_n^{4s}}{n^4}+\frac{\rho_n^{4s-2}}{n^5}}}\\%O\bb{\frac{\rho_n^{4s}/n^4(1+1/n\rho_n^2)}{N^2}}+O\bb{\frac{\rho_n^{2s}}{N^2n^5}}\\
  %  &=O\bb{\frac{1}{N^2}\max\bb{\frac{\rho_n^{2}}{n^5}(1+n\rho_n^2),}}
%\end{align*}
where the second term in step $(i)$ follows from Lemma~\ref{lem:E-perm-to-subset}. 



% For the second part,
% \begin{align*}
%     \var\bb{\sum_i H_1(i)^2}\leq E\bb{\sum_i H_1(i)^2}^2\leq E\bb{\frac{n}{r}\hat{T}_n}^2\leq n^2\rho_n^{2s}
% \end{align*}
% Putting everything together,
% \begin{align*}
%     \var\bb{E\bbb{\frac{1}{n^2}\sum_i \bb{\tilde{H}_1(i)-H_1(i)}^2|A,X}}&\leq \frac{\rho_n^{2s}}{n^7N^2}+\frac{\rho_n^{2s}}{n^6N^2}\leq C\frac{\rho_n^{2s}}{n^6N^2}
% \end{align*}
%Thus the variance of $1/n^2\sum_i(\tilde{H}_1(i)-H_1(i))^2$ is upper bounded as above:
% \begin{align*}
%     \var\bb{1/n^2\sum_i(\tilde{H}_1(i)-H_1(i))^2}&\leq \frac{\rho_n^s}{n^6N^3}\bb{1+N n\rho_n^s+Nn^2\rho_n^{2s}}
%     %O\bb{\frac{1}{N^2}\bb{\frac{\rho_n^{2s}}{n^7}+\frac{\rho_n^{2s}}{n^{2r+1}}+\frac{\rho_n^{4s}}{n^4}+\frac{\rho_n^{4s-2}}{n^5}}}
% \end{align*}
By Equation~\ref{eq:Ekn2}, we have the expectation of $\kappa_n^2$ is given by
$\Theta\bb{\frac{\rho_n^{s}}{Nn^2}(1+N n\rho_n^s)}$. 

% By Eq~\ref{eq:V2}, we have:
% \begin{align*}
%     \frac{V_2}{\frac{\rho_n^{s}}{Nn^2}(1+N n\rho_n^s)}&=o_P\bb{\frac{\rho_n^{2s}/n}{\rho_n^{s}/Nn^2(1+N n\rho_n^s)}}
%     =o_P\bb{\frac{Nn\rho_n^s}{1+N n\rho_n^s}}=o_P(1)\\
% \end{align*}

For $V_1$,  we have, for some constant $C_1$:%\bl{[checked-this is just $\var(V_1)$]}
\begin{align*}
    %\var\bb{\bcom^2}=\rd [\kappa_n^2 \text{is not what follows} ]\bl=
    \var\bb{V_1} = \frac{\rho_n^s}{n^6N^3}\bb{C_1(1+N n\rho_n^s)+o(Nn^2\rho_n^{s})}.%O\bb{\frac{\rho_n^s}{n^6N^3}\bb{1+N n\rho_n^s+Nn^2\rho_n^{2s}}}
\end{align*}
\bk


Finally  we have:
% \begin{align*}
%     P\bb{\frac{|V_1+V_2+V_3-(\sigma_n^2+\tilde{\sigma}_n^2)|}{\sigma_n^2+\tilde{\sigma}_n^2}\geq \epsilon}&\leq P\bb{\frac{|V_2-\sigma_n^2/r^2|}{E\kappa_n^2}\geq \frac{\epsilon}{2}}+P\bb{\frac{|V_1+V_3-EV_1|}{E\kappa_n^2}\geq \frac{\epsilon}{2}}\\
%     &\leq P\bb{\frac{|r^2V_2-\sigma_n^2|}{\sigma_n^2}\geq \frac{\epsilon}{2}}+P\bb{\frac{|V_1+V_3-EV_1|}{E\kappa_n^2}\geq \frac{\epsilon}{2}}\\
% \end{align*}
\begin{align}
    &P\bb{\frac{|V_1+V_2+V_3-(EV_1+\sigma_n^2/r^2)|}{\sigma_n^2/r^2+\tilde{\sigma}_n^2}
    \geq \epsilon}\notag\\
    &\leq P\bb{\frac{|V_1-EV_1|}{\sigma_n^2/r^2+\tilde{\sigma}_n^2}\geq \frac{\epsilon}{3}}+P\bb{\frac{|V_2-\sigma_n^2/r^2|}{\sigma_n^2/r^2+\tilde{\sigma}_n^2}}+P\bb{\frac{|V_3|}{\sigma_n^2/r^2+\tilde{\sigma}_n^2}\geq \frac{\epsilon}{3}}\notag\\
    &\leq \frac{9\var(V_1)}{(\sigma_n^2/r^2+\tilde{\sigma}_n^2)^2\epsilon^2}+P\bb{\frac{|V_2-\sigma_n^2/r^2|}{\sigma_n^2/r^2}\geq \frac{\epsilon}{3}}+\frac{9\var(V_3)}{(\sigma_n^2/r^2+\tilde{\sigma}_n^2)^2\epsilon^2}\label{eq:cheby}
\end{align}

When $Nn\rho_n^s\gg1$, $\sigma_n^2/r^2+\tilde{\sigma}_n^2$ is dominated by $\frac{\rho_n^{2s}}{n}$. When $Nn\rho_n^s\ll1\ll Nn^2\rho_n^s$, it is dominated by $\frac{\rho_n^{s}}{n^2N}$.  It is easy to check that when $Nn\rho_n^s\gg 1$, or $Nn\rho_n^s\ll 1 \ll Nn^2\rho_n^s$, we have $\var(V_1)/(E \bcom^2)^2\rightarrow 0$, which establishes consistency of the first term on the RHS of Eq~\ref{eq:cheby}. The second term was shown to go to zero in Eq~\ref{eq:varv2}. For the third term, using Eq~\ref{eq:varv3}, we see: %\bl{checked - true from S10}
%\rd
\begin{align*}
    \frac{\var(V_3)}{(\sigma_n^2/r^2+\tilde{\sigma}_n^2)^2}=\begin{cases}
    O\bb{\frac{1}{Nn^{r+2}\rho_n^{2s}}}+O\bb{\frac{1}{N\rho_n^sn^3}}&\mbox{When $N\gg \frac{1}{n\rho_n^s}$}\\
    O\bb{\frac{N}{n^r}}+O\bb{\frac{N\rho_n^s}{n}}&\mbox{When $\frac{1}{n^2\rho_n^s}\ll N\ll \frac{1}{n\rho_n^s}$}\\
    \end{cases}
\end{align*}
For simple cycles and acyclic subgraphs, one can verify that the above goes to zero.

Thus, we have:
\begin{align*}
    \frac{V_1+V_2+V_3-(\sigma_n^2/r^2+\tilde{\sigma}_n^2)}{\sigma_n^2/r^2+\tilde{\sigma}_n^2}&=\frac{V_1+V_2+V_3-(\sigma_n^2/r^2+EV_1/(1-1/n))}{\sigma_n^2/r^2+\tilde{\sigma}_n^2}\\
    &=\frac{V_1+V_2+V_3-(\sigma_n^2/r^2+EV_1)}{\sigma_n^2/r^2+\tilde{\sigma}_n^2}-\frac{1}{n-1}\frac{\tilde{\sigma}_n^2(1-1/n)}{\sigma_n^2/r^2+\tilde{\sigma}_n^2}\\
    &=\frac{V_1+V_2+V_3-(\sigma_n^2/r^2+EV_1)}{\sigma_n^2/r^2+\tilde{\sigma}_n^2}-O\bb{\frac{1}{n}}\\
    &\stackrel{P}{\rightarrow} 1,
\end{align*}
where the last line follows from Eq~\ref{eq:cheby}.
 

%Qiao: When $Nn\rho_n^s\gg1$, $(E(\kappa_n^2))^2$ is dominated by $\frac{\rho_n^{4s}}{n^2}$, we have $E\{\var(V_3|A,X)\}/(E(\kappa_n^2))^2 \rightarrow 0$. When $Nn\rho_n^s\ll1\ll Nn^2\rho_n^s$, $(E(\kappa_n^2))^2$ is dominated by $\frac{\rho_n^{2s}}{n^4N^2}$, we also have $E\{\var(V_3|A,X)\}/(E(\kappa_n^2))^2 \rightarrow 0$. (maybe move it to last paragraph where $(E(\kappa_n^2))^2$ is discussed. ) 

 \end{proof}

%If $Nn\rho^s\gg 1$, we have the variance is $O(\rho_n^{2s}/N^2n^5)$ and the expectation is $\Theta\bb{\rho_n^{2s}/n}$. Thus the expectation is a larger order than the standard deviation.

% If $Nn\rho_n^s\ll 1$, we have the variance is $O(\rho_n^{s}/N^3n^6)$ and the expectation is $\Theta\bb{\rho_n^{s}/Nn^2}$.
% Thus the expectation is a larger order than the standard deviation.
% \begin{align*}
%     \frac{\rho_n^{s/2}}{n^{3}N^{1.5}}&\ll \frac{\rho_n^{s}}{Nn^2}\\
%     n^2N\rho_n^s&\gg 1
% \end{align*}



\begin{lemma}\label{lem:rosenthal:V11}
Suppose that $R$ is acyclic or a simple cycle, $r \geq 2$, and $n \rho_n \rightarrow \infty$.  Then, \bk 
\begin{align*}
    %E\bbb{\var\bb{\frac{1}{n^2}\sum_i \bb{\tilde{H}_1(i)-H_1(i)}^2|A,X}}
    E\bbb{\bb{\tilde{H}_1(i)-H_1(i)}^4}
    \leq \frac{\rho_n^s}{n^3 \bk N^3}\bb{1+N n\rho_n^s}
\end{align*}
\end{lemma}
\begin{proof}


% Note that,
% \begin{align}\label{eq:V11-decomp}
%       %\var\bb{\frac{1}{n^2}\sum_i \bb{\tilde{H}_1(i)-H_1(i)}^2|A,X}
%       \var\bb{\frac{1}{n^2}\sum_i \bb{\tilde{H}_1(i)-H_1(i)}^2|A,X}&=\frac{1}{n^4} \sum_i \var\bbb{\bb{\tilde{H}_1(i)-H_1(i)}^2|A,X}
%     %  &=\frac{1}{N^2n^4}\sum_{i=1}^n\sum_{j=1}^N \var\bbb{\bb{\tilde{H}_{\pi_j}(i)-H_1(i)}^2|A,X}\\
%   %    &\leq \frac{1}{N^2n^4}\sum_{i=1}^n\sum_{j=1}^N E\bbb{\bb{\tilde{H}_{\pi_j}(i)-H_1(i)}^4|A,X}\\
% \end{align}
Note that,
\begin{align}
    %&\var\bbb{\left(\tilde{H}_1(i)-H_1(i)\right)^2|A,X}\notag\\
     &E\bbb{\bb{\tilde{H}_1(i)-H_1(i)}^4|A,X}\notag\\
    &\leq \frac{1}{N^4}\bb{C_1\sum_{j=1}^N E\bbb{\bb{H_{\pi_j}(i)-H_1(i)}^4|A,X}+C_2\bb{\sum_{j=1}^N E\bbb{\bb{H_{\pi_j}(i)-H_1(i)}^2|A,X}}^2}\label{eq:varh1}
\end{align}

Since, we now take an expectation of the RHS of above, we bound the first part with Rosenthal's inequality. For a given permutation $\pi$,
\begin{align}\label{eq:varh1-fourth}
&n^4 E\bbb{\bb{H_{\pi}(i)-H_1(i)}^4}\notag\\
&=n^4 E E\bbb{\bb{H_{\pi}(i)-H_1(i)}^4|X_i}\notag\\
&\leq C_1 E \sum_{S\in \mathcal{S}_\pi}  E\bbb{\bb{H(A_{S\cup i})-H_1(i)}^4|X_i}+C_2 E\bb{\sum_{S\in \mathcal{S}_\pi}  E\bbb{\bb{H(A_{S\cup i})-H_1(i)}^2|X_i}}^2\notag\\
&\leq C_1' n\rho_n^s+ C_2 E\bb{\sum_{S\in \mathcal{S}_\pi}  E\bbb{\bb{H(A_{S\cup i})-H_1(i)}^2|X_i}}^2\notag\\
&\leq C_1' n\rho_n^s+C_2'n^2\rho_n^{2s}
\end{align}

For the the last step Eq~\ref{eq:varh1-fourth}, we used
\begin{align*}
E\bb{\sum_{S\in \mathcal{S}_\pi}  E\bbb{\bb{H(A_{S\cup i})-H_1(i)}^2|X_i}}^2\leq n \sum_{S\in \mathcal{S}_\pi} E \bbb{E\bb{H(A_{S\cup i})-H_1(i)}^2|X_i}^2\leq n^2\rho_n^{2s}
\end{align*}
As for the second term in Eq~\ref{eq:varh1}, we have that:
%
\begin{align}
\begin{split}
\label{eq:rosenthal-var-term}
E\bb{\sum_{j=1}^N E\bbb{\bb{H_{\pi}(i)-H_1(i)}^2|A,X}}^2&\leq C_1 N\sum_{j=1}^N E\bb{E\bbb{\bb{H_{\pi_j}(i)-H_1(i)}^2|A,X}}^2\\
&\leq C_1' N^2 (\rho_n^{2s}/n^2+\rho_n^{4s-2}/n^2)\\
&= O(N^2\rho_n^{2s}/n^2)
\end{split}
\end{align}

To obtain the last step, observe that
\begin{align*}
    &E\bb{E\bbb{\bb{H_{\pi}(i)-H_1(i)}^2|A,X}}^2= E\bb{\frac{1}{(n-1)!}\sum_\pi \bb{H_{\pi}(i)-H_1(i)}^2}^2\\ 
    & = E\bb{\frac{1}{(n-1)!}\sum_\pi (H_{\pi}(i)-\cei)^2-(H_1(i)-\cei)^2}^2\\
    &\leq 2E\bb{\frac{1}{(n-1)!}\sum_\pi \bb{H_{\pi}(i)-\cei}^2}^2+2E\bbb{\bb{H_1(i)-\cei}^4}\\
    &\stackrel{(i)}{\leq} 4E\bb{\frac{1}{(n-1)!}\sum_\pi \bb{H_{\pi}(i)-\cei}^2}^2\\%+2E\bbb{\bb{H_1(i)-\cei}^4}\\
    &\leq  4E\bb{\frac{1}{n^2(n-1)!}\sum_{\pi}\bb{\sum_{S\in\mathcal{S}_\pi(i)} \bb{H(A_{S\cup i}-\cei}^2+\sum_{\stackrel{S\cap T=\phi}{S,T\in\mathcal{S}_\pi(i)}} (H(A_{S\cup i})-\cei)(H(A_{T\cup i})-\cei)}}^2\\
  % &+2E\bbb{\bb{H_1(i)-\cei}^4}\\
    &\leq 4E\bb{\frac{C H_1(i) + {\cei}^2}{n}+C'H'_1(i)}^2 = O\bb{\frac{\rho_n^{2s}}{n^2}}+O\bb{\frac{\rho_n^{4s-2}}{n^2}}
\end{align*}

Note that:
\begin{align*}
    &E(H'_1(i)^2|X_i)\\&=\frac{C}{n^{4(r-1)}}\sum_{\substack{S\cap T=\phi\\S'\cap T'=\phi}}E\bbb{H(A_{S\cup i})-\cei)H(A_{T\cup i})-\cei)H(A_{S'\cup i})-\cei)H(A_{T'\cup i})-\cei)|X_i}\\
    &=O\bb{\frac{\rho_n^{4s-2}}{n^2}} + O\left( \frac{\rho_n^{2s}}{n^{2(r-1)}} \right)
\end{align*}
The last line is true because the terms with the largest contribution are those with $|S\cap S'|=1$ and $|T\cap T'|=1$.  The latter term corresponds to the variance terms (i.e. $S=S'$, $T=T'$), which is $O\left( \frac{\rho_n^{2s}}{n^2} \right)$ for $r \geq 2$. 
% %Where $H'_1(i)$ is a local U statistics with expectation  $\Theta(\rho_n^{2s})$. FILLIN.

Step (i) follows from Jensen's inequality:
\begin{align*}
    \bb{H_1(i)-\cei}^2\leq \frac{1}{(n-1)!}\sum_\pi\bb{H_{\pi}(i)-\cei}^2
\end{align*}


Putting everything together,
\begin{align*}
   % &E \var\bbb{\left(\tilde{H}_1(i)-H_1(i)\right)^2|A,X}
   &E \bbb{\left(\tilde{H}_1(i)-H_1(i)\right)^4}
   \leq \frac{\rho_n^s}{N^3n^3}+\frac{\rho_n^{2s}}{n^2N^3}+\frac{\rho_n^{2s}}{N^2n^2}=O\bb{\frac{\rho_n^s}{N^3n^3}(1+N n\rho_n^s)},
\end{align*}
concluding the proof. 
\end{proof}



% \begin{lemma}
% \label{lemma-exp-second-moment}
% \begin{align*}
% E\bb{E\bbb{\bb{H_{\pi}(i)-H_1(i)}^2|A,X}}^2= O\bb{\frac{\rho_n^{2s}}{n^2}}+O\bb{\frac{\rho_n^{4s-2}}{n^2}}
% \end{align*}
% \end{lemma}
% \begin{proof}
% \begin{align*}
%     &E\bb{E\bbb{\bb{H_{\pi}(i)-H_1(i)}^2|A,X}}^2= E\bb{\frac{1}{(n-1)!}\sum_\pi \bb{H_{\pi}(i)-H_1(i)}^2}^2\\ 
%     & = E\bb{\frac{1}{(n-1)!}\sum_\pi (H_{\pi}(i)-\cei)^2-(H_1(i)-\cei)^2}^2\\
%     &\leq 2E\bb{\frac{1}{(n-1)!}\sum_\pi \bb{H_{\pi}(i)-\cei}^2}^2+2E\bbb{\bb{H_1(i)-\cei}^4}\\
%     &\stackrel{(i)}{\leq} 4E\bb{\frac{1}{(n-1)!}\sum_\pi \bb{H_{\pi}(i)-\cei}^2}^2\\%+2E\bbb{\bb{H_1(i)-\cei}^4}\\
%     &\leq  4E\bb{\frac{1}{n^2(n-1)!}\sum_{\pi}\bb{\sum_{S\in\mathcal{S}_\pi(i)} \bb{H(A_{S\cup i}-\cei}^2+\sum_{\stackrel{S\cap T=\phi}{S,T\in\mathcal{S}_\pi(i)}} (H(A_{S\cup i})-\cei)(H(A_{T\cup i})-\cei)}}^2\\
%   % &+2E\bbb{\bb{H_1(i)-\cei}^4}\\
%     &\leq 4E\bb{\frac{C H_1(i) + {\cei}^2}{n}+C'H'_1(i)}^2 = O\bb{\frac{\rho_n^{2s}}{n^2}}+O\bb{\frac{\rho_n^{4s-2}}{n^2}}
% \end{align*}

% Note that:
% \begin{align*}
%     E(H'_1(i)^2|X_i)&=\frac{C}{n^{4(r-1)}}\sum_{\substack{S\cap T=\phi\\S'\cap T'=\phi}}E\bbb{H(A_{S\cup i})-\cei)H(A_{T\cup i})-\cei)H(A_{S'\cup i})-\cei)H(A_{T'\cup i})-\cei)|X_i}\\
%     &=O\bb{\frac{\rho_n^{4s-2}}{n^2}} + O\left( \frac{\rho_n^{2s}}{n^{2(r-1)}} \right)
% \end{align*}
% The last line is true because the terms with the largest contribution are those with $|S\cap S'|=1$ and $|T\cap T'|=1$.  The latter term corresponds to the variance terms (i.e. $S=S'$, $T=T'$), which is $O\left( \frac{\rho_n^{2s}}{n^2} \right)$ for $r \geq 2$. 
%Where $H'_1(i)$ is a local U statistics with expectation  $\Theta(\rho_n^{2s})$. FILLIN.

% Step (i) follows from Jensen's inequality:
% \begin{align*}
%     \bb{H_1(i)-\cei}^2\leq \frac{1}{(n-1)!}\sum_\pi\bb{H_{\pi}(i)-\cei}^2
% \end{align*}

% \end{proof}


\begin{theorem}
%%%%%%%%% The commented out part below is already stated in Theorem 6 now %%%%%%%%%%


%Let the variance of the bootstrap estimator be given by
%\begin{align*}
%\bootsd^2 := \dfrac{c_n^2}{n^2}\sum_{i=1}^n (\tilde{H}_1(i) - \tilde{T}_n)^2.
%\end{align*}
%where $c_n=r$ when $Nn\rho_n^s\gg 1$ and $c_n=1$ otherwise. We have that if $ N = \omega(1/n \rho_n)$ or $N= \omega(1/n \rho_n), N=o(\omega(1/n \rho_n) $ 
%\begin{align*}
%\frac{\bootsd}{\nu_n} \xrightarrow{P} 1    
%\end{align*}
%Moreover,
Suppose that $\rho_n \rightarrow 0$, $r \geq 2$ and either $R$ is acyclic and $n \rho_n \rightarrow \infty$ or $R$ is a simple cycle and $n^{r-1} \rho_n^{r} \rightarrow \infty$.
When $N\gg 1/n^2\rho_n^s$, we have 
\begin{align*}
\sup_{t \in \mathcal{R}} |P( \tilde{T}_{n,L}^* - \tilde{T}_n   \leq t) - P( \tilde{T}_n - \theta_n   \leq t)     | \xrightarrow{P} 0.    
\end{align*}

\end{theorem}
\begin{proof}
Now, we verify the Berry-Esseen condition.  Observe that, for some $C>0$, the third central absolute moment of the bootstrap conditioned on the data $\psi_i$ may be upper-bounded as:
\begin{align*}
\psi_i \leq \frac{CE|\xi_i - 1|^3}{n^3} \left( |\tilde{H}_1(i) - H_1(i)|^3 +  |H_1(i) - \theta_n|^3 + |\tilde{T}_n - \hat{T}_n|^3 + |\hat{T}_n - \theta_n|^3   \right)       
\end{align*}
By Jensen's inequality, the latter two terms are again lower order. Therefore, by Lemma \ref{lemma:third-moment-randomized} and Lemma \ref{lem:proveconv}:
\begin{align*}
\Psi_n := \sum_{i=1}^n \psi_i = \underbrace{O_P\left( \frac{\rho_n^s}{n^4 N^2} \right) + O_P\left( \frac{\rho_n^{3s/2}}{n^{7/2} N^{3/2}} \right)}_{\text{contribution of randomization}} + \underbrace{O_P\left( \frac{\rho_n^{3s}}{n^2} \right)}_{\text{contribution of signal}}   
\end{align*}
Moreover, by definition of $\bootsd^2$ in Equation~\ref{eq:def-vnhat}, and %$\nu_n^2=E(\bootsd^2)$, 
$\nu_n^2:=c_n^2(\sigma_n^2/r^2+\tilde{\sigma}_n^2)$
from Theorem~\ref{lem:bootvarconc}, we have that when $N \gg 1/(n^2 \rho_n^s)$,
\begin{align}
\frac{\bootsd^2}{\nu_n^2} \xrightarrow{P} 1,     
\end{align}
%
where by Equation~\ref{eq:Ekn2}
,%
\begin{align*}
 \nu_n^2 = \underbrace{\Theta\left( \frac{\rho_n^s}{Nn^2} \right)}_{\text{contribution of randomization}} +  \underbrace{\Theta\left( \frac{\rho_n^{2s}}{n} \right)}_{\text{contribution of signal}}    
\end{align*}
%
Observe that when $N \gg 1/n \rho_n^s$, the signal dominates for both $\Psi_n$ and $\nu_n$.  When $1/n^2 \rho_n^s \ll N \ll 1/n \rho_n^s$, the randomization dominates and when $N= \Theta(1/n \rho_n^s)$ the contributions are the same order; in all cases:
$\Psi_n/\bootsd^{3/2} = o_P(1)$. Thus the desired CLT holds for the bootstrap.   
\end{proof}

\begin{comment}
\rd


% We will consider two cases: $N \gg \rho_n^s/n$ and $N \ll \rho_n^s/n$. 





% \begin{align}\label{eq:BE-decomp-ttnl-tnhat}
%     & \sup_{t\in R}\bigg{|}P\left(\frac{n^{1/2}(\ttnl-\Tilde{T}_n)}{r\rho_n^s}\leq t\mid A,X \right)-P\left(\frac{n^{1/2}(\hat{T}_n-\theta_n)}{r\rho_n^s}\leq t\right)\bigg{|} \nonumber \\ 
%     & \leq \sup_{t\in R}\bigg{|}P\left(\frac{n^{1/2}(\ttnl-\Tilde{T}_n)}{r\rho_n^s}\leq t \mid A,X\right)- \Phi(t)\bigg{|} + \sup_{t\in R}\bigg{|}P\left(\frac{n^{1/2}(\hat{T}_n-\theta_n)}{r\rho_n^s}\leq t\right)-\Phi(t)\bigg{|}
% \end{align}

\begin{align}\label{eq:BE-decomp-ttnl-tnhat}
    & \sup_{t\in R}\bigg{|}P\left(\frac{\ttnl-\Tilde{T}_n}{\sigma_n}\leq t\mid A,X \right)-P\left(\frac{\tilde{T}_n-\theta_n}{\sigma_n}\leq t\right)\bigg{|} \nonumber \\ 
    & \leq \sup_{t\in R}\bigg{|}P\left(\frac{\ttnl-\Tilde{T}_n}{\sigma_n}\leq t \mid A,X\right)- \Phi(t)\bigg{|} + \sup_{t\in R}\bigg{|}P\left(\frac{\hat{T}_n-\theta_n}{\sigma_n}\leq t\right)-\Phi(t)\bigg{|}
\end{align}




\begin{align}\label{eq:BE-decomp-ttnl-tnhat}
    & \sup_{t\in R}\bigg{|}P\left(\frac{\ttnl-\Tilde{T}_n}{\sigma_n}\leq t\mid A,X \right)-P\left(\frac{\hat{T}_n-\theta_n}{\sigma_n}\leq t\right)\bigg{|} \nonumber \\ 
    & \leq \sup_{t\in R}\bigg{|}P\left(\frac{\ttnl-\Tilde{T}_n}{\sigma_n}\leq t \mid A,X\right)- \Phi(t)\bigg{|} + \sup_{t\in R}\bigg{|}P\left(\frac{\hat{T}_n-\theta_n}{\sigma_n}\leq t\right)-\Phi(t)\bigg{|}
\end{align}



For the second term of Eq~\ref{eq:BE-decomp-ttnl-tnhat}, from Proposition~\ref{prop:ew} (proof in Section~\ref{sec:suppprop3}), we have 
\begin{align*}
    \sup_{t\in R} \bigg{|}P\left(\frac{\hat{T}_n-\theta_n}{\sigma_n}\right)-G(t)\bigg{|}=O(\mathcal{M}(n,\rho_n,R)).
\end{align*}
Combining with $G(t)$ defined in Eq~\ref{eq:edgeworth-gn}, we have 
\begin{align*}
     \sup_{t\in R} \bigg{|}P\left(\frac{\hat{T}_n-\theta_n}{\sigma_n}\right)-\Phi(t)\bigg{|} &\leq  \sup_{t\in R} \bigg{|}P\left(\frac{\hat{T}_n-\theta_n}{\sigma_n}\right)-G(t) \bigg{|} + \sup_{t\in R} \bigg{|}G(t)-\Phi(t)\bigg{|} \nonumber \\
     & = O(\mathcal{M}(n,\rho_n,R))+O\left(\frac{1}{n^{1/2}}\right).
\end{align*}


Now, invoking Proposition 1, we have for the bootstrap:
\begin{align*}
\sup_{t \in \mathbb{R}} \left|P\left(\frac{(\ttnl-\tilde{T}_n)}{\tilde{\sigma}} \leq t \right) - P( Z \leq t)\right| = O_P\left(\frac{1}{n\rho_n}\right)+O_P(n^{-1/2})+O_P\left(\frac{1}{Nn\rho_n^s}\right)   
\end{align*}

%Now let $J$ denote $\ttnl-\tilde{T}_n$ and $\tilde{\sigma}_a$ denote $\sqrt{\var{\ttnl-\tilde{T}_n|A,X}}$, we have

Since $\sigma_n$ is a constant with $\Theta(\frac{r\rho_n^s}{n^{1/2}})$, the above equation can be written as 
\begin{align}\label{eq:BE-tnhat-Phi}
      \sup_{t\in R} \bigg{|}P\left(\frac{n^{1/2}(\hat{T}_n-\theta_n)}{r\rho_n^s}\right)-\Phi(t)\bigg{|} = O(\mathcal{M}(n,\rho_n,R))+O_P\left(\frac{1}{n^{1/2}}\right).
 \end{align}
 Now for the first part of Eq~\ref{eq:BE-decomp-ttnl-tnhat}, let $\tilde{\sigma}_a^2 =\var(\ttnl|A,X)$. By Eq~\ref{eq:approx-var-2}, we have
 \begin{align}\label{eq:BE-define-sigratio}
     \frac{\tilde{\sigma}_a}{\tilde{\sigma}}= 1+O_P\left(\frac{1}{n\rho_n}\right)+O_P(n^{-1/2})+O_P\left(\frac{1}{Nn\rho_n^s} \right).
 \end{align}
 Denote $J=\frac{n^{1/2}(\ttnl-\Tilde{T}_n)}{r\rho_n^s}$, denote $Z$ is a standard normal random variable. The first part of Eq~\ref{eq:BE-decomp-ttnl-tnhat} is then 
\begin{align*}
    &\sup_{t\in R}|P(J\leq t \mid A,X) - P(Z\leq t)| 
    \\ &= \sup_{t\in R} |P(J \leq \tilde{\sigma}_a t\mid A,X)- P(Z \leq \tilde{\sigma}_a t)|
    \\ & \leq \underbrace{\sup_{t\in R}\bigg{|}P\left(\frac{J}{\tilde{\sigma}_a}\leq t\mid A,X\right)-P(Z\leq t) \bigg{|}}_{P_1} +\underbrace{\sup_{t \in R}|P(Z\leq t)- P(Z\leq \tilde{\sigma}_a t)|}_{P_2}
\end{align*}
Since $\frac{J}{\tilde{\sigma}_a}$ by definition is $\frac{\ttnl-\tilde{T}_n}{\sqrt{\var{\ttnl-\tilde{T}_n|A,X}}}$, by Eq~\ref{eq:BE-for-Q-2}, we have proved that $P_1=O_P(n^{-1/2})$.
For $P_2$, it is straightforward that, for some constant $C$ we have, 
\begin{align*}
    P_2=\sup_{t \in R}|P(z\leq t)- P(z\leq \tilde{\sigma}_a t)| &= \sup_{t \in R}|P(t\leq z \leq \tilde{\sigma}_a t)|=\sup_{t \in R}\bigg{|}\int_t^{t\tilde{\sigma}_a}\frac{1}{\sqrt{2\pi}}e^{-\frac{t^2}{2}}dt\bigg{|}\\
    &\leq (\tilde{\sigma}_a - 1) t e^{-\frac{t^2}{2}} \leq C(\tilde{\sigma}_a - 1).
\end{align*}
Putting $P_1$, $P_2$ and Eq~\ref{eq:BE-define-sigratio} together, we have bounded the first term of Eq~\ref{eq:BE-decomp-ttnl-tnhat}
\begin{align}\label{eq:BE-ttnl-Phi}
    \sup_{t\in R}\bigg{|}P\left(\frac{n^{1/2}(\ttnl-\Tilde{T}_n)}{r\rho_n^s}\leq t \mid A, X \right) - \Phi(t) \bigg{|} = O_P({n^{-1/2}}) + O_P\left(\frac{1}{n\rho_n}\right)+O_P\left(\frac{1}{Nn\rho_n^s} \right).
\end{align}

Combining Eq~\ref{eq:BE-tnhat-Phi} and Eq~\ref{eq:BE-ttnl-Phi} into Eq~\ref{eq:BE-decomp-ttnl-tnhat}, we have
\begin{align*}
    &\sup_{t\in R}\bigg{|}P\left(\frac{n^{1/2}(\ttnl-\Tilde{T}_n)}{r\rho_n^s}\leq t \mid A, X \right)-P\left(\frac{n^{1/2}(\hat{T}_n-\theta_n)}{r\rho_n^s}\leq t\right)\bigg{|}  \\&= O_P({n^{-1/2}}) + O_P\left(\frac{1}{n\rho_n}\right)+O_P\left(\frac{1}{Nn\rho_n^s} \right) + 
    O(\mathcal{M}(n,\rho_n,R).
\end{align*}
\bl
------------------------------------------------

% Now, we establish a CLT for the approximate count functional.  Our overall strategy for this part follows \citet{chen2019randomized}, but novel analysis is needed to establish intermediary lemmas. Let $Z \sim N(0,1)$ be independent of $A,X$ and $t' = \sqrt{\noisesd^2 + \sigma_n^2} \cdot t$. In addition, let $\noisesdax^2 = \var(\tilde{T}_n - \hat{T}_n \ | \ A,X)$ and $\noisesd^2 = E(\noisesdax^2)$.     We may further reduce the problem to establishing central limit theorems for the randomization and signal components separately as follows:

% % We start by conditioning on $A,X$ and establishing a Gaussian approximation for the noise.  Let $\noisesdax = \var(\tilde{T}_n - \hat{T}_n \ | \ A,X)$ and rearranging $\tilde{T}_n - \theta = \tilde{T}_n - \hat{T}_n + \hat{T}_n - \theta$ we have:
% \begin{align*}
% & \ \sup_{t \in \mathcal{R}} \left| P\left( \frac{\tilde{T}_n - \theta}{ \sqrt{\noisesd^2 + \sigma_n^2} } \leq t  \right) - \Phi(t)    \right|
% \\ \leq & \  \sup_{t' \in \mathcal{R}} \left|P\left( \frac{\tilde{T}_n - \hat{T}_n}{\noisesdax } \leq \frac{t'-(\hat{T}_n - \theta)}{\noisesdax}  \right) -\Phi\left(\frac{t'-(\hat{T}_n - \theta)}{\noisesd} \right) \right| 
% \\ + & \ \sup_{t' \in \mathcal{R}} \left| P\left(\frac{(\hat{T}_n - \theta) + \noisesd Z}{\sigma_n} \leq \frac{t^\prime}{\sigma_n} \right) - \Phi\left(\frac{t'}{\sqrt{\noisesd^2 + \sigma_n^2}} \right)   \right| = I +II 
% \end{align*}
% To show $I \rightarrow 0$, observe that:
% \begin{align*}
% I  \leq & \   E \left\{ \ \sup_{t' \in \mathcal{R}} \left|P\left( \frac{\tilde{T}_n - \hat{T}_n}{\noisesdax } \leq \frac{t'-(\hat{T}_n - \theta)}{\noisesdax} \ \biggr\rvert \  A,X  \right) -\Phi\left(\frac{t'-(\hat{T}_n - \theta)}{\noisesdax} \ \biggr\rvert \  A,X \right) \right| \ \right\}
%  \\ + & E \left\{ \ \sup_{t' \in \mathcal{R}} \left| \Phi\left(\frac{t'-(\hat{T}_n - \theta)}{\noisesdax} \ \biggr\rvert \  A,X \right) - \Phi\left(\frac{t'-(\hat{T}_n - \theta)}{\noisesd} \ \biggr\rvert \  A,X \right)  \right| \ \right\} = I_a + I_b
% \end{align*}

% For $I_a$, the Berry-Esseen Theorem implies that if:
% \begin{align}
% \label{eq:conditional-berry-esseen-condition}
% \frac{\frac{1}{n^3}\sum_{i=1}^n\E\left(|\tilde{H}_1(i) - H_1(i) |^3\ | \ A,X \right)}{\noisesdax^{3/2}} \xrightarrow{P} 0,
% \end{align}
% then:
% \begin{align*}
% \sup_{t' \in \mathcal{R}} \left|P\left( \frac{\tilde{T}_n - \hat{T}_n}{\noisesdax } \leq \frac{t'-(\hat{T}_n - \theta)}{\noisesdax} \ \biggr\rvert \ A, X  \right) -\Phi\left(\frac{t'-(\hat{T}_n - \theta)}{\noisesdax} \ \biggr\rvert \ A,X \right) \right| \xrightarrow{P} 0     
% \end{align*}
% By Lemma blah and Chebychev's inequality, we have that:
% \begin{align}
% \label{eq:noise-var-convergence}
% \frac{\noisesdax^2}{\noisesd^2} \xrightarrow{P} 1    
% \end{align}
% %
% where
% %
% \begin{align*}
%  \noisesd^2 := \E(\noisesdax^2) = \Theta\left( \frac{\rho_n^s}{Nn^2} \right)   
% \end{align*}
% %
% Moreover, by Lemma \ref{lemma:third-moment-randomized}, we have that:
% \begin{align*}
%  \frac{1}{n^3}\sum_{i=1}^n\E\left(|\tilde{H}_1(i) - H_1(i) |^3\ | \ A,X \right)= O_P\left( \frac{\rho_n^s}{n^4N^2} \right) + O_P\left(\frac{\rho_n^{3s/2}}{N^{3/2}n^{7/2}} \right)   
% \end{align*}
% Therefore, under the condition $N = \omega(1/n^2 \rho_n^s) $, Eq \ref{eq:conditional-berry-esseen-condition} holds and thus the expectation in converges to zero since the Kolmogorov distance is bounded.  Moreover, since Eq \ref{eq:noise-var-convergence} holds, we have that:
% %
% \begin{align*}
% \sup_{t' \in \mathcal{R}} \left|\Phi\left(\frac{t'-(\hat{T}_n - \theta)}{\noisesdax} \ \biggr\rvert \ A,X \right) - \Phi\left(\frac{t'-(\hat{T}_n - \theta)}{\noisesd} \ \biggr\rvert \ A,X \right)  \right| \xrightarrow{P} 0   
% \end{align*}
% Therefore by similar reasoning $I_b \rightarrow 0$.
% Now for $II$, for some $Z'$ independent of $Z$, by Theorem 1 of \citet{Bickel-Chen-Levina-method-of-moments} and P{\'o}lya's theorem:
% % Proposition~\ref{prop:ew} (proof in Section~\ref{sec:suppprop3}), 
% \begin{align*}
% II & \leq E \left\{\sup_{t' \in \mathcal{R}} \left| P\left(\frac{(\hat{T}_n - \theta)}{\sigma_n} \leq \frac{t^\prime - \noisesd Z}{\sigma_n} \ \biggr\rvert \ Z=z \right) - P\left(Z^\prime \leq \frac{t^\prime - \noisesd Z}{\sigma_n} \ \biggr\rvert \ Z=z \right) \right| \right\} \rightarrow 0
% % \Phi\left(\{t-(\hat{T}_n - \theta)\}/\noisesd \right)  & = P\left( \noisesd Z + (T_n - \theta) \leq  t    \right)
% % \\ &= E\left\{P\left( \frac{T_n - \theta}{\sigma_n} \leq \frac{t + \tilde{\sigma}_n Z}{\sigma_n} \ \biggr\rvert \ Z=z \right) \right\}
% % \\ &= P( \tilde{\sigma}_n Z + \sigma_n Z^\prime \leq t) + o(1)
% \end{align*}
% To conclude the proof, observe that:
% \begin{align*}
% P\left(Z^\prime \leq \frac{t^\prime - \noisesd Z}{\sigma_n} \right)
% = P(\sigma_n Z^\prime + \noisesd Z \leq t') = \Phi\left( \frac{t'}{\sqrt{\noisesd^2 +\sigma_n^2}}  \right)
% \end{align*}


\rd






% We again condition on $X_i$ and use law of iterated variance for $P_{2,2,i}$.  For $E(P_{2,2,i} \ | \ X_i)$, notice that we may interpret the summands as conditional covariances and observe that there are $O( n^{2r-k-2})$ terms such that $|S \cap T| = k$, with corresponding expectation upper bounded by $C\rho_n^{2s-k}$ for acyclic graphs and simple cycles for some $C > 0$. It follows that $\var(E(P_{2,2,i} \ | \ X_i)) = O( \rho_n^{4s-2}/n^{2})$.

% For $E(\var(P_{2,2,i} \ | \ X_i))$, we consider a variant of the Hoeffding decomposition.  For each possible cardinality of the intersection, consider a new kernel consisting of $2(r-1)-k$ nodes involving the sum of products of the form $\{H(A_{S \cup i}) - \cei\} \cdot \{H(A_{T \cup i } - \cei$, where $S 
% \cup T = \{ i_1, \ldots, i_{2(r-1)-k} \}$ and $|S \cap T| = k$.  Then,
% \begin{align*}
% P_{2,2,i} =  \frac{1}{(n-1)!}  \sum_{\pi} \sum_{k=1}^{r-2} \underbrace{\frac{ {n-1 \choose 2r-2-k }}{ {n-1 \choose r-1}^2} \sum_{|S \cap T| =k, S \cup T \in \mathbb{S_\pi}} \frac{\{H(A_{S \cup i}) - \cei\} \cdot \{H(A_{T \cup i }) - \cei) \}}{n/(2r-2-k)}}_{P_{2,2,i,\pi}}
% \end{align*}

% Since the subsets in the permutation are disjoint and there are at most $2 {2r-2-k \choose k}$ products defined on the same node set, we have that $\var(P_{2,2,i,\pi} \ | \ X_i) \leq C \rho_n^{2s-1}/n^2$ for some $C >0$.  Again using the fact that the variance of an average is upper bounded by the maximal variance, this implies that $ E(\var( P_{2,2,i} \ | \ X_i)) = O(\rho_n^{2s-1}/n^2)$.  Therefore the variance of the second term of $P_2$, which we denote $\var(P_{2,2})$, is $O( \rho_n^{2s-1}/N^2n^4)$.




% \begin{lemma} 
% If $n \rho_n \rightarrow \infty$ and $S$ is acyclic or a simple cycle with $r \geq 2$, we have for $k \geq 2$, 
% \begin{align*}
% \var(U_k/N n^k) = O\left( \frac{\rho_n^{4s-4}}{N^2n^4} \right) +  O\left( \frac{\rho_n^{2s}}{N^2n^6}   \right)
% \end{align*}
% For $k=1$, 
% \begin{align*}
% \var(U_1/N n) = O\left( \frac{\rho_n^{4s-2}}{N^2n^4} \right) +O\left( \frac{\rho_n^{2s}}{N^2n^5} \right)
% \end{align*}

% \end{lemma}
% \begin{lemma}\label{lem:p12}
% If $n \rho_n \rightarrow \infty$ and $S$ is acyclic or a simple cycle with $r \geq 2$, we have:
% \begin{align*}
% \var(P_{1,2}) = O\left( \frac{\rho_n^{4s}}{N^2n^4} \right)+O\left( \frac{\rho_n^{4s-2}}{N^2n^5} \right) +\bl O\left( \frac{\rho_n^{2s}}{N^2n^{2r+1}} \right)
% \end{align*}
% \end{lemma}
% \begin{proof}
% Now for $k=1$, consider the following decomposition: 


\begin{align*}
\frac{1}{Nn{n \choose 2r-1}}\sum_{|K| = 2r-1, \  } \frac{1}{2r-1}\sum_{S \cup T = K, i \in S \cap T }[H(A_S) - \theta_n^{(i)}] \cdot [H(A_T) -\theta_n^{(i)}]
\end{align*}

Observe that the inner sum may be written as:
\begin{align*}
& \ \frac{1}{2r-1}\sum_{S \cup T = K, i \in S \cap T }[H(A_S) - \theta_n^{(i)}] \cdot [H(A_T) -\theta_n^{(i)}] \\ =& \  \frac{1}{2r-1}\sum_{S \cup T = K }[H(A_S) - h(X_S)] \cdot [H(A_T) - h(X_T) ] 
\\    &+ \frac{1}{2r-1}\sum_{S \cup T = K, i \in S \cap T }[H(A_S) - h(X_S)] \cdot [h(X_T) - \theta_n^{(i)} ] 
\\  &+ \frac{1}{2r-1}\sum_{S \cup T = K, i \in S \cap T }[h(A_S) - \theta_n^{(i)}] \cdot [H(A_T) -h(X_T) ]  
\\ &+ \frac{1}{2r-1}\sum_{S \cup T = K, i \in S \cap T }[h(A_S) - \theta_n^{(i)}] \cdot [h(X_T) - \theta_n^{(i)}] 
\\ =& \ V_{1,K} + V_{2,K} + V_{3,K} + V_{4,K}, \ \text{say}.  
\end{align*}
So that:
\begin{align*}
&\frac{1}{Nn{n \choose 2r-1}}\sum_{|K| = 2r-1, \  } \frac{1}{2r-1}\sum_{S \cup T = K, i \in S \cap T }\{H(A_S) - \theta_n^{(i)}\} \cdot \{H(A_T) -\theta_n^{(i)}\} \\ &= \frac{1}{Nn{n \choose 2r-1}} \sum_{|K| = 2r-1} V_{1,K} + \frac{1}{Nn{n \choose 2r-1}} \sum_{|K| = 2r-1} V_{2,K} + \frac{1}{Nn{n \choose 2r-1}} \sum_{|K| = 2r-1} V_{3,K} + \frac{1}{Nn{n \choose 2r-1}} \sum_{|K| = 2r-1} V_{4,K}
\\ &= V_1 + V_2 + V_3 + V_4, \text{ say}. 
\end{align*}

We start by bounding $\var(V_1)$.  Since $A_S$ and $A_T$ share no edges, we have that:
\begin{align*}
\var(V_{1,K})&\leq  E(\var(V_{1,K} |X_i)) =   E\{\var(H_S | X_i) \  \var(H_T | X_i)\} 
\\ &= O( \rho_n^{2s})
\end{align*}
where above we used the fact that the variance of an average is upper bounded by the largest variance, which is simply the variance of any one of the terms since they are identically distributed.

Therefore, the contribution of the variance terms of the form $\var(V_{1,K})$ to $\var(V_1)$ is $O(\rho_n^{2s}/n^{2r-1}n^2N^2)$
Now for the contributions of the covariance terms to $V_{1}$,  it is immediately clear that the covariance is 0 if $(S,T)$ and $(S^\prime, T^\prime)$ are disjoint or share only a root node $i$.  

When the pairs share 3 nodes and an edge, the covariance is 0.  To see this, without loss of generality, assume that $S$ and $S^\prime$ share two nodes and an edge and $T$ and $T^\prime$ only share the root $i$.  Then,
% 
% that share 3 nodes (including a common root i) and an edge is 0.  To see this, without loss of generality, assume that $S$ and $S^\prime$ share two nodes and an edge and $T$ and $T^\prime$ only share the root $i$.  Then,
\begin{align*}
&\cov([H( A_S) - h(A_S)] \cdot [H( A_T) - h(A_T)], [H( A_{S^\prime}) - h(A_{S^\prime})] \cdot [H( A_{T^\prime}) - h(A_{T^\prime})]) 
\\ = & \  E\{E( [H( A_S) - h(A_S)] \cdot [H( A_{S^\prime}) - h(A_{S^\prime})] \ | \ X_1) \cdot  E([H( A_T) - h(A_T)] \cdot [H( A_{T^\prime}) - h(A_{T^\prime})] \ | \ X_1)\} = 0 
\end{align*}
% Now, consider the case where $(S,T)$ and $(S^\prime, T^\prime)$ share $4$ nodes, but are centered at different vertices.  Without loss of generality, suppose $S, S^\prime$ share node $k$, $T, T^\prime$ share node $l$, $(S,T)$ share node $i$, and $(S^\prime, T^\prime)$ shared node $j$.   Again, the covariance is zero by law of iterated covariance on the conditioning set $X_i, X_j,X_k,X_l$.  The asymmetric case where $S$ and $S^\prime$ share 3 nodes and $T$ and $T^\prime$ share one node is analogous. 

Thus, the dominant term is the case where $S$ and $S^\prime$ and $T$ and $T^\prime$ both share 2 nodes and an edge. There are $O(n^{4r-5})$ such terms, each with covariance upper bounded by $C\rho_n^{4s-2}$ for some $C >0$.  \bl Therefore, the contribution of such terms to the variance is $\rho_n^{4s-2}/N^2 n^4$. [Purna: is this not $\rho_n^{4s-2}/N^2 n^5$]\rd 

We now bound $\var(V_2)$ and $\var(V_3)$.  By law of iterated variance,
$\var(V_2) = E(\var(V_2 \ | X)$.  Observe that there are $O(n^{2r-1})$ variance terms of the order $\rho_n^{3s}$; therefore the total contribution is $O(\rho_n^{3s}/N^2 n^2 n^{2r-1})$. For the covariance terms, the leading term we have that $S$ and $S'$ and $T$ and $T'$ each share two vertices, with one also sharing an edge.  There are again $O(n^{4r-5})$ terms, where the conditional covariance is bounded by $C\rho_n^{2s-1}$ and the expectation component is $O(\rho_n^{2s-1})$.  Therefore, the total contribution of covariance terms is $O(\rho_n^{4s-2}/N^2n^5)$.  The variance for $V_3$ is analogous. 

Finally for $V_4$, observe that the kernel is degenerate of order 1. Therefore, $\var(V_4) = O(\rho_n^{4s}/N^2n^4)$.  
% \end{proof}
\begin{lemma} \label{lem:p22}
If $n \rho_n \rightarrow \infty$ and $S$ is acyclic or a simple cycle with $r \geq 2$, we have for $k \geq 2$, 
\begin{align*}
\var(P_{2,2}) = O\left( \frac{\rho_n^{4s}}{N^2n^4} \right) +  O\left( \frac{\rho_n^{4s-2}}{N^2n^5}   \right)
\end{align*}
% For $k=1$, 
% \begin{align*}
% \var(U_1/N n) = O\left( \frac{\rho_n^{4s-2}}{N^2n^4} \right) +O\left( \frac{\rho_n^{2s}}{N^2n^5} \right)
% \end{align*}

\end{lemma}

% \begin{proof}
% Note that $\var(P_{2,2})$ can be broken up into $\var E (P_{2,2}|X)$ and $E\bbb{\var (P_{2,2}|X)}$. 


% For the variance of the conditional expectation, we may express this term as a sum of noisy U-statistics of different orders:
% \begin{align*}
% P_{2,2} &\asymp \sum_{k=1}^{r-2}  \frac{1}{Nn^k {n \choose 2r-k }} \sum_{|K| = 2r-k} \frac{1}{2r-k} \sum_{S \cup T= K, i \in S \cap T} \{ H(A_S) - \cei\} \cdot \{ H(A_T) - \cei\}
%\\&= \sum_{k=1}^{r-2} \frac{U_k}{Nn^k} , \text{ say.}
%  \\ &= \sum_{k=1}^{r-1}  \frac{1}{Nn^k {n \choose 2r-k }} \sum_{|K| = 2r-k} \frac{1}{2r-k} \sum_{S \cup T= K} H(A_S)H(A_T)  
%  \\ & \ \ + \sum_{k=1}^{r-1}  \frac{1}{Nn^k {n \choose 2r-k }} \sum_{|K| = 2r-k} \frac{1}{2r-k} \sum_{S \cup T= K}   \left\{ \sum_{ i \in S \cap T} \cei \right\} \cdot H(A_S)
%   \\ & \ \ + \sum_{k=1}^{r-1}  \frac{1}{Nn^k {n \choose 2r-k }} \sum_{|K| = 2r-k} \frac{1}{2r-k} \sum_{S \cup T= K}   \left\{ \sum_{ i \in S \cap T} \cei \right\} \cdot H(A_T)
%   \\ & \ \ + \sum_{k=1}^{r-1}  \frac{1}{Nn^k} \frac{1}{n}\sum_{i=1}^n (\cei)^2 = P_{2,2,1}+ P_{2,2,2} + P_{2,2,3} + + P_{2,2,4}, \text{ say.} 
% 
% \end{align*} 
% For note that for $k=1$, the conditional expectation of the terms with $|S\cap T|=1$  is zero. For $k\geq 2$, the terms will have  a contribution of $\rho_n^{2s-(k-1)}$.
% For some function $g$ with finite second moment, the conditional expectation is given by:
\begin{align*}
    \frac{1}{{n\choose 2r-k}}\sum_{|S\cup T|=2r-k}E\bbb{(H(A_S)-\cei)(H(A_T)-\cei)|X}=\rho_n^{2s-k+1}\frac{\sum_{|S\cup T|=2r-k}g(X_{S\cup T})}{{n\choose 2r-k}}
\end{align*}
%This leads to $O\bb{\rho_n^{4s-2}/n^4N^2}$.

Note that the above is a U statistic and thus the variance of the conditional expectation of $P_{2,2}$ given by $O\bb{\frac{\rho_n^{4s-2k+2}}{N^2n^{2k+1}}}$. For $k\geq 2$, this is dominated by $O\bb{\frac{\rho_n^{4s-2}}{n^5N^2}}$.

% For computing the expectation of the conditional variance, we upper bound as follows: %$E\var (P_{2,2}|X)$
% %upper bounded by:
% \begin{align*}
%     \frac{1}{n^{4r}}\sum_{i,j}\sum_{\substack{S\neq T, S,T\in \mathbb{S}\{-i\}\\S'\neq T', S',T'\in \mathbb{S}\{-j\}}} E\bb{(H(A_{S\cup i})-\cei)(H(A_{T\cup i})-\cei)(H(A_{S'\cup j})-\theta^{(j)})(H(A_{T'\cup j})-\theta^{(j)})}
% \end{align*}
% \end{proof}

% %Another term which has $S\cap T=S'\cap T'$, contributes $n^{4r-3k}\rho_n^{4s-k+1}$ leading to $\rho_n^{4s+1}/(n\rho_n)^kn^{2k}$.
% %We will consider two different strategies for $k=1$ and $k >1$; for the former, we use degeneracy of the corresponding U-statistic kernel to get a sharper bound.

% % For $k >1$, we further break up $P_{2,2}$ as follows:
% % \begin{align*}
% %   \sum_{k>1} \frac{U_k}{Nn^k} &= \sum_{k>1}  \frac{1}{Nn^k {n \choose 2r-k }} \sum_{|K| = 2r-k} \frac{1}{2r-k} \sum_{S \cup T= K} H(A_S)H(A_T)  
% %  \\ & \ \ + \sum_{k>1}  \frac{1}{Nn^k {n \choose 2r-k }} \sum_{|K| = 2r-k} \frac{1}{2r-k} \sum_{S \cup T= K}   \left\{ \sum_{ i \in S \cap T} \cei \right\} \cdot H(A_S)
% %   \\ & \ \ + \sum_{k>1}  \frac{1}{Nn^k {n \choose 2r-k }} \sum_{|K| = 2r-k} \frac{1}{2r-k} \sum_{S \cup T= K}   \left\{ \sum_{ i \in S \cap T} \cei \right\} \cdot H(A_T)
% %   \\ & \ \ + \sum_{k>1}  \frac{1}{Nn^k} \frac{1}{n}\sum_{i=1}^n (\cei)^2 = P_{2,2,1}+ P_{2,2,2} + P_{2,2,3} + P_{2,2,4}, \text{ say.} 
% %   \end{align*}
% %  Now for $P_{2,2,1}$, we use law of iterated variance.  For the variance of the conditional expectation given $X$, observe that the resulting expectation is a U-statistic; therefore the contribution of the the $k$th term to the variance is $O(\rho_n^{4s-2k}/N^2n^{2k+1})$, which is upper bounded by $O(\rho_n^{2s+4}/N^2n^5)$.  
 
% %  Now, for the expectation of the variance conditional on $X$, we consider the contribution of conditional variance and covariance terms for some fixed $k >1$.  For the contribution of the covariance terms, suppose that $|S \cap T| = k$, $|S' \cap T'| = k$, and that $(S \cup T) \cap (S' \cup T') =q$ for $q \geq 2$.  There are $O(n^{4r-2k-q})$ such terms, with conditional covariance upper bounded by $C\rho_n^{4s-2k-q}$ for some $C>0$; therefore the conditional covariance is $O(  \rho_n^{4s-2k}/(N^2n^{2k}(n\rho_n)^q)$, which is further upper bounded by $O(\rho_n^{2s+4}/(N^2 n^4))$. 
% %  $|(S \cup T) \cap (S' \cup T')|=q$ for some $q \geq 2$, which implies that the subgraphs corresponding to $S \cup T$ and $S' \cup T'$ share at most $q$ edges. 
% %  Observe that there at most $O(n^{4r-2k-q_1-q_2+d})$ such vertex sets, with covariance conditional on $X$ is upper bounded by $\rho_n^{4s-2k -q_1 -q_2 + }$; therefore, the covariance is $O( \rho_n^{4s-2k}/(N^2 n^{2k}(n\rho_n)^{2q}))$, which is further upper bounded by $O( \rho_n^{2s+2}/ N^2 n^4)$. 
 
% { \color{orange}
% % Purna's stab at the above para.
 
%  Consider four subsets $S,T,S',T'$. There are 3 types of intersections. The first type are nodes \textit{only} in the intersection of a pair of subsets, and between six pairs. We will denote the size of  these intersections by $k_i,i\in[6]$. We will denote by $K$ the sum of $k_i's$. The second are nodes only in triple wise intersections with sizes $j_i,i\in[4]$. The total of these numbers is $J$. Finally there are nodes in the intersection between all four, whose size will be denoted by $J$. Note that for any given configuration of the sets (translating to a configuration of these numbers), there are a total of $n^{4r-(K+2L+3J)}$ nodes. This is because every node in the pairwise intersection gets counted twice. Those in three-way intersections get counted thrice and those in the four-way intersection get counted thrice. Finally note that there are a total of $K+L+J$ nodes such that each node belongs to some intersection (call this $I$). In order to find the number of edges, note that this intersection can be represented as four sets, which are $I\cap S,I\cap T$ etc. For each of these intersections, since we are allowing simple cycles or acyclic graphs,  note that we can have $|I\cup S|-1(|I\cup S|>0)$ edges. Thus the the total number of edges can be at most $|I|-1$ edges in the intersection. So the contribution of these numbers is
%  $$\frac{n^{4r-(K+2L+3J)}\rho_n^{4s-(K+L+J-1)}}{n^{4r}}=\frac{\rho_n^{4s+1}}{(n\rho_n)^{K+L+J}n^{L+2J}}$$
%  Now we consider some cases of configuration before summing over all $K,L,J$. We first note that all cases with $K\leq 3,L=0,J=0$ are zero. 
%  For $K=4,L=0,J=0$, the only possible case that contributes to the covariance is the one with $k_i=1,i\leq 4$. This contributes $\rho_n^{4s}/n^{4}$. Similarly note that if we have $K=5$, the contribution comes from $k_1=1,k_2=1,k_3=1,k_4=2$ which has contribution $\rho_n^{4s-1}/n^5$ and so on. Thus the terms contribute $\sum_{i\geq 0}\rho_n^{4s-i}/n^{4+i}=O\bb{\rho_n^{4s}/n^4}$. 
%  {\color{blue} We also consider the case where $K= 1,L= 2,J= 1$, this will contribute $\frac{\rho_n^{4s-1}}{n^5}$. }
%  Now we consider the case with $K= 2,L= 0,J= 1$. These terms will contribute $ \frac{\rho_n^{4s-2}}{n^5}$. In fact for $K=2,L\geq 1,J\geq 1$, we will have a contribution of
%  \begin{align*}
%      \frac{\rho_n^{4s+1}}{(n\rho_n)^4n^3}=\frac{\rho_n^{4s-2}}{(n\rho_n)n^6}
%  \end{align*}
 
%  Now we consider the terms of the form $K\geq 3,L\geq 0, J\geq 1$. These terms contribute:
%  \begin{align*}
%      \frac{\rho_n^{4s+1}}{(n\rho_n)^{4}n^{2}}=\frac{\rho_n^{4s-2}}{(n\rho_n)n^{5}}
%  \end{align*}
 
% Consider $C_{k,\ell,j}$ the covariance contribution for sets with $K=k,L=\ell,J=j$.  Putting everything together, we have:
%  \begin{align*}
%      \sum_{k,\ell,j\geq 0}C_{k,\ell,j}&=
%      \sum_{k< 4, \ell=j=0}C_{k,\ell,j}+\sum_{k\geq 4, \ell=j=0}C_{k,\ell,j}+{\color{blue}\sum_{k=1,\ell=2,j=0}C_{k,\ell,j}+}\sum_{k=2, \ell=0,j= 1}C_{k,\ell,j}\\
%      &\qquad +\sum_{k=2, \ell\geq 1,j\geq 1}C_{k,\ell,j}+\sum_{k\geq 3, \ell\geq 0,j\geq 1}C_{k,\ell,j}\\
%      &=0+O\bb{\frac{\rho_n^{4s}}{n^4}}+{\color{blue} O\bb{\frac{\rho_n^{4s-1}}{n^5}}+} O\bb{\frac{\rho_n^{4s-2}}{n^5}}.
%  \end{align*}
 
 
 
% For the conditional variance terms, observe that the variance for a given k is $O( \rho_n^{2s-k})$; therefore, the contribution of these terms is $O(\rho_n^{2s}/ N^2n^{2r+k} (n \rho_n)^k)$, which is further upper bounded by $O(\rho_n^{2s}/(N^2n^6))$. for $r \geq 2$, 
% For $P_{2,2,2}$ and $P_{2,2,3}$ we may use similar reasoning to conclude that they are of the same order as $P_{2,2,1}$.  Finally for $P_{2,2,4}$, we have the bound $O(\rho_n^{4s}/(N^2n^{2k+1}))$, which is of the desired order for $k>1$.   
\bl





\bk




% we have $O(n^2)$ terms; furthermore, for each term, there are $O(n)$ terms sharing a subset in common; when there is no subset in common, the conditional covariance is 0.  Therefore, the contribution of the covariance terms is  $O(\rho_n^{2s}/n)$.  The contribution of the variance terms is $O(\rho_n^s/n^3)$  Therefore, $E(\var(H_\pi - \theta_i)^2 \ | \ X_i) =O(\rho_n^s/n^3) +  O(\rho_n^{2s}/n)$.  Now, observe that $\var( E(H_\pi - \theta_i)^2 \ | \ X_i)) = O(\rho_n^{2s}/(n/r)^2)$ since all cross terms are zero.  Now, the variance of a mean is upper bounded by the maximum variance, we have that $\var(P_1) = O(\rho_n^{2s}/n^3 N^2)$.  For $\var(P_2)$, expanding the square and using the fact that $H_1^2(i) = H_1(i)$, we have that:
% \begin{align*}
% \var(P_2) \leq \frac{9}{n^4 N^2} \left( \var(\hat{T}_n) + \var\left(\sum_{i=1}^n \theta_n^{(i)} H_1(i)\right) + \sum_{i=1}^n\var( (\theta_n^{(i)})^2)
% \right)
% \end{align*}






% \textit{Proof of Theorem~\ref{thm: apprx-linear-bootstrap}(c)} 
% For the un-approximated linear bootstrap, there is no randomness in $\tilde{H}_1(i)$, since it equals $\hat{H}_1(i)$. Thus $\var(\tilde{H}_1(i)|A,X)=0$. So the result follows from Eq~\ref{eq:BE-esigma}.
% \end{proof}

\bk
\end{comment}
\begin{lemma}\label{lem:E-perm-to-subset}
\begin{align*}
\E\bbb{\mathrm{var}\{\tdh(i)\mid A,X\}}=\Theta\left(\frac{r\rho_n^{s}}{Nn}\right).
\end{align*}
\begin{proof}\normalfont
\begin{align*}
 \E\bbb{\var\{\tdh(i)\mid A,X)\}}&= \E\bbb{\var\left\{\frac{\sum_jH_{\pi_j}(i)}{N} \mid A,X\right\}} =\E\left(\frac{1}{N^2}\sum_j\var\{H_{\pi_j}(i)\mid A,X\}\right)\\
 &=\E\left(\frac{1}{N^2}\sum_j\E\{(H_{\pi_j}(i)-\theta)^2\mid A,X\}\right)\\
 &=\E\left(\frac{1}{N^2}\left[\sum_j\sum_{S\in \mathbb{S}_{\pi_j}}\frac{E\{H(A_{S\cup i}-\theta)^2\mid A,X\}}{(\frac{n-1}{r-1})^2}\right]\right)\\
 &=\frac{\var\{H(A_{S\cup i})\}}{N\frac{n-1}{r-1}}
\end{align*}

%\rd Why do we need Lemma S4 for proving this eqn?\bk

%We know from Lemma~\ref{lem:moments-z/x}, which is shown Supplementary Section~\ref{sec:suppthm23} that,
We further have,
\begin{align*}
   \var\{\hsxi\}=\var[E\{\hsxi\mid X\}]+E[\var\{\hsxi\mid X\}]=\Theta(\rho_n^s).
\end{align*}
Thus, we arrive at
\begin{align*}
\E\bbb{\var\{\tdh(i)\mid A,X)\}}=\Theta\left(\frac{r\rho_n^{s}}{Nn}\right).    
\end{align*}


\end{proof}
\end{lemma}



\section{Proof of Proposition~\ref{prop:ew}}
\label{sec:suppprop3}
\begin{proof}\normalfont
 In what follows, we prove Proposition~\ref{prop:ew} holds for Edgeworth expansion of a standardized count functional.  Our argument here is closely related to  \cite{zhang-xia-network-edgeworth}, thus we do not present the complete proof here. They have showed in Theorem 3.1 in the above reference, that under same conditions, Edgeworth Expansion for studentized $\hat{T}_n$, denote as $\tilde{G}_n(u)$ here, has the same property as Proposition~ \ref{prop:ew}. We have first derived our Edgeworth Expansion formula in eq~\ref{eq:edgeworth-gn} for standardized $\hat{T}_n$ instead of studentized $\hat{T}_n$ and we state the form of the characteristic function of $G_n(u)$ below:

\begin{proposition}\label{lm:chf_g}
We have:
\begin{align*}
    \psi_{G(n)}(t)&:= \int e^{itu}dG_n(u)\\
    &= e^{-\frac{t^2}{2}}\left(1- it^3\frac{1}{6n^{1/2}\tau_n^3}\left[E\{g_1^3(X_1)\}+3(r-1)E\{g_1(X_1)g_1(X_2)g_2(X_1,X_2)\}\right]\right).
\end{align*}
\end{proposition}

Our standardized $\hat{T}_n$, denote as $\tilde{T}_n$ can be decomposed into
\begin{equation*}%\label{eq:tnt-decomp}
    \tilde{T}_n:=\frac{\hat{T}_n-\theta_n}{\sigma_n} = \frac{T_n-\theta_n}{\sigma_n}+ \frac{\tnhat - T_n}{\sigma_n}= T_{n,1}+T_{n,2}  + O_P\left(\frac{1}{n} \right)+ R_n,
\end{equation*}
where
\begin{align*}
    &T_{n,1}= \frac{1}{n^{1/2}\tau_n}\sum_{i=1}^n g_1(X_i),
    &T_{n,2}= \frac{r-1}{n^{1/2}(n-1)\tau_n}\sum_{i<j}g_2(X_i,X_j), \ 
    &R_{n} =  \frac{\tnhat - T_n}{\sigma_n}.
   % & R_{n,1} = \text{Linear part of } \frac{\tnt - T_n}{\sigma_n},\\
\end{align*}


%It is not hard to check that our modified version of $\tilde{T}_n$ decomposition and $\psi_{G(n)}(t)$ satisfy the same conditions of Essen's Smoothing Lemma as $\psi_{\tilde{G}(n)}(t)$ in the above literature for Proposition~\ref{prop:ew} to hold. 
 We will begin by bounding $R_n$. Similar to the theory for U-statistics, the behavior is largely determined by a linear term.

Let:
\begin{equation*}\label{eq:linear-bern}
    R_{n,1} = \text{Linear part of } \frac{\tnhat - T_n}{\sigma_n}.
\end{equation*}
where the linear part has the form:
\begin{align*}
R_{n,1} = \frac{1}{{n \choose 2 }}\sum_{i<j} c_{ij} \left\{A_{ij} - \E(A_{ij} \mid  X_i, X_j) \right\}
\end{align*}
for $c_{ij} = c_{ij}(X_i,X_j,\rho_n) \asymp \rho_n^{-1}n^{-1/2}$ defined in Section 7 of the above reference.   Theorem 3.1(b) of the above authors establishes that:     

\begin{equation*}%\label{eq:rn-rn1}
     R_{n}- R_{n,1}= O_P( \mathcal{M}(n,\rho_n,R)),
\end{equation*}
% where $\mathcal{M}(n,\rho_n,R)$ 
% where
% \begin{equation*}
%      \mathcal{M}(\rho_n,)= \left\{\begin{array}{cc}
%         \rho_n^{-1} n^{-1}  & R \text{ is acyclic} \\
%         \rho_n^{-\frac{p}{2}}n^{-1} & R \text{ is cyclic}
%      \end{array}\right. .
% \end{equation*}
Under the assumed sparsity conditions, given $\mathbf{X}$, the distribution of $R_{n,1}$ permits the following (uniform) approximation by a Gaussian-distributed variable $Z_n$:
% \rd under the condition for $\rho_n$ in Assumption~\ref{ass:sparse} %Theorem~\ref{thm:ew-sd} \bk 
% according to the same paper, 
\begin{equation*}%\label{eq:rn1-zn}
    \sup_{u} \bigg{|}F_{R_{n,1}|X}(u)-F_{Z_n} \bigg{|}=O_P\left(\frac{1}{\rho_n^{1/2}n}\right),
\end{equation*}
where $Z_n\sim N(0,\frac{\sigma_w^2}{n\rho_n})$ and $\sigma_w^2$ is defined as the variance of Eq~\ref{eq:linear-bern}. Note that $\sigma_w \asymp 1$ when $n \xrightarrow[]{} \infty$.

Now to prove our theorem, we will show the three equations below. 
\begin{equation}\label{eq:decomp1}
    \sup_{u} \bigg{|}F_{\tnt}(u)-F_{T_{n,1}+T_{n,2}+R_n} \bigg{|}=O\left( \mathcal{M}(n,\rho_n,R)\right),
\end{equation}
\begin{equation}\label{eq:decomp2}
    \sup_{u} \bigg{|}F_{T_{n,1}+T_{n,2}+R_n}(u)-F_{T_{n,1}+T_{n,2}+ Z_n} \bigg{|}=O\left(\frac{1}{\rho_n^{1/2}n}\right),
\end{equation}
\begin{equation}\label{eq:decomp3}
    \sup_{u} \bigg{|}F_{T_{n,1}+T_{n,2}+ Z_n}-G_n(x) \bigg{|}=O\left(\frac{1}{n}\right),
\end{equation}

We prove Eq~\ref{eq:decomp3} using Esseen’s smoothing lemma from Section XVI.3 in \cite{feller-vol-2},
\begin{equation}\label{eq:essensmoothing}
\begin{split}
     &\sup_{u} \bigg{|}F_{T_{n,1}+T_{n,2}+ Z_n}(u)-G_n(x) \bigg{|} \\&\leq c_1\int_{-\gamma}^{\gamma}\frac{1}{t} \bigg{|}\psi_{F_{T_{n,1}+T_{n,2}+ Z_n}}(u) - \psi_{G_n}(t)  \bigg{|}dt + c_2 \sup_u\frac{G_n'(u)}{\gamma},
\end{split}
\end{equation}
where $\psi$ is the characteristic function. $\gamma$ is set to $n$. We omit the proof here as it is not hard to check by breaking the integral into $|t| \in (0,n^{\epsilon})$,$(n^{\epsilon},n^{1/2})$ and $(n^{1/2},n)$. Using similar arguments as Lemma 8.3 of \cite{zhang-xia-network-edgeworth}, we have Eq~\ref{eq:essensmoothing} and thus Eq~\ref{eq:decomp3} hold for our characteristic function in Proposition~\ref{lm:chf_g}.  It is also not hard to check that, using similar arguments of the above reference, under Assumption~\ref{ass:sparse}, Eq~\ref{eq:decomp1} and  Eq~\ref{eq:decomp2} hold given Eq~\ref{eq:decomp3}.
\end{proof}
\bk


\iffalse
\section{Proof of Proposition~\ref{prop:ew}}
\label{sec:suppprop3}
 In what follows, we derive an Edgeworth expansion for a standardized count functional.  Our argument here is closely related to \rd \cite{zhang-xia-network-edgeworth}\bk, but we present it for completeness. 
\begin{proof}\normalfont
% \cite{zhang-xia-network-edgeworth} have showed that $\tnt$ can be decomposed into the following form
Consider the following decomposition:
\begin{equation}\label{eq:tnt-decomp}
    \tilde{T}_n:=\frac{\hat{T}_n-\mu_n}{\sigma_n} = \frac{T_n-\mu_n}{\sigma_n}+ \frac{\tnhat - T_n}{\sigma_n}= T_{n,1}+T_{n,2}  + O_P\left(\frac{1}{n} \right)+ R_n,
\end{equation}
where
\begin{align*}
    &T_{n,1}= \frac{1}{n^{1/2}\tau_n}\sum_{i=1}^n g_1(X_i),
    &T_{n,2}= \frac{r-1}{n^{1/2}(n-1)\tau_n}\sum_{i<j}g_2(X_i,X_j), \ 
    &R_{n} =  \frac{\tnhat - T_n}{\sigma_n}.
   % & R_{n,1} = \text{Linear part of } \frac{\tnt - T_n}{\sigma_n},\\
\end{align*}
 We will begin by bounding $R_n$.  \bl [blue - propose to cut] [Theorem 3.1(b) of  \cite{zhang-xia-network-edgeworth} establishes a central limit theorem for $(\tnt - T_n)/\sigma_n$; ] \bk Similar to the theory for U-statistics, the behavior is largely determined by a linear term.

Let:
\begin{equation*}\label{eq:linear-bern}
    R_{n,1} = \text{Linear part of } \frac{\tnhat - T_n}{\sigma_n}.
\end{equation*}
where the linear part has the form:
\begin{align}
R_{n,1} = \frac{1}{{n \choose 2 }}\sum_{i<j} c_{ij} \left(A_{ij} - \E[A_{ij} \mid X_i, X_j] \right)
\end{align}
for $c_{ij} = c_{ij}(X_i,X_j,\rho_n) \asymp \rho_n^{-1}n^{-1/2}$ defined in Section 7 of the above reference.   Theorem 3.1(b) of the above authors establishes that:     

\begin{equation}\label{eq:rn-rn1}
     R_{n}- R_{n,1}= O_P( \mathcal{M}(n,\rho_n,R)),
\end{equation}
% where $\mathcal{M}(n,\rho_n,R)$ 
% where
% \begin{equation*}
%      \mathcal{M}(\rho_n,)= \left\{\begin{array}{cc}
%         \rho_n^{-1} n^{-1}  & R \text{ is acyclic} \\
%         \rho_n^{-\frac{p}{2}}n^{-1} & R \text{ is cyclic}
%      \end{array}\right. .
% \end{equation*}
Under the assumed sparsity conditions, given $\mathbf{X}$, the distribution of $R_{n,1}$ permits the following (uniform) approximation by a Gaussian-distributed variable $Z_n$:
% \rd under the condition for $\rho_n$ in Assumption~\ref{ass:sparse} %Theorem~\ref{thm:ew-sd} \bk 
% according to the same paper, 
\begin{equation}\label{eq:rn1-zn}
    \sup_{u} \bigg{|}F_{R_{n,1}|X}(u)-F_{Z_n} \bigg{|}=O_P\left(\frac{1}{\rho_n^{1/2}n}\right),
\end{equation}
where $Z_n\sim N(0,\frac{\sigma_w^2}{n\rho_n})$ and $\sigma_w^2$ is defined as the variance of Eq~\ref{eq:linear-bern}. Note that $\sigma_w \asymp 1$ when $n \xrightarrow[]{} \infty$.

Now to prove our theorem, we will show the three equations below. 
\begin{equation}\label{eq:decomp1}
    \sup_{u} \bigg{|}F_{\tnt}(u)-F_{T_{n,1}+T_{n,2}+R_n} \bigg{|}=O\left(\rd \mathcal{M}(\rho_n,n)\bk\right),
\end{equation}
\begin{equation}\label{eq:decomp2}
    \sup_{u} \bigg{|}F_{T_{n,1}+T_{n,2}+R_n}(u)-F_{T_{n,1}+T_{n,2}+ Z_n} \bigg{|}=O\left(\frac{1}{\rho_n^{1/2}n}\right),
\end{equation}
\begin{equation}\label{eq:decomp3}
    \sup_{u} \bigg{|}F_{T_{n,1}+T_{n,2}+ Z_n}-G_n(x) \bigg{|}=O\left(\frac{1}{n}\right),
\end{equation}


We first prove eq~\ref{eq:decomp1} and Eq~\ref{eq:decomp2} by assuming Eq~\ref{eq:decomp3} holds. 

%  We proceed by stating following lemma, which is closely related to the proof of Lemma 8.2 of \cite{zhang-xia-network-edgeworth}.  A proof is omitted, as it closely follows the proof of (8.32), pg 42 of the above reference. 
\begin{lemma}
Suppose that Eq~\ref{eq:decomp3} holds. Then, $F_{T_{n,1}+T_{n,2}+Z_n}(u)$ is Lipschitz.
\end{lemma}
The proof is omitted since it is closely related to the proof of Lemma 8.2 of \rd\cite{zhang-xia-network-edgeworth}\bk.
% \begin{proof}\normalfont
% % \text{Proof of $F_{T_{n,1}+T_{n,2}+Z_n}(u)$ is Lipschitz assuming eq~\ref{eq:decomp3} holds.}
% We have that:
% \begin{align*}
%     &P(T_{n,1}+T_{n,2}+ Z_n \leq u+a) - P(T_{n,1}+T_{n,2}+ Z_n \leq u) \\
%     & \leq |P(T_{n,1}+T_{n,2}+ Z_n \leq u+a)- G_n(u+a)|  + |G_n(u+a)-G_n(u)| \\ & + |G_n(u)-P(T_{n,1}+T_{n,2}+ Z_n \leq u) |,
% \end{align*}
% when Eq~\ref{eq:decomp3} holds, the first term and the third term is $O(\frac{1}{n})$ and the second term is less than equal to $Ma$, $M$ is a constant. Then the inequality above can be continued as
% \begin{align*}
%     P(T_{n,1}+T_{n,2}+ Z_n \leq u+a) - P(T_{n,1}+T_{n,2}+ Z_n \leq u) \leq Ma + O\left(\frac{1}{n} \right).
% \end{align*}

% % Thus, $F_{T_{n,1}+T_{n,2}+Z_n}(u)$ is Lipschitz assuming eq~\ref{eq:decomp3} holds.
% \end{proof}

Now \rd [applying this lemma from the above authors and] \bk continuing with our proof, since $R_n-Z_n=R_n-R_{n,1}+R_{n,1}-Z_n= O_P(\mathcal{M}(n,\rho_n R))$ and $F_{T_{n,1}+T_{n,2}+Z_n}(u)$ is Lipschitz, \bl [cut] [applying lemma 8.2 of \cite{zhang-xia-network-edgeworth}\bk, we have
\begin{equation}
    \sup_u  \bigg{|}F_{T_{n,1}+T_{n,2}+R_n}(u)-F_{T_{n,1}+T_{n,2}+Z_n}(u) \bigg{|} = O_P\left(\mathcal{M}(n, \rho_n, R) \right),
\end{equation}
which proves Eq~\ref{eq:decomp2}.\\
\\
Using  Eq~\ref{eq:tnt-decomp}, Eq~\ref{eq:rn-rn1} and Eq~\ref{eq:rn1-zn}, we have
\begin{equation*}
    \tnt = T_{n,1}+T_{n,2} + Z_n + O_P\left(\frac{1}{n\rho_n^{1/2}}\right) + O_P\left(\frac{1}{n}\right)+ O_P(\mathcal{M}(n, \rho_n, R) ).
\end{equation*}
Applying the same lemma to $\tnt$ and $T_{n,1}+T_{n,2}+Z_n$ gives us
\begin{equation}\label{eq:decomp1-intermediate1}
    \sup_u  \bigg{|}F_{\tnt}(u)-F_{T_{n,1}+T_{n,2}+Z_n}(u) \bigg{|} = O_P\left(\mathcal{M}(n, \rho_n, R) \bk\right).
\end{equation}

Combining Eq~\ref{eq:decomp2} and Eq~\ref{eq:decomp1-intermediate1}, we have Eq~\ref{eq:decomp1},
\begin{align*}
      &\sup_{u} \bigg{|}F_{\tnt}(u)-F_{T_{n,1}+T_{n,2}+R_n} \bigg{|}\\
      & \leq  \sup_u  \bigg{|}F_{\tnt}(u)-F_{T_{n,1}+T_{n,2}+Z_n(u)} \bigg{|} + 
      \sup_u  \bigg{|}F_{T_{n,1}+T_{n,2}+R_n(u)}- F_{T_{n,1}+T_{n,2}+Z_n(u)} \bigg{|}\\
      &=O\left(\mathcal{M}(n, \rho_n, R)\right). 
\end{align*}

We have proved Eq~\ref{eq:decomp1} and Eq~\ref{eq:decomp2} assuming Eq~\ref{eq:decomp3} holds. Now we prove Eq~\ref{eq:decomp3}.

We prove Eq~\ref{eq:decomp3} using Esseen’s smoothing lemma from Section XVI.3 in \cite{feller-vol-2},
\begin{equation}\label{eq:essensmoothing}
\begin{split}
     &\sup_{u} \bigg{|}F_{T_{n,1}+T_{n,2}+ Z_n}(u)-G_n(x) \bigg{|} \\&\leq c_1\int_{-\gamma}^{\gamma}\frac{1}{t} \bigg{|}\psi_{F_{T_{n,1}+T_{n,2}+ Z_n}}(u) - \psi_{G_n}(t)  \bigg{|}dt + c_2 \sup_u\frac{G_n'(u)}{\gamma},
\end{split}
\end{equation}
where $\psi$ is the characteristic function. $\gamma$ is set to $n$. Breaking the integral into $|t| \in (0,n^{\epsilon})$,$(n^{\epsilon},n^{1/2})$ and $(n^{1/2},n)$ and using the same arguments of lemma 8.3 part (b) and part (c) from \rd \cite{zhang-xia-network-edgeworth}\bk, we have 
\begin{equation}\label{eq:lm83pb}
    \int_{C_1n^{1/2}}^n \frac{E[e^{it(T_{n,1}+T_{n,2}+ Z_n)}]}{t} dt = O_P(n^{-1}),
\end{equation}
\begin{equation}\label{eq:lm83pc}
    \int_{n^{\epsilon}}^{C_1n^{1/2}} \frac{E[e^{it(T_{n,1}+T_{n,2}+ Z_n})]}{t} dt = O_P(n^{-1}),
\end{equation}
for small enough constant $C_1$, and $\rho_n \leq c_\rho(\log n)^{-1}$ for small enough $c_\rho$. \bk

Now we only need to prove similar arguments of their part (a) and (d) to our $G_n(u)$ defined in \ref{eq:edgeworth-gn}. We want to show our $G_n(u)$ satisfies that 
\begin{equation}\label{eq:lm83pa}
    \int_{n^{\epsilon}}^{n} \bigg{|}\frac{\psi_{G_n}(t)}{d} \bigg{|}dt=O_P\left(\frac{1}{n}\right),
\end{equation}
\begin{equation}\label{eq:lm83pd}
    \int_0^{n^{\epsilon}} \bigg{|}\frac{E[e^{it(T_{n,1}+T_{n,2}+ Z_n})]-\psi_{G_n}(t)}{t} \bigg{|}dt=O_P\left(\frac{1}{n\rho_n}\right)
\end{equation}

To prove $G_n(u)$ satisfies these conditions, we first state the form of the characteristic function of $G_n(u)$ below: 

\begin{proposition}\label{lm:chf_g}
We have:
\begin{equation*}
    \psi_{G(n)}(t):= \int e^{itu}dG_n(u)= e^{-\frac{t^2}{2}}\left(1- it^3\frac{1}{6n^{1/2}\tau_n^3}\{E[g_1^3(X_1)]+3(r-1)E[g_1(X_1)g_1(X_2)g_2(X_1,X_2)]\}\right).
\end{equation*}
\end{proposition}
% \begin{proof}\normalfont
% Denote $A=\frac{1}{6n^{1/2}\tau_n^3}\{E[g_1^3(X_1)]+3E[g_1(X_1)g_1(X_2)g_2(X_1,X_2)]\}$, then 
% \begin{equation*}
%     G_n(u)= \Phi(u) + \phi''(u)A; \ \ G_n'(u)= \phi(u)+ \phi'''(u)A.
%  \end{equation*}
%  %taking derivatives of $G_n$ with respect to $u$,
% %\begin{equation*}
% %    G_n'(u)= \phi(u)+ \phi'''(u)A.
% %\end{equation*}
% The characteristic function is thus
% \begin{equation*}
%     \psi_{G_n(u)}(t)= \int e^{itu} dG(u) = \int e^{itu}[\phi(u)-\phi'''(u)A]du .
% \end{equation*}
% Knowing $E_{\phi(u)}[e^{itu}]=e^{-\frac{t^2}{2}}$, simple algebra yields 
% \begin{equation*}
%     E_{\phi(u)}[ue^{itu}]=ite^{-\frac{t^2}{2}}; \  E_{\phi(u)}[u^3e^{itu}]=i(3t-t^3)e^{-\frac{t^2}{2}}.
% \end{equation*}
% Thus, putting them into the expression of characteristic function, we have,
% \begin{align*}
%     \psi_{G_n(u)}(t) &= e^{-\frac{t^2}{2}}- A\times \int e^{itu}\phi'''(u)du\\
%     &=  e^{-\frac{t^2}{2}}- A\times(3\int u e^{itu}\phi(u)du - \int u^3 e^{itu}\phi(u)du) \\
%     &= e^{-\frac{t^2}{2}}- A\times(3ite^{-\frac{t^2}{2}}-i(3t-t^3)e^{-\frac{t^2}{2}})\\
%     &= e^{-\frac{t^2}{2}}(1-Ait^3).
% \end{align*}
% Thus, we have established that: 
% \begin{equation*}
%     \psi_{G_n(u)}(t)= e^{-\frac{t^2}{2}}\left(1- it^3\frac{1}{6n^{1/2}\tau_n^3}\{E[g_1^3(X_1)]+3(r-1)E[g_1(X_1)g_1(X_2)g_2(X_1,X_2)]\}\right).
% \end{equation*}
% \end{proof}

Now we first verify $\psi_{G_n}$ satisfies Eq~\ref{eq:lm83pa}. Using then fact that $t^ke^{-\frac{t^2}{2}} \leq C_k$ for some constant $C_k$ depending on $k$ when $t>1$ for $k=-1,0,1,2,3,...,$, we have
\begin{equation*}
    \int_{n^{\epsilon}}^n \bigg{|}\frac{\psi_{G_n}(t)}{t} \bigg{|}dt \leq (C_{-1}+C_2)\int_{n^{\epsilon}}^\infty e^{-t^2/3}dt = O_P\left(\frac{1}{n}\right).
\end{equation*}

The rest of the proof verifies $\psi_{G_n}$ satisfies Eq~\ref{eq:lm83pd}. \bl [cut] [Similar to \cite{zhang-xia-network-edgeworth}]\bk We write $E[e^{it(T_{n,1}+T_{n,2}+ Z_n)}]$ into
\begin{equation}\label{eq:chftn1tn2zn}
    E[e^{it(T_{n,1}+T_{n,2}+ Z_n)}]=E\left[e^{it(T_{n,1}+T_{n,2})}\left\{1-\frac{\sigma_w^2t^2}{\rho_n n}+O_P\left(\frac{\sigma_w^4t^4}{\rho_n^2n^2}\right)\right\}\right]
\end{equation}
%\rd
 $\int_0^{n^{\epsilon}}\frac{\sigma_w^4t^4}{\rho_n^2n^2}t^{-1}dt=O_P(n^{-1})$ when $\rho_n=\Omega(\frac{1}{n^{1/2-\delta}})$, and $\epsilon=\delta/2$. \bk
We write  $E\left[e^{it(T_{n,1}+T_{n,2})}\right]$ into 
\begin{align}\label{eq:chftn1tn2}
    E\left[e^{it(T_{n,1}+T_{n,2})}\right]=E\left[e^{itT_{n,1}}\left\{1+itT_{n,2}+ O_P (t^2T_{n,2}^2)\right\}\right].
\end{align}
Since $T_{n,2}$ is $O_P(n^{-1/2})$, the last term $O_P\left(T_{n,2}^{*2}t^2\right))$ is $O_P(n^{-1})$, thus ignorable. From \cite{petrov2012sums} Section VI Lemma 4 \bl [cut] [and \cite{zhang-xia-network-edgeworth}]\bk, define $\phi_n(t)=E\left[e^{it\frac{g_1(X_1)}{n^{1/2}\tau_n}}\right]$, denote $\phi_n^n(t)$ as the characteristic function of $n$ independent sums of $g_1(X_i)$, $P_0,..,P_k$ are fixed polynomials of $t$, then
\begin{align*}
    &\phi_n^n(t)=e^{-\frac{t^2}{2}}\left(1-\frac{E[g_1(X_1)^3]it^3}{
    6n^{1/2}\tau_n^3}\right)+O_P(n^{-1}e^{-\frac{t^2}{4}}P_0(t))\\
    &\phi_n^{n-k}(t)=\phi_n^n(t)+O_P(n^{-1}e^{-\frac{t^2}{4}}P_k(t)).
\end{align*}
Thus, we have the first term in the RHS above is 
\begin{equation}\label{eq:chftn1tn2-p1}
    E[e^{itT_{n,1}}]= \phi_n^n(t)=e^{-\frac{t^2}{2}}\left(1-\frac{E[g_1(X_1)^3]it^3}{
    6n^{1/2}\tau_n^3}\right)+O_P(n^{-1}e^{-\frac{t^2}{4}}Poly(t)).
\end{equation}
\rd\cite{zhang-xia-network-edgeworth}\bk  gives the second term as
\begin{equation}\label{eq:chftn1tn2-p2}
\begin{split}
    E[e^{itT_{n,1}}itT_{n,2}]=e^{-\frac{t^2}{2}}\times \frac{-it^3(r-1)}{2n^{1/2}\tau_n^3}E[g_1(X_1)g_1(X_2)g_2(X_1,X_2)] \\+O_P(n^{-1}e^{-\frac{t^2}{4}}|t|Poly(t)),
\end{split}
\end{equation}
Putting back Eq~\ref{eq:chftn1tn2-p1} and Eq~\ref{eq:chftn1tn2-p2} back to Eq~\ref{eq:chftn1tn2}, we have
\begin{equation}\label{eq:chftn1tn2-final}
\begin{split}
      E\left[e^{it(T_{n,1}+T_{n,2})}\right] = e^{-\frac{t^2}{2}}&\left(1- it^3\frac{1}{6n^{1/2}\tau_n^3}[E[g_1^3(X_1)] \right.\\
      &\left.\phantom{\frac{a}{b}}+3(r-1)E[g_1(X_1)g_1(X_2)g_2(X_1,X_2)]]\right)\\
      &+ O_P(n^{-1}e^{-\frac{t^2}{4}}|t|Poly(t)).
\end{split}
\end{equation}

Finally, the integral of the remainder term in Eq~\ref{eq:chftn1tn2zn} follows same argument in \rd\cite{zhang-xia-network-edgeworth}\bk,
\begin{equation}\label{eq:chftn1tn2znrmd}
    \int_0^{n^{\epsilon}}   \bigg{|}E\left[e^{it(T_{n,1}+T_{n,2})}\frac{\sigma_w^2t^2}{\rho_n n}\right]\frac{1}{t} \bigg{|} = O(\rho_n^{-1}n^{-1}).
\end{equation}
Thus Eq~\ref{eq:lm83pd} follows from Eqs~\ref{eq:chftn1tn2zn},~\ref{eq:chftn1tn2-final},~\ref{eq:chftn1tn2znrmd} and Lemma~\ref{lm:chf_g}. We have proved that our $G_n$ satisfies  Eq~\ref{eq:lm83pa} and Eq~\ref{eq:lm83pd}.


Now combining Eqs~\ref{eq:lm83pb},~\ref{eq:lm83pc},~\ref{eq:lm83pa}, and Eq~\ref{eq:lm83pd} into Esseen's smoothing lemma (see Eq~\ref{eq:essensmoothing}) proves Eq~\ref{eq:decomp3}  under the condition $\rho_n = O_P((\log n)^{-1})$.  Then combining Eqs~\ref{eq:decomp3},~\ref{eq:decomp2},~\ref{eq:decomp1} yields Proposition~\ref{prop:ew}.
\end{proof}
\fi

 \section{Edgeworth expansion for weighted bootstrap - proofs of Theorem~\ref{thm:mbq-firstorder} and Corollary~\ref{thm:mbm-firstorder}}
 \label{sec:suppthm23}
% For any set set $S$ of $r$ nodes, $S=\{i_{1}\dots i_{r}\}$, denote $\W_S= \prod_{i \in S} \w_i$.
% Conditioned on the graph $A$ and $X$, we see that the hoeffding projections of the weighted bootstrap statistic gives: %the $X$ observed as $x$, $\tnt$ and $\hat{H}(x_i)$ for each $i$ are all observed.  $\hat{H}(x_i)$ is defined as
% \begin{equation*}
%     \begin{split}
%      &\hi= \frac{1}{{n-1 \choose r-1}}\sum_{S,i\in S}H(A_S), \\
%      &\hhij= \frac{1}{{n-2 \choose r-2}}\sum_{S,i,j\in S}H(A_S).
% \end{split}
% \end{equation*}
% Recall the definition of $\gi$ and $\gj$ from the main paper. To remind the reader, we have:

% \begin{equation*}
%     \begin{split}
%      &\gi= \frac{1}{{n-1 \choose r-1}}\sum_{S,i\in S}(H(A_S)-\tnhat), \\
%      &\ggij= \frac{1}{{n-2 \choose r-2}}\sum_{S,i,j\in S}(H(A_S)-\tnhat).
% \end{split}
% \end{equation*}

% We are interested in the Hoeffding decomposition [\rd Put eqn number from main \bk] of the following quantity. Below we derive the Hoeffding decomposition.
% %We define weighted boostrap of count statistic as $\vnhat$. Conditioned on A, Standardized $\vnhat$ can be written as follows using $\W_S=1$.
% \begin{equation}\label{eq:wb-def-vn}
%     \begin{split}
%         \frac{\vnhat-\tnhat}{\hat{\sigma}_n}&=\frac{\sum_S \W_S (\hat{H}(A_S)-\tnhat)}{{n \choose r} \hat{\sigma}_n} = \frac{\sum_S (\W_S-1)(\hat{H}(A_S)-\tnhat)}{{n \choose r} \hat{\sigma}_n} \\
%         &=\frac{r}{n\hat{\sigma}_n} \sum_i f_1(\w_i) + \frac{r(r-1)}{n(n-1)\hat{\sigma}_n} \sum_{1\leq i<j \leq n} f_2(\w_i,\w_j) + \rd R_n \bk.
%     \end{split}
% \end{equation}

% We now derive the Hoeffding projections.

% %Applying a Hoeffding decompsition to $\sum_S (\W_S-1)(\hat{H}(A_S)-\tnhat)/{n \choose r}$ above with respect to $\W$ yields

% %\begin{equation*}
% %    \begin{split}
% %       & f_1(\w_i)= E[\hat{H}(X_S,\\W_S)|\w_i,x_i]; \\
% %       & f_2(\w_i,w_j)=E[\hat{H}(X_S,\\W_S)|\w_i,x_i,\w_j,x_j].
% %    \end{split}
% %\end{equation*}
% %Equivalently , $g_1(x_i)$ and $g_2(x_i,x_j)$ can be written as 
% \begin{equation}
% \begin{split}
%     f_1(\w_i)&=E[\W_S (\hat{H}(A_S)-\tnhat)|\w_i]= (\w_i-1)(\hi-\tnhat)=(\w_i-1)\gi;\notag\\
%     f_2(\w_i,\w_j)&=E[\W_S (\hat{H}(A_S)-\tnhat)|\w_i,\w_j] \notag\\
%     &=(\w_i\w_j-\w_i-\w_j+1)(\hhij-\tnhat)\notag\\
%     &=(\w_i\w_j-1)(\hhij-\tnhat)-(\w_i-1)(\hi-\tnhat)-(\w_j-1)(\hj-\tnhat),\label{eq:wb-hp}
% \end{split}
% \end{equation}

% \rd The residual $R_n$ is essentially a sum of higher order Hoeffding projections, which are all uncorrelated. Therefore, we see that the variance of the third order term (the first one in the remainder) is $\dfrac{\sum_{ijk}  \hat{g}_3(i,j,k)^2}{\hat{\sigma}_n^2 {n\choose 3}} \times O(1/n^3)$. Note that  $\hat{g}_3(i,j,k)^2=O_P(\rho_n^{3s-3})$ for cyclic and $O_P(\rho_n^{3s-2})$ for acyclic subgraphs. This is because, for any two nonoverlapping $S,T$ (not containing $\{i,j,k\}$)  of size $r-3$, there are potentially three edges common between the subgraphs induced by $S\cup \{i,j,k\}$ and  $S\cup \{i,j,k\}$ for a cyclic subgraph, and two for an acyclic one.
% Thus we can show that the remainder is the same order as $O(\mathcal{M}(n,\rho_n,R))$.
\bk

%O\left(\frac{1}{n^{2/3-\epsilon}\rho_n}
%\rd needs to add lemma of $R_n$ is   $O_P(1/n)$ \\ \bk
%using the definition %$ \hat{H}_1(x_1)= E[\hat{H}(x_1,x_2,,,X_r)|x_1=x_1]$ and $\hat{H}_2(x_1,x_2)= E[\hat{H}(x_1,x_2,,,X_r)|x_1=x_1,x_2=x_2]$.

%We are now ready to present out theorem.

% \begin{theorem}
% Define
% \begin{equation*}
%     \gnhat(u) = \Phi(u) -\frac{(u^2-1)\phi(u)}{6n^{1/2}\hat{\tau}_n^3}\left[ \widehat{g_1}^3 + 3(r-1) \text{\ \stackon[-8pt]{$g_1(i)g_1(j)g_2(i,j)$}{\vstretch{1.5}{\hstretch{9.0}{\widehat{\phantom{\;}}}}}}\ \right],
% %\widehat{g_1(i)g_1(j)g_2(i,j)})\right]
% \end{equation*}
% where
% \begin{equation*}
% \begin{split}
%      &\text{ \stackon[-6pt]{$g_1^3$}{\vstretch{1}{\hstretch{2.0}{\widehat{\phantom{\;}}}}}}= \frac{1}{n}\sum_{i=1}^n (\hi - \tnhat)^3, \\
%      &\text{ \stackon[-8pt]{$g_1(i)g_1(j)g_2(i,j)$}{\vstretch{1.5}{\hstretch{13.0}{\widehat{\phantom{\;}}}}}}=\frac{1}{{n \choose 2}}\sum_{1 \leq i<j\leq n}(\hhij-\tnhat)(\hi -\tnhat)(\hj -\tnhat). %\rd \times \frac{n}{n-1}\bk.
% \end{split}
% \end{equation*}
%With probability tending to one, we have,
%$$\sup_u\left|P^*\left(\frac{\vnhat-\tnhat}{\shat}\leq u\right)-\gnhat(u)\right|=O\left(\frac{\log n}{n^{2/3}\rho_n}\right),$$
%where $P^*(.)$ simply defines the conditional probability of event (.) conditioned on $A$ and $X$.
%\end{theorem}

Using Eq~(10), we express our quadratic bootstrap statistic as:
\begin{align}\label{eq:cfbqform}
    \cfbq=\frac{\sum_i (\w_i-1)\gi}{n^{1/2}\hat{\tau}_n} +  &\frac{(r-1)\sum_{1\leq i <j \leq n}(\w_i\w_j-\w_i-\w_j+1) \tilde{g}_2(i,j)}{n^{1/2}(n-1)\hat{\tau}_n}  
\end{align}
We will first prove Theorem~\ref{thm:mbq-firstorder}. However in order to prove it we state a slightly different version of Theorem 3.1 in~\cite{wang-jing-weighted-bootstrap-u-statistics}\bk. The main difference is that one condition in the original lemma is not fulfilled in our case.  In particular, Bernoulli noise with $\rho_n \rightarrow 0$ blows up some terms that are needed to bound the error associated with the Edgeworth expansion.  However, a thorough examination reveals that the argument carries through with some modifications. \bk  %causes some issues, since in the original proof $l_{4,n}$ is bounded. A thorough examination shows however that the final error is scaled by a factor of $l_{4,n}$. This includes $|K_{2,n}|, I_{1,n}, I_{3,n}$ and $I_{4,n}$. We may therefore replace $l_{4}$ with the sequence $l_{4,n}$. 


Let
\begin{subequations}
\begin{align}\label{eq:alldefswangjing}
    \kn&=\frac{1}{n^{3/2}B_n^2}\sum_{1\leq i<j\leq n} b_{ni} b_{nj}  d_{nij}\E\{\y_1\y_2\psi(\y_1,\y_2)\}\\
    \lnone(x)&=\sum_{j=1}^n \left\{\E\Phi(x- b_{nj}\y_j/B_n)-\Phi(x)\right\}-\frac{1}{2}\Phi''(x)\\
    \lntwo(x)&=-\kn\Phi'''(x)\\
      E_{2n}(x)&= \Phi(x) + \lnone(x) + \lntwo(x),
\end{align}
\end{subequations}

\begin{lemma}\label{lem:wangjing}
Consider the following expression.
\begin{align}\label{eq:wangjingdecomp}
    V_n=\frac{1}{B_n}\sum_j  b_{nj} \y_j+\frac{1}{n^{3/2}} \sum_{i < j}   d_{nij} \psi(\y_i,\y_j),
\end{align}
where $B_n^2=\sum_j b_{nj}^2$. Let $\beta:=\E(|\y_1|^3)$ and $\ro=\E \{\psi^2(\y_1,\y_2)\}$, and let $\E(\y_1)=0$, $\E(\y_1^2)=1$ and  $\kappa(X_1)>0$ . Furthermore, let $\E\{\psi(\y_1,\y_2)\mid \y_t\}=0$ for all $1\leq t\leq n$.
For some constants $\ell_1$, $\ell_2$, $\ell_3$ the sequence $b_{n,i}$ satisfies %and $d_{n,ij}$ satisfies 
\begin{equation}\label{eq:wb-conds}
    \begin{split}
    &\frac{1}{n}\sum_{i=1}^n b_{n,i} ^2 \geq l_1 >0, \ \ \frac{1}{n}\sum_{i=1}^n |b_{n,i}| ^3 \leq l_2 \leq \infty, \\
%    &\frac{1}{mn}\sum_{i=1}^m\sum_{j=1,j\neq i}^{n} d_{n,ij}^2 \leq l_{4,n} \ \text{For any $m\geq 1$}
    \end{split}
\end{equation}

Furthermore, define $\alpha_{i}:=\frac{1}{n}\sum_{j\neq i} d_{nij}^2$.
and for sufficiently large $k$, define:
\begin{align}
    \label{eq:ddef}
    l_{4,n}=\frac{1}{n}\sum_{i=1}^n\alpha_{i}, \ \ \ \ s_n^2=\frac{1}{n}\sum_i\alpha_i^2-(l_{4,n})^2, \ \ \ \ l_{5,n} = l_{4,n} + k s_n
\end{align}


%Redoing of Theorem 3.1 in~\cite{wang-jing-weighted-bootstrap-u-statistics} when condition on $d_{nij}'s$ is not satisfied.
 If $\beta,\kappa(\y_1)$ and $\ro$ are bounded, then,
% \rd There exists
% a large enough constant $k$ independent of $n$ such that:\bk
\begin{align*}
    \sup_x|P(V_n\leq x)-E_{2n}(x)|= O\left(\frac{ l_{5,n}\log n}{n^{2/3}}\right),
\end{align*}

\end{lemma}


\iffalse
\begin{lemma}\label{lem:wangjing}
Consider the following expression.
\begin{align}\label{eq:wangjingdecomp}
    V_n=\frac{1}{B_n}\sum_j  b_{nj} \y_j+\frac{1}{n^{3/2}}  \sum_{i < j} \bk  d_{nij} \psi(\y_i,\y_j),
\end{align}
where $B_n^2=\sum_j b_{nj}^2$. Let $\beta:=\E(|\y_1|^3)$ and $\ro=\E [\psi^2(\y_1,\y_2)]$, and let $\E[\y_1]=0$, $\E[\y_1^2]=1$ and  $\kappa(X_1)>0$ \bk. Furthermore, let $\E[\psi(\y_1,\y_2)\mid \y_t]=0$ for all $1\leq t\leq n$.
For some constants $\ell_1$, $\ell_2$, $\ell_3$ and $l_{4,n}$, the sequence $b_{n,i}$ and $d_{n,ij}$ satisfies 
\begin{equation}\label{eq:wb-conds}
    \begin{split}
    &\frac{1}{n}\sum_{i=1}^n b_{n,i} ^2 \geq l_1 >0, \ \ \frac{1}{n}\sum_{i=1}^n |b_{n,i}| ^3 \leq l_2 \leq \infty, \\
    &\frac{1}{mn}\sum_{i=1}^m\sum_{j=1,j\neq i}^{n} d_{n,ij}^2 \leq l_{4,n} \ \text{For any $m\geq 1$}
    \end{split}
\end{equation}
%Redoing of Theorem 3.1 in~\cite{wang-jing-weighted-bootstrap-u-statistics} when condition on $d_{nij}'s$ is not satisfied.
If $\beta,\kappa(\y_1)$ and $\ro$ are bounded, we have:
\begin{align*}
    \sup_x|P(V_n\leq x)-E_{2n}(x)|= O\left(\frac{l_{4,n}\log n}{n^{2/3}}\right),
\end{align*}
\end{lemma}
\fi
  Intuitively, arguments for establishing rates of convergence for the Edgeworth expansions require comparing the characteristic function of the random variable of interest with the Fourier transform of the Edgeworth expansion.  To this end, the respective integrals are broken up into several pieces.  The bounds required in  (\ref{eq:wb-conds}) are used to estimate the error of the Edgeworth expansion in some of these steps, but appear as constants and are suppressed in the Big-O notation.  

On the other hand, as previously mentioned, it turns out that certain terms that appear as constants in \cite{wang-jing-weighted-bootstrap-u-statistics} blow up when perturbed by sparse network noise and appear in the rate.  In particular, the term $l_{5,n}$ arises from needing to bound $\frac{1}{m}\sum_{i=1}^m \alpha_i$ for all $m \leq M$ for some $M$ large enough.  

Since the data is fixed,  we may view $\alpha_1, \ldots, \alpha_n$ as constants. We therefore have the liberty of choosing a ``good set" in which $\alpha_i$ are well-behaved.  Without loss of generality, we may label these elements $\{\alpha_1, \ldots, \alpha_M\}$; the corresponding multiplier random variables are still independent. Even when there is no randomness, it turns out that a large proportion of $\{\alpha_1, \ldots \alpha_n\}$ must be within $k$ sample standard deviations of the sample mean $l_{4,n}$ for $k$ large enough. This observation, which we believe is novel in the bootstrap setting, allows us to establish a tight bound for $\frac{1}{m}\sum_{i=1}^m \alpha_i$ for all $m \leq M$.  We state this lemma below.   
% Before bounding this term, we will state and proof a lemma involving deviations of constants from a sample mean.  Our lemma is closely related to concentration of sums sampled without replacement from a finite population. In fact, it implies the without-replacement Chebychev inequality; see, for example, Corollary 1.2 of \citet{serfling-concentration-without-replacement}.  We will then use this lemma to construct a ``good set" for which $\alpha_i$ are well-behaved. 
%
\begin{lemma}
\label{lemma:deterministic-deviation-identity}
Let $x_1 ,\ldots, x_n$ be constants in $\mathbb{R}$ and let $\bar{x}_n = \frac{1}{n}\sum_{i=1}^n x_i$ and $s_n^2 = \frac{1}{n}\sum_{i=1}^n (x_i - \bar{x})^2$  Define the set:
\begin{align*}
    \Gamma_k =  \left\{x_i \geq \bar{x}_n + k s_n  \right\}
\end{align*}
Then,
\begin{align*}
|\Gamma_k| \leq \frac{n}{k^2} 
\end{align*}
\end{lemma}
\begin{proof}\normalfont
Observe that:
\begin{align*}
s_n^2 &\geq \frac{1}{n}\sum_{i \in \Gamma_k} (x_i-\bar{x}_n)^2
\\ &\geq \frac{1}{n}\sum_{i \in \Gamma_k} k^2 s_n^2  \implies  |\Gamma_k | \leq \frac{n}{k^2}  
\end{align*}
\end{proof}

\begin{remark}
Our lemma is closely related to concentration of sums sampled without replacement from a finite population. In fact, it implies the without-replacement Chebychev inequality; see, for example, Corollary 1.2 of \citet{serfling-concentration-without-replacement}.
\end{remark}

%
We will show that $\cfbq$ can be written as Eq~\ref{eq:wangjingdecomp}, with carefully chosen $\{ b_{ni}\}$ and $\{ d_{nij}\}$'s. We now present some accompanying Lemmas to show that Eq~\ref{eq:wb-conds} is satisfied with probability tending to 1. Proofs of Lemmas~\ref{lem:wangjing},~\ref{lem:proveconv},
% ~\ref{lem:proveconv2}
and~\ref{lem:thirdabsmoment} are provided in following subsections.

% \begin{lemma}\label{lem:proveconv2}
% Under the sparsity assumptions in Assumption~\ref{ass:sparse}, we show that, for large enough $C$, 
% \begin{align*}
% P\left(\max_i \sum_{j\neq i}\tilde{g}_2(i,j)^2/n\geq C\rho_n^{2s-1}\right)\rightarrow 1
%   %  P\left(\frac{\sum_{i=1}^m\sum_{j\neq i} |\ggij/\tau_n|^2}{mn}\leq n^{\epsilon}/\rho_n\right)&\rightarrow 1
% %   P\left(\frac{\sum_i |\gi|^3}{n\rho_n^s}\right)&\leq c\right)\rightarrow 1\\
% \end{align*}
% \end{lemma}
We present some useful results shown in \cite{zhang-xia-network-edgeworth} which we will use later in proofs of our theorems. 
\begin{lemma}\label{lem:moments-z/x}
Let $\hat{\tau}_n^2=\sum_i \gi^2/n$.  
We have, 
\begin{enumerate}
	\item For acyclic graphs, if $n\rho_n\rightarrow \infty$, and for cyclic graphs, if  $n\rho_n^r\rightarrow\infty$, from \cite{zhang-xia-network-edgeworth} Lemma 3.1 and its proof, we have:
	\begin{align}
	\frac{\hat{\tau}_n^2}{\tau_n^2}&=1+O_P\left(\frac{1}{n\rho_n}\right)+O_P\left(\frac{1}{\sqrt{n}}\right)\\
	E(|\gi-g_1(X_i)|/\rho_n^s)^2&=O(1/n\rho_n)
	\end{align}
	\item Under Assumption~\ref{ass:sparse}, we have
\begin{align}\label{eq:zxempiricalg13}
\left|\frac{\sum_j \hat{g}_1(i)^3}{n}-\E\{g_1(X_1)^3\}\right|=O_P\left(\rho_n^{3s-0.5}n^{-1/2}\right),
\end{align}
\begin{align}\label{eq:zxempiricalg1g1g2}
\left|\frac{\sum_{i<j} \gi\gj\ggij}{{n\choose 2}}-\E\{g_1(X_1)g_1(X_2)g_2(X_1,X_2)\}\right|=O_P\left(\rho_n^{3s-0.5}n^{-1/2}\right),
\end{align}
and
%\rd [This sounds wrong]
\begin{align}\label{eq:tauhaterr}
|\hat{\tau}_n^3-\tau_n^3|=O_P(\rho_n^{3s}/n^{1/2}).
\end{align}
\end{enumerate}

%We have $\hat{\tau}$ is $\Theta(\rho_n^s)$ and 



%We have $\hat{g}_1(i)$ converges to $g_1(i)$ with $\hat{g}_1(i)-g_1(i)=O_p(\rho_n^{s-0.5}/n^{1/2})$. We also have  $\sum_i\left(\frac{\gi}{\rho_n^s}\right)^2/n$ converges to a positive constant, and
\iffalse
and 
\begin{align}\label{eq:zxempiricalg13}
    \left|\frac{\sum_j \hat{g}_1(i)^3}{n}-\E\{g_1(X_1)^3\}\right|=O_P\left(\rho_n^{3s-0.5}n^{-1/2}\right),
\end{align}
\begin{align}\label{eq:zxempiricalg1g1g2}
    \left|\frac{\sum_{i<j} \gi\gj\ggij}{{n\choose 2}}-\E\{g_1(X_1)g_1(X_2)g_2(X_1,X_2)\}\right|=O_P\left(\rho_n^{3s-0.5}n^{-1/2}\right).
\end{align}
\fi
\iffalse
\begin{align}\label{eq:zxempirical}
    &\max\left\{\left|\frac{\sum_j \hat{g}_1(i)^3}{n}-\E\{g_1(X_1)^3\}\right|,\right.\notag\\
    &\left.\left|\frac{\sum_{i<j} \gi\gj\ggij}{{n\choose 2}}-\E\{g_1(X_1)g_1(X_2)g_2(X_1,X_2)\}\right|\right\}\notag\\
    &=O_P\left(\rho_n^{3s}n^{1/2}\mzx\right),
\end{align}
\fi
\end{lemma}



 \begin{lemma}\label{lem:proveconv-mean}
 Under the sparsity assumptions in Assumption~\ref{ass:sparse}, for large enough $C$, 
 \begin{align*}
 P\left(\frac{1}{n^2}\sum_i \sum_{j\neq i}\tilde{g}_2(i,j)^2\geq C\rho_n^{2s-1}\right)\rightarrow 1
   %  P\left(\frac{\sum_{i=1}^m\sum_{j\neq i} |\ggij/\tau_n|^2}{mn}\leq n^{\epsilon}/\rho_n\right)&\rightarrow 1
 %   P\left(\frac{\sum_i |\gi|^3}{n\rho_n^s}\right)&\leq c\right)\rightarrow 1\\
 \end{align*}
 \end{lemma}


\begin{lemma}\label{lem:proveconv}
Under the sparsity conditions in Assumption~\ref{ass:sparse} and for some arbitrary $\epsilon>0$,
\begin{align*}
    P\left(\frac{\sum_i |\gi/\rho_n^s|^3}{n}\leq c\right)&\rightarrow 1\\
    P\left(\frac{\sum_i |\gi/\rho_n^s|^2}{n}\geq c'\right)&\rightarrow 1,
%    P\left(\frac{\sum_i |\hhij/\shat|^2}{n}\geq c''\right)&\rightarrow 1\\
%   P\left(\frac{\sum_i |\gi|^3}{n\rho_n^s}\right)&\leq c\right)\rightarrow 1\\
\end{align*}
for positive constants $c,c'$ not depending on $n$.
\end{lemma}
%We will first show that, conditioned on the data, the CDF $\cfbq$ matches the asymptotic expansion in Pro~\ref{thm:ew-sd}. However the moments are replaced by their empirical counterparts. 
%Now we want to show 
%\begin{equation*}
%    \sup_u |F_{\tnas+\tnbs}(u)-\hat{G}_n(u)|= o(n^{-1/2}).
%\end{equation*}
%We begin by rewriting $\tnas+\tnbs$.
\begin{lemma}\label{lem:thirdabsmoment}
Let $\w_1$ be generated from the Gaussian product distribution. We have $\E|\w_1-1|^3<\infty$. 
\end{lemma}
Now we are ready to provide the proof.
\begin{proof}\normalfont[ of Theorem~\ref{thm:mbq-firstorder}]
It is easy to see from Eq~\ref{eq:cfbqform} that $\cfbq$ can be expressed as:

\iffalse
%Note also that, by construction we have $$ (see~\cite{Bentkus-edgeworth-symmetric}), $f_1$ and $f_2$ satisfies
\begin{align*}
    & E[f_1(\w_1) f_2(\w_1,\w_2)]=0\\
    & E[f_1(\w_1)^2 f_2(\w_1,\w_2)]=0.
\end{align*}
Thus, $\tnas+\tnbs$ can be written into a form which has been shown to be first order correct in~\rd \cite{wang-jing-weighted-bootstrap-u-statistics}\bk, Theorem 3.1.
\fi
\begin{equation*}
\begin{split}
     %\tnas + \tnbs &= \frac{1}{n^{1/2}\hat{\tau}_n}\sum_i (\w_i-1)(\hi -\tnhat) + ...\\ &\frac{r-1}{n^{1/2}(n-1)\hat{\tau}_n} \sum_{1\leq i <j \leq n}(\w_i\w_j-\w_i-\w_j+1) (\hhij-\tnhat) \\
     \cfbq& = \frac{\sum_i b_{n,i}\y_i }{B_n} + \frac{1}{n^{1/2}(n-1)}\sum_{1\leq i <j \leq n} \psi(\y_i,\y_j)d_{n,ij},
\end{split}
\end{equation*}
where we have:
\begin{subequations}\label{eq:wangjingbd}
\begin{align}
&\y_i=\w_i-1 ,\\
    &b_{n,i}= \frac{\gi}{\rho_n^s}, \\
     &B_n^2= \sum_{i=1}^n b_{n,i}^2,\\
    &d_{n,ij}= \frac{r-1}{\hat{\tau}_n}\tilde{g}_2(i,j) \times \frac{n}{n-1},\\
    &\psi(\w_i,\w_j)=\w_i\w_j-\w_i-\w_j+1.
\end{align}
\end{subequations}
\iffalse
\begin{equation*}
\begin{split}
    &b_{n,i}= \frac{\hi - \tnhat}{\rho_n^s}, \\
     &B_n^2= \sum_{i=1}^n b_{n,i}^2,\\
    &d_{n,ij}= \frac{r-1}{\hat{\tau}_n}(\hhij -\tnhat) \times \frac{n}{n-1}, \\
    &\psi(\w_i,\w_j)=\w_i\w_j-\w_i-\w_j+1.
\end{split}
\end{equation*}
\fi
Note that since $\hat{\tau}_n^2=\sum_i \gi^2/n$. Thus we use $B_n^2=n\hat{\tau}_n^2/\rho_n^{2s}$. Thus, $B_n^2=\sum_i b_{n,i}^2$. Furthermore, Lemma~\ref{lem:thirdabsmoment} shows that our $\w_i-1$ random variables have finite $\E\{|\xi_i-1|^3\}$.

Lemma~\ref{lem:proveconv} shows that the conditions in Eq~\ref{eq:wb-conds} are satisfied on a high probability set of $A,X$. 

\iffalse
In order to use Theorem 3.1, we need the following conditions. For some constant $l_1$, $l_2$, $l_3$ and $l_4$, the sequence $b_{n,i}$ and $d_{n,ij}$ satisfies 
\begin{equation}\label{eq:wb-conds}
    \begin{split}
    &\frac{1}{n}\sum_{i=1}^n b_{n,i} ^2 \geq l_1 >0, \ \ \frac{1}{n}\sum_{i=1}^n |b_{n,i}| ^3 \leq l_2 \leq \infty, \\
    &\frac{1}{mn}\sum_{i=1}^m\sum_{j=1,j\neq i}^{n} d_{n,ij}^2 \leq l_4 \  \text{For any $m\geq 1$}
    \end{split}
\end{equation}
Now we will show that the conditions in Theorem 3.1 are satisfied with high probability. 
\fi 

Using Lemma~\ref{lem:proveconv}, we see that the first two conditions in Eq~\ref{eq:wb-conds} are satisfied with probability tending to one under Assumption~\ref{ass:sparse}. Since $B_n^2/n=\sum_i b_{n,i}^2/n$ converges to a positive constant (see Lemma~\ref{lem:moments-z/x})%\cite{zhang-xia-network-edgeworth,network-jackknife-theory}\bk)
, the first condition holds. 
 Now, we need to bound $\ell_{4,n}$ and $s_n$ as defined Eq~\ref{eq:ddef}. First, %let $\alpha_{n,i}:=\sum_{j\neq i} \tilde{g}_2(i,j)^2/n\hat{\tau}_n$.
 let $\beta_{n,i}:=\sum_{j\neq i} \tilde{g}_2(i,j)^2/n$ and $\bar{\beta}_n=\sum_i\beta_{n,i}/n$. Also let $\gamma_n=\sum_i \beta_{n,i}^2/n-\bar{\beta}_n^2$. %$\ell_{4,n}=:\sum_{}$ 
Then $\ell_{4,n}=C\beta_{n,i}/\hat{\tau}_n^2$.
Note that using Lemma~\ref{lem:proveconv-mean}, we have, with probability tending to one, $\ell_{4,n}\leq C\rho_n^{-1}$. From  Lemma~\ref{lem:moments-z/x}, we have $\hat{\tau}_n$ is $\Theta(\rho_n^s)$.
 Furthermore, let $\hat{G}_2(i,j):=\hhij -h_2(X_i,X_j)$. 

We have
\begin{align*}
    \hat{G}_2(i,j)^2=\underbrace{\hat{G}_2(i,j)^2-\E\{\hat{G}_2(i,j)^2\mid X\}}_{\delta_{ij}}+\underbrace{\E\{\hat{G}_2(i,j)^2\mid X\}}_{O(\rho_n^{2s-1})}
\end{align*}
% Note that the second term is bounded by $ \rd C \bk \rho_{n}^{2s-1}$ a.s. as a result of the boundedness assumption.
We now will establish the $O(\rho_n^{2s-1})$ bound stated above for the second term. 
Let $\mathcal{S}^{ij}_r$ denote all subsets of size $r$ not containing $i,j$.
\begin{align*}
   \E\{\hat{G}_2(i,j)^2\mid X\}= \frac{\sum_{S,T\in \mathcal{S}^{ij}_r} \E\{H(A_{ij\cup S})H(A_{ij\cup T})\mid X\}}{{n-2\choose r-2}^2}
\end{align*}
In the above sum the terms with $|S\cap T|=0$ dominate, and for each of them the conditional expectation is bounded a.s. by $O(\rho_n^{2s-1})$ because of the boundedness of the graphon.
Now note that:
\begin{align*}
  % \tilde{g}_2(i,j)^2&=(\hhij-\tnhat)^2=\\
   %\beta_{n,i}&=\frac{1}{n}\sum_{j\neq i}(\hhij-\hi+\hi-\tnhat)^2\\
   %&=\frac{1}{n}\sum_{j\neq i}(\hhij-\hi)^2-(\hi-\tnhat)^2
   \tilde{g}_2(i,j)^2&\leq 3\left[\{\hhij -h_2(X_i,X_j)\}^2+\{h_2(X_i,X_j)-\theta_n\}^2+(\tnhat-\theta_n)^2\right]\\
   &\leq 3\{\hhij -h_2(X_i,X_j)\}^2+O(\rho_n^{2s-1})\\
%    \beta_{n,i}&\leq \frac{3}{n}\sum_{j\neq i}(\hhij -h_2(X_i,X_j))^2+\frac{1}{n}\sum_{j\neq i}(h_2(X_i,X_j)-\theta_n)^2+3(\tnhat-\theta_n)^2
\beta_{n,i}&\leq \frac{1}{n}\sum_{j\neq i}\delta_{ij}+O(\rho^{2s-1})\\
\gamma_n^2&\leq \frac{1}{n}\sum_i \beta_{n,i}^2\leq \frac{1}{n}\sum_i \left\{\frac{1}{n}\sum_{j\neq i}\delta_{ij}+O(\rho^{2s-1})\right\}^2\\
&\leq O(\rho^{4s-2})+\underbrace{\frac{1}{n}\sum_i \frac{1}{n}\sum_{j\neq i}\delta_{ij}^2}_{A}
\end{align*}

Now note that, $\E(\delta_{ij})=\E\{\E(\delta_{ij}\mid X)\}=0$. Thus, for all $i$,
\begin{align*}
\E(A)=\frac{1}{n}\sum_i\E \left\{\frac{1}{n}\sum_{j\neq i}\delta_{ij}\right\}^2=\frac{1}{n}\sum_i\var\left(\frac{1}{n}\sum_{j\neq i}\delta_{ij}\right)=O(\rho_n^{4s-3}/n)
\end{align*}

Thus, we have, for a large enough $C$,
\begin{align*}
    P\bb{\gamma_n^2\geq C \rho_n^{4s-2}}\leq P\bb{A\geq C'\rho_n^{4s-2}}\leq O\bb{\frac{\E(A)}{\rho_n^{4s-2}}}=O\bb{\frac{1}{n\rho_n}}
\end{align*}

\iffalse
%Since $\alpha_{n,i}$ are identically distributed, $E[l_{4,n}]=E[\alpha_{n,1}]$. As for $s_n^2$, we have:
\begin{align*}
    s_n^2&=E[s_n^2\mid X]+s_n^2-E[s_n^2\mid X]\\
\end{align*}
\begin{align}\label{eq:sn}
    \E s_n^2&= \frac{1}{n}\sum_{i=1}^{n}\E(\alpha_{n,i}-l_{4,n})^2=\E (\alpha_{n,i}-l_{4,n})^2\notag\\
    &\leq \E((\alpha_{n,i}-\E[\alpha_{n,i}]^2)+\E(l_{4,n}-\E[l_{n,4}])^2\\
    &=\var(\E[\alpha_{n,i}\mid X])+\E(\var(\alpha_{n,i}\mid X))+\var(\E[l_{n,4}\mid X])+\E(\var(l_{n,4}\mid X))\\
    &=O\bb{\frac{\rho_n^{-3}}{n}}
\end{align}
Thus, using Markov's inequality, we have:
\begin{align*}%\label{eq:sn}
  P\bb{s_n\geq \rho_n^{-1}}\leq \frac{\E s_n^2}{\rho_n^{-2}}=\frac{1}{n\rho_n}
\end{align*}

\fi

Therefore, since $s_n^2=\frac{(r-1)^2n^2}{(n-1)^2}\gamma_n/\hat{\tau}_n^2$, we have with probability tending to one,
$l_{4,n}+ks_n=O(\rho_n^{-1})$.

\bk
%As for the third condition, Lemma~\ref{lem:proveconv2} shows that on a high probability set,  for n large enough, we have $\max_i \sum_j  d_{nij}^2/n\leq l_{4,n}=O(1/\rho_n)$. This means the third condition is also satisfied on this high probability set. %causes some issues, since in the original proof $l_{4,n}$ is bounded. A thorough examination shows however that the final error is scaled by a factor of $l_{4,n}$. This includes $|K_{2,n}|, I_{1,n}, I_{3,n}$ and $I_{4,n}$. We may therefore replace $l_{4}$ with the sequence $l_{4,n}$. 

%Let $\m_i$ be $\w_i-1$.  
\iffalse
Now define 
\begin{equation}\label{eq:e2n}
      E_{2n}(u)= \Phi(u) + L_{1n}(u) + L_{2n}(u),
\end{equation}
where
\begin{equation*}
\begin{split}
     L_{1n}(u)=\sum_{i=1}^n (E \Phi (u -b_{n,i}(\w_i-1)/B_n)-\Phi(u)) -\frac{1}{2}\Phi''(u), \\
    L_{2n}(u)= - \frac{1}{n^{3/2}B_n^2}\sum_{1\leq i <j \leq n} b_{n,i}b_{n,j}d_{n,ij}E[(\w_i-1)(\w_j-1)\psi(\w_i,\w_j)].
\end{split}
\end{equation*}
\fi
%%\begin{equation*}
 %  \sup_u  \bigg{|}L_{1n}(u)+\frac{E(
%  \xi_i-1)^3}{6B_n^3}\sum_{i=1}^nb_{n,i}^3\Phi'''(u) \bigg{|} = o(n^{-1/2}). 
%\end{equation*}

%Define 
%\begin{equation*}
%    E_{2n}(u)= \Phi(u) + L_{1n}(u) + L_{2n}.
%\end{equation*}
%When $\E[\xi_i]=1$, $\E[(\xi_i-1)^2]=1$, and $E[\xi_i-1]^3=1$, and 
Since the first two conditions in eq~\ref{eq:wb-conds} are satisfied with probability tending to one, from \cite{wang-jing-weighted-bootstrap-u-statistics}  Theorem 3.1, we have,
\begin{equation*}
   \sup_u  \bigg{|}L_{1n}(u)+\frac{E(
   \xi_i-1)^3}{6B_n^3}\sum_{i=1}^nb_{n,i}^3\Phi'''(u) \bigg{|} = o_P(n^{-1/2}), 
\end{equation*}

Now we see that,
using the definitions of $L_{1n}$, $L_{2n}$ in Eq~\ref{eq:alldefswangjing}, plugging in definitions of $ b_{ni}$ and $ d_{nij}$'s from Eq~\ref{eq:wangjingbd}, and using the fact that $\E[\y_i\y_j\psi(\y_i,\y_j)]=\E[(\w_i-1)^2(\w_j-1)^2]=1$,
$$\sup_u |E_{2n}(u)-\gnhat(u)|=o_P(n^{-1/2}).$$
%$E_{2n}(u)$ can be written explicitly into 



Therefore, putting all the pieces together we see that
% with probability tending to 1,
% \begin{equation}\label{eq:tnasbserror}
%     \sup_{u}\bigg{|}P^*\left(\frac{\cfbq-\tnhat}{\hat{\sigma}_n}\leq u\right) -\gnhat(u)\bigg{|} = o\left(n^{-1/2}\right)+ O\left(\frac{\log n}{n^{2/3}\rho_n}\right)
% \end{equation}

\begin{equation}\label{eq:tnasbserror}
    \sup_{u}\bigg{|}P^*\left(\frac{\cfbq-\tnhat}{\hat{\sigma}_n}\leq u\right) -\gnhat(u)\bigg{|} = o_p\left(n^{-1/2}\right)+ O_P\left(\frac{\log n}{n^{2/3}\rho_n}\right)
\end{equation}



\end{proof}

Now we are ready to finish the proof of Corollary~\ref{thm:mbm-firstorder}.
\begin{proof}\normalfont[of Corollary~\ref{thm:mbm-firstorder}]
Here we take care of the error term in the Hoeffding projection in Eq~\ref{eq:boot-hoeff}. %\sout{For this we will use Lemma 8.2 in~\rd\cite{zhang-xia-network-edgeworth}\bk.} 
Set $X=\frac{\cfbm-\tnhat}{\shat}$, $Y=\cfbq$. From Eq~\ref{eq:boot-hoeff}, we see that $X=Y+R_n$, where $R_n =O_P(\mathcal{\delta}(n,\rho_n,R))$. Using Eq~\ref{eq:tnasbserror}, we see that on a high probability set,
\begin{align*}
    F_{Y}(u+a)-F_{Y}(u)&\leq |F_Y(u+a)-\gnhat(u+a)|+|\gnhat(u+a)-\gnhat(u)|+|\gnhat(u)-F_Y(u)| \\
    &\leq Ca+O\left(\frac{\log n}{n^{2/3}\rho_n}\right)
\end{align*}
Therefore, using Lemma 8.2 in~\cite{zhang-xia-network-edgeworth},
$$\sup_u\left|P^*\left(\frac{\cfbm-\tnhat}{\shat}\leq u\right)-\gnhat(u)\right|=o_P(n^{-1/2}) +  O_P\left(\frac{\log n}{n^{2/3}\rho_n}\right).$$

\end{proof}

\begin{proof}\normalfont[ of Lemma~\ref{lem:convEW}]

%\sout{As part of their proof of Theorem 3.2 ~\rd\cite{zhang-xia-network-edgeworth}\bk show that,}
\iffalse
\begin{align}\label{eq:zxempirical}
    &\max\left(\left|\frac{\sum_j \hat{g}_1(i)^3}{n}-\E[g_1(X_1)^3]\right|,\right.\notag\\
    &\left.\left|\frac{\sum_{i<j} \gi\gj\ggij}{{n\choose 2}}-\E[g_1(X_1)g_1(X_2)g_2(X_1,X_2)]\right|\right)\notag\\
    &=O_P\left(\rho_n^{3s}n^{1/2}\mzx\right),
\end{align}
and
\begin{align}\label{eq:tauhaterr}
    |\hat{\tau}_n^3-\tau_n^3|=O_P(\rho^{3s}/n^{1/2})
\end{align}
\fi
If we can establish Eq~\ref{eq:zxempiricalg1g1g2} and Eq~\ref{eq:tauhaterr} from Lemma~\ref{lem:moments-z/x} \bk for our empirical moments, we will get the desired result.
Note that our empirical moments involve the first term as well as a slight variation of the second term, which is given below.
\begin{align*}
   \widehat{E}_n\{ g_1(i)g_1(j)g_2(i,j) \}&=\frac{\sum_{i<j}\gi\gj\tilde{g}_2(i,j)}{{n\choose 2}}
\end{align*}
We will show that this follows from Eq~\ref{eq:zxempiricalg1g1g2}.
\begin{align*}
    &\frac{\sum_{i<j} \gi\gj\ggij}{{n\choose 2}}\\
    &=\frac{\sum_{i<j} \gi\gj(\tilde{g}_2(i,j)-\gi-\gj)}{{n\choose 2}}\\
    &=\frac{\sum_{i<j} \gi\gj\tilde{g}_2(i,j)}{{n\choose 2}}-\frac{\sum_{i\neq j}\gi\gj(\gi+\gj)}{2{n\choose 2}}\\
    &=\frac{\sum_{i<j} \gi\gj\tilde{g}_2(i,j)}{{n\choose 2}}-\frac{\sum_{i\neq j}\gi^2\gj}{{n\choose 2}}\\
    &=\frac{\sum_{i<j} \gi\gj\tilde{g}_2(i,j)}{{n\choose 2}}-\frac{(\sum_{i}\gi^2)(\sum_j\gj)-\sum_i \gi^3}{{n\choose 2}}\\
    &\stackrel{(i)}{=}\frac{\sum_{i<j} \gi\gj\tilde{g}_2(i,j)}{{n\choose 2}}+\frac{\sum_i \gi^3}{{n\choose 2}}\\
    &\stackrel{(ii)}{=}\frac{\sum_{i<j} \gi\gj\tilde{g}_2(i,j)}{{n\choose 2}}+O_P\left(\frac{\rho_n^{3s}}{n}\right)
\end{align*}
(i) uses the fact that $\sum_i\gi=0$. (ii) uses the fact that $\E\{g_1(X_1)^3\}=O(\rho_n^{3s})$ along with Eq~\ref{eq:zxempiricalg13}.
Hence from Eq~\ref{eq:zxempiricalg1g1g2} we have:
\begin{align*}
    &\left|\frac{\sum_{i<j} \gi\gj\tilde{g}_2(i,j)}{{n\choose 2}}-\E\{g_1(X_1)g_1(X_2)g_2(X_1,X_2)\}\right|\\
    &=\max\left\{O_P\left(\frac{\rho_n^{3s}}{n}\right), O_P\left(\rho_n^{3s-\frac{1}{2}}n^{-1/2}\right) %O_P\left(\rho^{3s}n^{1/2}\mzx\right)
    \right\}\\
    &=O_P\left(\rho_n^{3s-\frac{1}{2}}n^{-1/2}\right).
\end{align*}
This, along with Eqs~\ref{eq:zxempiricalg13} and~\ref{eq:tauhaterr} yields the result.
\end{proof}



\iffalse
\subsection{Proof of Lemma~\ref{lem:proveconv2}}
\begin{proof}\normalfont
%We will first do a direct variance calculation of $\ggij^2$.
Recall the definition of $\hhij$ from Eq~\ref{eq:hhij}.
\begin{align}\label{eq:g2upper}
    \tilde{g}_2(i,j)&=\hhij-\tnhat=(\hhij -h_2(X_i,X_j))+(h_2(X_i,X_j)-\theta_n)- \bk (\tnhat-\theta_n)\notag\\
    % \ggij^2
    \tilde{g}_2(i,j)^2 \bk
    &\leq 3\left((\hhij -h_2(X_i,X_j))^2+(h_2(X_i,X_j)-\theta_n)^2+(\tnhat-\theta_n)^2\right)
\end{align}
Since $\var(\tnhat)=O(\rho_n^{2s}/n)$ and the second term is bounded a.s. due to our boundedness assumption. We will just prove that
$\sum_{j\neq i} (\hhij -h_2(X_i,X_j))^2/(n-1)\rho_n^{2s}$ is bounded with high probability. It is not hard to check (also see~\rd\cite{zhang-xia-network-edgeworth}\bk) that
$$\E[(\hhij -h_2(X_i,X_j))^2/\rho_n^{2s}]=O(1/\rho_n)$$
Therefore,
\begin{align*}
   % \sum_{i=1}^m\sum_{j\neq i}E\ggij^2/(mn\rho^{2s})&=O(1/\rho_n)
    \sum_{j\neq i}\E\ggij^2/(n\rho^{2s})&=O(1/\rho_n)
\end{align*}
Furthermore, let $\hat{G}_2(i,j):=\hhij -h_2(X_i,X_j)$. 
\iffalse
Let
\begin{align*}
    \tilde{G}_2(i,j)=\hat{G}_2(i,j)^2-\E[\hat{G}_2(i,j)^2\mid X]
\end{align*}
\fi
We have
\begin{align*}
    \hat{G}_2(i,j)^2=\underbrace{\hat{G}_2(i,j)^2-\E[\hat{G}_2(i,j)^2\mid X]}_{\delta_{ij}\bk}+\underbrace{\E[\hat{G}_2(i,j)^2\mid X]}_{O(\rho_n^{2s-1})}
\end{align*}
% Note that the second term is bounded by $  C \bk \rho_{n}^{2s-1}$ a.s. as a result of the boundedness assumption.
 We now will establish the $O(\rho_n^{2s-1})$ bound stated above for the second term. \bk  
Let $\mathcal{S}^{ij}_r$ denote all subsets of size $r$ not containing $i,j$.
\begin{align*}
   \E[\hat{G}_2(i,j)^2\mid X]= \frac{\sum_{S,T\in \mathcal{S}^{ij}_r} \E[H(A_{ij\cup S})H(A_{ij\cup T})\mid X]}{{n-2\choose r-2}^2}
\end{align*}
In the above sum the terms with $|S\cap T|=0$ dominate, and for each of them the conditional expectation is bounded a.s. by $O(\rho_n^{2s-1})$ because of the boundedness of the graphon.

% Thus for any $i$, using Eq~\ref{eq:g2upper}, for some positive constant $C$,
% \begin{align}\label{eq:gtildebound}
% \frac{\sum_{j\neq i} \tilde{g}_2(i,j)^2}{n}&=C\left(\frac{\sum_{j\neq i}\delta_{ij}}{n}\right)+O(\rho_n^{2s-1})%\\
%     %\frac{\sum_{j\neq i} \hat{G}_2(i,j)^2}{n}&=\frac{\sum_{j\neq i}\delta_{ij}}{n}+O(\rho_n^{2s-1})
% \end{align}
We will analyze $\sum_j \delta_{ij}$. Note that $\E[\delta_{ij}|X]=0$.
%Then the variance of $\sum_j g'_2(i,j)^2/n$ is given by:
\begin{align}\label{eq:vardel}
    \var\left(\frac{1}{n}\sum_j \delta_{ij}\mid X\right)=\frac{\sum_i \var(\delta_{ij}\mid X)+2\sum_{k<\ell\neq i} \cov(\delta_{ik},\delta_{i\ell}\mid X)}{n^2}
\end{align}
%A quick calculation yields $\var(\delta_{ij})=\var(\delta_{ij}|A)=O(\rho_n^{4s-1})$ and $\cov(\delta(i,j),\delta(i,k))=\cov(\delta(i,j),\delta(i,k)|A)=O(\rho_n^{4s-1}/n)$. So the variance is $O(\rho_n^{4s}/n\rho_n)$.


\begin{align}
    \delta_{ij}=\frac{1}{{n-2\choose r-2}^2}\sum_{S,T\in \mathcal{S}^{ij}_r} \underbrace{H(A_{ij\cup S})H(A_{ij\cup T})-\E[H(A_{ij\cup S})H(A_{ij\cup T})\mid X]}_{H_{ij}'(S,T)}
\end{align}
For variance, we have:
\begin{align*}
    \var(\delta_{ij})&=\E\var(\delta_{ij}\mid X)\\
     &=\frac{ \sum\limits_{S_1\neq T_1, S_2\neq T_2\in \mathcal{S}^{ij}_r}\E\cov(H_{ij}'(S_1,T_1),H_{ij}'(S_2,T_2)\mid X)}{{n-2\choose r-2}^4}\\
      &=\frac{O\left({n-2\choose r-2}^4\rho_n^{4s-1}\right)}{{n-2\choose r-2}^4}=O(\rho_n^{4s-1})
   % &=\frac{\sum\limits_{S,T\in \mathcal{S}^{ij}_r} \E\var(H_{ij}'(S,T)\mid X)+2\sum\limits_{S_1\neq T_1, S_2\neq T_2\in \mathcal{S}^{ij}_r}\E\cov(H_{ij}'(S_1,T_1),H_{ij}'(S_2,T_2)\mid X)}{{n-2\choose r-2}^4}\\
   % &=\frac{{n-2\choose r-2}^2\rho_n^{4s-1}+O\left({n-2\choose r-2}^4\rho_n^{4s-1}\right)}{{n-2\choose r-2}^4}=O(\rho_n^{4s-1})
\end{align*}
The dominant term in the above sum is the one with $S_1, S_2, T_1, T_2$ all disjoint.
For covariance, for $i\neq j\neq k$ we have:
\begin{align*}
    \cov(\delta_{ij},\delta_{ik})&=\E\cov(\delta_{ij},\delta_{ik}\mid X)\\
    &=\frac{\sum\limits_{S_1\neq T_1 \in \bk \mathcal{S}^{ij}_r,S_2\neq T_2\in \mathcal{S}^{ik}_r} \E\cov (H_{ij}'(S_1,T_1),H_{ik}'(S_2,T_2)\mid X)}{{n-2\choose r-2}^4}\\
    &\stackrel{(i)}{=}\frac{O\left({n-3\choose 4(r-2)-1}\rho_n^{4s- 3\bk}\right)}{{n-2\choose r-2}^4}=O(\rho_n^{4s- 3 \bk}/n)
\end{align*}

Step (i) is true, because conditioned on $X$, there needs to be at lease one $u$ in common between $\{i,j\cup S_1\cup T_1\}$ and $\{i,k\cup S_2\cup T_2\}$ to have a nonzero covariance. This leads to only $4(r-2)-1$ choices, which dominates the sum. This along with Eq~\ref{eq:vardel} gives us:
$$\var\left(\sum_j \delta_{ij}/n\right)=\E\var\left(\sum_j \delta_{ij}/n\mid X\right)= O(\rho_n^{4s-3}/n).$$
%comment out the following section

Thus we have for large enough $C$,
\rd
not correct anymore 
\bk 
\begin{align*}
    P\left(\max_i \sum_{j\neq i}\tilde{g}_2(i,j)^2/n\geq C\rho_n^{2s-1}\right)&\leq n P\left( \sum_{j\neq 1}\tilde{g}_{1j}^2/n\geq C\rho_n^{2s-1)}\right)\\
    % (\text{Using Eq~\ref{eq:gtildebound}})
    \qquad\qquad&\leq nP\left( |\sum_{j\neq 1}\delta_{1j}/n+O(\rho_n^{2s-1})|\geq C\rho_n^{2s-1}\right)\\
    &\leq nP\left( |\sum_{j\neq 1}\delta_{1j}/n|\geq C'\rho_n^{2s-1}\right)\\
    &\leq C''\frac{n\rho_n^{4s-1}/n}{\rho_n^{4s-2}}=O\left(\rho_n\right)
 \end{align*}
 
 \rd 
 \iffalse
 Thus we have,
 \begin{align*}
    P\left(\max_i \sum_{j\neq i}\tilde{g}_2(i,j)^2/n\geq (\log n)^{1/2}\rho_n^{2s-1.5}\right)&\leq n P\left( \sum_{j\neq 1}\tilde{g}_{1j}^2/n\geq (\log n)^{1/2}\rho_n^{2s-1.5}\right)\\
    % (\text{Using Eq~\ref{eq:gtildebound}})
    \qquad\qquad&\leq nP\left( |\sum_{j\neq 1}\delta_{1j}/n+O(\rho_n^{2s-1})|\geq (\log n)^{1/2}\rho_n^{2s-1.5}\right)\\
    &\leq nP\left( |\sum_{j\neq 1}\delta_{1j}/n|\geq (\log n)^{1/2}\rho_n^{2s-1.5}\right)\\
    &\leq C''\frac{n\rho_n^{4s-3}/n}{ (\log n)^{1/2} \rho_n^{4s-3}} = O\left(\frac{1}{(\log n)^{1/2}}\right).
 \end{align*}
 \fi
%Now a Markov inequality yields the result.
\end{proof}
\fi


\subsection{Proof of Lemma~\ref{lem:proveconv-mean}}
\begin{proof}\normalfont
%We will first do a direct variance calculation of $\ggij^2$.
Recall the definition of $\hhij$ from Eq~\ref{eq:hhij}.
\begin{align*}%\label{eq:g2upper}
    \tilde{g}_2(i,j)&=\hhij-\tnhat=\{\hhij -h_2(X_i,X_j)\}+\{h_2(X_i,X_j\}-\theta_n)-  (\tnhat-\theta_n)\notag\\
    % \ggij^2
    \tilde{g}_2(i,j)^2 
    &\leq 3\left[\{\hhij -h_2(X_i,X_j)\}^2+\{h_2(X_i,X_j)-\theta_n\}^2+(\tnhat-\theta_n)^2\right].
\end{align*}
Since $\var(\tnhat)=O(\rho_n^{2s}/n)$ and the second term is bounded a.s. due to our boundedness assumption. We will just prove that
$\sum_{j\neq i} \{\hhij -h_2(X_i,X_j)\}^2/(n-1)\rho_n^{2s}$ is bounded with high probability. It is not hard to check %\sout{\bl [cut][(also see~\rd\cite{zhang-xia-network-edgeworth}\bk)]} \bk 
that
$$\E\{(\hhij -h_2(X_i,X_j))^2/\rho_n^{2s}\}=O(1/\rho_n)$$
Therefore,
\begin{align*}
   % \sum_{i=1}^m\sum_{j\neq i}E\ggij^2/(mn\rho_n^{2s})&=O(1/\rho_n)
    \sum_{j\neq i}\E\{\ggij^2/(n\rho_n^{2s})&=O(1/\rho_n)\}
\end{align*}
Furthermore, let $\hat{G}_2(i,j):=\hhij -h_2(X_i,X_j)$. 
\iffalse
Let
\begin{align*}
    \tilde{G}_2(i,j)=\hat{G}_2(i,j)^2-\E[\hat{G}_2(i,j)^2\mid X]
\end{align*}
\fi
We have
\begin{align*}
    \hat{G}_2(i,j)^2=\underbrace{\hat{G}_2(i,j)^2-\E\{\hat{G}_2(i,j)^2\mid X\}}_{\delta_{ij}}+\underbrace{\E\{\hat{G}_2(i,j)^2\mid X\}}_{O(\rho_n^{2s-1})}
\end{align*}
% Note that the second term is bounded by $ \rd C \bk \rho_{n}^{2s-1}$ a.s. as a result of the boundedness assumption.
 We now will establish the $O(\rho_n^{2s-1})$ bound stated above for the second term.  
Let $\mathcal{S}^{ij}_r$ denote all subsets of size $r$ not containing $i,j$.
\begin{align*}
   \E\{\hat{G}_2(i,j)^2\mid X\}= \frac{\sum_{S,T\in \mathcal{S}^{ij}_r} \E\{H(A_{ij\cup S})H(A_{ij\cup T})\mid X\}}{{n-2\choose r-2}^2}
\end{align*}
In the above sum the terms with $|S\cap T|=0$ dominate, and for each of them the conditional expectation is bounded a.s. by $O(\rho_n^{2s-1})$ because of the boundedness of the graphon.

% Thus for any $i$, using Eq~\ref{eq:g2upper}, for some positive constant $C$,
% \begin{align}\label{eq:gtildebound}
% \frac{\sum_{j\neq i} \tilde{g}_2(i,j)^2}{n}&=C\left(\frac{\sum_{j\neq i}\delta_{ij}}{n}\right)+O(\rho_n^{2s-1})%\\
%     %\frac{\sum_{j\neq i} \hat{G}_2(i,j)^2}{n}&=\frac{\sum_{j\neq i}\delta_{ij}}{n}+O(\rho_n^{2s-1})
% \end{align}
We will analyze $\sum_i\sum_{j\neq i}\delta_{ij}$. Note that $\E(\delta_{ij}\mid X)=0$.
%Then the variance of $\sum_j g'_2(i,j)^2/n$ is given by:
\begin{align}\label{eq:vardel2}
    \var\left(\frac{1}{n^2}\sum_i\sum_j \delta_{ij}\mid X\right)=\frac{\sum_i\sum_j \var(\delta_{ij}\mid X)+\sum_{i,k,k\neq i}\sum_{j,\ell,j\neq \ell} \cov(\delta_{ik},\delta_{j\ell}\mid X)}{n^4}
\end{align}
%A quick calculation yields $\var(\delta_{ij})=\var(\delta_{ij}\mid A)=O(\rho_n^{4s-1})$ and $\cov(\delta(i,j),\delta(i,k))=\cov(\delta(i,j),\delta(i,k)\mid A)=O(\rho_n^{4s-1}/n)$. So the variance is $O(\rho_n^{4s}/n\rho_n)$.


\begin{align*}
    \delta_{ij}=\frac{1}{{n-2\choose r-2}^2}\sum_{S,T\in \mathcal{S}^{ij}_r} \underbrace{H(A_{ij\cup S})H(A_{ij\cup T})-\E\{H(A_{ij\cup S})H(A_{ij\cup T})\mid X\}}_{H_{ij}'(S,T)}
\end{align*}
For variance, we have:
\iffalse
\begin{align*}
    \var(\delta_{ij})&=\E\{\var(\delta_{ij}\mid X)\}\\
     &=\frac{ \sum\limits_{S_1\neq T_1, S_2\neq T_2\in \mathcal{S}^{ij}_r}\E\{\cov(H_{ij}'(S_1,T_1),H_{ij}'(S_2,T_2)\mid X)\}}{{n-2\choose r-2}^4}\\
      &=\frac{O\left({n-2\choose r-2}^4\rho_n^{4s-1}\right)}{{n-2\choose r-2}^4}=O(\rho_n^{4s-3})
   % &=\frac{\sum\limits_{S,T\in \mathcal{S}^{ij}_r} \E\var(H_{ij}'(S,T)\mid X)+2\sum\limits_{S_1\neq T_1, S_2\neq T_2\in \mathcal{S}^{ij}_r}\E\cov(H_{ij}'(S_1,T_1),H_{ij}'(S_2,T_2)\mid X)}{{n-2\choose r-2}^4}\\
   % &=\frac{{n-2\choose r-2}^2\rho_n^{4s-1}+O\left({n-2\choose r-2}^4\rho_n^{4s-1}\right)}{{n-2\choose r-2}^4}=O(\rho_n^{4s-1})
\end{align*}
\fi
\begin{align*}
\var(\delta_{ij})&=\E\{\var(\delta_{ij}\mid X)\}\\
&=\frac{ \sum\limits_{S_1\neq T_1, S_2\neq T_2\in \mathcal{S}^{ij}_r}\E\{\cov(H_{ij}'(S_1,T_1),H_{ij}'(S_2,T_2)\mid X)\}}{{n-2\choose r-2}^4}\\
%&=\frac{O\left({n-2\choose r-2}^4\rho_n^{4s-1}\right)}{{n-2\choose r-2}^4}=O(\rho_n^{4s-3})
% &=\frac{\sum\limits_{S,T\in \mathcal{S}^{ij}_r} \E\var(H_{ij}'(S,T)\mid X)+2\sum\limits_{S_1\neq T_1, S_2\neq T_2\in \mathcal{S}^{ij}_r}\E\cov(H_{ij}'(S_1,T_1),H_{ij}'(S_2,T_2)\mid X)}{{n-2\choose r-2}^4}\\
% &=\frac{{n-2\choose r-2}^2\rho_n^{4s-1}+O\left({n-2\choose r-2}^4\rho_n^{4s-1}\right)}{{n-2\choose r-2}^4}=O(\rho_n^{4s-1})
\end{align*}

The dominant term in the above sum is the one with $S_1, S_2, T_1, T_2$ all disjoint. Consider any other term in the above sum where any pair of the subsets have $p$ nodes, $d$ edges in common and the rest are disjoint. In this case there are $2(r-2-p)+2(r-2)+p=4(r-2)-p$ choices of nodes and the number of edges are lower bounded by $4(s-1)+1-d=4s-3-d$ (since all pairs have $\{i,j\}$ in common). When $p\geq 1$, for acyclic graphs, $d\leq p-1$ and for general subgraphs with a cycle, $d\leq {p\choose 2}$. Thus, for $p\geq 0$, we have:
\begin{align*}
\frac{O\left(n^{4(r-2)-p}\rho_n^{4s-3-d}\right)}{{n-2\choose r-2}^4}=O(\rho_n^{4s-3})\times O\left(\frac{1}{n^p \rho_n^d}\right)
\end{align*}
Note that for acyclic graphs, it is easy to see that under our sparsity conditions the above is dominated by $p=0$. For general cyclic graphs, since $\rho_n= \omega(n^{-1/r})$, note that, since $p\leq r$,
\begin{align*}
n^p\rho_n^d\geq n^p\rho_n^{p(p-1)/2}\geq n^{p\left(1-\frac{p-1}{2r}\right)}\geq n^{\frac{p(r+1)}{2r}} \rightarrow \infty
\end{align*}
So, $\var(\delta_{ij})=O(\rho_n^{4s-3})$.



For covariance, for $i\neq j\neq k \neq \ell$, we have:
\begin{align*}
\cov(\delta_{ik},\delta_{j\ell})&=\E\{\cov(\delta_{ik},\delta_{j\ell}\mid X)\}\\
&=\frac{\sum\limits_{S_1\neq T_1 \in  \mathcal{S}^{ik}_r,S_2\neq T_2\in \mathcal{S}^{j\ell}_r} \E\{\cov (H_{ij}'(S_1,T_1),H_{ik}'(S_2,T_2)\mid X)\}}{{n-2\choose r-2}^4}
%&\stackrel{(i)}{=}\frac{O\left({n-4\choose 4(r-2)-2}\rho_n^{4s- 3}\right)}{{n-2\choose r-2}^4}=O(\rho_n^{4s-3}/n^2).
\end{align*}
Consider any two pairs of subsets with $p$ nodes and $d$ edges in common. First note that $p\geq 2$ in order to have a nonzero covariance. In this case there will be $4(r-2)-p$ choices for nodes, and $(2s-A_{ik})+(2s-A_{j\ell})-d\geq 4s-3-d$ edges.
\begin{align*}
=\frac{O\left(n^{4(r-2)-p}\rho_n^{4s-2-d}\right)}{{n-2\choose r-2}^4}=O\left(\frac{\rho_n^{4s-3}}{n^2}\right)\times O\left(\frac{1}{n^{p-2}\rho_n^{d-1}}\right).
\end{align*}
Note that, for acyclic graphs $d\leq p-1$ and hence the above is maximized at $p=2,d=1$ as long as $n\rho_n\rightarrow \infty$. 

For general cyclic subgraphs, $d\leq {p\choose 2}$.  Furthermore, since $p+2\leq r$, and $\rho_n=\omega(n^{-1/r})$, we have, for $p> 2$:
\begin{align*}
n^{p-2}\rho_n^{d-1}&=n^{p-2-\frac{1}{r}\left(\frac{p(p-1)}{2}-1\right)}\\
&=n^{p-2-\frac{(p-2)(p+1)}{2r}}=n^{(p-2)\left(1-\frac{p+1}{2r}\right)}\geq n^{(p-2)\frac{r+1}{2r}}\rightarrow \infty
\end{align*}
Thus under the conditions of Assumption~\ref{ass:sparse}, we have:
%As long as $n\rho_n\rightarrow \infty$ for acyclic graphs and $n\rho_n^2\rightarrow \infty$ for simple cycles, we see that the dominating term is given by $p=2$, and 
\begin{align*}
\cov(\delta_{ik},\delta_{j\ell})=O(\rho_n^{4s-3}/n^2)
\end{align*}
\bk
\iffalse
The dominant term in the above sum is the one with $S_1, S_2, T_1, T_2$ all disjoint.
For covariance, for $i\neq j\neq k \neq \ell$ we have:
\begin{align*}
    \cov(\delta_{ik},\delta_{j\ell})&=\E\{\cov(\delta_{ik},\delta_{j\ell}\mid X)\}\\
    &=\frac{\sum\limits_{S_1\neq T_1 \in  \mathcal{S}^{ik}_r,S_2\neq T_2\in \mathcal{S}^{j\ell}_r} \E\{\cov (H_{ij}'(S_1,T_1),H_{ik}'(S_2,T_2)\mid X)\}}{{n-2\choose r-2}^4}\\
    &\stackrel{(i)}{=}\frac{O\left({n-4\choose 4(r-2)-2}\rho_n^{4s- 3}\right)}{{n-2\choose r-2}^4}=O(\rho_n^{4s-3}/n^2).
\end{align*}
\fi
Step (i) is true, because conditioned on $X$, there needs to be at lease two nodes $u_1$, $u_2$ in common between $\{i,k\cup S_1\cup T_1\}$ and $\{j,\ell \cup S_2\cup T_2\}$ to have a nonzero covariance. This leads to only $4(r-2)-2$ choices, which dominates the sum. This along with Eq~\ref{eq:vardel2} gives us:
$$\var\left(\frac{1}{n^2}\sum_i\sum_{j \neq i} \delta_{ij}\right)=\E\left\{\var\left(\sum_i\sum_{j \neq i} \delta_{ij}/n^2\mid X\right)\right\}=O(\rho_n^{4s-3}/n^2).$$
%comment out the following section
%\bl Note that for covariance, if $k=\ell$ and $\{i,k\cup S_1\cup T_1\}$ and $\{j,\ell \cup S_2\cup T_2\}$ share a node $u_1$, $ \cov(\delta_{ik},\delta_{jk})=O(\rho_n^{4s-3}/n)$, but in Eq~\ref{eq:vardel2} there will only be $O(n^3)$ terms in the summation of covariance, instead of $O(n^4)$ terms. Thus will result in the same $\var\left(\sum_i\sum_j \delta_{ij}/n^2\right)$.


Thus we have for large enough $C$, we have

\begin{align*}
   P\left( \frac{1}{n^2}\sum_i\sum_{j\neq i}\tilde{g}_2(i,j)^2\geq C\rho_n^{2s-1}\right)
    % (\text{Using Eq~\ref{eq:gtildebound}})
   &\leq P\left( \bigg{|}\sum_i\sum_{j\neq i}\delta_{ij}/n^2+O(\rho_n^{2s-1})\bigg{|}\geq C\rho_n^{2s-1}\right)\\
    &\leq P\left( \sum_i\bigg{|}\sum_{j\neq i}\delta_{ij}/n^2\bigg{|}\geq C'\rho_n^{2s-1}\right)\\
    &\leq C''\frac{\rho_n^{4s-3}/n^2}{\rho_n^{4s-2}}=O\left(\frac{1}{n^2\rho_n}\right).
 \end{align*}
 

 \iffalse
 Thus we have,
 \begin{align*}
    P\left(\max_i \sum_{j\neq i}\tilde{g}_2(i,j)^2/n\geq (\log n)^{1/2}\rho_n^{2s-1.5}\right)&\leq n P\left( \sum_{j\neq 1}\tilde{g}_{1j}^2/n\geq (\log n)^{1/2}\rho_n^{2s-1.5}\right)\\
    % (\text{Using Eq~\ref{eq:gtildebound}})
    \qquad\qquad&\leq nP\left( |\sum_{j\neq 1}\delta_{1j}/n+O(\rho_n^{2s-1})|\geq (\log n)^{1/2}\rho_n^{2s-1.5}\right)\\
    &\leq nP\left( |\sum_{j\neq 1}\delta_{1j}/n|\geq (\log n)^{1/2}\rho_n^{2s-1.5}\right)\\
    &\leq C''\frac{n\rho_n^{4s-3}/n}{ (\log n)^{1/2} \rho_n^{4s-3}} = O\left(\frac{1}{(\log n)^{1/2}}\right).
 \end{align*}
 \fi
%Now a Markov inequality yields the result.
\end{proof}
\bk

\subsection{Proof of Lemma~\ref{lem:proveconv}}
\begin{proof}\normalfont
Let $\Delta_i:=|\gi-g_1(X_i)|/\rho_n^s$. We have:
\begin{align}\label{eq:b12}
    &\dfrac{\sum_{i}|\gi/\rho_n^s|^3}{n}\notag\\
    &\leq \dfrac{\sum_i \Delta_i^3}{n} + 3\dfrac{\sum_i |g_1(X_i)/\rho_n^s|\Delta_i^2}{n}+3\dfrac{\sum_i |g_1(X_i)/\rho_n^s|^2\Delta_i}{n}+\dfrac{\sum_i |g_1(X_i)/\rho_n^s|^3}{n}\notag\\
    &=B_1+B_2+B_3+B_4
\end{align}
First note that using the boundedness condition on the graphon, $|g_1(X_i)/\rho_n^s|$ is bounded. Hence $B_4\leq c$ a.s.
%\sout{Using the proof of Theorem 3.2 in~\rd\citep{zhang-xia-network-edgeworth}}
Using Lemma~\ref{lem:moments-z/x}\bk, we know that $E(\Delta_i)^2=O(1/n\rho_n)$.
Since $\sum_i \Delta_i\leq n^{1/2}{\sum_j \Delta_j^2}$, for the second term we have, for some $C > 0$ \bk:
\begin{align}\label{eq:b2}
    P(B_2\geq \epsilon)\leq \frac{n^{1/2} E\sum_i\Delta_i^2}{n\epsilon^2}\leq \frac{ C \bk }{n^{1/2}\rho_n\epsilon^2}
\end{align}
Furthermore,
\begin{align}\label{eq:b3}
    P(B_3\geq \epsilon)\leq \frac{ E\sum_i\Delta_i^2}{n\epsilon^2}\leq \frac{ C \bk}{n\rho_n\epsilon^2}.
\end{align}
By repeated application of Cauchy-Schwarz inequality, we have $(\sum_i x_i^3)^2\leq \sum_i x_i^2\sum_i x_i^4\leq (\sum_i x_i^2)^3$, we also have:
\begin{align*}
    P(B_1\geq \epsilon)\leq \frac{ E\sum_i\Delta_i^3}{n\epsilon^2}\leq \frac{(\sum_i E\Delta_i^2)^{3/2}}{n\epsilon^2}
    \leq \frac{C \bk }{n\rho_n^{3/2}\epsilon^2}
\end{align*}
Therefore, using the sparsity conditions in Assumption~\ref{ass:sparse}, we see that the first equation in the lemma statement is proved.

For the second, we use:
\begin{align*}
    \dfrac{\sum_{i}|\gi/\rho_n^s|^2}{n}&\geq \dfrac{\sum_i |g_1(X_i)/\rho_n^s|^2}{n} +\dfrac{\sum_i \Delta_i^2}{n} - 2\dfrac{\sum_i |g_1(X_i)/\rho_n^s|\Delta_i}{n}\\
    &=C_1+\alpha B_2-\beta B_3,
\end{align*}
where $\alpha,\beta$ are positive constants, and $B_2,B_3$ were defined in Eq~\ref{eq:b12}.
Using Assumption 2 part 1, \bk we see $C_1>0$, a.s. Also, now for a small enough constant $\epsilon$, using Eqs~\ref{eq:b2} and~\ref{eq:b3}, we see that the second equation in the lemma statement is proven.

\iffalse
%Finally, let $\delta_{ij}=|\ggij-g_2(i,j)|$
\begin{align*}
    \dfrac{\sum_{i=1}^m\sum_{j\neq i}|\ggij/\rho_n^s|^2}{n m}&\leq 2 \left(\dfrac{\sum_{i=1}^m\sum_{j\neq i}\hhij^2}{nm\rho_n^{2s}}+\dfrac{\sum_{i=1}^m\sum_{j=1}^nh_2(X_i,X_j)^2}{nm\rho_n^{2s}}\right)\\
    &\leq 2\frac{\sum_{i=1}^m(\sum_{j\neq i}\hhij)^2}{nm\rho_n^{2s}} +c\\
    &\leq c'\frac{(r-1)^2 \sum_{i=1}^m \hi ^2}{nm\rho_n^{2s}} +c\\
\end{align*}

The last step is true because 
$$\hi=\sum_{j\neq i}\hhij/(n-1),$$
since every rooted subgraph is overcounted by $r-1$.

\fi
\end{proof}



\subsection{Proof of Lemma~\ref{lem:wangjing}}
\begin{proof}\normalfont
%Recall that 
Define the following quantities.
\begin{align*}
    \gjt&=\E\{\exp(it b_{nj}\y_j/B_n)\}
    \end{align*}
    Also define $\phi_{1,n}$ and $\phi_{2,n}$ as:
    \begin{align*}
    \phi_{1,n}(t)&=e^{-t^2/2}\left[1+\sum_j\{\gjt-1\}+\frac{t^2}{2}\right]\\
    \phi_{2,n}(t)&=-t^2\kn \et.
    \end{align*}
    Finally define,
    \begin{align*}
    S_n&=\frac{1}{B_n}\sum_j  b_{nj} \y_j,\qquad
    \del_{n,m}=\frac{1}{n^{3/2}}\sum_{i=1}^{m-1}\sum_{j=i+1}^n d_{nij}\psi(\y_i,\y_j)\\
\end{align*}
As in the original proof, we define:
\begin{subequations}
\label{eq:ltophi}%(\rd did not check the first one \bk)
\begin{align}
    &\int_{-\infty}^\infty e^{itx} d\{\Phi(x)+\lnone\}dx=\phi_{1,n}(t)\\
    &\int_{-\infty}^\infty e^{itx} d \lntwo dx=it\phi_{2,n}(t)\\
    &\int_{-\infty}^\infty e^{itx}E_{2n}(x)= \phi_{1,n}(t)+it\phi_{2,n}(t)%\notag
\end{align}
\end{subequations}

Now, for some $c>0$ to be chosen later, from Esseen's smoothing lemma~\cite{petrov2012sums} and Eq~\ref{eq:ltophi} we have:
\begin{align}\label{eq:esseen}
    &\sup_x\bigg{|}P(V_n\leq x)-E_{2n}(x)\bigg{|}\notag\\
    &\leq \int_{|t|\leq n^{1-c}}|t|^{-1}|\E (e^{itV_n})-\phi_{1,n}(t)-it\phi_{2,n}(t)|dt+Cn^{c-1}\sup_x\left|\dfrac{d E_{2,n}(x)}{dx}\right|\notag\\
    &\leq \int_{|t|\leq n^{1-c}}|t|^{-1}|\E (e^{itV_n})-\phi_{1,n}(t)-it\phi_{2,n}(t)|dt+\frac{C_1(|\kn|+\beta)}{n^{1-c}}
\end{align}

The last line is true due to the following argument. Note that, for some $v_j$ in the $| b_{nj}\y_j/B_n|$ ball in the neighborhood of $x$, for $j\in\{1,\dots, n\}$,
\begin{align*}
    \frac{d\lnone(x)}{dx}&=\sum_{j=1}^n \left[\E\{\phi(x- b_{nj}\y_j/B_n)\}-\phi(x)\right]-\frac{1}{2}\Phi'''(x)\\
    &=\sum_{j=1}^n \E\left\{- b_{nj}\y_j/B_n\phi'(x)+ b_{nj}^2\y_j^2/2B_n^2\phi''(x)- b_{nj}^3\y_j^3/6B_n^3\phi'''(v_j)\right\}-\frac{1}{2}\Phi'''(x).
    \end{align*}
    Thus, we have:
    \begin{align*}
    \sup_x\left|\frac{d\lnone(x)}{dx}\right|&\leq \sum_{j=1}^n c_1\left\{ b_{nj}^2/B_n^2 |\phi''(x)|+ c_2| b_{nj}/B_n|^3\E(|\y_j^3|)|\phi'''(v_j)|\right\}+\frac{1}{2}|\Phi'''(x)| \\
    &\leq C+\E(|X_1|^3) \left(\sum_j | b_{nj}/B_n|^3\right)+C'\\
    &\leq C+\beta/n^{1/2}\leq C\beta\qquad\text{Since $\beta\geq 1$}
\end{align*}

Also note that, for any $\epsilon >0$, for $n$ large enough,
\begin{align*}
    \int_{|t|>n^\epsilon} |\phi_{1,n}(t)/t|dt&=O(1/n^{1-c})\\
    \int_{|t|>n^\epsilon} |\phi_{2,n}(t)/t|dt&=O(|\kn|/n^{1-c})
\end{align*}

Thus the main idea is that $E(e^{itV_n})$ behaves like $E(itS_n)+itE(itS_n\del_{n,n})$.
\begin{align*}
    &\int_{|t|\leq n^{1-c}}|t|^{-1}|\E (e^{itV_n})-\phi_{1,n}(t)-\phi_{2,n}(t)|dt\leq \sum_{j=1}^4I_{j,n}
\end{align*}

Going back to Eq~\ref{eq:esseen}, we break up the first part of the RHS into four parts, and the remainder gets absorbed into $O(|\kn+\beta|/n^{1-c})$ term in Eq~\ref{eq:esseen}. 

\begin{align*}
    |I_{1,n}|&=\int_{|t|<n^\epsilon}|t|^{-1}\left|\E (e^{it V_n})-E(itS_n)-itE(itS_n\del_{n,n})\right|dt\\
    |I_{2,n}|&=\int_{|t|<n^\epsilon}|t|^{-1}\left|\E (e^{it S_n})-\phi_{1,n}(t)\right|dt\\
    |I_{3,n}|&=\int_{|t|<n^\epsilon}\left|\E (\del_{n,n} e^{itS_n}) -\phi_{2,n}(t)\right|dt\\
    |I_{4,n}|&=\int_{n^\epsilon \leq |t|<n^{1-c}}|t|^{-1}\left|\E (e^{itV_n})\right|dt\\
\end{align*}
First we will bound some terms which will be used frequently. Since $ab\leq (a^2+b^2)/2$.
\begin{align}
    |\kn|&\leq \frac{C}{n^{3/2}B_n^2}\sum_{1\leq i<j\leq n} ( b_{ni}^2 b_{nj}^2+ d_{nij}^2)(1+\ro)\notag\\
    & \leq \frac{C(1+\ro)}{n^{3/2}B_n^2} \left\{\left(\sum_j b_{nj}^2\right)^2+\sum_{i<j} d_{nij}^2\right\}\notag\\
    &\leq \frac{C(1+\ro)}{n^{3/2}B_n^2}\left(B_n^4+l_{4,n} n^2\right)\notag\\
    &\leq \frac{C'(1+\ro)l_{4,n}}{n^{1/2}}\label{eq:knbound}
\end{align}


As for $\del_{n,n}$, we have:
\begin{align*}%\label{eq:delnn}
    E\del_{n,n}^2=\frac{\ro}{n^3}\sum_{i=1}^{n-1}\sum_{j=i+1}^n  d_{nij}^2=\frac{\ro l_{4,n}}{n}
\end{align*}
\bk
Furthermore we will use:
\begin{align}\label{eq:rem}
    R(z):=e^{iz}-1-iz\qquad |R(z)|\leq |z|^\alpha \ \ \text{for all } \alpha\in [1,2]
\end{align}
We will first bound $I_{1,n}$. Using Taylor expansion, for some $|\eta|\leq 1$,

\begin{align*}
    |\ione|&\leq \int_{|t|<n^\epsilon}|t|^{-1}t^2/2  |\E (\del_{n,n}^2 e^{itS_n}e^{it\del_{n,n}\eta})|dt\notag\\
    &\leq 1/2\int_{|t|<n^\epsilon}|t|  \E(\del_{n,n}^2)dt
    \leq C\frac{(1+\ro)l_{4,n}}{n^{1-2\epsilon}}
\end{align*}

Next we bound $\itwo$. 
% \rd Can do better under more conditions on $\sum_j b_{nj}^4$. \bk
Using a similar argument in the proof of the original version of this theorem, we have:%stated in \rd\citet{wang-jing-weighted-bootstrap-u-statistics}\bk, we have:
% as the original proof (\rd did not check Hall \bk), we have:
\begin{align*}
    |\itwo|&\leq \frac{C_1}{B_n^4}\sum_j  b_{nj}^4+C_2\left(\frac{1}{B_n^3}\sum_j | b_{nj}|^3E(|X_1|^3)\right)^2\\
    &\leq C_1n^{-2/3}+C_2\ro^2/n
\end{align*}
Now we do $\ithr$. Denote $Z_j= b_{nj}\y_j/B_n$ and $\psi_{ij}= d_{nij}\psi(\y_i,\y_j)$.
First note that
\begin{align}\label{eq:ltwomain}
    \E\{\psi_{ij}e^{it(Z_i+Z_j)}\}=-t^2\ell_{ij}+\theta_{1ij}(t),
\end{align}
where we have:
\begin{align}\label{eq:lij}
    \ell_{ij}&=\E\left(|\psi_{ij}Z_iZ_j |\right)\leq  | b_{ni} b_{nj} d_{nij}|/B_n^2|\E\{\y_i\y_j\psi(\y_i,\y_j)\}|\leq \ro^{1/2}( b_{ni}^2 b_{nj}^2+ d_{nij}^2)/B_n^2.
\end{align}
Using Eq~\ref{eq:rem} and the fact that $\E\{\psi(\y_i,\y_j)\}=0$ and $\E\{\psi(\y_i,\y_j)\mid \y_i\}=0$,
\begin{align*}%\label{eq:theta1ij}
    \tij&=\E(\psi_{ij}[it \{Z_i R(tZ_j)+Z_j R(tZ_i))+R(tZ_i)R(tZ_j)\}])\notag\\
    &\leq C|t|^{2.5}\E\left(|\psi_{ij}Z_iZ_j^{1.5}|+|\psi_{ij}Z_jZ_i^{1.5}|\right)\notag\\
    &\leq C|t|^{2.5}\E\{|\y_1\y_2^{1.5}\psi(\y_i,\y_j)|\}\left(| d_{nij} b_{ni} b_{nj}^{1.5}/B_n^{2.5}|+| d_{nij} b_{ni}^{1.5} b_{nj}/B_n^{2.5}|\right)\notag\\
    &\leq C|t|^{2.5}(\ro\beta)^{1/2}\left( d_{nij}^2+ b_{ni}^2| b_{nj}|^3+| b_{ni}|^3 b_{nj}^2\right)n^{-5/4}
\end{align*}
Using Eq~\ref{eq:ltwomain}, and setting $\prod_{k\neq i,j}\gamma_k(t)=e^{-t^2/2}+\ttij$ we see:
\begin{align*}
    E(\del_{n,n}e^{itS_n})&=n^{-3/2}\sum_{i<j}\E(\psi_{ij}e^{it S_n})
    =n^{-3/2}\sum_{i<j}\E\{\psi_{ij}e^{it(Z_i+Z_j)}\}\prod_{k\neq i,j}\gamma_k(t)\\
    &=n^{-3/2}\sum_{i<j}\{-t^2\lij+\tij(t)\}\left(e^{-t^2/2}+\ttij\right)\\
    &=n^{-3/2}\sum_{i<j}\{-t^2\lij e^{-t^2/2}+\tttij(t)\}=\underbrace{-\kn t^2 e^{-t^2/2}}_{\phi_{2,n}(t)}+\underbrace{n^{-3/2}\sum_{i<j} \tttij}_{\rnf},
\end{align*}

where using Lemma A.4 in~\cite{wang-jing-weighted-bootstrap-u-statistics}, for $|t|<n^\epsilon << n^{1/6}$
\begin{align*}
    |\ttij|&\leq \frac{C}{n^{1/2}}\left(\beta+\frac{ b_{nj}^2+ b_{ni}^2}{n^{1/2}}\right)(t^2+t^4)e^{-t^2/8}
\end{align*}
Furthermore, using Lemma A.4 and $\sum_i | b_{ni}|^3\leq \ell_2 n$
\begin{align*}
    |\tttij|&\leq t^2|\lij\ttij|+|\tij|\prod_{k\neq i,j}\gamma_k(t)\leq t^2|\lij\ttij|+4|\tij|e^{-t^2/8}\notag\\
    |\lij\ttij|&\leq \frac{C}{n^{1/2}}|\lij|\left(\beta+\frac{ b_{nj}^2+ b_{ni}^2}{n^{1/2}}\right)(t^2+t^4)e^{-t^2/8}
    \end{align*}
    Summing the above expression over $i<j$, we also have,
    \begin{align}\label{eq:tttij}
    &\sum_{i<j}|\lij\ttij|\notag\\
    &\leq C\lambda^{1/2}\left(\beta \frac{B_n^4+l_{4,n} n^2}{n^{3/2}}+\frac{\sum_{i<j}| d_{nij}|(| b_{ni}^3 b_{nj}|+| b_{ni} b_{nj}^3|)}{n^2}\right)(t^2+t^4)e^{-t^2/8}\notag\\
    & \leq C\lambda^{1/2}\left[\beta \frac{B_n^4+l_{4,n} n^2}{n^{3/2}}+\frac{c}{n^2}%\frac{\sum_{i<j}( d_{nij}^2+ b_{ni}^2)}{n}\right)
    \underbrace{\left\{\left(\sum_{i<j} d_{nij}^2\right)\left(\sum_{i<j} b_{ni}^6 b_{nj}^2\right)\right\}^{1/2}}_{A}\right](t^2+t^4)e^{-t^2/8}
\end{align}
To bound (A) we see:
\begin{align*}
    (A)&\leq %\frac{\sum_{i<j}( d_{nij}^2+ b_{ni}^2)}{n}\right)
    \left\{(n^2l_{4,n})(n\ell_2)\sum_{i<j} b_{ni}^3 b_{nj}^2\right\}^{1/2}\leq n^{3/2}(\ell_2l_{4,n})^{1/2}\left\{\left(\sum_{i} b_{ni}^3\right)\left(\sum_j b_{nj}^2\right)\right\}^{1/2}\\
&\leq c' n^{5/2}l_{4,n}^{1/2}\ell_2
\end{align*}
Plugging this back in Eq~\ref{eq:tttij}, and assuming WLOG $l_{4,n}\geq 1$,
\begin{align*}
    \sum_{i<j}|\lij\ttij|&\leq C'\lambda^{1/2}\left(\beta \frac{B_n^4+l_{4,n} n^2}{n^{3/2}}+\frac{1}{n^2} n^{5/2}\ell_2l_{4,n}^{1/2}\right)(t^2+t^4)e^{-t^2/8}\notag\\
    &\leq C'l_{4,n}\ro^{1/2}\beta n^{1/2}(t^2+t^4)e^{-t^2/8}
\end{align*}
Finally, we also have:
\begin{align*}
    \sum_{i<j}|\tij|&\leq C|t|^{2.5}(\ro\beta)^{1/2}
    \left(l_{4,n} n^2+2\ell_2 n B_n^2 \right)n^{-5/4}\leq C|t|^{2.5}(\ro\beta)^{1/2}l_{4,n}n^{1/4}
\end{align*}
Finally we have, since $t^4\leq |t|+|t|^6$, and $|t|^{2.5}\leq |t|+|t|^6$,
\begin{align*}
    \rnf&\leq n^{-3/2}\sum_{i<j}|\tttij|\leq n^{-3/2}\left(\sum_{i<j}t^2|\lij\ttij|+4\sum_{i<j}|\tij|e^{-t^2/8}e^{-t^2/8}\right)\\
    &\leq \left(t^2l_{4,n}\ro^{1/2}(t^2+t^4)e^{-t^2/8}n^{-1}+|t|^{2.5}(\ro\beta)^{1/2}l_{4,n}n^{-3/4}e^{-t^2/8}\right)\\
    &\leq l_{4,n}\left(\ro^{1/2}\beta n^{-1}+(\ro\beta)^{1/2}n^{-3/4}\right)(|t|+|t|^6)e^{-t^2/8}\\
    &\leq C'l_{4,n}\left(\beta^2 n^{-1}+(\ro+\beta)n^{-3/4}\right)(|t|+|t|^6)e^{-t^2/8}\\
\end{align*}
Finally, for $\ithr$, we have:
\begin{align*}
    |\ithr|&\leq \int_{|t|\leq n^\epsilon} |t|^{-1}\rnf dt\\
    &\leq  C'l_{4,n}\left(\beta^2 n^{-1}+(\ro+\beta)n^{-3/4}\right)\int_{|t|\leq n^\epsilon} (1+|t|^5)e^{-t^2/8} dt\\
    &\leq C'1'l_{4,n} \left(\beta^2 n^{-1}+(\ro+\beta)n^{-3/4}\right)
\end{align*}

Now we will bound $\ifour$. 
% Before bounding this term, we will state and proof a lemma involving deviations of constants from a sample mean.  Our lemma is closely related to concentration of sums sampled without replacement from a finite population. In fact, it implies the without-replacement Chebychev inequality; see, for example, Corollary 1.2 of \citet{serfling-concentration-without-replacement}.  We will then use this lemma to construct a ``good set" for which $\alpha_i$ are well-behaved.  

% \begin{lemma} Let $x_1 ,\ldots, x_n$ be constants in $\mathbb{R}$ and let $\bar{x}_n = \frac{1}{n}\sum_{i=1}^n x_i$ and $s_n^2 = \frac{1}{n}\sum_{i=1}^n (x_i - \bar{x})^2$  Define the set:
% \begin{align}
%     \Gamma_k =  b_{ni}gl\{x_i > \bar{x} + k s_n   b_{ni}gr\}
% \end{align}
% Then,
% \begin{align*}
% |\Gamma_k| \leq \frac{n}{k^2} 
% \end{align*}
% \end{lemma}
% \begin{proof}\normalfont
% Observe that:
% \begin{align*}
% s_n^2 &\geq \frac{1}{n}\sum_{i \in \Gamma_k} (x_i-\bar{x}_n)^2
% \\ &= \frac{1}{n}\sum_{i \in \Gamma_k} k^2 s_n^2  \implies  |\Gamma_k | \leq \frac{n}{k^2}  
% \end{align*}
% \end{proof}






Define $\Omega:=\{k:\min(1/2,\ell_2/\ell_1^{3/2})\leq n^{1/2}b_{n,k}/B_n\leq 2\ell_2/\ell_1^{3/2}\}$. Using Lemma A.5 in~\cite{wang-jing-weighted-bootstrap-u-statistics}\bk, we see that $|\Omega|\geq c_0 n$, for some $c_0\in (0,1)$. 


% Recall that $\alpha_{n,i}:=\sum_j d_{ij}^2/n$, $l_{4,n}:=\sum_i \alpha_{n,i}/n$, and $s_n^2:=\sum_i (\alpha_{ni}-l_{4,n})^2/n$. 
% Let $\Gamma:=\{i|\alpha_i\geq \bar{\alpha}+ks_n\}$. Note that:
% \begin{align*}
%     s_n^2&=\frac{1}{n}\sum_i (\alpha_i-\bar{\alpha})^2\geq \frac{1}{n}\sum_{i\in \Gamma} k^2s_n^2=\frac{k^2s_n^2|\Gamma|}{n}
% \\    & \implies  |\Gamma|\leq \frac{n}{k^2}
% \end{align*}
Now, let $\Gamma:=\{i \ | \ \alpha_i\geq \bar{\alpha}+ks_n\}$. Applying Lemma \ref{lemma:deterministic-deviation-identity} and setting $k=\sqrt{2/c_0}$, we see that $|\Gamma^c|\geq n (1-c_0/2)$. Therefore, $|\Gamma^c \cap \Omega|\geq n c_0/2$. Let $k_0=\lfloor c_0/2\rfloor.$

WLOG assume $b_{n,1}\dots b_{n,k_0n}\in \Omega\cap\Gamma^c$ and $\ell_2/\ell_1^{3/2}\geq 1/2$. Now for $m\in [2,k_0 n]$, we have:

%WLOG assume $b_{n,1}\dots b_{n,k_0n}\in \Omega$ and $\ell_2/\ell_1^{3/2}\geq 1/2$. Now for $m\in [2,k_0 n]$.
\begin{align*}
    S_m=\frac{1}{B_n}\sum_{k=1}^m b_{nk} \y_k\qquad S_m^{i,j}:=\frac{1}{B_n}\sum_{k\neq i,j}b_{nk} X_k
\end{align*}

For $1,\dots, m \leq k_0n$, we have:
\begin{align*}
    \frac{1}{mn}\sum_{i=1}\sum_{j=1,j\neq i} d_{nij}^2=\frac{1}{m}\sum_{i=1}^m\alpha_i\leq l_{4,n}+ks_n=:\ell_{5,n}
\end{align*}

As for $\del_{n,m}$, we have:
\begin{align}\label{eq:delnm}
    E(\del_{n,m}^2)=\frac{\ro}{n^3}\sum_{i=1}^{m-1}\sum_{j=i+1}^n  d_{nij}^2\leq \ro l_{5,n}\frac{m}{n^2}
\end{align}

Now we use the decomposition in~\cite{bickel1986edgeworth} (17)-(22).
\begin{align*}
    \E(e^{it V_n})&=\E\{e^{it (V_n-\del_{n,m})}e^{it \del_{n,m}}\}\\
    &=\E\{e^{it (V_n-\del_{n,m})}(1+it \del_{n,m})\}+R_{n,5}\\
    &=\E\{e^{it (V_n-\del_{n,m})}(1+it \del_{n,m})\}+Ct^2 \lambda  \lfn m/n^2\\
    &=\E\{e^{it (V_n-\del_{n,m})}\}+\frac{it}{n^{3/2}}\sum_{i=1}^m\sum_{j=i+1}^n 
    \underbrace{\E\{e^{it (V_n-\del_{n,m})}\psi_{ij}\}}_{D_{ij}}+Ct^2\ro \lfn \frac{m}{n^2}
    %&\stackrel{|.|}{\leq} |\E[e^{it (V_n-\del_{n,m})}(1+it \del_{n,m})]|+\\
\end{align*}
where the last line is obtained using Eqs~\ref{eq:rem} and~\ref{eq:delnm}, as follows:
\begin{align*}
    R_{n,5}\leq |\E\{e^{it (V_n-\del_{n,m})}t^2\del_{n,m}^2\}|\leq Ct^2 \lambda   l_{5,n} \bk m/n^2
\end{align*}
Note that $V_n-\del_{n,m}$ can be written as $S_{m-1}+Y_{m,n}$, where $Y_{m,n}$ does not depend on $\y_1,\dots,\y_{m-1}$. 
 So we will write:
 \begin{align*}
     \left|\sum_{i=1}^{m-1}\sum_{j=i+1}^n(D_{ij}) \right| &= \left|\sum_{i=1}^{m-1}\sum_{j=i+1}^n\E\{e^{it (S_{m-1}^{ij}+\psi_{ij}+Y_{m,n})}\psi_{ij}\} \right|\\
     &=\left|\sum_{i=1}^{m-1}\sum_{j=i+1}^n\E\{e^{it S_{m-1}^{ij}}\}\E\{e^{(\psi_{ij}+Y_{m,n})}\psi_{ij}\} \right| \\
     &\leq \sup_{i<j}|\E(e^{it S_{m-1}^{ij}})|\sum_{i=1}^{m-1}\sum_{j=i+1}^n\E(|\psi_{ij}|)\\
     &\leq \sup_{i<j}|\E(e^{it S_{m-1}^{ij}})|\sum_{i=1}^{m-1}\sum_{j=i+1}^n| d_{nij} | \E\{|\psi(\y_i,
     \y_j)|\}\\
     &\leq \ro^{1/2}\sup_{i<j}|\E(e^{it S_{m-1}^{ij}})|\sqrt{mn\sum_{i=1}^{m-1}\sum_{j=i+1}^n d_{nij}^2}\\
     &\leq \sqrt{\lambda  \lfn}\sup_{i<j}|\E(e^{it S_{m-1}^{ij}})| mn\\
 \end{align*}
 Plugging it back, we have:
 \begin{align}\label{eq:vncharac}
   |\E(e^{it V_n})|\leq   |\E(e^{it S_{m-1}})|+\frac{|t|}{n^{3/2}}\sqrt{\lambda  \lfn}\sup_{i<j}|\E(e^{it S_{m-1}^{ij}})| mn+Ct^2\lambda  \lfn \frac{m}{n^2}
 \end{align}
 Now, we have for $|t|\leq 1/4n^{1/2}/\E(|\y_1|^3)$
 \begin{align*}
     |\E(e^{itS_{m}})|\leq e^{-c_0 mt^2/n}\qquad |\E(e^{itS_{m}^{ij}})|\leq e^{-c_0(m-2)t^2/n}
 \end{align*}
 Taking $m=[6n\log n/c_0 t^2]+1$ (for a large enough $\epsilon$, this is still smaller than $k_0n$), from Eq~\ref{eq:vncharac} we have:
 \begin{align*}
     &\int_{n^\epsilon \leq |t|<1/4n^{1/2}/\E(|\y_1|^3)}|t|^{-1}\left|\E (e^{itV_n})\right|dt\\
     &\leq \int_{n^\epsilon \leq |t|<1/4n^{1/2}/\E(|\y_1|^3)} \left(\frac{e^{-c_0mt^2/n}}{|t|}+\frac{m}{n^{1/2}}\sqrt{\lambda  \lfn}e^{-c (m-2)t^2/n}+C|t|\lambda \lfn \frac{m}{n^2}\right)dt\\
     &\leq C'\lambda \lfn \frac{\log^2 n}{n}
 \end{align*}
 Now we will deal with the range $1/4n^{1/2}/\E(|\y_1|^3)\leq |t|\leq n^{1-c}$. Since $\kappa(\y_1)>0$, and hence for large enough $n$, 
 \begin{align*}
 |\gamma_k(t)|&\leq 1- \kappa(\y_1) \\
     |\E(e^{itS_{m}})|&\leq e^{-m\kappa(\y_1)}\\
     \E(e^{itS_{m}^{ij}})|&\leq e^{-(m-2)\kappa(\y_1)} 
 \end{align*}
 Using this in conjunction with Eq~\ref{eq:vncharac}, and setting $m=[4\log n/\kappa(\y_1)]+2$,
 \begin{align*}
      &\int_{1/4n^{1/2}/\E(|\y_1|^3)\leq |t|\leq n^{1-c}}|t|^{-1}\left|\E (e^{itV_n})\right|dt\\
      &\int_{1/4n^{1/2}/\E(|\y_1|^3)\leq |t|\leq n^{1-c}}\left(\frac{e^{-\kappa(\y_1)m}}{|t|}+\frac{m}{n^{1/2}}\sqrt{\lambda  \lfn}e^{-\kappa(\y_1)(m-2)}+C|t|\lambda \lfn \frac{m}{n^2}\right)\\
      &\leq C'\frac{\rho_n \lfn}{\kappa(\y_1)}\frac{\log n}{n^2}n^{2(1-c)}=C'\frac{\lambda  \lfn}{\kappa(\y_1)}\frac{\log n}{n^{2c}}
 \end{align*}
 
 Thus, using the bounds on $\ione,\itwo,\ithr$ and $\ifour$ along with Eq~\ref{eq:esseen}, Eq~\ref{eq:knbound} we get:
 \begin{align*}
     &\sup_x|P(V_n\leq x)-E_{2n}(x)|\\
     &\leq \sum_{i=1}^4 I_{n,i}+C'\frac{\beta+(1+\ro)l_{4,n}/n^{1/2}}{n^{1-c}}\\
     &\leq C\left(\frac{(1+\ro)l_{4,n}}{n^{1-2\epsilon}}+n^{-2/3}+l_{4,n}(\ro+\beta+\beta^2)n^{-3/4}+\frac{\lambda  \lfn}{\kappa(\y_1)}\frac{\log n}{n^{2c}}\right)+C'\frac{\beta+(1+\ro)l_{4,n}/n^{1/2}}{n^{1-c}}\\
     &\leq (l_{4,n}+ks_n)\frac{\log n}{n^{2/3}}
 \end{align*}
 The last line assumes $\beta,\ro$ and $\kappa(\y_1)$ are all bounded.
\end{proof}


\subsection{Proof of Lemma~\ref{lem:thirdabsmoment}}
\begin{proof}\normalfont
Let $X\sim N(1,c_1^2)$ and $Y\sim N(1,c_2^2)$ be two independent random variables. We have $\w_1=XY$.%Since $x^3$ is convex for $x>0$, using Jensen's inequality, we have:
\begin{align*}
    \E(|XY-1|^3) &\leq  \E(|XY|^3)+1+3\E(X^2|Y|)+3\E(|X|Y^2)\\
    &=\E(|X|^3)\E(|Y|^3)+3\E(X^2)\E(|Y|)+3\E(|X|)\E(Y^2)\\
    &<\infty
\end{align*}
The last step is true because both $\E(|X|^3)$ and $\E(|Y|^3)$ are bounded for bounded $c_1,c_2$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% commenting all of this out. 
\iffalse
Now we derive the characteristic function of $T_{n,1}^*+T_{n,2}^*$. 
\begin{equation} \label{eq:wb-chf-tn1tn2}
    E[e^{it(T_{n,1}^*+T_{n,2}^*)}]= E[e^{itT_{n,1}^*}(1+itT_{n,2}^*+  O_P\left(T_{n,2}^{*2}t^2\right))]
\end{equation}
Since $T_{n,2}^*$ is $O_P(n^{-1/2})$, the last term $O_P\left(T_{n,2}^{*2}t^2\right))$ is $O_P(n^{-1})$, thus ignorable. Now, we denote $\varphi_n^n$ the characteristic function of sum of $n$ independent but not identical distributed variables, $\varphi_{-ij}$ as $\varphi_n^n$ excluding variable $i$ and $j$th element in the sum.  Following \cite{petrov2012sums}  Chapter VI Lemma 11 \bk,  $|t| < n^{\epsilon}$ for a small enough fixed $\epsilon$, we have the first term in the RHS of  eq~\ref{eq:wb-chf-tn1tn2} is
\begin{align}\label{eq:wb-chf-tn1}
    E[e^{it T_{n,1}^*}]&= e^{-\frac{t^2}{2}}\left(1-\frac{it^3}{6n^{1/2}\tau^3}\underbrace{\frac{\sum_j E[(\w_j-1)^3(\hat{H}_1(x_j)-\tnhat)^3}{n}}_{D_n}\right) +O_P(n^{-1/2}e^{-t^2/2}Poly(t)).\\
     &\text{(if we take expectation jointly)}\\
     &= e^{-\frac{t^2}{2}}\left(1-\frac{it^3}{6n^{1/2}\tau^3} D_n\right) +O_P(n^{-1/2}e^{-t^2/2}Poly(t)).
\end{align}
For the second term in RHS in eq~\ref{eq:wb-chf-tn1tn2}, for $|t| < n^{\epsilon}$ we have  Purna fix, \bl

Let $\varphi_n^{-ij} $ be defined as follows:
\begin{align*}
    \varphi_n^{-ij} &= E \left[ \exp\left(\frac{it}{n^{1/2}\tau}\sum_{k\neq i,j}f_1(\w_i)\right)\right]\\
    &=e^{-\frac{t^2}{2}}\left(1-\frac{it^3}{6n^{1/2}\tau^3}\frac{\sum_{k\not\in \{i,j\}} E[(\w_k-1)^3(\hat{H}_1(x_k)-\tnhat)^3}{n-2}\right) +O_P(n^{-1/2}e^{-t^2/2}Poly(t))\\
    &=e^{-\frac{t^2}{2}}\left(1-\frac{it^3}{6n^{1/2}\tau^3}\underbrace{\frac{\sum_{k\not\in \{i,j\}} (\hat{H}_1(x_k)-\tnhat)^3}{n-2}}_{D_n^{-ij}}\right) +O_P(n^{-1/2}e^{-t^2/2}Poly(t))\\
\end{align*}

\begin{equation}\label{eq:wb-chf-tn1timestn2}
    \begin{split}
         E_*[e^{itT_{n,1}^*}\times it T_{n,2}^{*}] &= \sum_{i<j }\varphi_n^{-ij} E_*\left[e^{\frac{it f_1(\w_i)+f_1(\w_j)}{\taun^{1/2}}}\times it \frac{(r-1)}{n^{1/2}(n-1)\tau}\sum_{i<j}f_2(\w_i,\w_j)\right] \\
          &= \sum_{i<j} \varphi_n^{-ij} \times \frac{it(r-1)}{\taun^{1/2}(n-1)} E_*\left[\frac{it(f_1(\w_i)+f_1(\w_j))}{n^{1/2}\tau}\times  f_2(\w_i,\w_j)+...\right.\\
          &\left. \left(\frac{t (f_1(\w_i)+f_2(\w_j))}{n^{1/2}\tau^}\right)^2 f_2(\w_i,\w_j)+O\left(\frac{it(f_1(\w_i)+f_1(\w_j))}{n^{1/2}\tau}\right)^{3}f_2(
          \w_i,\w_j)\right]\\
          &=e^{-t^2/2}\frac{it(r-1)}{n^{1/2}(n-1)}\sum_{i<j}\left(t^2\frac{2\hat{g}_1(X_i)\hat{g}_1(X_j)\hat{g}_2(X_i,X_j)}{n^{1/2}\tau^2} ...\right.\\
          &+O\left(\frac{t^5 D_n^{-ij}}{n^{1/2}\tau^3}\frac{(\hat{g}_1(X_i)+\hat{g}_1(X_j))\hat{g}_2(X_i,X_j)}{n^{1/2}\tau^2} \right)
     \end{split}
\end{equation}
Taking an outer expectation w.r.t the data,
\begin{equation}\label{eq:wb-chf-tn1timestn2}
    \begin{split}
         E[e^{itT_{n,1}^*}\times it T_{n,2}^{*}] 
          &=e^{-t^2/2}{n\choose 2}\frac{it(r-1)}{n^{1/2}(n-1)}E\left[t^2\frac{2\hat{g}_1(X_i)\hat{g}_1(X_j)\hat{g}_2(X_i,X_j)}{n^{1/2}\tau^2} ...\right.\\
          &\left.+ O\left(\frac{t (\hat{g}_1(X_i)+\hat{g}_1(X_j))}{n^{1/2}\tau^}\right)^3 |\hat{g}_2(X_i,X_j)|+...\right.\\ &\left.+O\left(\frac{t^5 D_n^{-ij}}{n^{1/2}\tau^3}\frac{(\hat{g}_1(X_i)+\hat{g}_1(X_j))\hat{g}_2(X_i,X_j)}{n^{1/2}\tau^2} \right)\right]\\
          &=e^{-t^2/2}
          \left[\frac\right]
     \end{split}
\end{equation}
\begin{align*}
    \varphi_{-ij}(t)\frac{it(r-1)n^{1/2}}{2}E \bigg{\{}\frac{f_2(\w_1,\w_2)}{\tau}\times  \bigg{[}1+\frac{it}{\taun^{1/2}}(f_1(\w_1)+f_2(\w_2))- \\ &\frac{t^2}{n\tau^2}(f_1(\w_1)^2+f_2(\w_2)^2+2f_1(\w_1)f_2(\w_2))  \bigg{]} \bigg{\}} +O_P (n^{-1/2}e^{-t^2/2} |t|Poly(t))\\
        &= -\frac{it^3(r-1)}{2n^{1/2}\tau^3}e^{-t^2/2}E[f_1(\w_1)f_2(\w_2)f_2(\w_1,\w_2)] + O_P (n^{-1/2} e^{-t^2/2}|t|Poly(t))
\end{align*}
\bk The third equality in RHS of eq~\ref{eq:wb-chf-tn1timestn2} follows from the Hoeffding decompsition that 
\begin{align*}
    & E[f_1(\w_1) f_2(\w_1,\w_2)]=0\\
    & E[f_1(\w_1)^2 f_2(\w_1,\w_2)]=0.
\end{align*}
Now we look at the final RHS expression of eq~\ref{eq:wb-chf-tn1} and eq~\ref{eq:wb-chf-tn1timestn2}. Recall the definition of $g_1(x_i)$ and $g_2(x_i,x_j)$ in eq~\ref{eq:g1g2}. Thus, when the conditions of $\w_i$ below hold, 
\begin{equation*}
    E[\w_i]=1, \ \var[\w_i]=1, \ E[(\w_i-1)^3]=1, 
\end{equation*}
we have,
\begin{equation}\label{eq:wb-ef13-ef1f2}
\begin{split}
 &E[f_1(\w_1)^3]=E[(\w_1-1)^3(\hat{H}_1(x_1)-\tnhat)^3]=(\hat{H}_1(x_1)-\tnhat)^3, \\
       &E[f_1(\w_1)f_2(\w_2)f_2(\w_1,\w_2)]= (\w_1-1)(\hat{H}_1(x_1)-\tnhat)(\w_2-1)(\hat{H}_1(x_2)-\tnhat)\\ &\times[(\w_1 \w_2-1)(\hat{H}_2(x_i,x_j)-\tnhat)-(\w_1-1)(\hat{H}_1(x_1)-\tnhat)-(\w_2-1)(\hat{H}_1(x_2)-\tnhat)]\}\\
       &= E\{((\hat{H}_1(x_1)-\tnhat)(\hat{H}_1(x_2)-\tnhat)\times[(\hat{H}_2(x_i,x_j)-\tnhat)-(\hat{H}_1(x_1)-\tnhat)-(\hat{H}_1(x_2)-\tnhat)].%\\&= E[g_1(x_1)g_1(x_2)g_2(x_1,X2)].
\end{split}
\end{equation}

Thus, combining eq~\ref{eq:wb-chf-tn1tn2},eq~\ref{eq:wb-chf-tn1}, eq~\ref{eq:wb-chf-tn1timestn2} with eq~\ref{eq:wb-ef13-ef1f2} %and eq~\ref{eq:wb-vntn-to-tn1tn2},  
we have, for  a fixed small enougth $\epsilon$ and $|t|<n^\epsilon$,
\begin{equation*}\label{eq:wb-ftn-gn}
    \int_0^{n^{\epsilon}} \bigg{|}\frac{F_{T_{n,1}^*+T_{n,2}^*}(t)-\hat{G}_n(t)}{t} \bigg{|}=O_P(n^{-1/2}).
\end{equation*}

Now we prove for $|t| \in (n^\epsilon,n^{\delta})$ (for $1-c<\delta <1$ for small constant $c$), 
\begin{equation*}
    \int_{n^{\epsilon}}^{n^{\delta}} \bigg{|}\frac{F_{T_{n,1}^*+T_{n,2}^*}(t)-\hat{G}_n(t)}{t} \bigg{|}=O_P(n^{-1/2}).
\end{equation*}
From \cite{zhang-xia-network-edgeworth}, we know 
\begin{equation*}
     \int_{n^{\epsilon}}^{n^{\delta}} \bigg{|}\frac{\hat{G}_n(t)}{t} \bigg{|}=O_P(n^{-1}).
\end{equation*}
Thus we want to show 
\begin{equation*}
    \int_{n^{\epsilon}}^{n^{\delta}} \bigg{|}\frac{F_{T_{n,1}^*+T_{n,2}^*}(t)}{t} \bigg{|}= small ?\bk 
\end{equation*}
%For the ease of notation, from below we denote 
Following \cite{bickel1986edgeworth}, we define
\begin{equation*}
    \dnm = \frac{r(r-1)}{n(n-1)\hat{\sigma}_n}\times \sum_{i=1}^m\sum_{j>i}f_2(\w_i,\w_j).
\end{equation*}
Then we have 
\begin{equation*}
    \tnas+\tnbs -\dnm =  \underbrace{\frac{\sum_{i=1}^mf_1(\w_i)}{n\hat{\sigma}_n}}_{y_1}+\underbrace{\frac{\sum_{i=m+1}^n\sum_{j>i}f_2(\w_i,\w_j)}{n(n-1)\hat{\sigma}_n}+\frac{\sum_{i=m+1}^nf_1(\w_i)}{n\hat{\sigma}_n}}_{y_2},
\end{equation*}
where $y_1$ and $y_2$ are independent. 
Now we rewrite $E[e^{it(\tnas+\tnbs)}]$ into
\begin{equation*}
    \begin{split}
     E[e^{it(\tnas+\tnbs)}] &=   E\left[e^{it(\tnas+\tnbs-\dnm)}\left(1+\sum_{\nu=1}^{r-1}(it)^{\nu}\dnm  +  O_P(\dnm^r t^r)\right)\right] \bk \\
     & = \sum_{\nu=0}^{r-1} (it)^{\nu}J_{r,\nu} +  O_P(n^{-r/2} t^r) \bk,
    \end{split}
\end{equation*}
where 
\begin{equation*}
    J_{r,\nu}= E[e^{it(y_1+y_2)}\dnm^{\nu}] =  E\left[e^{it(y_1+y_2)}\sum_{S'}\prod_{\{i,j\}\in S'}f_2(\w_1,\w_2)/\hat{\sigma}_n^{\nu}\right],
\end{equation*}
in which $S'$ denotes a set of node pairs, $|S'|=\nu$. Denote $N_{S'}=\left\{i | \text{ exist } j\neq i, (i,j) \in S' \right\}$,then $|N_S'| \leq 2\nu$. Let $\bar{N}_{S'}$ be $\{1:m\} $ excluding $N_S$. $|\bar{N}_{S'}| \geq m-2\nu$. Then we can further write $J_{r,\nu}$ into
\begin{equation*}
    J_{r,\nu}=\sum_{S'\in \mathcal{S'}}\sum_{k\in\bar{N}_{S'}}E[e^{itf_1(\w_k)/\hat{\sigma}_n}]E[e^{it(y_2+\sum_{k \in N_S}f_1(\w_k))/\hat{\sigma}_n}].
\end{equation*}
For the first term of the RHS above, we have
\begin{equation*}
\begin{split}
      \psi_{k}^n(t)&= E[e^{itf_1(\w_k)/\hat{\sigma}_n}]= 1+E(itf_1(\w_k)/\hat{\sigma}_n)-\frac{t^2}{\hat{\sigma}_n^2}E(f_1(\w_k)^2)  ?? +O\left(\frac{t^2}{\sigma_n^2}\right)\bk   \leq 1-\frac{c_k^2}{\hat{\sigma}_n^2}t^2,\bk
\end{split}
\end{equation*}
for $\alpha < 1$ and $t< \epsilonn^{1/2}$ and $c_k=\hat{H}_1(x_k)-\tnhat$. Thus,
\begin{equation*}
    \prod_{k\in N_{S'}}\psi_{k}^n(t) \leq e^{-\alpha\sum_{k\in N_{S'}}c_k^2/\hat{\sigma}^2_n}.
\end{equation*}
\fi 
%%%%%%%%%%%%%%%%%%%%%%%%
%Thus, combining eq~\ref{eq:wb-chf-tn1} and eq~\ref{eq:wb-chf-tn1timestn2} into \ref{eq:wb-chf-tn1tn2}, we proved that the the characteristic function of $(T_{n,1}^*+T_{n,2}^*)$ is 
%\begin{equation*}%\label{eq:wb-chftn1tn2-final}
%\begin{split}
%      E\left[e^{it(T_{n,1}^*+T_{n,2}^*)}\right] = e^{-\frac{t^2}{2}}\left(1- it^3\frac{1}{6n^{1/2}\tau^3}[E[g_1^3(x_1)] +3(r-1)E[g_1(x_1)g_1(x_2)g_2(x_1,x_2)]]\right)\\
 %     + O_P(n^{-1}e^{-\frac{t^2}{4}}|t|Poly(t)).
%\end{split}
%end{equation*}



% \clearpage
% % b_{ni}bliography{references}
%  b_{ni}bliography{paper-draft/network_mb.bib}



% \end{document}



\input{supp-addsmf3.tex}




\bk



\section{Additional experiments}
\label{sec:addlexp}
In this section we provide additional experiment results that were left out from the main text for space concerns.


%\subsection{Competing algorithms}
%In this section, we describe normalization for the completing methods for count functionals and their smooth functions. %For triangles and V stars, for 

\iffalse
%\subsection{Additional Experiments}
We have shown timing results for triangle and two-star frequencies for the \sbm model against sample size $n$ in the main paper. Now we show below the computation time of triangles and two-star frequencies in \smg. 

\begin{figure*}
\centering
\begin{tabular}{cc}
     \includegraphics[ trim=0em 1em 0em 5em, clip,width=  .45\textwidth]{plots2/time-tri-smg.pdf}
     &\includegraphics[ trim=0em 1em 0em 5em, clip,width=  .45\textwidth]{plots2/time-ts-smg.pdf} 
\end{tabular}
\caption{From left to right, we present log of computation time of triangle frequencies in SM-G and two-star frequencies of SM-G against sample size $n$. }
%\label{plot:additional-timing}
\end{figure*}
\fi

\subsection{Simulation study for \smg and additional results for \sbm}
Here we first present experimental results on the smooth graphon model from~\cite{zhang2017smooth} (\smg)  with  $w(u,v)=(u ^2+v^2)/3\times cos(1/(u^2+v^2))+0.15$.  This graphon is continuous and high rank in contrast to the first graphon, which is piece-wise constant and low rank.  %Note for the \ls method applied to the smooth graphon \smg model, we use the \usvt algorithm to estimate the number of latent variables.
\begin{figure}[h]
\vspace{-5mm}
\centering
%\begin{tikzpicture}[zoomboxarray,  zoomboxarray inner gap=.5cm, zoomboxarray columns=1, zoomboxarray rows=1]
 %   \node [image node] { \includegraphics[width=0.35\textwidth]{plots2/sbm-triangles.pdf}};
 %  % \zoombox{0.175,0.9}
 %   \zoombox[magnification=2]{.15,.7}
   % \zoombox{0.15,0.3}
    %\zoombox[magnification=10]{0.86,0.35}
%\end{tikzpicture}
\begin{tikzpicture}[zoomboxarray,
zoomboxarray inner gap=.5cm, 
zoomboxarray columns=1, 
zoomboxarray rows=1]
    \node [image node] { \includegraphics[width=0.35\textwidth]{plots2/ng2-triangles.pdf} };
   % \zoombox{0.175,0.9}
    \zoombox[magnification=2]{.15,.7}
   % \zoombox{0.15,0.3}
    %\zoombox[magnification=10]{0.86,0.35}
\end{tikzpicture}\\
%\begin{tikzpicture}[zoomboxarray,
%zoomboxarray inner gap=.5cm, 
%zoomboxarray columns=1, 
%zoomboxarray rows=1]
%    \node [image node] { \includegraphics[width=0.35\textwidth]{plots2/sbm-triangles-centerbytnhat.pdf} };
   % \zoombox{0.175,0.9}
%    \zoombox[magnification=2]{.15,.7}
   % \zoombox{0.15,0.3}
    %\zoombox[magnification=10]{0.86,0.35}
%\end{tikzpicture}\\
\begin{tikzpicture}[zoomboxarray,
zoomboxarray inner gap=.5cm, 
zoomboxarray columns=1, 
zoomboxarray rows=1]
    \node [image node] { \includegraphics[width=0.35\textwidth]{plots2/ng2-triangles-centerbytnhat.pdf} };
   % \zoombox{0.175,0.9}
    \zoombox[magnification=2]{.15,.7}
   % \zoombox{0.15,0.3}
    %\zoombox[magnification=10]{0.86,0.35}
\end{tikzpicture}
\vspace{-3mm}
\caption{We plot \KL{$F_n$}{$F_n^*$} \bk for triangle density for all methods on the $Y$ axis, where $F_n^*(t)$ corresponds to the appropriate resampling distribution. We vary the sparsity parameter $\rho_n$ on the $X$ axis. The networks are simulated from \smg. The first row are centered at bootstrap mean and normalized by variance estimation from each method $\hat{\sigma}_n$  The second row is centered by triangles density estimated on the whole graph (\mblapx is centered at approximate triangle density estimated from the whole graph) and normalized by $\hat{\sigma}_n$.}
\label{plot:cdf-error-smg}
\end{figure}


\begin{figure}[!htb]
%\begin{tabular}{cc}
     \includegraphics[trim=2em 2em 0em 0em, clip, width=  .5\textwidth]{plots2/corrected-triangles-sbm.pdf}%&\includegraphics[trim=2em 2em 0em 0em, clip,width=  .5\textwidth]{plots2/corrected-triangles-ng2.pdf}\\
     \includegraphics[trim=2em 2em 0em 0em, clip,width=  .5\textwidth]{plots2/corrected-trans-sbm-new.pdf}%&\includegraphics[trim=2em 2em 0em 0em, clip,width=  .5\textwidth]{plots2/corrected-trans-ng2-new.pdf}%\\
   % (A)&(B)
%\end{tabular}
\caption{ We present coverage of  95\% Bootstrap Percentile CI with correction for triangles (left) and transitivity coefficient (right) of the \smg model  with $\rho_n$ varying from $0.05$ to $1$.}
\label{plot:coverage-smg}
\end{figure}


 Figure~\ref{plot:cdf-error-smg} and Figure~\ref{plot:coverage-smg} show simulation results of triangles and transitivity for \smg. We show in Figure~\ref{plot:cdf-error-smg}  the maximum of (absolute) difference of the bootstrap CDF $F_n^*$ over the $[-3,3]$ range  (\KL{$F_n$}{$F_n^*$}) for triangles density from the true CDF $F_n$ for sparsity parameter $\rho_n$ varying from $0.05$ to $1$. We show the average of the expected difference over 30 independent runs along with error-bars. In Figure~\ref{plot:coverage-smg}, we show the $95\%$ CI coverage for triangles and transitivity. 
 
 Figure~\ref{plot:cdf-vstar-error} and Figure~\ref{plot:coverage-vs} show additional simulation results for two-stars for both \sbm and \smg. The results of two-stars are similar to those of triangles in the main paper. 

\begin{figure}[H]
%\vskip 0.2in
\begin{tabular}{c}
    \includegraphics[width=  0.45\textwidth]{plots2/sbm-vstar.pdf} 
    \includegraphics[width=  0.45\textwidth]{plots2/ng2-vstar.pdf}\\
    \includegraphics[width=  0.45\textwidth]{plots2/sbm-vstar-centerbytnhat.pdf}\includegraphics[width=  0.45\textwidth]{plots2/ng2-vstar-centerbytnhat.pdf}
  %   \vspace{-2em}
    
%     \includegraphics[trim=0em 1em 0em 5em, clip, width=  \textwidth]{plots/EW-MB-trans-nobar.pdf}
  %     \vspace{-1em}
    %\vspace{-4em}
%    \includegraphics[width=  0.8\textwidth,height=0.4\textwidth]{plots/EW-MB-twostars-nobar.pdf}\\
\end{tabular}
 \caption{We plot  \KL{$F_n$}{$F_n^*$}  for two-star density for all methods on the $Y$ axis, where $F_n^*(t)$ corresponds to the appropriate resampling distribution. We vary the sparsity parameter $\rho_n$ on the $X$ axis. The networks in the left column are simulated from \sbm and those in the right column are simulated from \smg. The first row is centered at bootstrap mean and normalized by variance estimation from each method $\hat{\sigma}_n$  The second row is centered by triangles density estimated on the whole graph (\mblapx is centered at approximate triangle density estimated from the whole graph) and normalized by $\hat{\sigma}_n$. }
%\begin{center}
\label{plot:cdf-vstar-error}
\end{figure}

\begin{figure}[H]
\begin{tabular}{cc}
     \includegraphics[trim=2.5em 2.5em 0em 0em, clip, width=  0.45\textwidth]{plots2/corrected-vs-sbm.pdf}&
     \includegraphics[trim=2.5em 2.5em 0em 0em, clip,width=  0.45\textwidth]{plots2/corrected-vs-ng2.pdf}%\\
      %  \includegraphics[trim=3em 3em 0em 0em, clip, width=  0.45\textwidth]{plots2/correct-v-nocorrect-vs-sbm.pdf}&\includegraphics[trim=3em 3em 0em 0em, clip,width=  0.45\textwidth]{plots2/correct-v-nocorrect-vs-ng2.pdf}\\
   % (A)&(B)
\end{tabular}
\caption{We present coverage of  95\% Bootstrap Percentile CI with correction for two-stars of the \sbm (left) and \smg (right) models  in $\rho_n$ from $0.05$ to $1$. } \label{plot:coverage-vs}
\end{figure}

\paragraph{Timing results for \smg.}
In Figure~\ref{fig:4cycle-timing-ng2} we show logarithm of running time for four-cycles count against growing $n$ for \smg model. 

\begin{figure}[H]
%\begin{tabular}{cc}
\centering
    \includegraphics[width=  .5\textwidth]{plots2/runtime-ng2-fi.pdf} %&
     %\includegraphics[width=  .5\textwidth]{plots2/runtime-ng2-fi.pdf}\\
     %(A)&(B)
%\end{tabular}
\caption{Logarithm of running time for  four-cycles in  \smg  against sample size $n$.}
\label{fig:4cycle-timing-ng2}
\end{figure}

\iffalse
In addition to transitivity CDF Error from SBM, we also show here the transitivity CDF error from SM-G.
\begin{figure*}[h]
\begin{center}
\includegraphics[width=  .5\textwidth]{plots/EW-MB-trans-nobar-smg.pdf}
\caption{ $\E|F_n(u)-F_n^*(u)|$ for the transitivity coefficient of the SM-G model. }
\end{center}
\label{plot:trans-smg}
\end{figure*}
\fi

\subsection{Real data experiments on voting similarities of U.S. Congress}
In this section, we apply our algorithms to compare networks representing the voting similarities of U.S. Congress.
\begin{figure}[H]
	\centering
	\includegraphics[width= \textwidth]{plots2/house-threshold-illustration.png}
	\caption{Threshold for forming edges between congress members calculated from histograms of same-party (SP) and cross-party (CP) agreements, illustrated with example of 81st Congress and 109th Congress}
	\label{fig:votethreshold}
\end{figure}
We use roll call vote data from the U.S. House of Representatives~\citep{voteview} from 1949 (commencement of the 81$^{st}$ Congress) to 2012 (adjournment of 112$^{nd}$ Congress). Each Congress forms a network of representatives (nodes).  An edge between a node pair is formed when the number of agreements, i.e. number of times they both vote \textit{yay} or \textit{nay}  exceeds a threshold computed by~\citep{andris2015votethreshold} of this congress. The threshold is computed by constructing histograms of same-party pairs’ number of agreements and cross-party pair’s number of agreements and using the intersection point of the two histograms as the threshold. We will denote same-party by \texttt{SP} and cross-party by \texttt{CP}. For example, the threshold value is $124$ for $81$st Congress and $766$ for $109^{th}$ Congress as illustrated in Figure~\ref{fig:votethreshold}.
%Now we have a vote record network formed between members for each Congress. 
For each network, we calculate the normalized cross-party edge density and cross-party triangle density, and perform our bootstrap methods on these quantities.  We construct 95\%  second-order corrected Confidence Intervals from  the MB-Q method and present the CIs over $81$st to $112$nd Congress.  Note that the CIs are adjusted by Bonferonni Correction where  $\alpha=1-0.05/32$ for $32$ experiment congresses. 

In Figure~\ref{fig:voteCI}, we can see a significant decrease in cross party edge densities and cross party triangle densities over the years,  suggesting a trend of decreasing bipartisan agreement.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.45\textwidth]{plots2/house-year-mb-cped-bc-quantile-mblinqua.pdf}
    \includegraphics[width=0.45\textwidth]{plots2/house-year-mb-cptri-bc-quantile-mblinqua.pdf}
    \caption{Bonferroni-adjusted 95\% second-order corrected CI for cross party edge density (left) and cross party triangle density (right) from 1949 (commencement of the 81st Congress) to 2012 (adjournment of 112nd Congress).}
    \label{fig:voteCI}
\end{figure}

%%\iffalse
%%\rd REMOVE?
%%We also present here the average timing for $32$ congresses each method takes.
%%%\begin{figure}[H]
%    %\centering
% %   \includegraphics[width=0.47\textwidth]{plots2/runtime-cped.pdf}
% %   \includegraphics[width=0.47\textwidth]{plots2/runtime-cptri.pdf}
% %   \caption{Time in seconds for each method takes on average for $32$ congresses, on cross-party edge density (Left) and cross-party triangle density (Right).}
%  %  \label{fig:votetiming}
%%\end{figure}
%
%%\fi
%%\rd
%%To further illustrate our approximated linear bootstrap algorithm on large sparse networks, we apply \mblapx on Facebook page network dataset. %In the first example, we use the Facebook college network data from \cite{nr}. We compare three college pairs, Yale and Harvard, Duke and Wake Forest University (WFU), Auburn and UGA. Yale and Harvard are both Ivy League colleges; Duke and Wake Forest are both large universities in North Carolina; Auburn and UGA are both large public land-grant research university in the South.  We compare each pair using \mblapx constructed $90\%$ CI of triangles, two-stars and three-paths. Figure~\ref{fig:fb-colleges} shows that triangles can significantly separate all three pairs. Harvard has significantly more normalized counts of triangles compared to Yale, and so does Duke to its comparison Wake Forest, and UGA to Auburn. \sout{Table~\ref{tab:fb-colleges-summary} summarizes the size, edge density and time cost for each network and count statistic.}\bl The size of the networks in this study ranges from around $5000$ to $25000$, edge density ranges from $0.004$ to $0.011$. For example, for UGA of size $24389$ and edge density $0.004$, our approximate three-path calculation takes $18$min $23$s (in total 1103 s) while brute force counting does not finish in $24$ hours. 
%
%
%%\begin{figure}
% %   \centering
%   %    \scriptsize
%   % \begin{tabular}{ccc}
%   % \includegraphics[width=0.3\textwidth]{plots2/Bonf-Colleges_wUGA_CI_tri.pdf}
%  %  &\includegraphics[width=0.3\textwidth]{plots2/Bonf-Colleges_wUGA_CI_vstar.pdf}
%   % &\includegraphics[width=0.3\textwidth]{plots2/Bonf-Colleges_wUGA_CI_3path.pdf}\\
%   % Triangles & two-stars & Three-paths \\
%   % \end{tabular}
%   % \caption{Bonferroni-adjusted $90\%$ CI for three pairs of college comparison with triangles, two-stars and three-path using \mblapx algorithm.}
%    %\label{fig:fb-colleges}
%%\end{figure}
%\iffalse
%\begin{table}[h]
%\scriptsize
%\centering
%\begin{tabular}{|l|c|c|c|c|c|}
%\hline
%        & \multicolumn{1}{l|}{Size} & \multicolumn{1}{l|}{Edge Density} & \multicolumn{1}{l|}{Time Cost (Triangles)} & \multicolumn{1}{l|}{Time Cost (two-stars)} & \multicolumn{1}{l|}{Time Cost (Three-paths)} \\ \hline
%Yale    & 8578                      & 0.011                              & 27.88s                                     & 53.71s                                   & 288.64s                                      \\ \hline
%Harvard & 15126                     & 0.007                              & 62.39s                                     & 134.64s                                  & 691.29s                                      \\ \hline
%Duke    & 9895                      & 0.010                              & 35.18s                                     & 68.10s                                   & 360.51s                                      \\ \hline
%WFU     & 5372                      & 0.019                              & 17.66s                                     & 32.66s                                   & 173.56s                                      \\ \hline
%Auburn  & 18448                     & 0.005                              & 76.81s                                     & 176.90s                                  & 830.76s                                      \\ \hline
%UGA     & 24389                     & 0.004                              & 100.80s                                    & 237.14s                                  & 1103.07s                                     \\ \hline
%\end{tabular}
%\caption{Summaries of size, edge density and time cost for each network and count statistics in the Facebook colleges dataset.}
%\label{tab:fb-colleges-summary}
%
%\boxed{\bl Summarize \ the \ table! }
%\end{table}
%\fi
\subsection{Detailed network statistics and timing for Facebook page networks}
Table~\ref{tab:fb-pages-summary} summarizes the size, edge density, and time cost for different count functionals using our approximate linear bootstraps in the example of Facebook page categories.

\begin{table}[h]
\centering
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|}
\hline
            & Size  & Edge Density & Time Cost (Triangles) & Time Cost (two-stars) & Time Cost (Three-paths) \\ \hline
Athletes    & 13866 & 0.0009       & 11.47s                & 18.40s              & 65.51s                  \\ \hline
Politicians & 5908  & 0.0024       & 2.99s                 & 5.28s               & 47.54s                  \\ \hline
Artists     & 50515 & 0.0006       & 163.15s               & 278.03s             & 843.27s                 \\ \hline
\end{tabular}
\caption{Summaries of size, edge density and time cost for each network and count statistics in the Facebook page dataset.}
\label{tab:fb-pages-summary}
\end{table}

%\section{Fast Precompuation for Approximate Linear Bootstrap in Triangles, two-stars and Three-paths}\label{sec:suppalgapx}
\section{Detailed pseudocode for algorithms}\label{sec:suppalgapx}

In this section, we provide detailed algorithms of our proposed procedures. Algorithm~\ref{alg:apx} presents explicit algorithms of our linear bootstrap and approximated linear bootstrap procedure. Algorithm~\ref{alg:ho} provided explicit algorithms for our proposed higher order correct procedures including quadratic and multiplicative bootstrap procedures. 

%Algorithm~\ref{alg:apx_pretri} and Algorithm~\ref{alg:apx_prevs} and Algorithm~\ref{alg:apx_pre3path} explicitly provide fast pre-compuation algorithms to calculate $\tdu$ and $\tdh(i)$ in Eq~\ref{eq:define-h1-tilde} for triangles, two-stars and three-paths as described in Section~\ref{subsec:fast-linear-boot} and implemented in real data examples in Section~\ref{sec:realdata}.% The key of the faster precomputation is that we do not do a full permutation as suggested by $H_{\pi}$ in Eq~\ref{eq:define-h1-tilde}, but we sample index of $i$'s neighbours in the permuted sequence and only check the disjoint subsets including the neighbours in the permutation.   
 %Note that Algorithm~\ref{alg:apx_pre3path} for three-paths is similar to Algorithm~\ref{alg:apx_prevs} for two-stars, except that each bucket of the permutation sequence has three nodes in Algorithm~\ref{alg:apx_pre3path} but two nodes in Algorithm~\ref{alg:apx_prevs}. 
 
 Algorithm~\ref{alg:apx_pretri} and Algorithm~\ref{alg:apx_prevs} explicitly provide fast precomputation algorithms to calculate $\tdu$ and $\tdh(i)$ in Eq~\ref{eq:define-h1-tilde} for triangles, and two-stars as described in Section~\ref{subsec:fast-linear-boot} and implemented in real data examples in Section~\ref{sec:realdata}.% The key of the faster precomputation is that we do not do a full permutation as suggested by $H_{\pi}$ in Eq~\ref{eq:define-h1-tilde}, but we sample index of $i$'s neighbours in the permuted sequence and only check the disjoint subsets including the neighbours in the permutation.   
   Note that the corresponding algorithm for three-paths is similar to Algorithm~\ref{alg:apx_prevs}, except that each bucket of the permutation sequence has three nodes. Hence one needs to sample twice the degree of the root node to emulate the buckets which have a neighbor of the root node. We omit the details.% in Algorithm~\ref{alg:apx_pre3path} but two nodes in Algorithm~\ref{alg:apx_prevs}. 


\begin{algorithm}	
\SetAlgoLined
%\KwResult{}
\textbf{Input:} Network $A$, motif $R$, number of resamples $B$,  $\texttt{approximate}\in \{True,False\}$, parameter $u$\\
\textbf{If} $\texttt{approximate}=True$\\
%\vskip 0.5em
\hspace{1em}Compute $\{\tdh(i)\}_{i=1}^n$,   $\tilde{T}_n$ (Eq~\ref{eq:define-h1-tilde}) and $\tilde{\tau}_n$ (Eq~\ref{eq:define-taun-tilde})\\
\textbf{Else}\\
\vskip 0.5em
\hspace{1em}Compute $\hat{T}_n$, (Eq~\ref{eq:cf}), $\{\hat{g}_1(i)\}_{i=1}^n$    (Eq~\ref{eq:g1hat}) and $\hat{\tau}_n$ (Eq~\ref{eq:tauhat})\\
\textbf{End}\\
 \For{$j\in\{1,\dots, B\}$}{	
  Generate $n$ weights $\boldsymbol{\xi}^{(j)}=\{\w^{(j)}_i,i=1,\dots, n\}_{j=1}^B$ using Eq~\ref{eq:gaussproduct}\\
  \textbf{If} $\texttt{approximate}=True$\\
  \text{\hspace{1em} $T_n^*(j)\leftarrow  \ttnl$ (using Eq~\ref{eq:define-tnl-tilde}.)}\\
  \textbf{Else}\\
   \text{\hspace{1em} $T_n^*(j)\leftarrow  \cfbl$ (using Eq~\ref{eq:cfbl}.)}\\
 \textbf{End}\\
}
 Return $\dfrac{1}{B}\sum_j \mathbbm{1}\left(\dfrac{T_n^*(j)-\tilde{T}_n}{\frac{r}{n^{1/2}}\tilde{\tau}_n}\leq u\right)$
 %\ifthenelse
% Compute $\hat{T}^*_{n,a}$ from
 %$\boldsymbol{\xi}^{(j)}$, and $A$
 \caption{\label{alg:apx}Construction of linear or approximated linear bootstrap estimate of CDF}
\end{algorithm}


\begin{algorithm}[H]
\SetAlgoLined
%\KwResult{}
%\hline 
\vskip 0.1em
\textbf{Input:} Network $A$, motif $R$, number of resamples $B$, choice of bootstrap procedure $a\in\{M,Q\}$, parameter $u$\\
%\hline
\vskip 0.5em
Compute $\cfhat$ (Eq~\ref{eq:cf}), $\{\hat{g}_1(i)\}_{i=1}^n$ (Eq~\ref{eq:g1hat}), $\{\hat{g}_2(i,j)\}_{i=1}^n$ (Eq~\ref{eq:g2hat}) and $\hat{\tau}_n$ (Eq~\ref{eq:tauhat})
\vskip 0.5em
 \For{$j\in\{1,\dots, B\}$}{
  Generate $n$ weights $\boldsymbol{\xi}^{(j)}=\{\w^{(j)}_i,i=1,\dots, n\}_{j=1}^B$ using Eq~\ref{eq:gaussproduct}\\
   \textbf{If} $a=M$\\
  \text{\hspace{1em} $T_n^*(j)\leftarrow  \cfbm$ (using Eq~\ref{eq:multiplicative-bootstrap}.)}\\
  %\textbf{Else if} $a=Q$\\
  \textbf{Else}\\
  \text{\hspace{1em} $T_n^*(j)\leftarrow  \cfbq$ (using Eq~\ref{eq:cfbq}.)}\\
 %\textbf{Else}\\
  %\text{\hspace{1em} $T_n^*(j)\leftarrow  \cfbl$ (using Eq~\ref{eq:cfbl}.)}\\
 \textbf{End}\\
}
 Return $\dfrac{1}{B}\sum_j \mathbbm{1}\left(\dfrac{T_n^*(j)-\cfhat}{\frac{r}{n^{1/2}}\hat{\tau}_n}\leq u\right)$
 
 %\ifthenelse
% Compute $\hat{T}^*_{n,a}$ from
 %$\boldsymbol{\xi}^{(j)}$, and $A$
 \caption{\label{alg:ho}Construction of quadratic or multiplier bootstrap estimate of CDF}
\end{algorithm}


\rd
\rd
\begin{algorithm}	
\SetAlgoLined
%\KwResult{}
\textbf{Input:} Network A, size of network n,  number of samples N, r=3;\\
 \For{$i\in\{1,\dots, n\}$}{	
  $\texttt{nbs}\_{\texttt{i}}\leftarrow$ neighbors of node i; 
  $\texttt{deg}\_i\leftarrow$degree of i; 
  count=0;\\
    \For{$j\in\{1,\dots, N\}$}{
   \texttt{pos}$\leftarrow$ randomly sampled $\texttt{deg}\_i$ indices without replacement from $\{1\dots n-1\}$; \\ 
   (\texttt{indices}, \texttt{sorted})$\leftarrow$ sort(\texttt{pos}); \\
   ii=0; \\
  \While{ii $<$ \texttt{deg\_i}}{
  \texttt{curr} = \texttt{indices}(ii);
  \texttt{next} = \texttt{indices}(ii+1);\\
  \texttt{currnb}= \texttt{nbs}\_{\texttt{i}}(\texttt{sorted}(ii));
  \texttt{nextnb}=\texttt{nbs}\_{\texttt{i}}(\texttt{sorted}(ii+1));\\
 \textbf{if} (mod(\texttt{curr}, r-1) ==1 and \texttt{next}==\texttt{curr}+1):\\
       $\qquad$ \texttt{count}=\texttt{count}+A(\texttt{currnb},\texttt{nextnb}); ii=ii+1;\\
        \textbf{Else}:\\
 $\qquad$ continue;\\
     ii=ii+1\\
  \textbf{End}\\
  }\vspace{4mm}
 \textbf{End}\\
} \vspace{4mm}
  M(i) $\leftarrow$ (r-1)$\times$\texttt{count}/(N(n-1));\\
   \textbf{End}\\
}
 Return M where $\tdh(i)=M(i)/\rho_n^s$ and $\tdu=\frac{1}{n}\sum_{i=1}^n\tdh(i)$
 %\ifthenelse
% Compute $\hat{T}^*_{n,a}$ from
 %$\boldsymbol{\xi}^{(j)}$, and $A$
\caption{\label{alg:apx_pretri} Fast precomputation of approximating $\tdu$ and $\tdh(i)$ for triangles}
\end{algorithm}

\rd
\begin{algorithm}[htb]
\SetAlgoLined
%\KwResult{}
\textbf{Input:} Network $A$, size of network $n$, number of samples $N$, r=3;\\
 \For{$i\in\{1,\dots, n\}$}{	
   $\texttt{nbs}\_{\texttt{i}}\leftarrow$ neighbors of node i; $\texttt{deg}\_{\texttt{i}}\leftarrow$degree of i;  \texttt{count}=0;\\
    \For{$j\in\{1,\dots, N\}$}{
  \texttt{pos}$\leftarrow$ randomly sampled $\texttt{deg}\_{\texttt{i}}$ indices without replacement from $\{1:n-1\}$; \\ 
  \texttt{posConc} $\leftarrow$ randomly sample $\min(\texttt{deg}\_{\texttt{i}},n-1-\texttt{deg}\_{\texttt{i}})$ indices without replacement from $\{1:n\}\setminus\{i \cup \texttt{nbs}\_{\texttt{i}}\}$;\\
  % \texttt{indices}=sort(S); \texttt{sorted}=sort index(S);\\
    (\texttt{indices}, \texttt{sorted})$\leftarrow$ sort(\texttt{pos}); ConcurrentID=0; ii=0; \\
  \While{$ii < \texttt{deg}\_{\texttt{i}}$}{
    t=0; \texttt{curr} = \texttt{indices}(ii);  \texttt{next}=0; \texttt{nextnb}=0;\\
    \textbf{If} ($ii+1 > \texttt{deg}\_{\texttt{i}}-1$): \texttt{next} = -1;\\
    \textbf{Else}: \texttt{next} = \texttt{indices}(ii+1);
            \texttt{nextnb}=\texttt{nbs}\_{\texttt{i}}(\texttt{sorted}(ii+1));\\
    \texttt{currnb}= \texttt{nbs}\_{\texttt{i}}(\texttt{sorted}(ii));\\     
    \textbf{If} (\texttt{next}!=-1 and (mod(\texttt{curr},2)==1 and \texttt{next}==\texttt{curr}+1)):\\
            $\qquad$  \textbf{If}(A(\texttt{currnb},\texttt{nextnb})==0): t=1;\\
             $\qquad$ ii=ii+1;\\
    \textbf{Else}:\\
    \vspace{-3mm}
           $\qquad$    \texttt{concurrent} = \texttt{posConc}(ConcurrentID);\\
           $\qquad$    \textbf{If} (A(\texttt{currnb},\texttt{concurrent})==1): t=1;\\
           $\qquad$    ConcurrentID=ConcurrentID+1;\\
    \texttt{count}=\texttt{count}+t; \  ii=ii+1;\\
  \textbf{End}\\
  }\vspace{4mm}
 \textbf{End}\\
} \vspace{4mm}
  M(i)=(r-1)$\times$\texttt{count}/(N(n-1));\\
 % \vspace{-2mm}
   \textbf{End}\\
}
\vspace{2mm}
 Return $M$ where $\tdh(i)=M(i)/\rho_n^s$ and $\tdu=\frac{1}{n}\sum_{i=1}^n\tdh(i)$
 %\ifthenelse
% Compute $\hat{T}^*_{n,a}$ from
 %$\boldsymbol{\xi}^{(j)}$, and $A$
 \caption{\label{alg:apx_prevs} Fast precomputation of approximating $\tdu$ and $\tdh(i)$ for two-stars}
\end{algorithm}


\iffalse
\begin{algorithm}	
\SetAlgoLined
%\KwResult{}
\textbf{Input:} Network $A$, size of network $n$, number of samples $N$\\%motif $R$, numbers of nodes in the motif $r$, number of samples $N$\\
 \For{$i\in\{1,\dots, n\}$}{	
  $nbs\_i\leftarrow \text{neighbors of node $i$}$; 
  $d_i\leftarrow \text{degree of $i$}$; 
  $u=0$;\\
    \For{$j\in\{1,\dots, N\}$}{
  $S$= randomly sample $d_i$ integers without replacement from $\{1,n-1\}$;\\ 
  Sconc = randomly sample $2\texttt{deg}\_{\texttt{i}}$ indexes without replacement from $\{1:n\setminus i\}$ and excluding the neighbours;\\
   indexes=sort(S); \texttt{sorted}=sort index(S); ConcurrentID=0; ii=0; \\
  \While{$ii < d_i$}{
    t=0; curr=indexes(ii); next=0; nextnext=0;nextnb=0;nextnextnb=0;\\
    \textbf{If} ($ii+1 > (d_i-1)$):next = -1; nextnext=-1;\\
    \textbf{Else}:
    next = indexes(ii+1);
            nextnb=nbs(\texttt{sorted}(ii+1));\\
     $\qquad$    \textbf{If}($ii+1 > (d_i-2)$): nextnext=-1;\\
     $\qquad$ \textbf{Else}:nextnext=indexes(ii+2);
              nextnextnb=nbs(\texttt{sorted}(ii+2));\\
    currnb= nbs(\texttt{sorted}(ii));
    SS1=\{curr,next,nextnext\}; SS2=\{curr,next\};\\
    \textbf{If} (nextnext!=-1 and InSameBucket(SS1)==1): t=0;
            ii=ii+2;\\
            \textbf{Else If} (next!=-1 and InSameBucket(SS2)==1): \\
             $\qquad$ concurrent = Sconc(ConcurrentID);\\
              %$\qquad$t=(1-A(currnb,concurrent))*A(nextnb,concurrent)*(1-A(currnb,nextnb)) + (1-A(nextnb,concurrent))*A(currnb,concurrent)*(1-A(currnb,nextnb));\\
             $\qquad$ Check \textbf{If}(i,currnb,nextnb,concurrent forms a three-path):t=1;\\
             $\qquad$ ii=ii+1;
            ConcurrentID=ConcurrentID+1;\\
    \textbf{Else}\\
             $\qquad$ concurrent = Sconc(ConcurrentID);\\
             $\qquad$ concurrentnxt = Sconc(ConcurrentID+1);\\
             %$\qquad$ \textbf{If} (currnb, concurrent concurrentnxt forms a two-star with either concurrent or concurrentnxt as hub): t=1;\\
             $\qquad$ Check \textbf{If} (i,currnb, concurrent concurrentnxt forms a three-path): t=1;\\ $\qquad$ConcurrentID=ConcurrentID+2;\\
    u=u+t;
    ii=ii+1;\\
  \textbf{End}\\
  }\vspace{4mm}
 \textbf{End}\\
} \vspace{4mm}
  M(i)=u/(N*(n-1)/(r-1));\\
   \textbf{End}\\
}
 Return $M$ where $\tdh(i)=M(i)/\rho_n^s$ and $\tdu=\frac{1}{n}\sum_{i=1}^n\tdh(i)$
 %\ifthenelse
% Compute $\hat{T}^*_{n,a}$ from
 %$\boldsymbol{\xi}^{(j)}$, and $A$
 \caption{\label{alg:apx_pre3path} Fast precomputation of approximating $\tdu$ and $\tdh(i)$ for Three-paths}
\end{algorithm}
\fi
\bk
